GWTC-4.0: Population Properties of Merging Compact Binaries

We detail the population properties of merging compact objects using 158 mergers from the cumulative Gravitational-Wave Transient Catalog 4.0, which includes three types of binary mergers: binary neutron star, neutron star--black hole binary, and binary black hole mergers. We resolve multiple over- and under-densities in the black hole mass distribution: features persist at primary masses of $10\,M_\odot$ and $35\,M_\odot$ with a possible third feature at $\sim 20\,M_\odot$. These are departures from an otherwise power-law-like continuum that steepens above $35\,M_\odot$. Binary black holes with primary masses near $10\,M_\odot$ are more likely to have less massive secondaries, with a mass ratio distribution peaking at $q = 0.74^{+0.13}_{-0.13}$, potentially a signature of stable mass transfer during binary evolution. Black hole spins are inferred to be non-extremal, with 90\% of black holes having $\chi < 0.57$, and preferentially aligned with binary orbits, implying many merging binaries form in isolation. However, we find a significant fraction, 0.24-0.42, of binaries have negative effective inspiral spins, suggesting many could be formed dynamically in gas-free environments. We find evidence for correlation between effective inspiral spin and mass ratio, though it is unclear if this is driven by variation in the mode of the distribution or the width. (Abridged)

==> macros_from_json.tex <==
\makeatletter\newcommand\BBHMassModelBayesFactors[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BBHMassModelBayesFactors@out{\{"default\_dominant\_mode": 71, "default\_subdominant\_mode": 29, "pl2pk1": "{-}0.06", "pl2pk3": "{-}0.34", "plp": "{-}2.43"\}}\else\ifnum\pdfstrcmp{#1}{default_dominant_mode}=0\def\BBHMassModelBayesFactors@out{71}\else\ifnum\pdfstrcmp{#1}{default_subdominant_mode}=0\def\BBHMassModelBayesFactors@out{29}\else\ifnum\pdfstrcmp{#1}{pl2pk1}=0\def\BBHMassModelBayesFactors@out{{-}0.06}\else\ifnum\pdfstrcmp{#1}{pl2pk3}=0\def\BBHMassModelBayesFactors@out{{-}0.34}\else\ifnum\pdfstrcmp{#1}{plp}=0\def\BBHMassModelBayesFactors@out{{-}2.43}\else\def\BBHMassModelBayesFactors@out{??}\fi\fi\fi\fi\fi\fi\BBHMassModelBayesFactors@out}\makeatother
\makeatletter\newcommand\BsplineChiEff[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineChiEff@out{\{"chi\_eff": \{"percent\_less\_zero": \{"median": "43.1", "error plus": "6.4", "error minus": "6.4", "5th percentile": "36.7", "95th percentile": "49.5"\}, "1st\_percentile": \{"median": "{-}0.44", "error plus": "0.06", "error minus": "0.06", "5th percentile": "{-}0.51", "95th percentile": "{-}0.38"\}\}\}}\else\ifnum\pdfstrcmp{#1}{chi_eff}=0\let\BsplineChiEff@out\BsplineChiEff@I\else\def\BsplineChiEff@out{??}\fi\fi\BsplineChiEff@out}\newcommand\BsplineChiEff@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineChiEff@I@out{\{"percent\_less\_zero": \{"median": "43.1", "error plus": "6.4", "error minus": "6.4", "5th percentile": "36.7", "95th percentile": "49.5"\}, "1st\_percentile": \{"median": "{-}0.44", "error plus": "0.06", "error minus": "0.06", "5th percentile": "{-}0.51", "95th percentile": "{-}0.38"\}\}}\else\ifnum\pdfstrcmp{#1}{percent_less_zero}=0\let\BsplineChiEff@I@out\BsplineChiEff@II\else\ifnum\pdfstrcmp{#1}{1st_percentile}=0\let\BsplineChiEff@I@out\BsplineChiEff@III\else\def\BsplineChiEff@I@out{??}\fi\fi\fi\BsplineChiEff@I@out}\newcommand\BsplineChiEff@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineChiEff@II@out{\{"median": "43.1", "error plus": "6.4", "error minus": "6.4", "5th percentile": "36.7", "95th percentile": "49.5"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineChiEff@II@out{43.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineChiEff@II@out{6.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineChiEff@II@out{6.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineChiEff@II@out{36.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineChiEff@II@out{49.5}\else\def\BsplineChiEff@II@out{??}\fi\fi\fi\fi\fi\fi\BsplineChiEff@II@out}\newcommand\BsplineChiEff@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineChiEff@III@out{\{"median": "{-}0.44", "error plus": "0.06", "error minus": "0.06", "5th percentile": "{-}0.51", "95th percentile": "{-}0.38"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineChiEff@III@out{{-}0.44}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineChiEff@III@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineChiEff@III@out{0.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineChiEff@III@out{{-}0.51}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineChiEff@III@out{{-}0.38}\else\def\BsplineChiEff@III@out{??}\fi\fi\fi\fi\fi\fi\BsplineChiEff@III@out}\makeatother
\makeatletter\newcommand\BsplineIID[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@out{\{"mass\_1": \{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}, "ppd": \{"median": "10", "error plus": "24", "error minus": "2.2", "5th percentile": "8.2", "95th percentile": "34"\}\}, "mass\_ratio": \{"peak": \{"median": "0.75", "error plus": "0.11", "error minus": "0.16", "5th percentile": "0.59", "95th percentile": "0.86"\}, "ppd": \{"median": "0.71", "error plus": "0.22", "error minus": "0.31", "5th percentile": "0.40", "95th percentile": "0.94"\}\}, "a": \{"peak": \{"median": "0.095", "error plus": "0.17", "error minus": "0.095", "5th percentile": 0, "95th percentile": "0.26"\}, "ppd": \{"median": "0.30", "error plus": "0.61", "error minus": "0.27", "5th percentile": "0.028", "95th percentile": "0.90"\}\}, "cos\_tilt": \{"peak": \{"median": "0.17", "error plus": "0.79", "error minus": "0.41", "5th percentile": "{-}0.23", "95th percentile": "0.96"\}, "ppd": \{"median": "0.11", "error plus": "0.78", "error minus": "0.93", "5th percentile": "{-}0.82", "95th percentile": "0.88"\}\}, "redshift": \{"ppd": \{"median": "1.5", "error plus": "0.79", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}\}, "rate\_at\_z\_0{-}2": \{"median": "38", "error plus": "19", "error minus": "10", "5th percentile": "27", "95th percentile": "57"\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\BsplineIID@out\BsplineIID@I\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\BsplineIID@out\BsplineIID@II\else\ifnum\pdfstrcmp{#1}{a}=0\let\BsplineIID@out\BsplineIID@III\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\BsplineIID@out\BsplineIID@IV\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\BsplineIID@out\BsplineIID@V\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\BsplineIID@out\BsplineIID@VI\else\def\BsplineIID@out{??}\fi\fi\fi\fi\fi\fi\fi\BsplineIID@out}\newcommand\BsplineIID@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@I@out{\{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}, "ppd": \{"median": "10", "error plus": "24", "error minus": "2.2", "5th percentile": "8.2", "95th percentile": "34"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\BsplineIID@I@out\BsplineIID@VII\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\BsplineIID@I@out\BsplineIID@VIII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIID@I@out\BsplineIID@IX\else\def\BsplineIID@I@out{??}\fi\fi\fi\fi\BsplineIID@I@out}\newcommand\BsplineIID@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@II@out{\{"peak": \{"median": "0.75", "error plus": "0.11", "error minus": "0.16", "5th percentile": "0.59", "95th percentile": "0.86"\}, "ppd": \{"median": "0.71", "error plus": "0.22", "error minus": "0.31", "5th percentile": "0.40", "95th percentile": "0.94"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineIID@II@out\BsplineIID@X\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIID@II@out\BsplineIID@XI\else\def\BsplineIID@II@out{??}\fi\fi\fi\BsplineIID@II@out}\newcommand\BsplineIID@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@III@out{\{"peak": \{"median": "0.095", "error plus": "0.17", "error minus": "0.095", "5th percentile": 0, "95th percentile": "0.26"\}, "ppd": \{"median": "0.30", "error plus": "0.61", "error minus": "0.27", "5th percentile": "0.028", "95th percentile": "0.90"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineIID@III@out\BsplineIID@XII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIID@III@out\BsplineIID@XIII\else\def\BsplineIID@III@out{??}\fi\fi\fi\BsplineIID@III@out}\newcommand\BsplineIID@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@IV@out{\{"peak": \{"median": "0.17", "error plus": "0.79", "error minus": "0.41", "5th percentile": "{-}0.23", "95th percentile": "0.96"\}, "ppd": \{"median": "0.11", "error plus": "0.78", "error minus": "0.93", "5th percentile": "{-}0.82", "95th percentile": "0.88"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineIID@IV@out\BsplineIID@XIV\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIID@IV@out\BsplineIID@XV\else\def\BsplineIID@IV@out{??}\fi\fi\fi\BsplineIID@IV@out}\newcommand\BsplineIID@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@V@out{\{"ppd": \{"median": "1.5", "error plus": "0.79", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}\}}\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIID@V@out\BsplineIID@XVI\else\def\BsplineIID@V@out{??}\fi\fi\BsplineIID@V@out}\newcommand\BsplineIID@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@VI@out{\{"median": "38", "error plus": "19", "error minus": "10", "5th percentile": "27", "95th percentile": "57"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@VI@out{38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@VI@out{19}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@VI@out{10}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@VI@out{27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@VI@out{57}\else\def\BsplineIID@VI@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@VI@out}\newcommand\BsplineIID@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@VII@out{\{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@VII@out{10.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@VII@out{0.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@VII@out{0.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@VII@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@VII@out{10.8}\else\def\BsplineIID@VII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@VII@out}\newcommand\BsplineIID@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@VIII@out{\{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@VIII@out{33.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@VIII@out{2.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@VIII@out{4.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@VIII@out{29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@VIII@out{36}\else\def\BsplineIID@VIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@VIII@out}\newcommand\BsplineIID@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@IX@out{\{"median": "10", "error plus": "24", "error minus": "2.2", "5th percentile": "8.2", "95th percentile": "34"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@IX@out{10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@IX@out{24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@IX@out{2.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@IX@out{8.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@IX@out{34}\else\def\BsplineIID@IX@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@IX@out}\newcommand\BsplineIID@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@X@out{\{"median": "0.75", "error plus": "0.11", "error minus": "0.16", "5th percentile": "0.59", "95th percentile": "0.86"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@X@out{0.75}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@X@out{0.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@X@out{0.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@X@out{0.59}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@X@out{0.86}\else\def\BsplineIID@X@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@X@out}\newcommand\BsplineIID@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@XI@out{\{"median": "0.71", "error plus": "0.22", "error minus": "0.31", "5th percentile": "0.40", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@XI@out{0.71}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@XI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@XI@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@XI@out{0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@XI@out{0.94}\else\def\BsplineIID@XI@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@XI@out}\newcommand\BsplineIID@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@XII@out{\{"median": "0.095", "error plus": "0.17", "error minus": "0.095", "5th percentile": 0, "95th percentile": "0.26"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@XII@out{0.095}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@XII@out{0.17}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@XII@out{0.095}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@XII@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@XII@out{0.26}\else\def\BsplineIID@XII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@XII@out}\newcommand\BsplineIID@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@XIII@out{\{"median": "0.30", "error plus": "0.61", "error minus": "0.27", "5th percentile": "0.028", "95th percentile": "0.90"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@XIII@out{0.30}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@XIII@out{0.61}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@XIII@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@XIII@out{0.028}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@XIII@out{0.90}\else\def\BsplineIID@XIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@XIII@out}\newcommand\BsplineIID@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@XIV@out{\{"median": "0.17", "error plus": "0.79", "error minus": "0.41", "5th percentile": "{-}0.23", "95th percentile": "0.96"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@XIV@out{0.17}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@XIV@out{0.79}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@XIV@out{0.41}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@XIV@out{{-}0.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@XIV@out{0.96}\else\def\BsplineIID@XIV@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@XIV@out}\newcommand\BsplineIID@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@XV@out{\{"median": "0.11", "error plus": "0.78", "error minus": "0.93", "5th percentile": "{-}0.82", "95th percentile": "0.88"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@XV@out{0.11}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@XV@out{0.78}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@XV@out{0.93}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@XV@out{{-}0.82}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@XV@out{0.88}\else\def\BsplineIID@XV@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@XV@out}\newcommand\BsplineIID@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIID@XVI@out{\{"median": "1.5", "error plus": "0.79", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIID@XVI@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIID@XVI@out{0.79}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIID@XVI@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIID@XVI@out{0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIID@XVI@out{2.3}\else\def\BsplineIID@XVI@out{??}\fi\fi\fi\fi\fi\fi\BsplineIID@XVI@out}\makeatother
\makeatletter\newcommand\BsplineIIDnoGW[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@out{\{"mass\_1": \{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "1.9", "error minus": "4.5", "5th percentile": "29", "95th percentile": "35"\}, "ppd": \{"median": "10", "error plus": "23", "error minus": "2.6", "5th percentile": "7.8", "95th percentile": "34"\}\}, "mass\_ratio": \{"peak": \{"median": "0.75", "error plus": "0.11", "error minus": "0.15", "5th percentile": "0.60", "95th percentile": "0.86"\}, "ppd": \{"median": "0.71", "error plus": "0.22", "error minus": "0.32", "5th percentile": "0.39", "95th percentile": "0.93"\}\}, "a": \{"peak": \{"median": "0.090", "error plus": "0.19", "error minus": "0.090", "5th percentile": 0, "95th percentile": "0.28"\}, "ppd": \{"median": "0.30", "error plus": "0.59", "error minus": "0.28", "5th percentile": "0.028", "95th percentile": "0.90"\}\}, "cos\_tilt": \{"peak": \{"median": "0.16", "error plus": "0.84", "error minus": "0.37", "5th percentile": "{-}0.20", "95th percentile": "1.0"\}, "ppd": \{"median": "0.11", "error plus": "0.78", "error minus": "0.93", "5th percentile": "{-}0.82", "95th percentile": "0.89"\}\}, "redshift": \{"ppd": \{"median": "1.5", "error plus": "0.84", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}\}, "rate\_at\_z\_0{-}2": \{"median": "39", "error plus": "19", "error minus": "11", "5th percentile": "27", "95th percentile": "57"\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\BsplineIIDnoGW@out\BsplineIIDnoGW@I\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\BsplineIIDnoGW@out\BsplineIIDnoGW@II\else\ifnum\pdfstrcmp{#1}{a}=0\let\BsplineIIDnoGW@out\BsplineIIDnoGW@III\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\BsplineIIDnoGW@out\BsplineIIDnoGW@IV\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\BsplineIIDnoGW@out\BsplineIIDnoGW@V\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\BsplineIIDnoGW@out\BsplineIIDnoGW@VI\else\def\BsplineIIDnoGW@out{??}\fi\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@out}\newcommand\BsplineIIDnoGW@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@I@out{\{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "1.9", "error minus": "4.5", "5th percentile": "29", "95th percentile": "35"\}, "ppd": \{"median": "10", "error plus": "23", "error minus": "2.6", "5th percentile": "7.8", "95th percentile": "34"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\BsplineIIDnoGW@I@out\BsplineIIDnoGW@VII\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\BsplineIIDnoGW@I@out\BsplineIIDnoGW@VIII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIIDnoGW@I@out\BsplineIIDnoGW@IX\else\def\BsplineIIDnoGW@I@out{??}\fi\fi\fi\fi\BsplineIIDnoGW@I@out}\newcommand\BsplineIIDnoGW@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@II@out{\{"peak": \{"median": "0.75", "error plus": "0.11", "error minus": "0.15", "5th percentile": "0.60", "95th percentile": "0.86"\}, "ppd": \{"median": "0.71", "error plus": "0.22", "error minus": "0.32", "5th percentile": "0.39", "95th percentile": "0.93"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineIIDnoGW@II@out\BsplineIIDnoGW@X\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIIDnoGW@II@out\BsplineIIDnoGW@XI\else\def\BsplineIIDnoGW@II@out{??}\fi\fi\fi\BsplineIIDnoGW@II@out}\newcommand\BsplineIIDnoGW@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@III@out{\{"peak": \{"median": "0.090", "error plus": "0.19", "error minus": "0.090", "5th percentile": 0, "95th percentile": "0.28"\}, "ppd": \{"median": "0.30", "error plus": "0.59", "error minus": "0.28", "5th percentile": "0.028", "95th percentile": "0.90"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineIIDnoGW@III@out\BsplineIIDnoGW@XII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIIDnoGW@III@out\BsplineIIDnoGW@XIII\else\def\BsplineIIDnoGW@III@out{??}\fi\fi\fi\BsplineIIDnoGW@III@out}\newcommand\BsplineIIDnoGW@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@IV@out{\{"peak": \{"median": "0.16", "error plus": "0.84", "error minus": "0.37", "5th percentile": "{-}0.20", "95th percentile": "1.0"\}, "ppd": \{"median": "0.11", "error plus": "0.78", "error minus": "0.93", "5th percentile": "{-}0.82", "95th percentile": "0.89"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineIIDnoGW@IV@out\BsplineIIDnoGW@XIV\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIIDnoGW@IV@out\BsplineIIDnoGW@XV\else\def\BsplineIIDnoGW@IV@out{??}\fi\fi\fi\BsplineIIDnoGW@IV@out}\newcommand\BsplineIIDnoGW@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@V@out{\{"ppd": \{"median": "1.5", "error plus": "0.84", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}\}}\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineIIDnoGW@V@out\BsplineIIDnoGW@XVI\else\def\BsplineIIDnoGW@V@out{??}\fi\fi\BsplineIIDnoGW@V@out}\newcommand\BsplineIIDnoGW@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@VI@out{\{"median": "39", "error plus": "19", "error minus": "11", "5th percentile": "27", "95th percentile": "57"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@VI@out{39}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@VI@out{19}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@VI@out{11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@VI@out{27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@VI@out{57}\else\def\BsplineIIDnoGW@VI@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@VI@out}\newcommand\BsplineIIDnoGW@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@VII@out{\{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@VII@out{10.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@VII@out{0.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@VII@out{0.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@VII@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@VII@out{10.8}\else\def\BsplineIIDnoGW@VII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@VII@out}\newcommand\BsplineIIDnoGW@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@VIII@out{\{"median": "33.5", "error plus": "1.9", "error minus": "4.5", "5th percentile": "29", "95th percentile": "35"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@VIII@out{33.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@VIII@out{1.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@VIII@out{4.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@VIII@out{29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@VIII@out{35}\else\def\BsplineIIDnoGW@VIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@VIII@out}\newcommand\BsplineIIDnoGW@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@IX@out{\{"median": "10", "error plus": "23", "error minus": "2.6", "5th percentile": "7.8", "95th percentile": "34"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@IX@out{10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@IX@out{23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@IX@out{2.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@IX@out{7.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@IX@out{34}\else\def\BsplineIIDnoGW@IX@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@IX@out}\newcommand\BsplineIIDnoGW@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@X@out{\{"median": "0.75", "error plus": "0.11", "error minus": "0.15", "5th percentile": "0.60", "95th percentile": "0.86"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@X@out{0.75}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@X@out{0.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@X@out{0.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@X@out{0.60}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@X@out{0.86}\else\def\BsplineIIDnoGW@X@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@X@out}\newcommand\BsplineIIDnoGW@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@XI@out{\{"median": "0.71", "error plus": "0.22", "error minus": "0.32", "5th percentile": "0.39", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@XI@out{0.71}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@XI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@XI@out{0.32}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@XI@out{0.39}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@XI@out{0.93}\else\def\BsplineIIDnoGW@XI@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@XI@out}\newcommand\BsplineIIDnoGW@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@XII@out{\{"median": "0.090", "error plus": "0.19", "error minus": "0.090", "5th percentile": 0, "95th percentile": "0.28"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@XII@out{0.090}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@XII@out{0.19}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@XII@out{0.090}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@XII@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@XII@out{0.28}\else\def\BsplineIIDnoGW@XII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@XII@out}\newcommand\BsplineIIDnoGW@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@XIII@out{\{"median": "0.30", "error plus": "0.59", "error minus": "0.28", "5th percentile": "0.028", "95th percentile": "0.90"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@XIII@out{0.30}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@XIII@out{0.59}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@XIII@out{0.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@XIII@out{0.028}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@XIII@out{0.90}\else\def\BsplineIIDnoGW@XIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@XIII@out}\newcommand\BsplineIIDnoGW@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@XIV@out{\{"median": "0.16", "error plus": "0.84", "error minus": "0.37", "5th percentile": "{-}0.20", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@XIV@out{0.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@XIV@out{0.84}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@XIV@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@XIV@out{{-}0.20}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@XIV@out{1.0}\else\def\BsplineIIDnoGW@XIV@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@XIV@out}\newcommand\BsplineIIDnoGW@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@XV@out{\{"median": "0.11", "error plus": "0.78", "error minus": "0.93", "5th percentile": "{-}0.82", "95th percentile": "0.89"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@XV@out{0.11}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@XV@out{0.78}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@XV@out{0.93}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@XV@out{{-}0.82}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@XV@out{0.89}\else\def\BsplineIIDnoGW@XV@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@XV@out}\newcommand\BsplineIIDnoGW@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineIIDnoGW@XVI@out{\{"median": "1.5", "error plus": "0.84", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineIIDnoGW@XVI@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineIIDnoGW@XVI@out{0.84}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineIIDnoGW@XVI@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineIIDnoGW@XVI@out{0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineIIDnoGW@XVI@out{2.3}\else\def\BsplineIIDnoGW@XVI@out{??}\fi\fi\fi\fi\fi\fi\BsplineIIDnoGW@XVI@out}\makeatother
\makeatletter\newcommand\BsplineNonIID[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@out{\{"mass\_1": \{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}, "ppd": \{"median": "10", "error plus": "24", "error minus": "2.2", "5th percentile": "8.2", "95th percentile": "34"\}\}, "mass\_ratio": \{"peak": \{"median": "0.75", "error plus": "0.10", "error minus": "0.15", "5th percentile": "0.60", "95th percentile": "0.85"\}, "ppd": \{"median": "0.71", "error plus": "0.22", "error minus": "0.32", "5th percentile": "0.40", "95th percentile": "0.93"\}\}, "a\_1": \{"peak": \{"median": "0.12", "error plus": "0.18", "error minus": "0.12", "5th percentile": 0, "95th percentile": "0.30"\}, "ppd": \{"median": "0.30", "error plus": "0.61", "error minus": "0.27", "5th percentile": "0.029", "95th percentile": "0.91"\}\}, "a\_2": \{"peak": \{"median": "0.16", "error plus": "0.31", "error minus": "0.16", "5th percentile": 0, "95th percentile": "0.47"\}, "ppd": \{"median": "0.37", "error plus": "0.55", "error minus": "0.33", "5th percentile": "0.036", "95th percentile": "0.91"\}\}, "cos\_tilt\_1": \{"peak": \{"median": "0.12", "error plus": "0.88", "error minus": "0.56", "5th percentile": "{-}0.44", "95th percentile": "1.0"\}, "ppd": \{"median": "0.071", "error plus": "0.82", "error minus": "0.92", "5th percentile": "{-}0.85", "95th percentile": "0.89"\}\}, "cos\_tilt\_2": \{"peak": \{"median": "0.25", "error plus": "0.75", "error minus": "0.61", "5th percentile": "{-}0.36", "95th percentile": "1.0"\}, "ppd": \{"median": "0.12", "error plus": "0.77", "error minus": "0.96", "5th percentile": "{-}0.84", "95th percentile": "0.89"\}\}, "redshift": \{"ppd": \{"median": "1.5", "error plus": "0.84", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}\}, "rate\_at\_z\_0{-}2": \{"median": "38", "error plus": "21", "error minus": "11", "5th percentile": "27", "95th percentile": "59"\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\BsplineNonIID@out\BsplineNonIID@I\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\BsplineNonIID@out\BsplineNonIID@II\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\BsplineNonIID@out\BsplineNonIID@III\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\BsplineNonIID@out\BsplineNonIID@IV\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\BsplineNonIID@out\BsplineNonIID@V\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\BsplineNonIID@out\BsplineNonIID@VI\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\BsplineNonIID@out\BsplineNonIID@VII\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\BsplineNonIID@out\BsplineNonIID@VIII\else\def\BsplineNonIID@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\BsplineNonIID@out}\newcommand\BsplineNonIID@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@I@out{\{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}, "ppd": \{"median": "10", "error plus": "24", "error minus": "2.2", "5th percentile": "8.2", "95th percentile": "34"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\BsplineNonIID@I@out\BsplineNonIID@IX\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\BsplineNonIID@I@out\BsplineNonIID@X\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIID@I@out\BsplineNonIID@XI\else\def\BsplineNonIID@I@out{??}\fi\fi\fi\fi\BsplineNonIID@I@out}\newcommand\BsplineNonIID@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@II@out{\{"peak": \{"median": "0.75", "error plus": "0.10", "error minus": "0.15", "5th percentile": "0.60", "95th percentile": "0.85"\}, "ppd": \{"median": "0.71", "error plus": "0.22", "error minus": "0.32", "5th percentile": "0.40", "95th percentile": "0.93"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIID@II@out\BsplineNonIID@XII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIID@II@out\BsplineNonIID@XIII\else\def\BsplineNonIID@II@out{??}\fi\fi\fi\BsplineNonIID@II@out}\newcommand\BsplineNonIID@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@III@out{\{"peak": \{"median": "0.12", "error plus": "0.18", "error minus": "0.12", "5th percentile": 0, "95th percentile": "0.30"\}, "ppd": \{"median": "0.30", "error plus": "0.61", "error minus": "0.27", "5th percentile": "0.029", "95th percentile": "0.91"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIID@III@out\BsplineNonIID@XIV\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIID@III@out\BsplineNonIID@XV\else\def\BsplineNonIID@III@out{??}\fi\fi\fi\BsplineNonIID@III@out}\newcommand\BsplineNonIID@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@IV@out{\{"peak": \{"median": "0.16", "error plus": "0.31", "error minus": "0.16", "5th percentile": 0, "95th percentile": "0.47"\}, "ppd": \{"median": "0.37", "error plus": "0.55", "error minus": "0.33", "5th percentile": "0.036", "95th percentile": "0.91"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIID@IV@out\BsplineNonIID@XVI\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIID@IV@out\BsplineNonIID@XVII\else\def\BsplineNonIID@IV@out{??}\fi\fi\fi\BsplineNonIID@IV@out}\newcommand\BsplineNonIID@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@V@out{\{"peak": \{"median": "0.12", "error plus": "0.88", "error minus": "0.56", "5th percentile": "{-}0.44", "95th percentile": "1.0"\}, "ppd": \{"median": "0.071", "error plus": "0.82", "error minus": "0.92", "5th percentile": "{-}0.85", "95th percentile": "0.89"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIID@V@out\BsplineNonIID@XVIII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIID@V@out\BsplineNonIID@XIX\else\def\BsplineNonIID@V@out{??}\fi\fi\fi\BsplineNonIID@V@out}\newcommand\BsplineNonIID@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@VI@out{\{"peak": \{"median": "0.25", "error plus": "0.75", "error minus": "0.61", "5th percentile": "{-}0.36", "95th percentile": "1.0"\}, "ppd": \{"median": "0.12", "error plus": "0.77", "error minus": "0.96", "5th percentile": "{-}0.84", "95th percentile": "0.89"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIID@VI@out\BsplineNonIID@XX\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIID@VI@out\BsplineNonIID@XXI\else\def\BsplineNonIID@VI@out{??}\fi\fi\fi\BsplineNonIID@VI@out}\newcommand\BsplineNonIID@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@VII@out{\{"ppd": \{"median": "1.5", "error plus": "0.84", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}\}}\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIID@VII@out\BsplineNonIID@XXII\else\def\BsplineNonIID@VII@out{??}\fi\fi\BsplineNonIID@VII@out}\newcommand\BsplineNonIID@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@VIII@out{\{"median": "38", "error plus": "21", "error minus": "11", "5th percentile": "27", "95th percentile": "59"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@VIII@out{38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@VIII@out{21}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@VIII@out{11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@VIII@out{27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@VIII@out{59}\else\def\BsplineNonIID@VIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@VIII@out}\newcommand\BsplineNonIID@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@IX@out{\{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@IX@out{10.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@IX@out{0.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@IX@out{0.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@IX@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@IX@out{10.8}\else\def\BsplineNonIID@IX@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@IX@out}\newcommand\BsplineNonIID@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@X@out{\{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@X@out{33.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@X@out{2.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@X@out{4.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@X@out{29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@X@out{36}\else\def\BsplineNonIID@X@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@X@out}\newcommand\BsplineNonIID@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XI@out{\{"median": "10", "error plus": "24", "error minus": "2.2", "5th percentile": "8.2", "95th percentile": "34"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XI@out{10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XI@out{24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XI@out{2.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XI@out{8.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XI@out{34}\else\def\BsplineNonIID@XI@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XI@out}\newcommand\BsplineNonIID@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XII@out{\{"median": "0.75", "error plus": "0.10", "error minus": "0.15", "5th percentile": "0.60", "95th percentile": "0.85"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XII@out{0.75}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XII@out{0.10}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XII@out{0.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XII@out{0.60}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XII@out{0.85}\else\def\BsplineNonIID@XII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XII@out}\newcommand\BsplineNonIID@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XIII@out{\{"median": "0.71", "error plus": "0.22", "error minus": "0.32", "5th percentile": "0.40", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XIII@out{0.71}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XIII@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XIII@out{0.32}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XIII@out{0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XIII@out{0.93}\else\def\BsplineNonIID@XIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XIII@out}\newcommand\BsplineNonIID@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XIV@out{\{"median": "0.12", "error plus": "0.18", "error minus": "0.12", "5th percentile": 0, "95th percentile": "0.30"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XIV@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XIV@out{0.18}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XIV@out{0.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XIV@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XIV@out{0.30}\else\def\BsplineNonIID@XIV@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XIV@out}\newcommand\BsplineNonIID@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XV@out{\{"median": "0.30", "error plus": "0.61", "error minus": "0.27", "5th percentile": "0.029", "95th percentile": "0.91"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XV@out{0.30}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XV@out{0.61}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XV@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XV@out{0.029}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XV@out{0.91}\else\def\BsplineNonIID@XV@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XV@out}\newcommand\BsplineNonIID@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XVI@out{\{"median": "0.16", "error plus": "0.31", "error minus": "0.16", "5th percentile": 0, "95th percentile": "0.47"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XVI@out{0.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XVI@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XVI@out{0.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XVI@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XVI@out{0.47}\else\def\BsplineNonIID@XVI@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XVI@out}\newcommand\BsplineNonIID@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XVII@out{\{"median": "0.37", "error plus": "0.55", "error minus": "0.33", "5th percentile": "0.036", "95th percentile": "0.91"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XVII@out{0.37}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XVII@out{0.55}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XVII@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XVII@out{0.036}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XVII@out{0.91}\else\def\BsplineNonIID@XVII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XVII@out}\newcommand\BsplineNonIID@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XVIII@out{\{"median": "0.12", "error plus": "0.88", "error minus": "0.56", "5th percentile": "{-}0.44", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XVIII@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XVIII@out{0.88}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XVIII@out{0.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XVIII@out{{-}0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XVIII@out{1.0}\else\def\BsplineNonIID@XVIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XVIII@out}\newcommand\BsplineNonIID@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XIX@out{\{"median": "0.071", "error plus": "0.82", "error minus": "0.92", "5th percentile": "{-}0.85", "95th percentile": "0.89"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XIX@out{0.071}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XIX@out{0.82}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XIX@out{0.92}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XIX@out{{-}0.85}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XIX@out{0.89}\else\def\BsplineNonIID@XIX@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XIX@out}\newcommand\BsplineNonIID@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XX@out{\{"median": "0.25", "error plus": "0.75", "error minus": "0.61", "5th percentile": "{-}0.36", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XX@out{0.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XX@out{0.75}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XX@out{0.61}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XX@out{{-}0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XX@out{1.0}\else\def\BsplineNonIID@XX@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XX@out}\newcommand\BsplineNonIID@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XXI@out{\{"median": "0.12", "error plus": "0.77", "error minus": "0.96", "5th percentile": "{-}0.84", "95th percentile": "0.89"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XXI@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XXI@out{0.77}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XXI@out{0.96}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XXI@out{{-}0.84}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XXI@out{0.89}\else\def\BsplineNonIID@XXI@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XXI@out}\newcommand\BsplineNonIID@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIID@XXII@out{\{"median": "1.5", "error plus": "0.84", "error minus": "1.1", "5th percentile": "0.41", "95th percentile": "2.3"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIID@XXII@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIID@XXII@out{0.84}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIID@XXII@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIID@XXII@out{0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIID@XXII@out{2.3}\else\def\BsplineNonIID@XXII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIID@XXII@out}\makeatother
\makeatletter\newcommand\BsplineNonIIDnoGW[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@out{\{"mass\_1": \{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}, "ppd": \{"median": "10", "error plus": "23", "error minus": "2.6", "5th percentile": "7.8", "95th percentile": "33"\}\}, "mass\_ratio": \{"peak": \{"median": "0.74", "error plus": "0.10", "error minus": "0.16", "5th percentile": "0.58", "95th percentile": "0.84"\}, "ppd": \{"median": "0.70", "error plus": "0.23", "error minus": "0.33", "5th percentile": "0.37", "95th percentile": "0.93"\}\}, "a\_1": \{"peak": \{"median": "0.11", "error plus": "0.15", "error minus": "0.11", "5th percentile": 0, "95th percentile": "0.26"\}, "ppd": \{"median": "0.28", "error plus": "0.62", "error minus": "0.25", "5th percentile": "0.028", "95th percentile": "0.90"\}\}, "a\_2": \{"peak": \{"median": "0.21", "error plus": "0.31", "error minus": "0.21", "5th percentile": 0, "95th percentile": "0.52"\}, "ppd": \{"median": "0.38", "error plus": "0.53", "error minus": "0.34", "5th percentile": "0.039", "95th percentile": "0.91"\}\}, "cos\_tilt\_1": \{"peak": \{"median": "0.099", "error plus": "0.90", "error minus": "0.49", "5th percentile": "{-}0.39", "95th percentile": "1.0"\}, "ppd": \{"median": "0.071", "error plus": "0.82", "error minus": "0.91", "5th percentile": "{-}0.84", "95th percentile": "0.89"\}\}, "cos\_tilt\_2": \{"peak": \{"median": "0.23", "error plus": "0.77", "error minus": "1.0", "5th percentile": "{-}0.79", "95th percentile": "1.0"\}, "ppd": \{"median": "0.11", "error plus": "0.77", "error minus": "0.97", "5th percentile": "{-}0.86", "95th percentile": "0.88"\}\}, "redshift": \{"ppd": \{"median": "1.7", "error plus": "0.65", "error minus": "1.2", "5th percentile": "0.50", "95th percentile": "2.3"\}\}, "rate\_at\_z\_0{-}2": \{"median": "43", "error plus": "37", "error minus": "13", "5th percentile": "30", "95th percentile": "80"\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@I\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@II\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@III\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@IV\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@V\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@VI\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@VII\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\BsplineNonIIDnoGW@out\BsplineNonIIDnoGW@VIII\else\def\BsplineNonIIDnoGW@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@out}\newcommand\BsplineNonIIDnoGW@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@I@out{\{"peak\_1\_location": \{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}, "peak\_2\_location": \{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}, "ppd": \{"median": "10", "error plus": "23", "error minus": "2.6", "5th percentile": "7.8", "95th percentile": "33"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\BsplineNonIIDnoGW@I@out\BsplineNonIIDnoGW@IX\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\BsplineNonIIDnoGW@I@out\BsplineNonIIDnoGW@X\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIIDnoGW@I@out\BsplineNonIIDnoGW@XI\else\def\BsplineNonIIDnoGW@I@out{??}\fi\fi\fi\fi\BsplineNonIIDnoGW@I@out}\newcommand\BsplineNonIIDnoGW@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@II@out{\{"peak": \{"median": "0.74", "error plus": "0.10", "error minus": "0.16", "5th percentile": "0.58", "95th percentile": "0.84"\}, "ppd": \{"median": "0.70", "error plus": "0.23", "error minus": "0.33", "5th percentile": "0.37", "95th percentile": "0.93"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIIDnoGW@II@out\BsplineNonIIDnoGW@XII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIIDnoGW@II@out\BsplineNonIIDnoGW@XIII\else\def\BsplineNonIIDnoGW@II@out{??}\fi\fi\fi\BsplineNonIIDnoGW@II@out}\newcommand\BsplineNonIIDnoGW@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@III@out{\{"peak": \{"median": "0.11", "error plus": "0.15", "error minus": "0.11", "5th percentile": 0, "95th percentile": "0.26"\}, "ppd": \{"median": "0.28", "error plus": "0.62", "error minus": "0.25", "5th percentile": "0.028", "95th percentile": "0.90"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIIDnoGW@III@out\BsplineNonIIDnoGW@XIV\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIIDnoGW@III@out\BsplineNonIIDnoGW@XV\else\def\BsplineNonIIDnoGW@III@out{??}\fi\fi\fi\BsplineNonIIDnoGW@III@out}\newcommand\BsplineNonIIDnoGW@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@IV@out{\{"peak": \{"median": "0.21", "error plus": "0.31", "error minus": "0.21", "5th percentile": 0, "95th percentile": "0.52"\}, "ppd": \{"median": "0.38", "error plus": "0.53", "error minus": "0.34", "5th percentile": "0.039", "95th percentile": "0.91"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIIDnoGW@IV@out\BsplineNonIIDnoGW@XVI\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIIDnoGW@IV@out\BsplineNonIIDnoGW@XVII\else\def\BsplineNonIIDnoGW@IV@out{??}\fi\fi\fi\BsplineNonIIDnoGW@IV@out}\newcommand\BsplineNonIIDnoGW@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@V@out{\{"peak": \{"median": "0.099", "error plus": "0.90", "error minus": "0.49", "5th percentile": "{-}0.39", "95th percentile": "1.0"\}, "ppd": \{"median": "0.071", "error plus": "0.82", "error minus": "0.91", "5th percentile": "{-}0.84", "95th percentile": "0.89"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIIDnoGW@V@out\BsplineNonIIDnoGW@XVIII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIIDnoGW@V@out\BsplineNonIIDnoGW@XIX\else\def\BsplineNonIIDnoGW@V@out{??}\fi\fi\fi\BsplineNonIIDnoGW@V@out}\newcommand\BsplineNonIIDnoGW@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@VI@out{\{"peak": \{"median": "0.23", "error plus": "0.77", "error minus": "1.0", "5th percentile": "{-}0.79", "95th percentile": "1.0"\}, "ppd": \{"median": "0.11", "error plus": "0.77", "error minus": "0.97", "5th percentile": "{-}0.86", "95th percentile": "0.88"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\BsplineNonIIDnoGW@VI@out\BsplineNonIIDnoGW@XX\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIIDnoGW@VI@out\BsplineNonIIDnoGW@XXI\else\def\BsplineNonIIDnoGW@VI@out{??}\fi\fi\fi\BsplineNonIIDnoGW@VI@out}\newcommand\BsplineNonIIDnoGW@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@VII@out{\{"ppd": \{"median": "1.7", "error plus": "0.65", "error minus": "1.2", "5th percentile": "0.50", "95th percentile": "2.3"\}\}}\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\BsplineNonIIDnoGW@VII@out\BsplineNonIIDnoGW@XXII\else\def\BsplineNonIIDnoGW@VII@out{??}\fi\fi\BsplineNonIIDnoGW@VII@out}\newcommand\BsplineNonIIDnoGW@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@VIII@out{\{"median": "43", "error plus": "37", "error minus": "13", "5th percentile": "30", "95th percentile": "80"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@VIII@out{43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@VIII@out{37}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@VIII@out{13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@VIII@out{30}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@VIII@out{80}\else\def\BsplineNonIIDnoGW@VIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@VIII@out}\newcommand\BsplineNonIIDnoGW@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@IX@out{\{"median": "10.1", "error plus": "0.7", "error minus": "0.7", "5th percentile": "9", "95th percentile": "10.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@IX@out{10.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@IX@out{0.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@IX@out{0.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@IX@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@IX@out{10.8}\else\def\BsplineNonIIDnoGW@IX@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@IX@out}\newcommand\BsplineNonIIDnoGW@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@X@out{\{"median": "33.5", "error plus": "2.2", "error minus": "4.5", "5th percentile": "29", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@X@out{33.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@X@out{2.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@X@out{4.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@X@out{29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@X@out{36}\else\def\BsplineNonIIDnoGW@X@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@X@out}\newcommand\BsplineNonIIDnoGW@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XI@out{\{"median": "10", "error plus": "23", "error minus": "2.6", "5th percentile": "7.8", "95th percentile": "33"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XI@out{10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XI@out{23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XI@out{2.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XI@out{7.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XI@out{33}\else\def\BsplineNonIIDnoGW@XI@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XI@out}\newcommand\BsplineNonIIDnoGW@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XII@out{\{"median": "0.74", "error plus": "0.10", "error minus": "0.16", "5th percentile": "0.58", "95th percentile": "0.84"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XII@out{0.74}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XII@out{0.10}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XII@out{0.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XII@out{0.58}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XII@out{0.84}\else\def\BsplineNonIIDnoGW@XII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XII@out}\newcommand\BsplineNonIIDnoGW@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XIII@out{\{"median": "0.70", "error plus": "0.23", "error minus": "0.33", "5th percentile": "0.37", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XIII@out{0.70}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XIII@out{0.23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XIII@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XIII@out{0.37}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XIII@out{0.93}\else\def\BsplineNonIIDnoGW@XIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XIII@out}\newcommand\BsplineNonIIDnoGW@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XIV@out{\{"median": "0.11", "error plus": "0.15", "error minus": "0.11", "5th percentile": 0, "95th percentile": "0.26"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XIV@out{0.11}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XIV@out{0.15}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XIV@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XIV@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XIV@out{0.26}\else\def\BsplineNonIIDnoGW@XIV@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XIV@out}\newcommand\BsplineNonIIDnoGW@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XV@out{\{"median": "0.28", "error plus": "0.62", "error minus": "0.25", "5th percentile": "0.028", "95th percentile": "0.90"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XV@out{0.28}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XV@out{0.62}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XV@out{0.25}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XV@out{0.028}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XV@out{0.90}\else\def\BsplineNonIIDnoGW@XV@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XV@out}\newcommand\BsplineNonIIDnoGW@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XVI@out{\{"median": "0.21", "error plus": "0.31", "error minus": "0.21", "5th percentile": 0, "95th percentile": "0.52"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XVI@out{0.21}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XVI@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XVI@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XVI@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XVI@out{0.52}\else\def\BsplineNonIIDnoGW@XVI@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XVI@out}\newcommand\BsplineNonIIDnoGW@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XVII@out{\{"median": "0.38", "error plus": "0.53", "error minus": "0.34", "5th percentile": "0.039", "95th percentile": "0.91"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XVII@out{0.38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XVII@out{0.53}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XVII@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XVII@out{0.039}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XVII@out{0.91}\else\def\BsplineNonIIDnoGW@XVII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XVII@out}\newcommand\BsplineNonIIDnoGW@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XVIII@out{\{"median": "0.099", "error plus": "0.90", "error minus": "0.49", "5th percentile": "{-}0.39", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XVIII@out{0.099}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XVIII@out{0.90}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XVIII@out{0.49}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XVIII@out{{-}0.39}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XVIII@out{1.0}\else\def\BsplineNonIIDnoGW@XVIII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XVIII@out}\newcommand\BsplineNonIIDnoGW@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XIX@out{\{"median": "0.071", "error plus": "0.82", "error minus": "0.91", "5th percentile": "{-}0.84", "95th percentile": "0.89"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XIX@out{0.071}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XIX@out{0.82}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XIX@out{0.91}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XIX@out{{-}0.84}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XIX@out{0.89}\else\def\BsplineNonIIDnoGW@XIX@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XIX@out}\newcommand\BsplineNonIIDnoGW@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XX@out{\{"median": "0.23", "error plus": "0.77", "error minus": "1.0", "5th percentile": "{-}0.79", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XX@out{0.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XX@out{0.77}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XX@out{1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XX@out{{-}0.79}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XX@out{1.0}\else\def\BsplineNonIIDnoGW@XX@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XX@out}\newcommand\BsplineNonIIDnoGW@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XXI@out{\{"median": "0.11", "error plus": "0.77", "error minus": "0.97", "5th percentile": "{-}0.86", "95th percentile": "0.88"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XXI@out{0.11}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XXI@out{0.77}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XXI@out{0.97}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XXI@out{{-}0.86}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XXI@out{0.88}\else\def\BsplineNonIIDnoGW@XXI@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XXI@out}\newcommand\BsplineNonIIDnoGW@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\BsplineNonIIDnoGW@XXII@out{\{"median": "1.7", "error plus": "0.65", "error minus": "1.2", "5th percentile": "0.50", "95th percentile": "2.3"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\BsplineNonIIDnoGW@XXII@out{1.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\BsplineNonIIDnoGW@XXII@out{0.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\BsplineNonIIDnoGW@XXII@out{1.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\BsplineNonIIDnoGW@XXII@out{0.50}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\BsplineNonIIDnoGW@XXII@out{2.3}\else\def\BsplineNonIIDnoGW@XXII@out{??}\fi\fi\fi\fi\fi\fi\BsplineNonIIDnoGW@XXII@out}\makeatother
\makeatletter\newcommand\counts[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\counts@out{\{"FAROnePerYear": \{"O4aBNS": 0, "O4aNSBH": 1, "O4aBBH": 84, "O4aTotal": 85, "O3bBNS": 0, "O3bNSBH": 2, "O3bBBH": 23, "O3bTotal": 25, "O3aBNS": 1, "O3aNSBH": 2, "O3aBBH": 36, "O3aTotal": 39, "O2BNS": 1, "O2NSBH": 0, "O2BBH": 7, "O2Total": 8, "O1BNS": 0, "O1NSBH": 0, "O1BBH": 3, "O1Total": 3, "totalBNS": 2, "totalNSBH": 5, "totalBBH": 153, "total": 160\}, "FAROnePerFourYears": \{"O4aBNS": 0, "O4aNSBH": 1, "O4aBBH": 76, "O4aTotal": 77, "O3bBNS": 0, "O3bNSBH": 2, "O3bBBH": 21, "O3bTotal": 23, "O3aBNS": 1, "O3aNSBH": 0, "O3aBBH": 31, "O3aTotal": 32, "O2BNS": 1, "O2NSBH": 0, "O2BBH": 7, "O2Total": 8, "O1BNS": 0, "O1NSBH": 0, "O1BBH": 3, "O1Total": 3, "totalBNS": 2, "totalNSBH": 3, "totalBBH": 138, "total": 143\}, "combined": \{"total": 158\}\}}\else\ifnum\pdfstrcmp{#1}{FAROnePerYear}=0\let\counts@out\counts@I\else\ifnum\pdfstrcmp{#1}{FAROnePerFourYears}=0\let\counts@out\counts@II\else\ifnum\pdfstrcmp{#1}{combined}=0\let\counts@out\counts@III\else\def\counts@out{??}\fi\fi\fi\fi\counts@out}\newcommand\counts@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\counts@I@out{\{"O4aBNS": 0, "O4aNSBH": 1, "O4aBBH": 84, "O4aTotal": 85, "O3bBNS": 0, "O3bNSBH": 2, "O3bBBH": 23, "O3bTotal": 25, "O3aBNS": 1, "O3aNSBH": 2, "O3aBBH": 36, "O3aTotal": 39, "O2BNS": 1, "O2NSBH": 0, "O2BBH": 7, "O2Total": 8, "O1BNS": 0, "O1NSBH": 0, "O1BBH": 3, "O1Total": 3, "totalBNS": 2, "totalNSBH": 5, "totalBBH": 153, "total": 160\}}\else\ifnum\pdfstrcmp{#1}{O4aBNS}=0\def\counts@I@out{0}\else\ifnum\pdfstrcmp{#1}{O4aNSBH}=0\def\counts@I@out{1}\else\ifnum\pdfstrcmp{#1}{O4aBBH}=0\def\counts@I@out{84}\else\ifnum\pdfstrcmp{#1}{O4aTotal}=0\def\counts@I@out{85}\else\ifnum\pdfstrcmp{#1}{O3bBNS}=0\def\counts@I@out{0}\else\ifnum\pdfstrcmp{#1}{O3bNSBH}=0\def\counts@I@out{2}\else\ifnum\pdfstrcmp{#1}{O3bBBH}=0\def\counts@I@out{23}\else\ifnum\pdfstrcmp{#1}{O3bTotal}=0\def\counts@I@out{25}\else\ifnum\pdfstrcmp{#1}{O3aBNS}=0\def\counts@I@out{1}\else\ifnum\pdfstrcmp{#1}{O3aNSBH}=0\def\counts@I@out{2}\else\ifnum\pdfstrcmp{#1}{O3aBBH}=0\def\counts@I@out{36}\else\ifnum\pdfstrcmp{#1}{O3aTotal}=0\def\counts@I@out{39}\else\ifnum\pdfstrcmp{#1}{O2BNS}=0\def\counts@I@out{1}\else\ifnum\pdfstrcmp{#1}{O2NSBH}=0\def\counts@I@out{0}\else\ifnum\pdfstrcmp{#1}{O2BBH}=0\def\counts@I@out{7}\else\ifnum\pdfstrcmp{#1}{O2Total}=0\def\counts@I@out{8}\else\ifnum\pdfstrcmp{#1}{O1BNS}=0\def\counts@I@out{0}\else\ifnum\pdfstrcmp{#1}{O1NSBH}=0\def\counts@I@out{0}\else\ifnum\pdfstrcmp{#1}{O1BBH}=0\def\counts@I@out{3}\else\ifnum\pdfstrcmp{#1}{O1Total}=0\def\counts@I@out{3}\else\ifnum\pdfstrcmp{#1}{totalBNS}=0\def\counts@I@out{2}\else\ifnum\pdfstrcmp{#1}{totalNSBH}=0\def\counts@I@out{5}\else\ifnum\pdfstrcmp{#1}{totalBBH}=0\def\counts@I@out{153}\else\ifnum\pdfstrcmp{#1}{total}=0\def\counts@I@out{160}\else\def\counts@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\counts@I@out}\newcommand\counts@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\counts@II@out{\{"O4aBNS": 0, "O4aNSBH": 1, "O4aBBH": 76, "O4aTotal": 77, "O3bBNS": 0, "O3bNSBH": 2, "O3bBBH": 21, "O3bTotal": 23, "O3aBNS": 1, "O3aNSBH": 0, "O3aBBH": 31, "O3aTotal": 32, "O2BNS": 1, "O2NSBH": 0, "O2BBH": 7, "O2Total": 8, "O1BNS": 0, "O1NSBH": 0, "O1BBH": 3, "O1Total": 3, "totalBNS": 2, "totalNSBH": 3, "totalBBH": 138, "total": 143\}}\else\ifnum\pdfstrcmp{#1}{O4aBNS}=0\def\counts@II@out{0}\else\ifnum\pdfstrcmp{#1}{O4aNSBH}=0\def\counts@II@out{1}\else\ifnum\pdfstrcmp{#1}{O4aBBH}=0\def\counts@II@out{76}\else\ifnum\pdfstrcmp{#1}{O4aTotal}=0\def\counts@II@out{77}\else\ifnum\pdfstrcmp{#1}{O3bBNS}=0\def\counts@II@out{0}\else\ifnum\pdfstrcmp{#1}{O3bNSBH}=0\def\counts@II@out{2}\else\ifnum\pdfstrcmp{#1}{O3bBBH}=0\def\counts@II@out{21}\else\ifnum\pdfstrcmp{#1}{O3bTotal}=0\def\counts@II@out{23}\else\ifnum\pdfstrcmp{#1}{O3aBNS}=0\def\counts@II@out{1}\else\ifnum\pdfstrcmp{#1}{O3aNSBH}=0\def\counts@II@out{0}\else\ifnum\pdfstrcmp{#1}{O3aBBH}=0\def\counts@II@out{31}\else\ifnum\pdfstrcmp{#1}{O3aTotal}=0\def\counts@II@out{32}\else\ifnum\pdfstrcmp{#1}{O2BNS}=0\def\counts@II@out{1}\else\ifnum\pdfstrcmp{#1}{O2NSBH}=0\def\counts@II@out{0}\else\ifnum\pdfstrcmp{#1}{O2BBH}=0\def\counts@II@out{7}\else\ifnum\pdfstrcmp{#1}{O2Total}=0\def\counts@II@out{8}\else\ifnum\pdfstrcmp{#1}{O1BNS}=0\def\counts@II@out{0}\else\ifnum\pdfstrcmp{#1}{O1NSBH}=0\def\counts@II@out{0}\else\ifnum\pdfstrcmp{#1}{O1BBH}=0\def\counts@II@out{3}\else\ifnum\pdfstrcmp{#1}{O1Total}=0\def\counts@II@out{3}\else\ifnum\pdfstrcmp{#1}{totalBNS}=0\def\counts@II@out{2}\else\ifnum\pdfstrcmp{#1}{totalNSBH}=0\def\counts@II@out{3}\else\ifnum\pdfstrcmp{#1}{totalBBH}=0\def\counts@II@out{138}\else\ifnum\pdfstrcmp{#1}{total}=0\def\counts@II@out{143}\else\def\counts@II@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\counts@II@out}\newcommand\counts@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\counts@III@out{\{"total": 158\}}\else\ifnum\pdfstrcmp{#1}{total}=0\def\counts@III@out{158}\else\def\counts@III@out{??}\fi\fi\counts@III@out}\makeatother
\makeatletter\newcommand\DefaultBBHDominantMode[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@out{\{"alpha\_1": \{"median": "1.7", "error plus": "1.1", "error minus": "1.8", "5th percentile": "{-}0.036", "95th percentile": "2.8"\}, "alpha\_2": \{"median": "4.6", "error plus": "1.5", "error minus": "1.2", "5th percentile": "3.4", "95th percentile": "6.1"\}, "beta": \{"median": "1.2", "error plus": "1.2", "error minus": "0.99", "5th percentile": "0.17", "95th percentile": "2.4"\}, "mlow\_1": \{"median": "5.0", "error plus": "3.2", "error minus": "1.8", "5th percentile": "3.2", "95th percentile": "8.2"\}, "mlow\_2": \{"median": "3.6", "error plus": "1.4", "error minus": "0.53", "5th percentile": "3.0", "95th percentile": "4.9"\}, "break\_mass": \{"median": "36", "error plus": "12", "error minus": "13", "5th percentile": "23", "95th percentile": "48"\}, "mpp\_1": \{"median": "9.8", "error plus": "0.51", "error minus": "1.3", "5th percentile": "8.5", "95th percentile": "10"\}, "mpp\_2": \{"median": "33", "error plus": "2.8", "error minus": "2.1", "5th percentile": "31", "95th percentile": "36"\}, "sigpp\_1": \{"median": "0.65", "error plus": "0.96", "error minus": "0.34", "5th percentile": "0.30", "95th percentile": "1.6"\}, "sigpp\_2": \{"median": "3.1", "error plus": "2.7", "error minus": "2.0", "5th percentile": "1.1", "95th percentile": "5.9"\}, "delta\_m\_1": \{"median": "4.3", "error plus": "4.9", "error minus": "4.0", "5th percentile": "0.32", "95th percentile": "9.2"\}, "delta\_m\_2": \{"median": "5.0", "error plus": "3.9", "error minus": "4.4", "5th percentile": "0.54", "95th percentile": "8.9"\}, "lam\_0": \{"median": "0.38", "error plus": "0.27", "error minus": "0.21", "5th percentile": "0.18", "95th percentile": "0.65"\}, "lam\_1": \{"median": "0.57", "error plus": "0.22", "error minus": "0.26", "5th percentile": "0.32", "95th percentile": "0.79"\}, "mu\_chi": \{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}, "sigma\_chi": \{"median": "0.33", "error plus": "0.079", "error minus": "0.078", "5th percentile": "0.25", "95th percentile": "0.41"\}, "xi\_spin": \{"median": "0.65", "error plus": "0.32", "error minus": "0.53", "5th percentile": "0.12", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.42", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}, "sigma\_spin": \{"median": "1.2", "error plus": "2.4", "error minus": "0.78", "5th percentile": "0.44", "95th percentile": "3.6"\}, "lamb": \{"median": "3.1", "error plus": "0.95", "error minus": "0.99", "5th percentile": "2.1", "95th percentile": "4.1"\}, "rate": \{"median": "16", "error plus": "5.8", "error minus": "4.3", "5th percentile": "12", "95th percentile": "22"\}, "mass\_1": \{"powerlaw\_slope\_18{-}19": \{"median": "1.7", "error plus": "1.1", "error minus": "1.7", "5th percentile": "{-}0.0049", "95th percentile": "2.8"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "33.3", "error plus": "2.1", "error minus": "2.7", "5th percentile": "31", "95th percentile": "35"\}, "peak\_2\_percent": 95.7\}, "alpha\_diff": \{"median": "{-}3.0", "error plus": "1.9", "error minus": "2.2", "5th percentile": "{-}5.1", "95th percentile": "{-}1.0"\}, "alpha\_diff\_perc": 99.0, "mass\_ratio": \{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}, "a\_1": \{"peak": \{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}, "a\_2": \{"peak": \{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}, "cos\_tilt\_1": \{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}\}, "cos\_tilt\_2": \{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}\}, "redshift": \{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.5", "error minus": "6.5", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.39", "error minus": "0.98", "5th percentile": "0.50", "95th percentile": "1.9"\}\}, "mu\_plus\_sig": \{"median": "37", "error plus": "3.9", "error minus": "2.9", "5th percentile": "34", "95th percentile": "41"\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@I\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@II\else\ifnum\pdfstrcmp{#1}{beta}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@III\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@IV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@VI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@VII\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@VIII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@IX\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@X\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XI\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XIII\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XIV\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XV\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XVI\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XVII\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XIX\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XX\else\ifnum\pdfstrcmp{#1}{rate}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXI\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXII\else\ifnum\pdfstrcmp{#1}{alpha_diff}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXIII\else\ifnum\pdfstrcmp{#1}{alpha_diff_perc}=0\def\DefaultBBHDominantMode@out{99.0}\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXIV\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXV\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXVI\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXVII\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXVIII\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXIX\else\ifnum\pdfstrcmp{#1}{mu_plus_sig}=0\let\DefaultBBHDominantMode@out\DefaultBBHDominantMode@XXX\else\def\DefaultBBHDominantMode@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@out}\newcommand\DefaultBBHDominantMode@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@I@out{\{"median": "1.7", "error plus": "1.1", "error minus": "1.8", "5th percentile": "{-}0.036", "95th percentile": "2.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@I@out{1.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@I@out{1.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@I@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@I@out{{-}0.036}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@I@out{2.8}\else\def\DefaultBBHDominantMode@I@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@I@out}\newcommand\DefaultBBHDominantMode@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@II@out{\{"median": "4.6", "error plus": "1.5", "error minus": "1.2", "5th percentile": "3.4", "95th percentile": "6.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@II@out{4.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@II@out{1.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@II@out{1.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@II@out{3.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@II@out{6.1}\else\def\DefaultBBHDominantMode@II@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@II@out}\newcommand\DefaultBBHDominantMode@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@III@out{\{"median": "1.2", "error plus": "1.2", "error minus": "0.99", "5th percentile": "0.17", "95th percentile": "2.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@III@out{0.99}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@III@out{0.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@III@out{2.4}\else\def\DefaultBBHDominantMode@III@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@III@out}\newcommand\DefaultBBHDominantMode@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@IV@out{\{"median": "5.0", "error plus": "3.2", "error minus": "1.8", "5th percentile": "3.2", "95th percentile": "8.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@IV@out{5.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@IV@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@IV@out{8.2}\else\def\DefaultBBHDominantMode@IV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@IV@out}\newcommand\DefaultBBHDominantMode@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@V@out{\{"median": "3.6", "error plus": "1.4", "error minus": "0.53", "5th percentile": "3.0", "95th percentile": "4.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@V@out{3.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@V@out{1.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@V@out{0.53}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@V@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@V@out{4.9}\else\def\DefaultBBHDominantMode@V@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@V@out}\newcommand\DefaultBBHDominantMode@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@VI@out{\{"median": "36", "error plus": "12", "error minus": "13", "5th percentile": "23", "95th percentile": "48"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@VI@out{36}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@VI@out{12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@VI@out{13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@VI@out{23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@VI@out{48}\else\def\DefaultBBHDominantMode@VI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@VI@out}\newcommand\DefaultBBHDominantMode@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@VII@out{\{"median": "9.8", "error plus": "0.51", "error minus": "1.3", "5th percentile": "8.5", "95th percentile": "10"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@VII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@VII@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@VII@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@VII@out{8.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@VII@out{10}\else\def\DefaultBBHDominantMode@VII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@VII@out}\newcommand\DefaultBBHDominantMode@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@VIII@out{\{"median": "33", "error plus": "2.8", "error minus": "2.1", "5th percentile": "31", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@VIII@out{33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@VIII@out{2.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@VIII@out{2.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@VIII@out{31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@VIII@out{36}\else\def\DefaultBBHDominantMode@VIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@VIII@out}\newcommand\DefaultBBHDominantMode@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@IX@out{\{"median": "0.65", "error plus": "0.96", "error minus": "0.34", "5th percentile": "0.30", "95th percentile": "1.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@IX@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@IX@out{0.96}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@IX@out{0.30}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@IX@out{1.6}\else\def\DefaultBBHDominantMode@IX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@IX@out}\newcommand\DefaultBBHDominantMode@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@X@out{\{"median": "3.1", "error plus": "2.7", "error minus": "2.0", "5th percentile": "1.1", "95th percentile": "5.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@X@out{3.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@X@out{2.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@X@out{2.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@X@out{1.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@X@out{5.9}\else\def\DefaultBBHDominantMode@X@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@X@out}\newcommand\DefaultBBHDominantMode@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XI@out{\{"median": "4.3", "error plus": "4.9", "error minus": "4.0", "5th percentile": "0.32", "95th percentile": "9.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XI@out{4.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XI@out{4.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XI@out{4.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XI@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XI@out{9.2}\else\def\DefaultBBHDominantMode@XI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XI@out}\newcommand\DefaultBBHDominantMode@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XII@out{\{"median": "5.0", "error plus": "3.9", "error minus": "4.4", "5th percentile": "0.54", "95th percentile": "8.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XII@out{5.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XII@out{3.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XII@out{4.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XII@out{0.54}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XII@out{8.9}\else\def\DefaultBBHDominantMode@XII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XII@out}\newcommand\DefaultBBHDominantMode@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XIII@out{\{"median": "0.38", "error plus": "0.27", "error minus": "0.21", "5th percentile": "0.18", "95th percentile": "0.65"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XIII@out{0.38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XIII@out{0.27}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XIII@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XIII@out{0.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XIII@out{0.65}\else\def\DefaultBBHDominantMode@XIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XIII@out}\newcommand\DefaultBBHDominantMode@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XIV@out{\{"median": "0.57", "error plus": "0.22", "error minus": "0.26", "5th percentile": "0.32", "95th percentile": "0.79"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XIV@out{0.57}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XIV@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XIV@out{0.26}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XIV@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XIV@out{0.79}\else\def\DefaultBBHDominantMode@XIV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XIV@out}\newcommand\DefaultBBHDominantMode@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XV@out{\{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XV@out{0.088}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XV@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XV@out{0.080}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XV@out{0.0080}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XV@out{0.22}\else\def\DefaultBBHDominantMode@XV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XV@out}\newcommand\DefaultBBHDominantMode@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XVI@out{\{"median": "0.33", "error plus": "0.079", "error minus": "0.078", "5th percentile": "0.25", "95th percentile": "0.41"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XVI@out{0.33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XVI@out{0.079}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XVI@out{0.078}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XVI@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XVI@out{0.41}\else\def\DefaultBBHDominantMode@XVI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XVI@out}\newcommand\DefaultBBHDominantMode@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XVII@out{\{"median": "0.65", "error plus": "0.32", "error minus": "0.53", "5th percentile": "0.12", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XVII@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XVII@out{0.32}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XVII@out{0.53}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XVII@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XVII@out{0.97}\else\def\DefaultBBHDominantMode@XVII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XVII@out}\newcommand\DefaultBBHDominantMode@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XVIII@out{\{"median": "0.42", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XVIII@out{0.42}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XVIII@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XVIII@out{0.83}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XVIII@out{{-}0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XVIII@out{0.94}\else\def\DefaultBBHDominantMode@XVIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XVIII@out}\newcommand\DefaultBBHDominantMode@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XIX@out{\{"median": "1.2", "error plus": "2.4", "error minus": "0.78", "5th percentile": "0.44", "95th percentile": "3.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XIX@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XIX@out{2.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XIX@out{0.78}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XIX@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XIX@out{3.6}\else\def\DefaultBBHDominantMode@XIX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XIX@out}\newcommand\DefaultBBHDominantMode@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XX@out{\{"median": "3.1", "error plus": "0.95", "error minus": "0.99", "5th percentile": "2.1", "95th percentile": "4.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XX@out{3.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XX@out{0.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XX@out{0.99}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XX@out{2.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XX@out{4.1}\else\def\DefaultBBHDominantMode@XX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XX@out}\newcommand\DefaultBBHDominantMode@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXI@out{\{"median": "16", "error plus": "5.8", "error minus": "4.3", "5th percentile": "12", "95th percentile": "22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXI@out{16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXI@out{5.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXI@out{4.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXI@out{12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXI@out{22}\else\def\DefaultBBHDominantMode@XXI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXI@out}\newcommand\DefaultBBHDominantMode@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXII@out{\{"powerlaw\_slope\_18{-}19": \{"median": "1.7", "error plus": "1.1", "error minus": "1.7", "5th percentile": "{-}0.0049", "95th percentile": "2.8"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "33.3", "error plus": "2.1", "error minus": "2.7", "5th percentile": "31", "95th percentile": "35"\}, "peak\_2\_percent": 95.7\}}\else\ifnum\pdfstrcmp{#1}{powerlaw_slope_18-19}=0\let\DefaultBBHDominantMode@XXII@out\DefaultBBHDominantMode@XXXI\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\DefaultBBHDominantMode@XXII@out\DefaultBBHDominantMode@XXXII\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\DefaultBBHDominantMode@XXII@out\DefaultBBHDominantMode@XXXIII\else\ifnum\pdfstrcmp{#1}{peak_2_percent}=0\def\DefaultBBHDominantMode@XXII@out{95.7}\else\def\DefaultBBHDominantMode@XXII@out{??}\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXII@out}\newcommand\DefaultBBHDominantMode@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXIII@out{\{"median": "{-}3.0", "error plus": "1.9", "error minus": "2.2", "5th percentile": "{-}5.1", "95th percentile": "{-}1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXIII@out{{-}3.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXIII@out{1.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXIII@out{2.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXIII@out{{-}5.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXIII@out{{-}1.0}\else\def\DefaultBBHDominantMode@XXIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXIII@out}\newcommand\DefaultBBHDominantMode@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXIV@out{\{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHDominantMode@XXIV@out\DefaultBBHDominantMode@XXXIV\else\def\DefaultBBHDominantMode@XXIV@out{??}\fi\fi\DefaultBBHDominantMode@XXIV@out}\newcommand\DefaultBBHDominantMode@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXV@out{\{"peak": \{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHDominantMode@XXV@out\DefaultBBHDominantMode@XXXV\else\def\DefaultBBHDominantMode@XXV@out{??}\fi\fi\DefaultBBHDominantMode@XXV@out}\newcommand\DefaultBBHDominantMode@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXVI@out{\{"peak": \{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHDominantMode@XXVI@out\DefaultBBHDominantMode@XXXVI\else\def\DefaultBBHDominantMode@XXVI@out{??}\fi\fi\DefaultBBHDominantMode@XXVI@out}\newcommand\DefaultBBHDominantMode@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXVII@out{\{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHDominantMode@XXVII@out\DefaultBBHDominantMode@XXXVII\else\def\DefaultBBHDominantMode@XXVII@out{??}\fi\fi\DefaultBBHDominantMode@XXVII@out}\newcommand\DefaultBBHDominantMode@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXVIII@out{\{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHDominantMode@XXVIII@out\DefaultBBHDominantMode@XXXVIII\else\def\DefaultBBHDominantMode@XXVIII@out{??}\fi\fi\DefaultBBHDominantMode@XXVIII@out}\newcommand\DefaultBBHDominantMode@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXIX@out{\{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.5", "error minus": "6.5", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.39", "error minus": "0.98", "5th percentile": "0.50", "95th percentile": "1.9"\}\}}\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\DefaultBBHDominantMode@XXIX@out\DefaultBBHDominantMode@XXXIX\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\DefaultBBHDominantMode@XXIX@out\DefaultBBHDominantMode@XL\else\def\DefaultBBHDominantMode@XXIX@out{??}\fi\fi\fi\DefaultBBHDominantMode@XXIX@out}\newcommand\DefaultBBHDominantMode@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXX@out{\{"median": "37", "error plus": "3.9", "error minus": "2.9", "5th percentile": "34", "95th percentile": "41"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXX@out{37}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXX@out{3.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXX@out{2.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXX@out{34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXX@out{41}\else\def\DefaultBBHDominantMode@XXX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXX@out}\newcommand\DefaultBBHDominantMode@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXI@out{\{"median": "1.7", "error plus": "1.1", "error minus": "1.7", "5th percentile": "{-}0.0049", "95th percentile": "2.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXI@out{1.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXI@out{1.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXI@out{1.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXI@out{{-}0.0049}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXI@out{2.8}\else\def\DefaultBBHDominantMode@XXXI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXI@out}\newcommand\DefaultBBHDominantMode@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXII@out{\{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXII@out{0.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXII@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXII@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXII@out{10.1}\else\def\DefaultBBHDominantMode@XXXII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXII@out}\newcommand\DefaultBBHDominantMode@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXIII@out{\{"median": "33.3", "error plus": "2.1", "error minus": "2.7", "5th percentile": "31", "95th percentile": "35"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXIII@out{33.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXIII@out{2.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXIII@out{2.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXIII@out{31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXIII@out{35}\else\def\DefaultBBHDominantMode@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXIII@out}\newcommand\DefaultBBHDominantMode@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXIV@out{\{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXIV@out{1.0}\else\def\DefaultBBHDominantMode@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXIV@out}\newcommand\DefaultBBHDominantMode@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXV@out{\{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXV@out{0.088}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXV@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXV@out{0.080}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXV@out{0.0080}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXV@out{0.22}\else\def\DefaultBBHDominantMode@XXXV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXV@out}\newcommand\DefaultBBHDominantMode@XXXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXVI@out{\{"median": "0.088", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0080", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXVI@out{0.088}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXVI@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXVI@out{0.080}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXVI@out{0.0080}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXVI@out{0.22}\else\def\DefaultBBHDominantMode@XXXVI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXVI@out}\newcommand\DefaultBBHDominantMode@XXXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXVII@out{\{"median": "0.43", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXVII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXVII@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXVII@out{0.83}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXVII@out{{-}0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXVII@out{0.94}\else\def\DefaultBBHDominantMode@XXXVII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXVII@out}\newcommand\DefaultBBHDominantMode@XXXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXVIII@out{\{"median": "0.43", "error plus": "0.51", "error minus": "0.83", "5th percentile": "{-}0.40", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXVIII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXVIII@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXVIII@out{0.83}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXVIII@out{{-}0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXVIII@out{0.94}\else\def\DefaultBBHDominantMode@XXXVIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXVIII@out}\newcommand\DefaultBBHDominantMode@XXXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XXXIX@out{\{"median": "29", "error plus": "8.5", "error minus": "6.5", "5th percentile": "22", "95th percentile": "37"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XXXIX@out{29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XXXIX@out{8.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XXXIX@out{6.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XXXIX@out{22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XXXIX@out{37}\else\def\DefaultBBHDominantMode@XXXIX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XXXIX@out}\newcommand\DefaultBBHDominantMode@XL[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHDominantMode@XL@out{\{"median": "1.5", "error plus": "0.39", "error minus": "0.98", "5th percentile": "0.50", "95th percentile": "1.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHDominantMode@XL@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHDominantMode@XL@out{0.39}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHDominantMode@XL@out{0.98}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHDominantMode@XL@out{0.50}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHDominantMode@XL@out{1.9}\else\def\DefaultBBHDominantMode@XL@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHDominantMode@XL@out}\makeatother
\makeatletter\newcommand\defaultbbhgwtcthree[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@out{\{"alpha\_1": \{"median": "1.5", "error plus": "3.7", "error minus": "4.1", "5th percentile": "{-}2.6", "95th percentile": "5.3"\}, "alpha\_2": \{"median": "4.2", "error plus": "3.7", "error minus": "5.7", "5th percentile": "{-}1.5", "95th percentile": "7.9"\}, "beta": \{"median": "1.4", "error plus": "2.2", "error minus": "1.4", "5th percentile": "{-}0.075", "95th percentile": "3.6"\}, "mlow\_1": \{"median": "5.1", "error plus": "3.6", "error minus": "1.9", "5th percentile": "3.2", "95th percentile": "8.7"\}, "mlow\_2": \{"median": "3.5", "error plus": "1.3", "error minus": "0.46", "5th percentile": "3.0", "95th percentile": "4.8"\}, "break\_mass": \{"median": "34", "error plus": "13", "error minus": "13", "5th percentile": "22", "95th percentile": "48"\}, "mpp\_1": \{"median": "10", "error plus": "0.63", "error minus": "2.2", "5th percentile": "7.9", "95th percentile": "11"\}, "mpp\_2": \{"median": "31", "error plus": "5.0", "error minus": "4.9", "5th percentile": "26", "95th percentile": "36"\}, "sigpp\_1": \{"median": "0.67", "error plus": "1.6", "error minus": "0.44", "5th percentile": "0.22", "95th percentile": "2.2"\}, "sigpp\_2": \{"median": "6.5", "error plus": "3.1", "error minus": "4.9", "5th percentile": "1.6", "95th percentile": "9.7"\}, "delta\_m\_1": \{"median": "4.1", "error plus": "5.0", "error minus": "3.8", "5th percentile": "0.30", "95th percentile": "9.2"\}, "delta\_m\_2": \{"median": "3.9", "error plus": "5.1", "error minus": "3.6", "5th percentile": "0.32", "95th percentile": "9.0"\}, "lam\_0": \{"median": "0.25", "error plus": "0.39", "error minus": "0.21", "5th percentile": "0.041", "95th percentile": "0.63"\}, "lam\_1": \{"median": "0.65", "error plus": "0.20", "error minus": "0.36", "5th percentile": "0.29", "95th percentile": "0.85"\}, "mu\_chi": \{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.012", "95th percentile": "0.26"\}, "sigma\_chi": \{"median": "0.28", "error plus": "0.11", "error minus": "0.096", "5th percentile": "0.19", "95th percentile": "0.40"\}, "xi\_spin": \{"median": "0.60", "error plus": "0.36", "error minus": "0.51", "5th percentile": "0.092", "95th percentile": "0.96"\}, "mu\_spin": \{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}, "sigma\_spin": \{"median": "1.3", "error plus": "2.4", "error minus": "0.93", "5th percentile": "0.40", "95th percentile": "3.7"\}, "lamb": \{"median": "2.6", "error plus": "1.8", "error minus": "1.8", "5th percentile": "0.87", "95th percentile": "4.4"\}, "rate": \{"median": "17", "error plus": "10", "error minus": "6.5", "5th percentile": "11", "95th percentile": "28"\}, "mass\_1": \{"powerlaw\_slope\_18{-}19": \{"median": "0.0049", "error plus": "2.8", "error minus": "3.0", "5th percentile": "{-}3.0", "95th percentile": "2.8"\}, "peak\_1\_location": \{"median": "10", "error plus": "0.6", "error minus": "1.0", "5th percentile": "9", "95th percentile": "10.7"\}, "peak\_2\_location": \{"median": "30.7", "error plus": "4.6", "error minus": "5.3", "5th percentile": "25", "95th percentile": "35"\}, "peak\_2\_percent": 95.19999999999999\}, "alpha\_diff": \{"median": "{-}3.2", "error plus": "8.8", "error minus": "5.1", "5th percentile": "{-}8.2", "95th percentile": "5.6"\}, "alpha\_diff\_perc": 78.0, "mass\_ratio": \{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}, "a\_1": \{"peak": \{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.013", "95th percentile": "0.26"\}\}, "a\_2": \{"peak": \{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.013", "95th percentile": "0.26"\}\}, "cos\_tilt\_1": \{"peak": \{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}\}, "cos\_tilt\_2": \{"peak": \{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}\}, "redshift": \{"rate\_at\_z\_0{-}2": \{"median": "28", "error plus": "12", "error minus": "8.8", "5th percentile": "19", "95th percentile": "40"\}, "ppd": \{"median": "1.5", "error plus": "0.39", "error minus": "1.0", "5th percentile": "0.47", "95th percentile": "1.9"\}\}, "mu\_plus\_sig": \{"median": "37", "error plus": "4.6", "error minus": "3.5", "5th percentile": "34", "95th percentile": "42"\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@I\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@II\else\ifnum\pdfstrcmp{#1}{beta}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@III\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@IV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@VI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@VII\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@VIII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@IX\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@X\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XI\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XIII\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XIV\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XV\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XVI\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XVII\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XIX\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XX\else\ifnum\pdfstrcmp{#1}{rate}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXI\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXII\else\ifnum\pdfstrcmp{#1}{alpha_diff}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXIII\else\ifnum\pdfstrcmp{#1}{alpha_diff_perc}=0\def\defaultbbhgwtcthree@out{78.0}\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXIV\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXV\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXVI\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXVII\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXVIII\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXIX\else\ifnum\pdfstrcmp{#1}{mu_plus_sig}=0\let\defaultbbhgwtcthree@out\defaultbbhgwtcthree@XXX\else\def\defaultbbhgwtcthree@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@out}\newcommand\defaultbbhgwtcthree@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@I@out{\{"median": "1.5", "error plus": "3.7", "error minus": "4.1", "5th percentile": "{-}2.6", "95th percentile": "5.3"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@I@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@I@out{3.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@I@out{4.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@I@out{{-}2.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@I@out{5.3}\else\def\defaultbbhgwtcthree@I@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@I@out}\newcommand\defaultbbhgwtcthree@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@II@out{\{"median": "4.2", "error plus": "3.7", "error minus": "5.7", "5th percentile": "{-}1.5", "95th percentile": "7.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@II@out{4.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@II@out{3.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@II@out{5.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@II@out{{-}1.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@II@out{7.9}\else\def\defaultbbhgwtcthree@II@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@II@out}\newcommand\defaultbbhgwtcthree@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@III@out{\{"median": "1.4", "error plus": "2.2", "error minus": "1.4", "5th percentile": "{-}0.075", "95th percentile": "3.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@III@out{1.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@III@out{2.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@III@out{1.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@III@out{{-}0.075}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@III@out{3.6}\else\def\defaultbbhgwtcthree@III@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@III@out}\newcommand\defaultbbhgwtcthree@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@IV@out{\{"median": "5.1", "error plus": "3.6", "error minus": "1.9", "5th percentile": "3.2", "95th percentile": "8.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@IV@out{5.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@IV@out{3.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@IV@out{1.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@IV@out{8.7}\else\def\defaultbbhgwtcthree@IV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@IV@out}\newcommand\defaultbbhgwtcthree@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@V@out{\{"median": "3.5", "error plus": "1.3", "error minus": "0.46", "5th percentile": "3.0", "95th percentile": "4.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@V@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@V@out{1.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@V@out{0.46}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@V@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@V@out{4.8}\else\def\defaultbbhgwtcthree@V@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@V@out}\newcommand\defaultbbhgwtcthree@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@VI@out{\{"median": "34", "error plus": "13", "error minus": "13", "5th percentile": "22", "95th percentile": "48"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@VI@out{34}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@VI@out{13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@VI@out{13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@VI@out{22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@VI@out{48}\else\def\defaultbbhgwtcthree@VI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@VI@out}\newcommand\defaultbbhgwtcthree@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@VII@out{\{"median": "10", "error plus": "0.63", "error minus": "2.2", "5th percentile": "7.9", "95th percentile": "11"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@VII@out{10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@VII@out{0.63}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@VII@out{2.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@VII@out{7.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@VII@out{11}\else\def\defaultbbhgwtcthree@VII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@VII@out}\newcommand\defaultbbhgwtcthree@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@VIII@out{\{"median": "31", "error plus": "5.0", "error minus": "4.9", "5th percentile": "26", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@VIII@out{31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@VIII@out{5.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@VIII@out{4.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@VIII@out{26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@VIII@out{36}\else\def\defaultbbhgwtcthree@VIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@VIII@out}\newcommand\defaultbbhgwtcthree@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@IX@out{\{"median": "0.67", "error plus": "1.6", "error minus": "0.44", "5th percentile": "0.22", "95th percentile": "2.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@IX@out{0.67}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@IX@out{1.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@IX@out{0.44}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@IX@out{0.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@IX@out{2.2}\else\def\defaultbbhgwtcthree@IX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@IX@out}\newcommand\defaultbbhgwtcthree@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@X@out{\{"median": "6.5", "error plus": "3.1", "error minus": "4.9", "5th percentile": "1.6", "95th percentile": "9.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@X@out{6.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@X@out{3.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@X@out{4.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@X@out{1.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@X@out{9.7}\else\def\defaultbbhgwtcthree@X@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@X@out}\newcommand\defaultbbhgwtcthree@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XI@out{\{"median": "4.1", "error plus": "5.0", "error minus": "3.8", "5th percentile": "0.30", "95th percentile": "9.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XI@out{4.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XI@out{5.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XI@out{3.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XI@out{0.30}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XI@out{9.2}\else\def\defaultbbhgwtcthree@XI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XI@out}\newcommand\defaultbbhgwtcthree@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XII@out{\{"median": "3.9", "error plus": "5.1", "error minus": "3.6", "5th percentile": "0.32", "95th percentile": "9.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XII@out{3.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XII@out{5.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XII@out{3.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XII@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XII@out{9.0}\else\def\defaultbbhgwtcthree@XII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XII@out}\newcommand\defaultbbhgwtcthree@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XIII@out{\{"median": "0.25", "error plus": "0.39", "error minus": "0.21", "5th percentile": "0.041", "95th percentile": "0.63"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XIII@out{0.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XIII@out{0.39}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XIII@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XIII@out{0.041}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XIII@out{0.63}\else\def\defaultbbhgwtcthree@XIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XIII@out}\newcommand\defaultbbhgwtcthree@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XIV@out{\{"median": "0.65", "error plus": "0.20", "error minus": "0.36", "5th percentile": "0.29", "95th percentile": "0.85"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XIV@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XIV@out{0.20}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XIV@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XIV@out{0.29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XIV@out{0.85}\else\def\defaultbbhgwtcthree@XIV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XIV@out}\newcommand\defaultbbhgwtcthree@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XV@out{\{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.012", "95th percentile": "0.26"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XV@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XV@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XV@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XV@out{0.012}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XV@out{0.26}\else\def\defaultbbhgwtcthree@XV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XV@out}\newcommand\defaultbbhgwtcthree@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XVI@out{\{"median": "0.28", "error plus": "0.11", "error minus": "0.096", "5th percentile": "0.19", "95th percentile": "0.40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XVI@out{0.28}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XVI@out{0.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XVI@out{0.096}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XVI@out{0.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XVI@out{0.40}\else\def\defaultbbhgwtcthree@XVI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XVI@out}\newcommand\defaultbbhgwtcthree@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XVII@out{\{"median": "0.60", "error plus": "0.36", "error minus": "0.51", "5th percentile": "0.092", "95th percentile": "0.96"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XVII@out{0.60}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XVII@out{0.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XVII@out{0.51}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XVII@out{0.092}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XVII@out{0.96}\else\def\defaultbbhgwtcthree@XVII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XVII@out}\newcommand\defaultbbhgwtcthree@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XVIII@out{\{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XVIII@out{0.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XVIII@out{0.46}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XVIII@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XVIII@out{{-}0.58}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XVIII@out{0.95}\else\def\defaultbbhgwtcthree@XVIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XVIII@out}\newcommand\defaultbbhgwtcthree@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XIX@out{\{"median": "1.3", "error plus": "2.4", "error minus": "0.93", "5th percentile": "0.40", "95th percentile": "3.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XIX@out{1.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XIX@out{2.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XIX@out{0.93}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XIX@out{0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XIX@out{3.7}\else\def\defaultbbhgwtcthree@XIX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XIX@out}\newcommand\defaultbbhgwtcthree@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XX@out{\{"median": "2.6", "error plus": "1.8", "error minus": "1.8", "5th percentile": "0.87", "95th percentile": "4.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XX@out{2.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XX@out{1.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XX@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XX@out{0.87}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XX@out{4.4}\else\def\defaultbbhgwtcthree@XX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XX@out}\newcommand\defaultbbhgwtcthree@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXI@out{\{"median": "17", "error plus": "10", "error minus": "6.5", "5th percentile": "11", "95th percentile": "28"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXI@out{17}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXI@out{10}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXI@out{6.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXI@out{11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXI@out{28}\else\def\defaultbbhgwtcthree@XXI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXI@out}\newcommand\defaultbbhgwtcthree@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXII@out{\{"powerlaw\_slope\_18{-}19": \{"median": "0.0049", "error plus": "2.8", "error minus": "3.0", "5th percentile": "{-}3.0", "95th percentile": "2.8"\}, "peak\_1\_location": \{"median": "10", "error plus": "0.6", "error minus": "1.0", "5th percentile": "9", "95th percentile": "10.7"\}, "peak\_2\_location": \{"median": "30.7", "error plus": "4.6", "error minus": "5.3", "5th percentile": "25", "95th percentile": "35"\}, "peak\_2\_percent": 95.19999999999999\}}\else\ifnum\pdfstrcmp{#1}{powerlaw_slope_18-19}=0\let\defaultbbhgwtcthree@XXII@out\defaultbbhgwtcthree@XXXI\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\defaultbbhgwtcthree@XXII@out\defaultbbhgwtcthree@XXXII\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\defaultbbhgwtcthree@XXII@out\defaultbbhgwtcthree@XXXIII\else\ifnum\pdfstrcmp{#1}{peak_2_percent}=0\def\defaultbbhgwtcthree@XXII@out{95.19999999999999}\else\def\defaultbbhgwtcthree@XXII@out{??}\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXII@out}\newcommand\defaultbbhgwtcthree@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXIII@out{\{"median": "{-}3.2", "error plus": "8.8", "error minus": "5.1", "5th percentile": "{-}8.2", "95th percentile": "5.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXIII@out{{-}3.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXIII@out{8.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXIII@out{5.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXIII@out{{-}8.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXIII@out{5.6}\else\def\defaultbbhgwtcthree@XXIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXIII@out}\newcommand\defaultbbhgwtcthree@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXIV@out{\{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhgwtcthree@XXIV@out\defaultbbhgwtcthree@XXXIV\else\def\defaultbbhgwtcthree@XXIV@out{??}\fi\fi\defaultbbhgwtcthree@XXIV@out}\newcommand\defaultbbhgwtcthree@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXV@out{\{"peak": \{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.013", "95th percentile": "0.26"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhgwtcthree@XXV@out\defaultbbhgwtcthree@XXXV\else\def\defaultbbhgwtcthree@XXV@out{??}\fi\fi\defaultbbhgwtcthree@XXV@out}\newcommand\defaultbbhgwtcthree@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXVI@out{\{"peak": \{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.013", "95th percentile": "0.26"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhgwtcthree@XXVI@out\defaultbbhgwtcthree@XXXVI\else\def\defaultbbhgwtcthree@XXVI@out{??}\fi\fi\defaultbbhgwtcthree@XXVI@out}\newcommand\defaultbbhgwtcthree@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXVII@out{\{"peak": \{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhgwtcthree@XXVII@out\defaultbbhgwtcthree@XXXVII\else\def\defaultbbhgwtcthree@XXVII@out{??}\fi\fi\defaultbbhgwtcthree@XXVII@out}\newcommand\defaultbbhgwtcthree@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXVIII@out{\{"peak": \{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhgwtcthree@XXVIII@out\defaultbbhgwtcthree@XXXVIII\else\def\defaultbbhgwtcthree@XXVIII@out{??}\fi\fi\defaultbbhgwtcthree@XXVIII@out}\newcommand\defaultbbhgwtcthree@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXIX@out{\{"rate\_at\_z\_0{-}2": \{"median": "28", "error plus": "12", "error minus": "8.8", "5th percentile": "19", "95th percentile": "40"\}, "ppd": \{"median": "1.5", "error plus": "0.39", "error minus": "1.0", "5th percentile": "0.47", "95th percentile": "1.9"\}\}}\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\defaultbbhgwtcthree@XXIX@out\defaultbbhgwtcthree@XXXIX\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\defaultbbhgwtcthree@XXIX@out\defaultbbhgwtcthree@XL\else\def\defaultbbhgwtcthree@XXIX@out{??}\fi\fi\fi\defaultbbhgwtcthree@XXIX@out}\newcommand\defaultbbhgwtcthree@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXX@out{\{"median": "37", "error plus": "4.6", "error minus": "3.5", "5th percentile": "34", "95th percentile": "42"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXX@out{37}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXX@out{4.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXX@out{3.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXX@out{34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXX@out{42}\else\def\defaultbbhgwtcthree@XXX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXX@out}\newcommand\defaultbbhgwtcthree@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXI@out{\{"median": "0.0049", "error plus": "2.8", "error minus": "3.0", "5th percentile": "{-}3.0", "95th percentile": "2.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXI@out{0.0049}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXI@out{2.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXI@out{3.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXI@out{{-}3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXI@out{2.8}\else\def\defaultbbhgwtcthree@XXXI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXI@out}\newcommand\defaultbbhgwtcthree@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXII@out{\{"median": "10", "error plus": "0.6", "error minus": "1.0", "5th percentile": "9", "95th percentile": "10.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXII@out{10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXII@out{0.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXII@out{1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXII@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXII@out{10.7}\else\def\defaultbbhgwtcthree@XXXII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXII@out}\newcommand\defaultbbhgwtcthree@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXIII@out{\{"median": "30.7", "error plus": "4.6", "error minus": "5.3", "5th percentile": "25", "95th percentile": "35"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXIII@out{30.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXIII@out{4.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXIII@out{5.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXIII@out{25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXIII@out{35}\else\def\defaultbbhgwtcthree@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXIII@out}\newcommand\defaultbbhgwtcthree@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXIV@out{\{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXIV@out{1.0}\else\def\defaultbbhgwtcthree@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXIV@out}\newcommand\defaultbbhgwtcthree@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXV@out{\{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.013", "95th percentile": "0.26"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXV@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXV@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXV@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXV@out{0.013}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXV@out{0.26}\else\def\defaultbbhgwtcthree@XXXV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXV@out}\newcommand\defaultbbhgwtcthree@XXXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXVI@out{\{"median": "0.12", "error plus": "0.14", "error minus": "0.11", "5th percentile": "0.013", "95th percentile": "0.26"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXVI@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXVI@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXVI@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXVI@out{0.013}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXVI@out{0.26}\else\def\defaultbbhgwtcthree@XXXVI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXVI@out}\newcommand\defaultbbhgwtcthree@XXXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXVII@out{\{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXVII@out{0.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXVII@out{0.46}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXVII@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXVII@out{{-}0.58}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXVII@out{0.95}\else\def\defaultbbhgwtcthree@XXXVII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXVII@out}\newcommand\defaultbbhgwtcthree@XXXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXVIII@out{\{"median": "0.48", "error plus": "0.46", "error minus": "1.1", "5th percentile": "{-}0.58", "95th percentile": "0.95"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXVIII@out{0.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXVIII@out{0.46}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXVIII@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXVIII@out{{-}0.58}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXVIII@out{0.95}\else\def\defaultbbhgwtcthree@XXXVIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXVIII@out}\newcommand\defaultbbhgwtcthree@XXXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XXXIX@out{\{"median": "28", "error plus": "12", "error minus": "8.8", "5th percentile": "19", "95th percentile": "40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XXXIX@out{28}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XXXIX@out{12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XXXIX@out{8.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XXXIX@out{19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XXXIX@out{40}\else\def\defaultbbhgwtcthree@XXXIX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XXXIX@out}\newcommand\defaultbbhgwtcthree@XL[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhgwtcthree@XL@out{\{"median": "1.5", "error plus": "0.39", "error minus": "1.0", "5th percentile": "0.47", "95th percentile": "1.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhgwtcthree@XL@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhgwtcthree@XL@out{0.39}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhgwtcthree@XL@out{1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhgwtcthree@XL@out{0.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhgwtcthree@XL@out{1.9}\else\def\defaultbbhgwtcthree@XL@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhgwtcthree@XL@out}\makeatother
\makeatletter\newcommand\defaultbbh[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@out{\{"alpha\_1": \{"median": "1.7", "error plus": "1.2", "error minus": "1.8", "5th percentile": "{-}0.058", "95th percentile": "2.9"\}, "alpha\_2": \{"median": "4.5", "error plus": "1.6", "error minus": "1.3", "5th percentile": "3.2", "95th percentile": "6.1"\}, "beta": \{"median": "1.2", "error plus": "1.2", "error minus": "1.0", "5th percentile": "0.17", "95th percentile": "2.4"\}, "mlow\_1": \{"median": "5.1", "error plus": "3.2", "error minus": "1.8", "5th percentile": "3.2", "95th percentile": "8.2"\}, "mlow\_2": \{"median": "3.6", "error plus": "1.4", "error minus": "0.52", "5th percentile": "3.0", "95th percentile": "4.9"\}, "break\_mass": \{"median": "36", "error plus": "12", "error minus": "13", "5th percentile": "23", "95th percentile": "48"\}, "mpp\_1": \{"median": "9.8", "error plus": "0.50", "error minus": "1.3", "5th percentile": "8.5", "95th percentile": "10"\}, "mpp\_2": \{"median": "33", "error plus": "3.0", "error minus": "5.7", "5th percentile": "27", "95th percentile": "36"\}, "sigpp\_1": \{"median": "0.65", "error plus": "0.93", "error minus": "0.34", "5th percentile": "0.31", "95th percentile": "1.6"\}, "sigpp\_2": \{"median": "3.9", "error plus": "5.1", "error minus": "2.6", "5th percentile": "1.3", "95th percentile": "9.0"\}, "delta\_m\_1": \{"median": "4.3", "error plus": "4.9", "error minus": "4.0", "5th percentile": "0.33", "95th percentile": "9.2"\}, "delta\_m\_2": \{"median": "4.9", "error plus": "4.0", "error minus": "4.3", "5th percentile": "0.58", "95th percentile": "8.9"\}, "lam\_0": \{"median": "0.36", "error plus": "0.28", "error minus": "0.21", "5th percentile": "0.15", "95th percentile": "0.64"\}, "lam\_1": \{"median": "0.59", "error plus": "0.22", "error minus": "0.26", "5th percentile": "0.32", "95th percentile": "0.80"\}, "mu\_chi": \{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0078", "95th percentile": "0.22"\}, "sigma\_chi": \{"median": "0.33", "error plus": "0.077", "error minus": "0.081", "5th percentile": "0.25", "95th percentile": "0.41"\}, "xi\_spin": \{"median": "0.65", "error plus": "0.31", "error minus": "0.53", "5th percentile": "0.12", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}, "sigma\_spin": \{"median": "1.2", "error plus": "2.3", "error minus": "0.78", "5th percentile": "0.44", "95th percentile": "3.5"\}, "lamb": \{"median": "3.2", "error plus": "0.94", "error minus": "1.00", "5th percentile": "2.2", "95th percentile": "4.1"\}, "rate": \{"median": "16", "error plus": "5.8", "error minus": "4.3", "5th percentile": "12", "95th percentile": "22"\}, "mass\_1": \{"powerlaw\_slope\_18{-}19": \{"median": "1.5", "error plus": "1.2", "error minus": "1.9", "5th percentile": "{-}0.45", "95th percentile": "2.7"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "32.7", "error plus": "2.7", "error minus": "6.5", "5th percentile": "26", "95th percentile": "35"\}, "peak\_2\_percent": 87.3\}, "alpha\_diff": \{"median": "{-}2.9", "error plus": "2.3", "error minus": "2.4", "5th percentile": "{-}5.3", "95th percentile": "{-}0.64"\}, "alpha\_diff\_perc": 97.7, "mass\_ratio": \{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}, "a\_1": \{"peak": \{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}, "a\_2": \{"peak": \{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}, "cos\_tilt\_1": \{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}\}, "cos\_tilt\_2": \{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}\}, "redshift": \{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.5", "error minus": "6.5", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.39", "error minus": "0.97", "5th percentile": "0.50", "95th percentile": "1.9"\}\}, "mu\_plus\_sig": \{"median": "37", "error plus": "3.7", "error minus": "3.0", "5th percentile": "34", "95th percentile": "40"\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\defaultbbh@out\defaultbbh@I\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\defaultbbh@out\defaultbbh@II\else\ifnum\pdfstrcmp{#1}{beta}=0\let\defaultbbh@out\defaultbbh@III\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\defaultbbh@out\defaultbbh@IV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\defaultbbh@out\defaultbbh@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\defaultbbh@out\defaultbbh@VI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\defaultbbh@out\defaultbbh@VII\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\defaultbbh@out\defaultbbh@VIII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\defaultbbh@out\defaultbbh@IX\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\defaultbbh@out\defaultbbh@X\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\defaultbbh@out\defaultbbh@XI\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\defaultbbh@out\defaultbbh@XII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\defaultbbh@out\defaultbbh@XIII\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\defaultbbh@out\defaultbbh@XIV\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\defaultbbh@out\defaultbbh@XV\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\defaultbbh@out\defaultbbh@XVI\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\defaultbbh@out\defaultbbh@XVII\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\defaultbbh@out\defaultbbh@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\defaultbbh@out\defaultbbh@XIX\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\defaultbbh@out\defaultbbh@XX\else\ifnum\pdfstrcmp{#1}{rate}=0\let\defaultbbh@out\defaultbbh@XXI\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\defaultbbh@out\defaultbbh@XXII\else\ifnum\pdfstrcmp{#1}{alpha_diff}=0\let\defaultbbh@out\defaultbbh@XXIII\else\ifnum\pdfstrcmp{#1}{alpha_diff_perc}=0\def\defaultbbh@out{97.7}\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\defaultbbh@out\defaultbbh@XXIV\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\defaultbbh@out\defaultbbh@XXV\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\defaultbbh@out\defaultbbh@XXVI\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\defaultbbh@out\defaultbbh@XXVII\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\defaultbbh@out\defaultbbh@XXVIII\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\defaultbbh@out\defaultbbh@XXIX\else\ifnum\pdfstrcmp{#1}{mu_plus_sig}=0\let\defaultbbh@out\defaultbbh@XXX\else\def\defaultbbh@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\defaultbbh@out}\newcommand\defaultbbh@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@I@out{\{"median": "1.7", "error plus": "1.2", "error minus": "1.8", "5th percentile": "{-}0.058", "95th percentile": "2.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@I@out{1.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@I@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@I@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@I@out{{-}0.058}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@I@out{2.9}\else\def\defaultbbh@I@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@I@out}\newcommand\defaultbbh@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@II@out{\{"median": "4.5", "error plus": "1.6", "error minus": "1.3", "5th percentile": "3.2", "95th percentile": "6.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@II@out{4.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@II@out{1.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@II@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@II@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@II@out{6.1}\else\def\defaultbbh@II@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@II@out}\newcommand\defaultbbh@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@III@out{\{"median": "1.2", "error plus": "1.2", "error minus": "1.0", "5th percentile": "0.17", "95th percentile": "2.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@III@out{1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@III@out{0.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@III@out{2.4}\else\def\defaultbbh@III@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@III@out}\newcommand\defaultbbh@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@IV@out{\{"median": "5.1", "error plus": "3.2", "error minus": "1.8", "5th percentile": "3.2", "95th percentile": "8.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@IV@out{5.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@IV@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@IV@out{8.2}\else\def\defaultbbh@IV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@IV@out}\newcommand\defaultbbh@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@V@out{\{"median": "3.6", "error plus": "1.4", "error minus": "0.52", "5th percentile": "3.0", "95th percentile": "4.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@V@out{3.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@V@out{1.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@V@out{0.52}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@V@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@V@out{4.9}\else\def\defaultbbh@V@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@V@out}\newcommand\defaultbbh@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@VI@out{\{"median": "36", "error plus": "12", "error minus": "13", "5th percentile": "23", "95th percentile": "48"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@VI@out{36}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@VI@out{12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@VI@out{13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@VI@out{23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@VI@out{48}\else\def\defaultbbh@VI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@VI@out}\newcommand\defaultbbh@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@VII@out{\{"median": "9.8", "error plus": "0.50", "error minus": "1.3", "5th percentile": "8.5", "95th percentile": "10"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@VII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@VII@out{0.50}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@VII@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@VII@out{8.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@VII@out{10}\else\def\defaultbbh@VII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@VII@out}\newcommand\defaultbbh@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@VIII@out{\{"median": "33", "error plus": "3.0", "error minus": "5.7", "5th percentile": "27", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@VIII@out{33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@VIII@out{3.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@VIII@out{5.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@VIII@out{27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@VIII@out{36}\else\def\defaultbbh@VIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@VIII@out}\newcommand\defaultbbh@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@IX@out{\{"median": "0.65", "error plus": "0.93", "error minus": "0.34", "5th percentile": "0.31", "95th percentile": "1.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@IX@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@IX@out{0.93}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@IX@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@IX@out{1.6}\else\def\defaultbbh@IX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@IX@out}\newcommand\defaultbbh@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@X@out{\{"median": "3.9", "error plus": "5.1", "error minus": "2.6", "5th percentile": "1.3", "95th percentile": "9.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@X@out{3.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@X@out{5.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@X@out{2.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@X@out{1.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@X@out{9.0}\else\def\defaultbbh@X@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@X@out}\newcommand\defaultbbh@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XI@out{\{"median": "4.3", "error plus": "4.9", "error minus": "4.0", "5th percentile": "0.33", "95th percentile": "9.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XI@out{4.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XI@out{4.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XI@out{4.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XI@out{0.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XI@out{9.2}\else\def\defaultbbh@XI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XI@out}\newcommand\defaultbbh@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XII@out{\{"median": "4.9", "error plus": "4.0", "error minus": "4.3", "5th percentile": "0.58", "95th percentile": "8.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XII@out{4.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XII@out{4.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XII@out{4.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XII@out{0.58}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XII@out{8.9}\else\def\defaultbbh@XII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XII@out}\newcommand\defaultbbh@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XIII@out{\{"median": "0.36", "error plus": "0.28", "error minus": "0.21", "5th percentile": "0.15", "95th percentile": "0.64"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XIII@out{0.36}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XIII@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XIII@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XIII@out{0.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XIII@out{0.64}\else\def\defaultbbh@XIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XIII@out}\newcommand\defaultbbh@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XIV@out{\{"median": "0.59", "error plus": "0.22", "error minus": "0.26", "5th percentile": "0.32", "95th percentile": "0.80"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XIV@out{0.59}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XIV@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XIV@out{0.26}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XIV@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XIV@out{0.80}\else\def\defaultbbh@XIV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XIV@out}\newcommand\defaultbbh@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XV@out{\{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0078", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XV@out{0.085}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XV@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XV@out{0.077}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XV@out{0.0078}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XV@out{0.22}\else\def\defaultbbh@XV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XV@out}\newcommand\defaultbbh@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XVI@out{\{"median": "0.33", "error plus": "0.077", "error minus": "0.081", "5th percentile": "0.25", "95th percentile": "0.41"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XVI@out{0.33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XVI@out{0.077}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XVI@out{0.081}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XVI@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XVI@out{0.41}\else\def\defaultbbh@XVI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XVI@out}\newcommand\defaultbbh@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XVII@out{\{"median": "0.65", "error plus": "0.31", "error minus": "0.53", "5th percentile": "0.12", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XVII@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XVII@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XVII@out{0.53}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XVII@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XVII@out{0.97}\else\def\defaultbbh@XVII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XVII@out}\newcommand\defaultbbh@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XVIII@out{\{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XVIII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XVIII@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XVIII@out{0.79}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XVIII@out{{-}0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XVIII@out{0.94}\else\def\defaultbbh@XVIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XVIII@out}\newcommand\defaultbbh@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XIX@out{\{"median": "1.2", "error plus": "2.3", "error minus": "0.78", "5th percentile": "0.44", "95th percentile": "3.5"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XIX@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XIX@out{2.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XIX@out{0.78}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XIX@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XIX@out{3.5}\else\def\defaultbbh@XIX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XIX@out}\newcommand\defaultbbh@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XX@out{\{"median": "3.2", "error plus": "0.94", "error minus": "1.00", "5th percentile": "2.2", "95th percentile": "4.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XX@out{3.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XX@out{0.94}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XX@out{1.00}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XX@out{2.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XX@out{4.1}\else\def\defaultbbh@XX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XX@out}\newcommand\defaultbbh@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXI@out{\{"median": "16", "error plus": "5.8", "error minus": "4.3", "5th percentile": "12", "95th percentile": "22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXI@out{16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXI@out{5.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXI@out{4.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXI@out{12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXI@out{22}\else\def\defaultbbh@XXI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXI@out}\newcommand\defaultbbh@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXII@out{\{"powerlaw\_slope\_18{-}19": \{"median": "1.5", "error plus": "1.2", "error minus": "1.9", "5th percentile": "{-}0.45", "95th percentile": "2.7"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "32.7", "error plus": "2.7", "error minus": "6.5", "5th percentile": "26", "95th percentile": "35"\}, "peak\_2\_percent": 87.3\}}\else\ifnum\pdfstrcmp{#1}{powerlaw_slope_18-19}=0\let\defaultbbh@XXII@out\defaultbbh@XXXI\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\defaultbbh@XXII@out\defaultbbh@XXXII\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\defaultbbh@XXII@out\defaultbbh@XXXIII\else\ifnum\pdfstrcmp{#1}{peak_2_percent}=0\def\defaultbbh@XXII@out{87.3}\else\def\defaultbbh@XXII@out{??}\fi\fi\fi\fi\fi\defaultbbh@XXII@out}\newcommand\defaultbbh@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXIII@out{\{"median": "{-}2.9", "error plus": "2.3", "error minus": "2.4", "5th percentile": "{-}5.3", "95th percentile": "{-}0.64"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXIII@out{{-}2.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXIII@out{2.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXIII@out{2.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXIII@out{{-}5.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXIII@out{{-}0.64}\else\def\defaultbbh@XXIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXIII@out}\newcommand\defaultbbh@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXIV@out{\{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbh@XXIV@out\defaultbbh@XXXIV\else\def\defaultbbh@XXIV@out{??}\fi\fi\defaultbbh@XXIV@out}\newcommand\defaultbbh@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXV@out{\{"peak": \{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbh@XXV@out\defaultbbh@XXXV\else\def\defaultbbh@XXV@out{??}\fi\fi\defaultbbh@XXV@out}\newcommand\defaultbbh@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXVI@out{\{"peak": \{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0080", "95th percentile": "0.22"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbh@XXVI@out\defaultbbh@XXXVI\else\def\defaultbbh@XXVI@out{??}\fi\fi\defaultbbh@XXVI@out}\newcommand\defaultbbh@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXVII@out{\{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbh@XXVII@out\defaultbbh@XXXVII\else\def\defaultbbh@XXVII@out{??}\fi\fi\defaultbbh@XXVII@out}\newcommand\defaultbbh@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXVIII@out{\{"peak": \{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbh@XXVIII@out\defaultbbh@XXXVIII\else\def\defaultbbh@XXVIII@out{??}\fi\fi\defaultbbh@XXVIII@out}\newcommand\defaultbbh@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXIX@out{\{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.5", "error minus": "6.5", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.39", "error minus": "0.97", "5th percentile": "0.50", "95th percentile": "1.9"\}\}}\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\defaultbbh@XXIX@out\defaultbbh@XXXIX\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\defaultbbh@XXIX@out\defaultbbh@XL\else\def\defaultbbh@XXIX@out{??}\fi\fi\fi\defaultbbh@XXIX@out}\newcommand\defaultbbh@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXX@out{\{"median": "37", "error plus": "3.7", "error minus": "3.0", "5th percentile": "34", "95th percentile": "40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXX@out{37}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXX@out{3.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXX@out{3.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXX@out{34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXX@out{40}\else\def\defaultbbh@XXX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXX@out}\newcommand\defaultbbh@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXI@out{\{"median": "1.5", "error plus": "1.2", "error minus": "1.9", "5th percentile": "{-}0.45", "95th percentile": "2.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXI@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXI@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXI@out{1.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXI@out{{-}0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXI@out{2.7}\else\def\defaultbbh@XXXI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXI@out}\newcommand\defaultbbh@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXII@out{\{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXII@out{0.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXII@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXII@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXII@out{10.1}\else\def\defaultbbh@XXXII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXII@out}\newcommand\defaultbbh@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXIII@out{\{"median": "32.7", "error plus": "2.7", "error minus": "6.5", "5th percentile": "26", "95th percentile": "35"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXIII@out{32.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXIII@out{2.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXIII@out{6.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXIII@out{26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXIII@out{35}\else\def\defaultbbh@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXIII@out}\newcommand\defaultbbh@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXIV@out{\{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXIV@out{1.0}\else\def\defaultbbh@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXIV@out}\newcommand\defaultbbh@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXV@out{\{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0080", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXV@out{0.085}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXV@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXV@out{0.077}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXV@out{0.0080}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXV@out{0.22}\else\def\defaultbbh@XXXV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXV@out}\newcommand\defaultbbh@XXXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXVI@out{\{"median": "0.085", "error plus": "0.14", "error minus": "0.077", "5th percentile": "0.0080", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXVI@out{0.085}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXVI@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXVI@out{0.077}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXVI@out{0.0080}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXVI@out{0.22}\else\def\defaultbbh@XXXVI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXVI@out}\newcommand\defaultbbh@XXXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXVII@out{\{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXVII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXVII@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXVII@out{0.79}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXVII@out{{-}0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXVII@out{0.94}\else\def\defaultbbh@XXXVII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXVII@out}\newcommand\defaultbbh@XXXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXVIII@out{\{"median": "0.43", "error plus": "0.51", "error minus": "0.79", "5th percentile": "{-}0.36", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXVIII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXVIII@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXVIII@out{0.79}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXVIII@out{{-}0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXVIII@out{0.94}\else\def\defaultbbh@XXXVIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXVIII@out}\newcommand\defaultbbh@XXXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XXXIX@out{\{"median": "29", "error plus": "8.5", "error minus": "6.5", "5th percentile": "22", "95th percentile": "37"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XXXIX@out{29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XXXIX@out{8.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XXXIX@out{6.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XXXIX@out{22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XXXIX@out{37}\else\def\defaultbbh@XXXIX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XXXIX@out}\newcommand\defaultbbh@XL[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbh@XL@out{\{"median": "1.5", "error plus": "0.39", "error minus": "0.97", "5th percentile": "0.50", "95th percentile": "1.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbh@XL@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbh@XL@out{0.39}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbh@XL@out{0.97}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbh@XL@out{0.50}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbh@XL@out{1.9}\else\def\defaultbbh@XL@out{??}\fi\fi\fi\fi\fi\fi\defaultbbh@XL@out}\makeatother
\makeatletter\newcommand\defaultbbhnoGWttoott[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@out{\{"alpha\_1": \{"median": "1.6", "error plus": "1.2", "error minus": "1.8", "5th percentile": "{-}0.17", "95th percentile": "2.8"\}, "alpha\_2": \{"median": "5.2", "error plus": "1.7", "error minus": "1.5", "5th percentile": "3.7", "95th percentile": "6.9"\}, "beta": \{"median": "1.0", "error plus": "1.2", "error minus": "0.95", "5th percentile": "0.069", "95th percentile": "2.2"\}, "mlow\_1": \{"median": "5.0", "error plus": "2.8", "error minus": "1.8", "5th percentile": "3.2", "95th percentile": "7.8"\}, "mlow\_2": \{"median": "3.5", "error plus": "1.4", "error minus": "0.49", "5th percentile": "3.0", "95th percentile": "4.9"\}, "break\_mass": \{"median": "38", "error plus": "11", "error minus": "10", "5th percentile": "27", "95th percentile": "49"\}, "mpp\_1": \{"median": "9.8", "error plus": "0.50", "error minus": "1.1", "5th percentile": "8.7", "95th percentile": "10"\}, "mpp\_2": \{"median": "32", "error plus": "3.6", "error minus": "6.2", "5th percentile": "26", "95th percentile": "36"\}, "sigpp\_1": \{"median": "0.70", "error plus": "0.86", "error minus": "0.37", "5th percentile": "0.33", "95th percentile": "1.6"\}, "sigpp\_2": \{"median": "4.1", "error plus": "4.9", "error minus": "2.9", "5th percentile": "1.3", "95th percentile": "9.1"\}, "delta\_m\_1": \{"median": "4.6", "error plus": "4.5", "error minus": "4.2", "5th percentile": "0.42", "95th percentile": "9.1"\}, "delta\_m\_2": \{"median": "5.1", "error plus": "3.8", "error minus": "4.6", "5th percentile": "0.52", "95th percentile": "8.9"\}, "lam\_0": \{"median": "0.36", "error plus": "0.28", "error minus": "0.21", "5th percentile": "0.15", "95th percentile": "0.64"\}, "lam\_1": \{"median": "0.59", "error plus": "0.21", "error minus": "0.28", "5th percentile": "0.32", "95th percentile": "0.81"\}, "mu\_chi": \{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}, "sigma\_chi": \{"median": "0.31", "error plus": "0.069", "error minus": "0.077", "5th percentile": "0.23", "95th percentile": "0.38"\}, "xi\_spin": \{"median": "0.64", "error plus": "0.33", "error minus": "0.52", "5th percentile": "0.13", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.48", "error plus": "0.47", "error minus": "0.88", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}, "sigma\_spin": \{"median": "1.4", "error plus": "2.2", "error minus": "0.84", "5th percentile": "0.52", "95th percentile": "3.6"\}, "lamb": \{"median": "3.2", "error plus": "0.95", "error minus": "0.98", "5th percentile": "2.3", "95th percentile": "4.2"\}, "rate": \{"median": "16", "error plus": "5.7", "error minus": "4.5", "5th percentile": "11", "95th percentile": "22"\}, "mass\_1": \{"powerlaw\_slope\_18{-}19": \{"median": "1.3", "error plus": "1.3", "error minus": "2.0", "5th percentile": "{-}0.63", "95th percentile": "2.6"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "32.4", "error plus": "3.0", "error minus": "6.8", "5th percentile": "26", "95th percentile": "35"\}, "peak\_2\_percent": 82.39999999999999\}, "alpha\_diff": \{"median": "{-}3.7", "error plus": "2.4", "error minus": "2.3", "5th percentile": "{-}6.0", "95th percentile": "{-}1.4"\}, "alpha\_diff\_perc": 99.3, "mass\_ratio": \{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}, "a\_1": \{"peak": \{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}\}, "a\_2": \{"peak": \{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}\}, "cos\_tilt\_1": \{"peak": \{"median": "0.48", "error plus": "0.47", "error minus": "0.87", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}\}, "cos\_tilt\_2": \{"peak": \{"median": "0.48", "error plus": "0.47", "error minus": "0.87", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}\}, "redshift": \{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.1", "error minus": "6.4", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.38", "error minus": "0.97", "5th percentile": "0.52", "95th percentile": "1.9"\}\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@I\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@II\else\ifnum\pdfstrcmp{#1}{beta}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@III\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@IV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@VI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@VII\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@VIII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@IX\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@X\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XI\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XIII\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XIV\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XV\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XVI\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XVII\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XIX\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XX\else\ifnum\pdfstrcmp{#1}{rate}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXI\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXII\else\ifnum\pdfstrcmp{#1}{alpha_diff}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXIII\else\ifnum\pdfstrcmp{#1}{alpha_diff_perc}=0\def\defaultbbhnoGWttoott@out{99.3}\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXIV\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXV\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXVI\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXVII\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXVIII\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\defaultbbhnoGWttoott@out\defaultbbhnoGWttoott@XXIX\else\def\defaultbbhnoGWttoott@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@out}\newcommand\defaultbbhnoGWttoott@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@I@out{\{"median": "1.6", "error plus": "1.2", "error minus": "1.8", "5th percentile": "{-}0.17", "95th percentile": "2.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@I@out{1.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@I@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@I@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@I@out{{-}0.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@I@out{2.8}\else\def\defaultbbhnoGWttoott@I@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@I@out}\newcommand\defaultbbhnoGWttoott@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@II@out{\{"median": "5.2", "error plus": "1.7", "error minus": "1.5", "5th percentile": "3.7", "95th percentile": "6.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@II@out{5.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@II@out{1.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@II@out{1.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@II@out{3.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@II@out{6.9}\else\def\defaultbbhnoGWttoott@II@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@II@out}\newcommand\defaultbbhnoGWttoott@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@III@out{\{"median": "1.0", "error plus": "1.2", "error minus": "0.95", "5th percentile": "0.069", "95th percentile": "2.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@III@out{1.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@III@out{0.95}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@III@out{0.069}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@III@out{2.2}\else\def\defaultbbhnoGWttoott@III@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@III@out}\newcommand\defaultbbhnoGWttoott@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@IV@out{\{"median": "5.0", "error plus": "2.8", "error minus": "1.8", "5th percentile": "3.2", "95th percentile": "7.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@IV@out{5.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@IV@out{2.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@IV@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@IV@out{7.8}\else\def\defaultbbhnoGWttoott@IV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@IV@out}\newcommand\defaultbbhnoGWttoott@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@V@out{\{"median": "3.5", "error plus": "1.4", "error minus": "0.49", "5th percentile": "3.0", "95th percentile": "4.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@V@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@V@out{1.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@V@out{0.49}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@V@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@V@out{4.9}\else\def\defaultbbhnoGWttoott@V@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@V@out}\newcommand\defaultbbhnoGWttoott@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@VI@out{\{"median": "38", "error plus": "11", "error minus": "10", "5th percentile": "27", "95th percentile": "49"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@VI@out{38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@VI@out{11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@VI@out{10}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@VI@out{27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@VI@out{49}\else\def\defaultbbhnoGWttoott@VI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@VI@out}\newcommand\defaultbbhnoGWttoott@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@VII@out{\{"median": "9.8", "error plus": "0.50", "error minus": "1.1", "5th percentile": "8.7", "95th percentile": "10"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@VII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@VII@out{0.50}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@VII@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@VII@out{8.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@VII@out{10}\else\def\defaultbbhnoGWttoott@VII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@VII@out}\newcommand\defaultbbhnoGWttoott@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@VIII@out{\{"median": "32", "error plus": "3.6", "error minus": "6.2", "5th percentile": "26", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@VIII@out{32}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@VIII@out{3.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@VIII@out{6.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@VIII@out{26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@VIII@out{36}\else\def\defaultbbhnoGWttoott@VIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@VIII@out}\newcommand\defaultbbhnoGWttoott@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@IX@out{\{"median": "0.70", "error plus": "0.86", "error minus": "0.37", "5th percentile": "0.33", "95th percentile": "1.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@IX@out{0.70}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@IX@out{0.86}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@IX@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@IX@out{0.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@IX@out{1.6}\else\def\defaultbbhnoGWttoott@IX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@IX@out}\newcommand\defaultbbhnoGWttoott@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@X@out{\{"median": "4.1", "error plus": "4.9", "error minus": "2.9", "5th percentile": "1.3", "95th percentile": "9.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@X@out{4.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@X@out{4.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@X@out{2.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@X@out{1.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@X@out{9.1}\else\def\defaultbbhnoGWttoott@X@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@X@out}\newcommand\defaultbbhnoGWttoott@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XI@out{\{"median": "4.6", "error plus": "4.5", "error minus": "4.2", "5th percentile": "0.42", "95th percentile": "9.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XI@out{4.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XI@out{4.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XI@out{4.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XI@out{0.42}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XI@out{9.1}\else\def\defaultbbhnoGWttoott@XI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XI@out}\newcommand\defaultbbhnoGWttoott@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XII@out{\{"median": "5.1", "error plus": "3.8", "error minus": "4.6", "5th percentile": "0.52", "95th percentile": "8.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XII@out{5.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XII@out{3.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XII@out{4.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XII@out{0.52}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XII@out{8.9}\else\def\defaultbbhnoGWttoott@XII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XII@out}\newcommand\defaultbbhnoGWttoott@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XIII@out{\{"median": "0.36", "error plus": "0.28", "error minus": "0.21", "5th percentile": "0.15", "95th percentile": "0.64"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XIII@out{0.36}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XIII@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XIII@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XIII@out{0.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XIII@out{0.64}\else\def\defaultbbhnoGWttoott@XIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XIII@out}\newcommand\defaultbbhnoGWttoott@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XIV@out{\{"median": "0.59", "error plus": "0.21", "error minus": "0.28", "5th percentile": "0.32", "95th percentile": "0.81"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XIV@out{0.59}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XIV@out{0.21}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XIV@out{0.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XIV@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XIV@out{0.81}\else\def\defaultbbhnoGWttoott@XIV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XIV@out}\newcommand\defaultbbhnoGWttoott@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XV@out{\{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XV@out{0.096}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XV@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XV@out{0.087}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XV@out{0.0090}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XV@out{0.23}\else\def\defaultbbhnoGWttoott@XV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XV@out}\newcommand\defaultbbhnoGWttoott@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XVI@out{\{"median": "0.31", "error plus": "0.069", "error minus": "0.077", "5th percentile": "0.23", "95th percentile": "0.38"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XVI@out{0.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XVI@out{0.069}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XVI@out{0.077}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XVI@out{0.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XVI@out{0.38}\else\def\defaultbbhnoGWttoott@XVI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XVI@out}\newcommand\defaultbbhnoGWttoott@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XVII@out{\{"median": "0.64", "error plus": "0.33", "error minus": "0.52", "5th percentile": "0.13", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XVII@out{0.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XVII@out{0.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XVII@out{0.52}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XVII@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XVII@out{0.97}\else\def\defaultbbhnoGWttoott@XVII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XVII@out}\newcommand\defaultbbhnoGWttoott@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XVIII@out{\{"median": "0.48", "error plus": "0.47", "error minus": "0.88", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XVIII@out{0.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XVIII@out{0.47}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XVIII@out{0.88}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XVIII@out{{-}0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XVIII@out{0.95}\else\def\defaultbbhnoGWttoott@XVIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XVIII@out}\newcommand\defaultbbhnoGWttoott@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XIX@out{\{"median": "1.4", "error plus": "2.2", "error minus": "0.84", "5th percentile": "0.52", "95th percentile": "3.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XIX@out{1.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XIX@out{2.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XIX@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XIX@out{0.52}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XIX@out{3.6}\else\def\defaultbbhnoGWttoott@XIX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XIX@out}\newcommand\defaultbbhnoGWttoott@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XX@out{\{"median": "3.2", "error plus": "0.95", "error minus": "0.98", "5th percentile": "2.3", "95th percentile": "4.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XX@out{3.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XX@out{0.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XX@out{0.98}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XX@out{2.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XX@out{4.2}\else\def\defaultbbhnoGWttoott@XX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XX@out}\newcommand\defaultbbhnoGWttoott@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXI@out{\{"median": "16", "error plus": "5.7", "error minus": "4.5", "5th percentile": "11", "95th percentile": "22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXI@out{16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXI@out{5.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXI@out{4.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXI@out{11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXI@out{22}\else\def\defaultbbhnoGWttoott@XXI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXI@out}\newcommand\defaultbbhnoGWttoott@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXII@out{\{"powerlaw\_slope\_18{-}19": \{"median": "1.3", "error plus": "1.3", "error minus": "2.0", "5th percentile": "{-}0.63", "95th percentile": "2.6"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "32.4", "error plus": "3.0", "error minus": "6.8", "5th percentile": "26", "95th percentile": "35"\}, "peak\_2\_percent": 82.39999999999999\}}\else\ifnum\pdfstrcmp{#1}{powerlaw_slope_18-19}=0\let\defaultbbhnoGWttoott@XXII@out\defaultbbhnoGWttoott@XXX\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\defaultbbhnoGWttoott@XXII@out\defaultbbhnoGWttoott@XXXI\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\defaultbbhnoGWttoott@XXII@out\defaultbbhnoGWttoott@XXXII\else\ifnum\pdfstrcmp{#1}{peak_2_percent}=0\def\defaultbbhnoGWttoott@XXII@out{82.39999999999999}\else\def\defaultbbhnoGWttoott@XXII@out{??}\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXII@out}\newcommand\defaultbbhnoGWttoott@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXIII@out{\{"median": "{-}3.7", "error plus": "2.4", "error minus": "2.3", "5th percentile": "{-}6.0", "95th percentile": "{-}1.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXIII@out{{-}3.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXIII@out{2.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXIII@out{2.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXIII@out{{-}6.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXIII@out{{-}1.4}\else\def\defaultbbhnoGWttoott@XXIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXIII@out}\newcommand\defaultbbhnoGWttoott@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXIV@out{\{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhnoGWttoott@XXIV@out\defaultbbhnoGWttoott@XXXIII\else\def\defaultbbhnoGWttoott@XXIV@out{??}\fi\fi\defaultbbhnoGWttoott@XXIV@out}\newcommand\defaultbbhnoGWttoott@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXV@out{\{"peak": \{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhnoGWttoott@XXV@out\defaultbbhnoGWttoott@XXXIV\else\def\defaultbbhnoGWttoott@XXV@out{??}\fi\fi\defaultbbhnoGWttoott@XXV@out}\newcommand\defaultbbhnoGWttoott@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXVI@out{\{"peak": \{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhnoGWttoott@XXVI@out\defaultbbhnoGWttoott@XXXV\else\def\defaultbbhnoGWttoott@XXVI@out{??}\fi\fi\defaultbbhnoGWttoott@XXVI@out}\newcommand\defaultbbhnoGWttoott@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXVII@out{\{"peak": \{"median": "0.48", "error plus": "0.47", "error minus": "0.87", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhnoGWttoott@XXVII@out\defaultbbhnoGWttoott@XXXVI\else\def\defaultbbhnoGWttoott@XXVII@out{??}\fi\fi\defaultbbhnoGWttoott@XXVII@out}\newcommand\defaultbbhnoGWttoott@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXVIII@out{\{"peak": \{"median": "0.48", "error plus": "0.47", "error minus": "0.87", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\defaultbbhnoGWttoott@XXVIII@out\defaultbbhnoGWttoott@XXXVII\else\def\defaultbbhnoGWttoott@XXVIII@out{??}\fi\fi\defaultbbhnoGWttoott@XXVIII@out}\newcommand\defaultbbhnoGWttoott@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXIX@out{\{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.1", "error minus": "6.4", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.38", "error minus": "0.97", "5th percentile": "0.52", "95th percentile": "1.9"\}\}}\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\defaultbbhnoGWttoott@XXIX@out\defaultbbhnoGWttoott@XXXVIII\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\defaultbbhnoGWttoott@XXIX@out\defaultbbhnoGWttoott@XXXIX\else\def\defaultbbhnoGWttoott@XXIX@out{??}\fi\fi\fi\defaultbbhnoGWttoott@XXIX@out}\newcommand\defaultbbhnoGWttoott@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXX@out{\{"median": "1.3", "error plus": "1.3", "error minus": "2.0", "5th percentile": "{-}0.63", "95th percentile": "2.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXX@out{1.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXX@out{1.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXX@out{2.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXX@out{{-}0.63}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXX@out{2.6}\else\def\defaultbbhnoGWttoott@XXX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXX@out}\newcommand\defaultbbhnoGWttoott@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXI@out{\{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXI@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXI@out{0.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXI@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXI@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXI@out{10.1}\else\def\defaultbbhnoGWttoott@XXXI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXI@out}\newcommand\defaultbbhnoGWttoott@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXII@out{\{"median": "32.4", "error plus": "3.0", "error minus": "6.8", "5th percentile": "26", "95th percentile": "35"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXII@out{32.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXII@out{3.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXII@out{6.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXII@out{26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXII@out{35}\else\def\defaultbbhnoGWttoott@XXXII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXII@out}\newcommand\defaultbbhnoGWttoott@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXIII@out{\{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXIII@out{1.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXIII@out{0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXIII@out{0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXIII@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXIII@out{1.0}\else\def\defaultbbhnoGWttoott@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXIII@out}\newcommand\defaultbbhnoGWttoott@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXIV@out{\{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXIV@out{0.096}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXIV@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXIV@out{0.087}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXIV@out{0.0090}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXIV@out{0.23}\else\def\defaultbbhnoGWttoott@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXIV@out}\newcommand\defaultbbhnoGWttoott@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXV@out{\{"median": "0.096", "error plus": "0.13", "error minus": "0.087", "5th percentile": "0.0090", "95th percentile": "0.23"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXV@out{0.096}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXV@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXV@out{0.087}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXV@out{0.0090}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXV@out{0.23}\else\def\defaultbbhnoGWttoott@XXXV@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXV@out}\newcommand\defaultbbhnoGWttoott@XXXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXVI@out{\{"median": "0.48", "error plus": "0.47", "error minus": "0.87", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXVI@out{0.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXVI@out{0.47}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXVI@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXVI@out{{-}0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXVI@out{0.95}\else\def\defaultbbhnoGWttoott@XXXVI@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXVI@out}\newcommand\defaultbbhnoGWttoott@XXXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXVII@out{\{"median": "0.48", "error plus": "0.47", "error minus": "0.87", "5th percentile": "{-}0.40", "95th percentile": "0.95"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXVII@out{0.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXVII@out{0.47}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXVII@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXVII@out{{-}0.40}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXVII@out{0.95}\else\def\defaultbbhnoGWttoott@XXXVII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXVII@out}\newcommand\defaultbbhnoGWttoott@XXXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXVIII@out{\{"median": "29", "error plus": "8.1", "error minus": "6.4", "5th percentile": "22", "95th percentile": "37"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXVIII@out{29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXVIII@out{8.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXVIII@out{6.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXVIII@out{22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXVIII@out{37}\else\def\defaultbbhnoGWttoott@XXXVIII@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXVIII@out}\newcommand\defaultbbhnoGWttoott@XXXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultbbhnoGWttoott@XXXIX@out{\{"median": "1.5", "error plus": "0.38", "error minus": "0.97", "5th percentile": "0.52", "95th percentile": "1.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\defaultbbhnoGWttoott@XXXIX@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\defaultbbhnoGWttoott@XXXIX@out{0.38}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\defaultbbhnoGWttoott@XXXIX@out{0.97}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\defaultbbhnoGWttoott@XXXIX@out{0.52}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\defaultbbhnoGWttoott@XXXIX@out{1.9}\else\def\defaultbbhnoGWttoott@XXXIX@out{??}\fi\fi\fi\fi\fi\fi\defaultbbhnoGWttoott@XXXIX@out}\makeatother
\makeatletter\newcommand\DefaultBBHSubdominantMode[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@out{\{"alpha\_1": \{"median": "1.7", "error plus": "1.4", "error minus": "1.9", "5th percentile": "{-}0.16", "95th percentile": "3.1"\}, "alpha\_2": \{"median": "4.4", "error plus": "1.8", "error minus": "1.6", "5th percentile": "2.8", "95th percentile": "6.1"\}, "beta": \{"median": "1.2", "error plus": "1.2", "error minus": "1.0", "5th percentile": "0.17", "95th percentile": "2.4"\}, "mlow\_1": \{"median": "5.1", "error plus": "3.1", "error minus": "1.9", "5th percentile": "3.2", "95th percentile": "8.2"\}, "mlow\_2": \{"median": "3.5", "error plus": "1.4", "error minus": "0.52", "5th percentile": "3.0", "95th percentile": "4.9"\}, "break\_mass": \{"median": "36", "error plus": "12", "error minus": "13", "5th percentile": "23", "95th percentile": "48"\}, "mpp\_1": \{"median": "9.8", "error plus": "0.46", "error minus": "1.3", "5th percentile": "8.5", "95th percentile": "10"\}, "mpp\_2": \{"median": "29", "error plus": "2.9", "error minus": "3.6", "5th percentile": "26", "95th percentile": "32"\}, "sigpp\_1": \{"median": "0.66", "error plus": "0.88", "error minus": "0.34", "5th percentile": "0.31", "95th percentile": "1.5"\}, "sigpp\_2": \{"median": "7.3", "error plus": "2.3", "error minus": "2.5", "5th percentile": "4.8", "95th percentile": "9.6"\}, "delta\_m\_1": \{"median": "4.4", "error plus": "4.8", "error minus": "4.0", "5th percentile": "0.37", "95th percentile": "9.2"\}, "delta\_m\_2": \{"median": "4.8", "error plus": "4.2", "error minus": "4.2", "5th percentile": "0.59", "95th percentile": "9.0"\}, "lam\_0": \{"median": "0.31", "error plus": "0.28", "error minus": "0.20", "5th percentile": "0.10", "95th percentile": "0.59"\}, "lam\_1": \{"median": "0.62", "error plus": "0.20", "error minus": "0.27", "5th percentile": "0.35", "95th percentile": "0.83"\}, "mu\_chi": \{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0075", "95th percentile": "0.22"\}, "sigma\_chi": \{"median": "0.32", "error plus": "0.073", "error minus": "0.083", "5th percentile": "0.24", "95th percentile": "0.40"\}, "xi\_spin": \{"median": "0.67", "error plus": "0.30", "error minus": "0.55", "5th percentile": "0.12", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}, "sigma\_spin": \{"median": "1.2", "error plus": "2.1", "error minus": "0.78", "5th percentile": "0.47", "95th percentile": "3.4"\}, "lamb": \{"median": "3.2", "error plus": "0.94", "error minus": "1.0", "5th percentile": "2.2", "95th percentile": "4.2"\}, "rate": \{"median": "16", "error plus": "5.6", "error minus": "4.4", "5th percentile": "12", "95th percentile": "22"\}, "mass\_1": \{"powerlaw\_slope\_18{-}19": \{"median": "0.72", "error plus": "1.4", "error minus": "1.7", "5th percentile": "{-}1.0", "95th percentile": "2.1"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "28.3", "error plus": "3.0", "error minus": "4.4", "5th percentile": "24", "95th percentile": "31"\}, "peak\_2\_percent": 66.60000000000001\}, "alpha\_diff": \{"median": "{-}2.7", "error plus": "2.9", "error minus": "2.9", "5th percentile": "{-}5.6", "95th percentile": "0.14"\}, "alpha\_diff\_perc": 94.4, "mass\_ratio": \{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}, "a\_1": \{"peak": \{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0073", "95th percentile": "0.22"\}\}, "a\_2": \{"peak": \{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0073", "95th percentile": "0.22"\}\}, "cos\_tilt\_1": \{"peak": \{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}\}, "cos\_tilt\_2": \{"peak": \{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}\}, "redshift": \{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.0", "error minus": "6.7", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.38", "error minus": "0.97", "5th percentile": "0.51", "95th percentile": "1.9"\}\}, "mu\_plus\_sig": \{"median": "36", "error plus": "3.6", "error minus": "3.6", "5th percentile": "33", "95th percentile": "40"\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@I\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@II\else\ifnum\pdfstrcmp{#1}{beta}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@III\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@IV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@VI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@VII\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@VIII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@IX\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@X\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XI\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XIII\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XIV\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XV\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XVI\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XVII\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XIX\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XX\else\ifnum\pdfstrcmp{#1}{rate}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXI\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXII\else\ifnum\pdfstrcmp{#1}{alpha_diff}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXIII\else\ifnum\pdfstrcmp{#1}{alpha_diff_perc}=0\def\DefaultBBHSubdominantMode@out{94.4}\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXIV\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXV\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXVI\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXVII\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXVIII\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXIX\else\ifnum\pdfstrcmp{#1}{mu_plus_sig}=0\let\DefaultBBHSubdominantMode@out\DefaultBBHSubdominantMode@XXX\else\def\DefaultBBHSubdominantMode@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@out}\newcommand\DefaultBBHSubdominantMode@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@I@out{\{"median": "1.7", "error plus": "1.4", "error minus": "1.9", "5th percentile": "{-}0.16", "95th percentile": "3.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@I@out{1.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@I@out{1.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@I@out{1.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@I@out{{-}0.16}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@I@out{3.1}\else\def\DefaultBBHSubdominantMode@I@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@I@out}\newcommand\DefaultBBHSubdominantMode@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@II@out{\{"median": "4.4", "error plus": "1.8", "error minus": "1.6", "5th percentile": "2.8", "95th percentile": "6.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@II@out{4.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@II@out{1.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@II@out{1.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@II@out{2.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@II@out{6.1}\else\def\DefaultBBHSubdominantMode@II@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@II@out}\newcommand\DefaultBBHSubdominantMode@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@III@out{\{"median": "1.2", "error plus": "1.2", "error minus": "1.0", "5th percentile": "0.17", "95th percentile": "2.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@III@out{1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@III@out{0.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@III@out{2.4}\else\def\DefaultBBHSubdominantMode@III@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@III@out}\newcommand\DefaultBBHSubdominantMode@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@IV@out{\{"median": "5.1", "error plus": "3.1", "error minus": "1.9", "5th percentile": "3.2", "95th percentile": "8.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@IV@out{5.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@IV@out{3.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@IV@out{1.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@IV@out{8.2}\else\def\DefaultBBHSubdominantMode@IV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@IV@out}\newcommand\DefaultBBHSubdominantMode@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@V@out{\{"median": "3.5", "error plus": "1.4", "error minus": "0.52", "5th percentile": "3.0", "95th percentile": "4.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@V@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@V@out{1.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@V@out{0.52}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@V@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@V@out{4.9}\else\def\DefaultBBHSubdominantMode@V@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@V@out}\newcommand\DefaultBBHSubdominantMode@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@VI@out{\{"median": "36", "error plus": "12", "error minus": "13", "5th percentile": "23", "95th percentile": "48"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@VI@out{36}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@VI@out{12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@VI@out{13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@VI@out{23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@VI@out{48}\else\def\DefaultBBHSubdominantMode@VI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@VI@out}\newcommand\DefaultBBHSubdominantMode@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@VII@out{\{"median": "9.8", "error plus": "0.46", "error minus": "1.3", "5th percentile": "8.5", "95th percentile": "10"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@VII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@VII@out{0.46}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@VII@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@VII@out{8.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@VII@out{10}\else\def\DefaultBBHSubdominantMode@VII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@VII@out}\newcommand\DefaultBBHSubdominantMode@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@VIII@out{\{"median": "29", "error plus": "2.9", "error minus": "3.6", "5th percentile": "26", "95th percentile": "32"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@VIII@out{29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@VIII@out{2.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@VIII@out{3.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@VIII@out{26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@VIII@out{32}\else\def\DefaultBBHSubdominantMode@VIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@VIII@out}\newcommand\DefaultBBHSubdominantMode@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@IX@out{\{"median": "0.66", "error plus": "0.88", "error minus": "0.34", "5th percentile": "0.31", "95th percentile": "1.5"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@IX@out{0.66}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@IX@out{0.88}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@IX@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@IX@out{1.5}\else\def\DefaultBBHSubdominantMode@IX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@IX@out}\newcommand\DefaultBBHSubdominantMode@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@X@out{\{"median": "7.3", "error plus": "2.3", "error minus": "2.5", "5th percentile": "4.8", "95th percentile": "9.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@X@out{7.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@X@out{2.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@X@out{2.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@X@out{4.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@X@out{9.6}\else\def\DefaultBBHSubdominantMode@X@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@X@out}\newcommand\DefaultBBHSubdominantMode@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XI@out{\{"median": "4.4", "error plus": "4.8", "error minus": "4.0", "5th percentile": "0.37", "95th percentile": "9.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XI@out{4.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XI@out{4.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XI@out{4.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XI@out{0.37}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XI@out{9.2}\else\def\DefaultBBHSubdominantMode@XI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XI@out}\newcommand\DefaultBBHSubdominantMode@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XII@out{\{"median": "4.8", "error plus": "4.2", "error minus": "4.2", "5th percentile": "0.59", "95th percentile": "9.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XII@out{4.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XII@out{4.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XII@out{4.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XII@out{0.59}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XII@out{9.0}\else\def\DefaultBBHSubdominantMode@XII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XII@out}\newcommand\DefaultBBHSubdominantMode@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XIII@out{\{"median": "0.31", "error plus": "0.28", "error minus": "0.20", "5th percentile": "0.10", "95th percentile": "0.59"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XIII@out{0.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XIII@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XIII@out{0.20}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XIII@out{0.10}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XIII@out{0.59}\else\def\DefaultBBHSubdominantMode@XIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XIII@out}\newcommand\DefaultBBHSubdominantMode@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XIV@out{\{"median": "0.62", "error plus": "0.20", "error minus": "0.27", "5th percentile": "0.35", "95th percentile": "0.83"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XIV@out{0.62}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XIV@out{0.20}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XIV@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XIV@out{0.35}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XIV@out{0.83}\else\def\DefaultBBHSubdominantMode@XIV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XIV@out}\newcommand\DefaultBBHSubdominantMode@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XV@out{\{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0075", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XV@out{0.079}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XV@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XV@out{0.072}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XV@out{0.0075}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XV@out{0.22}\else\def\DefaultBBHSubdominantMode@XV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XV@out}\newcommand\DefaultBBHSubdominantMode@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XVI@out{\{"median": "0.32", "error plus": "0.073", "error minus": "0.083", "5th percentile": "0.24", "95th percentile": "0.40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XVI@out{0.32}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XVI@out{0.073}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XVI@out{0.083}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XVI@out{0.24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XVI@out{0.40}\else\def\DefaultBBHSubdominantMode@XVI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XVI@out}\newcommand\DefaultBBHSubdominantMode@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XVII@out{\{"median": "0.67", "error plus": "0.30", "error minus": "0.55", "5th percentile": "0.12", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XVII@out{0.67}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XVII@out{0.30}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XVII@out{0.55}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XVII@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XVII@out{0.97}\else\def\DefaultBBHSubdominantMode@XVII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XVII@out}\newcommand\DefaultBBHSubdominantMode@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XVIII@out{\{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XVIII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XVIII@out{0.50}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XVIII@out{0.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XVIII@out{{-}0.29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XVIII@out{0.93}\else\def\DefaultBBHSubdominantMode@XVIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XVIII@out}\newcommand\DefaultBBHSubdominantMode@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XIX@out{\{"median": "1.2", "error plus": "2.1", "error minus": "0.78", "5th percentile": "0.47", "95th percentile": "3.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XIX@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XIX@out{2.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XIX@out{0.78}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XIX@out{0.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XIX@out{3.4}\else\def\DefaultBBHSubdominantMode@XIX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XIX@out}\newcommand\DefaultBBHSubdominantMode@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XX@out{\{"median": "3.2", "error plus": "0.94", "error minus": "1.0", "5th percentile": "2.2", "95th percentile": "4.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XX@out{3.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XX@out{0.94}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XX@out{1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XX@out{2.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XX@out{4.2}\else\def\DefaultBBHSubdominantMode@XX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XX@out}\newcommand\DefaultBBHSubdominantMode@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXI@out{\{"median": "16", "error plus": "5.6", "error minus": "4.4", "5th percentile": "12", "95th percentile": "22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXI@out{16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXI@out{5.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXI@out{4.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXI@out{12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXI@out{22}\else\def\DefaultBBHSubdominantMode@XXI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXI@out}\newcommand\DefaultBBHSubdominantMode@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXII@out{\{"powerlaw\_slope\_18{-}19": \{"median": "0.72", "error plus": "1.4", "error minus": "1.7", "5th percentile": "{-}1.0", "95th percentile": "2.1"\}, "peak\_1\_location": \{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}, "peak\_2\_location": \{"median": "28.3", "error plus": "3.0", "error minus": "4.4", "5th percentile": "24", "95th percentile": "31"\}, "peak\_2\_percent": 66.60000000000001\}}\else\ifnum\pdfstrcmp{#1}{powerlaw_slope_18-19}=0\let\DefaultBBHSubdominantMode@XXII@out\DefaultBBHSubdominantMode@XXXI\else\ifnum\pdfstrcmp{#1}{peak_1_location}=0\let\DefaultBBHSubdominantMode@XXII@out\DefaultBBHSubdominantMode@XXXII\else\ifnum\pdfstrcmp{#1}{peak_2_location}=0\let\DefaultBBHSubdominantMode@XXII@out\DefaultBBHSubdominantMode@XXXIII\else\ifnum\pdfstrcmp{#1}{peak_2_percent}=0\def\DefaultBBHSubdominantMode@XXII@out{66.60000000000001}\else\def\DefaultBBHSubdominantMode@XXII@out{??}\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXII@out}\newcommand\DefaultBBHSubdominantMode@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXIII@out{\{"median": "{-}2.7", "error plus": "2.9", "error minus": "2.9", "5th percentile": "{-}5.6", "95th percentile": "0.14"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXIII@out{{-}2.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXIII@out{2.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXIII@out{2.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXIII@out{{-}5.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXIII@out{0.14}\else\def\DefaultBBHSubdominantMode@XXIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXIII@out}\newcommand\DefaultBBHSubdominantMode@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXIV@out{\{"peak": \{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHSubdominantMode@XXIV@out\DefaultBBHSubdominantMode@XXXIV\else\def\DefaultBBHSubdominantMode@XXIV@out{??}\fi\fi\DefaultBBHSubdominantMode@XXIV@out}\newcommand\DefaultBBHSubdominantMode@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXV@out{\{"peak": \{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0073", "95th percentile": "0.22"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHSubdominantMode@XXV@out\DefaultBBHSubdominantMode@XXXV\else\def\DefaultBBHSubdominantMode@XXV@out{??}\fi\fi\DefaultBBHSubdominantMode@XXV@out}\newcommand\DefaultBBHSubdominantMode@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXVI@out{\{"peak": \{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0073", "95th percentile": "0.22"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHSubdominantMode@XXVI@out\DefaultBBHSubdominantMode@XXXVI\else\def\DefaultBBHSubdominantMode@XXVI@out{??}\fi\fi\DefaultBBHSubdominantMode@XXVI@out}\newcommand\DefaultBBHSubdominantMode@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXVII@out{\{"peak": \{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHSubdominantMode@XXVII@out\DefaultBBHSubdominantMode@XXXVII\else\def\DefaultBBHSubdominantMode@XXVII@out{??}\fi\fi\DefaultBBHSubdominantMode@XXVII@out}\newcommand\DefaultBBHSubdominantMode@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXVIII@out{\{"peak": \{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\DefaultBBHSubdominantMode@XXVIII@out\DefaultBBHSubdominantMode@XXXVIII\else\def\DefaultBBHSubdominantMode@XXVIII@out{??}\fi\fi\DefaultBBHSubdominantMode@XXVIII@out}\newcommand\DefaultBBHSubdominantMode@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXIX@out{\{"rate\_at\_z\_0{-}2": \{"median": "29", "error plus": "8.0", "error minus": "6.7", "5th percentile": "22", "95th percentile": "37"\}, "ppd": \{"median": "1.5", "error plus": "0.38", "error minus": "0.97", "5th percentile": "0.51", "95th percentile": "1.9"\}\}}\else\ifnum\pdfstrcmp{#1}{rate_at_z_0-2}=0\let\DefaultBBHSubdominantMode@XXIX@out\DefaultBBHSubdominantMode@XXXIX\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\DefaultBBHSubdominantMode@XXIX@out\DefaultBBHSubdominantMode@XL\else\def\DefaultBBHSubdominantMode@XXIX@out{??}\fi\fi\fi\DefaultBBHSubdominantMode@XXIX@out}\newcommand\DefaultBBHSubdominantMode@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXX@out{\{"median": "36", "error plus": "3.6", "error minus": "3.6", "5th percentile": "33", "95th percentile": "40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXX@out{36}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXX@out{3.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXX@out{3.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXX@out{33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXX@out{40}\else\def\DefaultBBHSubdominantMode@XXX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXX@out}\newcommand\DefaultBBHSubdominantMode@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXI@out{\{"median": "0.72", "error plus": "1.4", "error minus": "1.7", "5th percentile": "{-}1.0", "95th percentile": "2.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXI@out{0.72}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXI@out{1.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXI@out{1.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXI@out{{-}1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXI@out{2.1}\else\def\DefaultBBHSubdominantMode@XXXI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXI@out}\newcommand\DefaultBBHSubdominantMode@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXII@out{\{"median": "9.8", "error plus": "0.3", "error minus": "0.6", "5th percentile": "9", "95th percentile": "10.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXII@out{0.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXII@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXII@out{9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXII@out{10.1}\else\def\DefaultBBHSubdominantMode@XXXII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXII@out}\newcommand\DefaultBBHSubdominantMode@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXIII@out{\{"median": "28.3", "error plus": "3.0", "error minus": "4.4", "5th percentile": "24", "95th percentile": "31"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXIII@out{28.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXIII@out{3.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXIII@out{4.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXIII@out{24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXIII@out{31}\else\def\DefaultBBHSubdominantMode@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXIII@out}\newcommand\DefaultBBHSubdominantMode@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXIV@out{\{"median": "1.0", "error plus": 0, "error minus": 0, "5th percentile": "1.0", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXIV@out{0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXIV@out{1.0}\else\def\DefaultBBHSubdominantMode@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXIV@out}\newcommand\DefaultBBHSubdominantMode@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXV@out{\{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0073", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXV@out{0.079}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXV@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXV@out{0.072}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXV@out{0.0073}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXV@out{0.22}\else\def\DefaultBBHSubdominantMode@XXXV@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXV@out}\newcommand\DefaultBBHSubdominantMode@XXXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXVI@out{\{"median": "0.079", "error plus": "0.14", "error minus": "0.072", "5th percentile": "0.0073", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXVI@out{0.079}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXVI@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXVI@out{0.072}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXVI@out{0.0073}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXVI@out{0.22}\else\def\DefaultBBHSubdominantMode@XXXVI@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXVI@out}\newcommand\DefaultBBHSubdominantMode@XXXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXVII@out{\{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXVII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXVII@out{0.50}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXVII@out{0.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXVII@out{{-}0.29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXVII@out{0.93}\else\def\DefaultBBHSubdominantMode@XXXVII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXVII@out}\newcommand\DefaultBBHSubdominantMode@XXXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXVIII@out{\{"median": "0.43", "error plus": "0.50", "error minus": "0.72", "5th percentile": "{-}0.29", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXVIII@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXVIII@out{0.50}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXVIII@out{0.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXVIII@out{{-}0.29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXVIII@out{0.93}\else\def\DefaultBBHSubdominantMode@XXXVIII@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXVIII@out}\newcommand\DefaultBBHSubdominantMode@XXXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XXXIX@out{\{"median": "29", "error plus": "8.0", "error minus": "6.7", "5th percentile": "22", "95th percentile": "37"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XXXIX@out{29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XXXIX@out{8.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XXXIX@out{6.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XXXIX@out{22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XXXIX@out{37}\else\def\DefaultBBHSubdominantMode@XXXIX@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XXXIX@out}\newcommand\DefaultBBHSubdominantMode@XL[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\DefaultBBHSubdominantMode@XL@out{\{"median": "1.5", "error plus": "0.38", "error minus": "0.97", "5th percentile": "0.51", "95th percentile": "1.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\DefaultBBHSubdominantMode@XL@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\DefaultBBHSubdominantMode@XL@out{0.38}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\DefaultBBHSubdominantMode@XL@out{0.97}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\DefaultBBHSubdominantMode@XL@out{0.51}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\DefaultBBHSubdominantMode@XL@out{1.9}\else\def\DefaultBBHSubdominantMode@XL@out{??}\fi\fi\fi\fi\fi\fi\DefaultBBHSubdominantMode@XL@out}\makeatother
\makeatletter\newcommand\defaultVersusBSplineSpinMagnitudes[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\defaultVersusBSplineSpinMagnitudes@out{\{"discrepancy percentile for chi=0.8": 85, "discrepancy percentile for chi=0.9": 96, "discrepancy percentile for chi=1.0": 98, "chi at discrepancy=90": 0.83\}}\else\ifnum\pdfstrcmp{#1}{discrepancy percentile for chi=0.8}=0\def\defaultVersusBSplineSpinMagnitudes@out{85}\else\ifnum\pdfstrcmp{#1}{discrepancy percentile for chi=0.9}=0\def\defaultVersusBSplineSpinMagnitudes@out{96}\else\ifnum\pdfstrcmp{#1}{discrepancy percentile for chi=1.0}=0\def\defaultVersusBSplineSpinMagnitudes@out{98}\else\ifnum\pdfstrcmp{#1}{chi at discrepancy=90}=0\def\defaultVersusBSplineSpinMagnitudes@out{0.83}\else\def\defaultVersusBSplineSpinMagnitudes@out{??}\fi\fi\fi\fi\fi\defaultVersusBSplineSpinMagnitudes@out}\makeatother
\makeatletter\newcommand\EpsSkewNormalChiEff[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@out{\{"param": \{"mu\_chi\_eff": \{"median": {-}0.05, "5th percentile": {-}0.1, "95th percentile": 0.01, "error plus": 0.06, "error minus": 0.04\}, "sigma\_chi\_eff": \{"median": 0.1, "5th percentile": 0.08, "95th percentile": 0.12, "error plus": 0.02, "error minus": 0.02\}, "mu\_chi\_p": \{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.07, "error minus": 0.07\}, "sigma\_chi\_p": \{"median": 0.19, "5th percentile": 0.13, "95th percentile": 0.31, "error plus": 0.12, "error minus": 0.06\}, "eps\_chi\_eff": \{"median": {-}0.68, "5th percentile": {-}0.96, "95th percentile": {-}0.21, "error plus": 0.47, "error minus": 0.28\}, "percent of epsilon less than zero": 99.3, "min\_chi\_eff": \{"median": {-}0.11, "5th percentile": {-}0.2, "95th percentile": {-}0.08, "error plus": 0.04, "error minus": 0.08\}, "f\_neg\_chi\_eff": \{"median": 0.34, "5th percentile": 0.26, "95th percentile": 0.42, "error plus": 0.08, "error minus": 0.09\}\}, "ppd": \{"chi\_eff": \{"median": 0.03, "5th percentile": {-}0.09, "95th percentile": 0.25, "spin at peak": {-}0.03\}, "chi\_p": \{"median": 0.34, "5th percentile": 0.07, "95th percentile": 0.68, "spin at peak": 0.33\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\EpsSkewNormalChiEff@out\EpsSkewNormalChiEff@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\EpsSkewNormalChiEff@out\EpsSkewNormalChiEff@II\else\def\EpsSkewNormalChiEff@out{??}\fi\fi\fi\EpsSkewNormalChiEff@out}\newcommand\EpsSkewNormalChiEff@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@I@out{\{"mu\_chi\_eff": \{"median": {-}0.05, "5th percentile": {-}0.1, "95th percentile": 0.01, "error plus": 0.06, "error minus": 0.04\}, "sigma\_chi\_eff": \{"median": 0.1, "5th percentile": 0.08, "95th percentile": 0.12, "error plus": 0.02, "error minus": 0.02\}, "mu\_chi\_p": \{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.07, "error minus": 0.07\}, "sigma\_chi\_p": \{"median": 0.19, "5th percentile": 0.13, "95th percentile": 0.31, "error plus": 0.12, "error minus": 0.06\}, "eps\_chi\_eff": \{"median": {-}0.68, "5th percentile": {-}0.96, "95th percentile": {-}0.21, "error plus": 0.47, "error minus": 0.28\}, "percent of epsilon less than zero": 99.3, "min\_chi\_eff": \{"median": {-}0.11, "5th percentile": {-}0.2, "95th percentile": {-}0.08, "error plus": 0.04, "error minus": 0.08\}, "f\_neg\_chi\_eff": \{"median": 0.34, "5th percentile": 0.26, "95th percentile": 0.42, "error plus": 0.08, "error minus": 0.09\}\}}\else\ifnum\pdfstrcmp{#1}{mu_chi_eff}=0\let\EpsSkewNormalChiEff@I@out\EpsSkewNormalChiEff@III\else\ifnum\pdfstrcmp{#1}{sigma_chi_eff}=0\let\EpsSkewNormalChiEff@I@out\EpsSkewNormalChiEff@IV\else\ifnum\pdfstrcmp{#1}{mu_chi_p}=0\let\EpsSkewNormalChiEff@I@out\EpsSkewNormalChiEff@V\else\ifnum\pdfstrcmp{#1}{sigma_chi_p}=0\let\EpsSkewNormalChiEff@I@out\EpsSkewNormalChiEff@VI\else\ifnum\pdfstrcmp{#1}{eps_chi_eff}=0\let\EpsSkewNormalChiEff@I@out\EpsSkewNormalChiEff@VII\else\ifnum\pdfstrcmp{#1}{percent of epsilon less than zero}=0\def\EpsSkewNormalChiEff@I@out{99.3}\else\ifnum\pdfstrcmp{#1}{min_chi_eff}=0\let\EpsSkewNormalChiEff@I@out\EpsSkewNormalChiEff@VIII\else\ifnum\pdfstrcmp{#1}{f_neg_chi_eff}=0\let\EpsSkewNormalChiEff@I@out\EpsSkewNormalChiEff@IX\else\def\EpsSkewNormalChiEff@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@I@out}\newcommand\EpsSkewNormalChiEff@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@II@out{\{"chi\_eff": \{"median": 0.03, "5th percentile": {-}0.09, "95th percentile": 0.25, "spin at peak": {-}0.03\}, "chi\_p": \{"median": 0.34, "5th percentile": 0.07, "95th percentile": 0.68, "spin at peak": 0.33\}\}}\else\ifnum\pdfstrcmp{#1}{chi_eff}=0\let\EpsSkewNormalChiEff@II@out\EpsSkewNormalChiEff@X\else\ifnum\pdfstrcmp{#1}{chi_p}=0\let\EpsSkewNormalChiEff@II@out\EpsSkewNormalChiEff@XI\else\def\EpsSkewNormalChiEff@II@out{??}\fi\fi\fi\EpsSkewNormalChiEff@II@out}\newcommand\EpsSkewNormalChiEff@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@III@out{\{"median": {-}0.05, "5th percentile": {-}0.1, "95th percentile": 0.01, "error plus": 0.06, "error minus": 0.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@III@out{{-}0.05}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@III@out{{-}0.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@III@out{0.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\EpsSkewNormalChiEff@III@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\EpsSkewNormalChiEff@III@out{0.04}\else\def\EpsSkewNormalChiEff@III@out{??}\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@III@out}\newcommand\EpsSkewNormalChiEff@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@IV@out{\{"median": 0.1, "5th percentile": 0.08, "95th percentile": 0.12, "error plus": 0.02, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@IV@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@IV@out{0.08}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@IV@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\EpsSkewNormalChiEff@IV@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\EpsSkewNormalChiEff@IV@out{0.02}\else\def\EpsSkewNormalChiEff@IV@out{??}\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@IV@out}\newcommand\EpsSkewNormalChiEff@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@V@out{\{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.07, "error minus": 0.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@V@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@V@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@V@out{0.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\EpsSkewNormalChiEff@V@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\EpsSkewNormalChiEff@V@out{0.07}\else\def\EpsSkewNormalChiEff@V@out{??}\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@V@out}\newcommand\EpsSkewNormalChiEff@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@VI@out{\{"median": 0.19, "5th percentile": 0.13, "95th percentile": 0.31, "error plus": 0.12, "error minus": 0.06\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@VI@out{0.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@VI@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@VI@out{0.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\EpsSkewNormalChiEff@VI@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\EpsSkewNormalChiEff@VI@out{0.06}\else\def\EpsSkewNormalChiEff@VI@out{??}\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@VI@out}\newcommand\EpsSkewNormalChiEff@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@VII@out{\{"median": {-}0.68, "5th percentile": {-}0.96, "95th percentile": {-}0.21, "error plus": 0.47, "error minus": 0.28\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@VII@out{{-}0.68}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@VII@out{{-}0.96}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@VII@out{{-}0.21}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\EpsSkewNormalChiEff@VII@out{0.47}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\EpsSkewNormalChiEff@VII@out{0.28}\else\def\EpsSkewNormalChiEff@VII@out{??}\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@VII@out}\newcommand\EpsSkewNormalChiEff@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@VIII@out{\{"median": {-}0.11, "5th percentile": {-}0.2, "95th percentile": {-}0.08, "error plus": 0.04, "error minus": 0.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@VIII@out{{-}0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@VIII@out{{-}0.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@VIII@out{{-}0.08}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\EpsSkewNormalChiEff@VIII@out{0.04}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\EpsSkewNormalChiEff@VIII@out{0.08}\else\def\EpsSkewNormalChiEff@VIII@out{??}\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@VIII@out}\newcommand\EpsSkewNormalChiEff@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@IX@out{\{"median": 0.34, "5th percentile": 0.26, "95th percentile": 0.42, "error plus": 0.08, "error minus": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@IX@out{0.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@IX@out{0.42}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\EpsSkewNormalChiEff@IX@out{0.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\EpsSkewNormalChiEff@IX@out{0.09}\else\def\EpsSkewNormalChiEff@IX@out{??}\fi\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@IX@out}\newcommand\EpsSkewNormalChiEff@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@X@out{\{"median": 0.03, "5th percentile": {-}0.09, "95th percentile": 0.25, "spin at peak": {-}0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@X@out{0.03}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@X@out{{-}0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@X@out{0.25}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\EpsSkewNormalChiEff@X@out{{-}0.03}\else\def\EpsSkewNormalChiEff@X@out{??}\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@X@out}\newcommand\EpsSkewNormalChiEff@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\EpsSkewNormalChiEff@XI@out{\{"median": 0.34, "5th percentile": 0.07, "95th percentile": 0.68, "spin at peak": 0.33\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\EpsSkewNormalChiEff@XI@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\EpsSkewNormalChiEff@XI@out{0.07}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\EpsSkewNormalChiEff@XI@out{0.68}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\EpsSkewNormalChiEff@XI@out{0.33}\else\def\EpsSkewNormalChiEff@XI@out{??}\fi\fi\fi\fi\fi\EpsSkewNormalChiEff@XI@out}\makeatother
\makeatletter\newcommand\ExampleModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@out{\{"param": \{"alpha": \{"median": 2.1, "error plus": 1.3, "error minus": 1.2, "5th percentile": 0.9, "95th percentile": 3.4\}, "m\_min": \{"median": 5.1, "5th percentile": 2.1, "95th percentile": 7.3\}, "m\_max": \{"median": 90.1, "5th percentile": 85.3, "95th percentile": 103.7\}\}, "ppd": \{"mass\_1\_source": \{"median": 28.7, "5th percentile": 8.1, "95th percentile": 87.3\}, "mass\_2\_source": \{"median": 22.7, "5th percentile": 6.3, "95th percentile": 54.1\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\ExampleModel@out\ExampleModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\ExampleModel@out\ExampleModel@II\else\def\ExampleModel@out{??}\fi\fi\fi\ExampleModel@out}\newcommand\ExampleModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@I@out{\{"alpha": \{"median": 2.1, "error plus": 1.3, "error minus": 1.2, "5th percentile": 0.9, "95th percentile": 3.4\}, "m\_min": \{"median": 5.1, "5th percentile": 2.1, "95th percentile": 7.3\}, "m\_max": \{"median": 90.1, "5th percentile": 85.3, "95th percentile": 103.7\}\}}\else\ifnum\pdfstrcmp{#1}{alpha}=0\let\ExampleModel@I@out\ExampleModel@III\else\ifnum\pdfstrcmp{#1}{m_min}=0\let\ExampleModel@I@out\ExampleModel@IV\else\ifnum\pdfstrcmp{#1}{m_max}=0\let\ExampleModel@I@out\ExampleModel@V\else\def\ExampleModel@I@out{??}\fi\fi\fi\fi\ExampleModel@I@out}\newcommand\ExampleModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@II@out{\{"mass\_1\_source": \{"median": 28.7, "5th percentile": 8.1, "95th percentile": 87.3\}, "mass\_2\_source": \{"median": 22.7, "5th percentile": 6.3, "95th percentile": 54.1\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1_source}=0\let\ExampleModel@II@out\ExampleModel@VI\else\ifnum\pdfstrcmp{#1}{mass_2_source}=0\let\ExampleModel@II@out\ExampleModel@VII\else\def\ExampleModel@II@out{??}\fi\fi\fi\ExampleModel@II@out}\newcommand\ExampleModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@III@out{\{"median": 2.1, "error plus": 1.3, "error minus": 1.2, "5th percentile": 0.9, "95th percentile": 3.4\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\ExampleModel@III@out{2.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\ExampleModel@III@out{1.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\ExampleModel@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\ExampleModel@III@out{0.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\ExampleModel@III@out{3.4}\else\def\ExampleModel@III@out{??}\fi\fi\fi\fi\fi\fi\ExampleModel@III@out}\newcommand\ExampleModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@IV@out{\{"median": 5.1, "5th percentile": 2.1, "95th percentile": 7.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\ExampleModel@IV@out{5.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\ExampleModel@IV@out{2.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\ExampleModel@IV@out{7.3}\else\def\ExampleModel@IV@out{??}\fi\fi\fi\fi\ExampleModel@IV@out}\newcommand\ExampleModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@V@out{\{"median": 90.1, "5th percentile": 85.3, "95th percentile": 103.7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\ExampleModel@V@out{90.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\ExampleModel@V@out{85.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\ExampleModel@V@out{103.7}\else\def\ExampleModel@V@out{??}\fi\fi\fi\fi\ExampleModel@V@out}\newcommand\ExampleModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@VI@out{\{"median": 28.7, "5th percentile": 8.1, "95th percentile": 87.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\ExampleModel@VI@out{28.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\ExampleModel@VI@out{8.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\ExampleModel@VI@out{87.3}\else\def\ExampleModel@VI@out{??}\fi\fi\fi\fi\ExampleModel@VI@out}\newcommand\ExampleModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\ExampleModel@VII@out{\{"median": 22.7, "5th percentile": 6.3, "95th percentile": 54.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\ExampleModel@VII@out{22.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\ExampleModel@VII@out{6.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\ExampleModel@VII@out{54.1}\else\def\ExampleModel@VII@out{??}\fi\fi\fi\fi\ExampleModel@VII@out}\makeatother
\makeatletter\newcommand\FgmcRates[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FgmcRates@out{\{"RatesBBH": \{"median": "15.1", "5th percentile": "13.1", "95th percentile": "17.3", "error plus": "2.2", "error minus": "2.01", "mean": "15.2"\}, "RatesBNS": \{"median": "137", "5th percentile": "30.9", "95th percentile": "361", "error plus": "224", "error minus": "106", "mean": "159"\}, "RatesNSBH": \{"median": "67.1", "5th percentile": "22.2", "95th percentile": "143", "error plus": "76.1", "error minus": "44.9", "mean": "72.9"\}\}}\else\ifnum\pdfstrcmp{#1}{RatesBBH}=0\let\FgmcRates@out\FgmcRates@I\else\ifnum\pdfstrcmp{#1}{RatesBNS}=0\let\FgmcRates@out\FgmcRates@II\else\ifnum\pdfstrcmp{#1}{RatesNSBH}=0\let\FgmcRates@out\FgmcRates@III\else\def\FgmcRates@out{??}\fi\fi\fi\fi\FgmcRates@out}\newcommand\FgmcRates@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FgmcRates@I@out{\{"median": "15.1", "5th percentile": "13.1", "95th percentile": "17.3", "error plus": "2.2", "error minus": "2.01", "mean": "15.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FgmcRates@I@out{15.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FgmcRates@I@out{13.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FgmcRates@I@out{17.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FgmcRates@I@out{2.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FgmcRates@I@out{2.01}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FgmcRates@I@out{15.2}\else\def\FgmcRates@I@out{??}\fi\fi\fi\fi\fi\fi\fi\FgmcRates@I@out}\newcommand\FgmcRates@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FgmcRates@II@out{\{"median": "137", "5th percentile": "30.9", "95th percentile": "361", "error plus": "224", "error minus": "106", "mean": "159"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FgmcRates@II@out{137}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FgmcRates@II@out{30.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FgmcRates@II@out{361}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FgmcRates@II@out{224}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FgmcRates@II@out{106}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FgmcRates@II@out{159}\else\def\FgmcRates@II@out{??}\fi\fi\fi\fi\fi\fi\fi\FgmcRates@II@out}\newcommand\FgmcRates@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FgmcRates@III@out{\{"median": "67.1", "5th percentile": "22.2", "95th percentile": "143", "error plus": "76.1", "error minus": "44.9", "mean": "72.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FgmcRates@III@out{67.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FgmcRates@III@out{22.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FgmcRates@III@out{143}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FgmcRates@III@out{76.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FgmcRates@III@out{44.9}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FgmcRates@III@out{72.9}\else\def\FgmcRates@III@out{??}\fi\fi\fi\fi\fi\fi\fi\FgmcRates@III@out}\makeatother
\makeatletter\newcommand\FullMassSpectrumBGPPeakSignificance[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPPeakSignificance@out{\{"m1\_peaks": \{"(9, 12)": 77\}, "m2\_peaks": \{"(1, 2)": 99, "(7.23021864, 9.2586008)": 97\}\}}\else\ifnum\pdfstrcmp{#1}{m1_peaks}=0\let\FullMassSpectrumBGPPeakSignificance@out\FullMassSpectrumBGPPeakSignificance@I\else\ifnum\pdfstrcmp{#1}{m2_peaks}=0\let\FullMassSpectrumBGPPeakSignificance@out\FullMassSpectrumBGPPeakSignificance@II\else\def\FullMassSpectrumBGPPeakSignificance@out{??}\fi\fi\fi\FullMassSpectrumBGPPeakSignificance@out}\newcommand\FullMassSpectrumBGPPeakSignificance@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPPeakSignificance@I@out{\{"(9, 12)": 77\}}\else\ifnum\pdfstrcmp{#1}{(9, 12)}=0\def\FullMassSpectrumBGPPeakSignificance@I@out{77}\else\def\FullMassSpectrumBGPPeakSignificance@I@out{??}\fi\fi\FullMassSpectrumBGPPeakSignificance@I@out}\newcommand\FullMassSpectrumBGPPeakSignificance@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPPeakSignificance@II@out{\{"(1, 2)": 99, "(7.23021864, 9.2586008)": 97\}}\else\ifnum\pdfstrcmp{#1}{(1, 2)}=0\def\FullMassSpectrumBGPPeakSignificance@II@out{99}\else\ifnum\pdfstrcmp{#1}{(7.23021864, 9.2586008)}=0\def\FullMassSpectrumBGPPeakSignificance@II@out{97}\else\def\FullMassSpectrumBGPPeakSignificance@II@out{??}\fi\fi\fi\FullMassSpectrumBGPPeakSignificance@II@out}\makeatother
\makeatletter\newcommand\FullMassSpectrumBGPRate[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPRate@out{\{"R\_BNS": \{"50th\_percentile": 49, "5th\_percentile": 8, "95th\_percentile": 170, "error\_plus": 121, "error\_minus": 42, "mean": 63.83278679172662\}, "R\_NSBH": \{"50th\_percentile": 30, "5th\_percentile": 9, "95th\_percentile": 84, "error\_plus": 54, "error\_minus": 21, "mean": 36.45956698365504\}, "R\_BBH": \{"50th\_percentile": 19, "5th\_percentile": 15, "95th\_percentile": 26, "error\_plus": 7, "error\_minus": 5, "mean": 19.83182217256504\}, "R\_NS{-}Gap": \{"50th\_percentile": 15, "5th\_percentile": 1, "95th\_percentile": 61, "error\_plus": 46, "error\_minus": 14, "mean": 21.135299049905807\}, "R\_BH{-}Gap": \{"50th\_percentile": 1.5, "5th\_percentile": 0.2, "95th\_percentile": 6.3, "error\_plus": 4.9, "error\_minus": 1.3, "mean": 2.1710767640642694\}, "R\_Full": \{"50th\_percentile": 110, "5th\_percentile": 50, "95th\_percentile": 240, "error\_plus": 130, "error\_minus": 60, "mean": 120.1241759479467\}\}}\else\ifnum\pdfstrcmp{#1}{R_BNS}=0\let\FullMassSpectrumBGPRate@out\FullMassSpectrumBGPRate@I\else\ifnum\pdfstrcmp{#1}{R_NSBH}=0\let\FullMassSpectrumBGPRate@out\FullMassSpectrumBGPRate@II\else\ifnum\pdfstrcmp{#1}{R_BBH}=0\let\FullMassSpectrumBGPRate@out\FullMassSpectrumBGPRate@III\else\ifnum\pdfstrcmp{#1}{R_NS-Gap}=0\let\FullMassSpectrumBGPRate@out\FullMassSpectrumBGPRate@IV\else\ifnum\pdfstrcmp{#1}{R_BH-Gap}=0\let\FullMassSpectrumBGPRate@out\FullMassSpectrumBGPRate@V\else\ifnum\pdfstrcmp{#1}{R_Full}=0\let\FullMassSpectrumBGPRate@out\FullMassSpectrumBGPRate@VI\else\def\FullMassSpectrumBGPRate@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumBGPRate@out}\newcommand\FullMassSpectrumBGPRate@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPRate@I@out{\{"50th\_percentile": 49, "5th\_percentile": 8, "95th\_percentile": 170, "error\_plus": 121, "error\_minus": 42, "mean": 63.83278679172662\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumBGPRate@I@out{49}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumBGPRate@I@out{8}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumBGPRate@I@out{170}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumBGPRate@I@out{121}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumBGPRate@I@out{42}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FullMassSpectrumBGPRate@I@out{63.83278679172662}\else\def\FullMassSpectrumBGPRate@I@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumBGPRate@I@out}\newcommand\FullMassSpectrumBGPRate@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPRate@II@out{\{"50th\_percentile": 30, "5th\_percentile": 9, "95th\_percentile": 84, "error\_plus": 54, "error\_minus": 21, "mean": 36.45956698365504\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumBGPRate@II@out{30}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumBGPRate@II@out{9}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumBGPRate@II@out{84}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumBGPRate@II@out{54}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumBGPRate@II@out{21}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FullMassSpectrumBGPRate@II@out{36.45956698365504}\else\def\FullMassSpectrumBGPRate@II@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumBGPRate@II@out}\newcommand\FullMassSpectrumBGPRate@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPRate@III@out{\{"50th\_percentile": 19, "5th\_percentile": 15, "95th\_percentile": 26, "error\_plus": 7, "error\_minus": 5, "mean": 19.83182217256504\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumBGPRate@III@out{19}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumBGPRate@III@out{15}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumBGPRate@III@out{26}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumBGPRate@III@out{7}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumBGPRate@III@out{5}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FullMassSpectrumBGPRate@III@out{19.83182217256504}\else\def\FullMassSpectrumBGPRate@III@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumBGPRate@III@out}\newcommand\FullMassSpectrumBGPRate@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPRate@IV@out{\{"50th\_percentile": 15, "5th\_percentile": 1, "95th\_percentile": 61, "error\_plus": 46, "error\_minus": 14, "mean": 21.135299049905807\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumBGPRate@IV@out{15}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumBGPRate@IV@out{1}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumBGPRate@IV@out{61}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumBGPRate@IV@out{46}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumBGPRate@IV@out{14}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FullMassSpectrumBGPRate@IV@out{21.135299049905807}\else\def\FullMassSpectrumBGPRate@IV@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumBGPRate@IV@out}\newcommand\FullMassSpectrumBGPRate@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPRate@V@out{\{"50th\_percentile": 1.5, "5th\_percentile": 0.2, "95th\_percentile": 6.3, "error\_plus": 4.9, "error\_minus": 1.3, "mean": 2.1710767640642694\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumBGPRate@V@out{1.5}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumBGPRate@V@out{0.2}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumBGPRate@V@out{6.3}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumBGPRate@V@out{4.9}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumBGPRate@V@out{1.3}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FullMassSpectrumBGPRate@V@out{2.1710767640642694}\else\def\FullMassSpectrumBGPRate@V@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumBGPRate@V@out}\newcommand\FullMassSpectrumBGPRate@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumBGPRate@VI@out{\{"50th\_percentile": 110, "5th\_percentile": 50, "95th\_percentile": 240, "error\_plus": 130, "error\_minus": 60, "mean": 120.1241759479467\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumBGPRate@VI@out{110}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumBGPRate@VI@out{50}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumBGPRate@VI@out{240}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumBGPRate@VI@out{130}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumBGPRate@VI@out{60}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\FullMassSpectrumBGPRate@VI@out{120.1241759479467}\else\def\FullMassSpectrumBGPRate@VI@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumBGPRate@VI@out}\makeatother
\makeatletter\newcommand\FullMassSpectrumMerged[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumMerged@out{\{"R\_BNS": \{"50th\_percentile": 77, "95th\_percentile": 250, "5th\_percentile": 7.6, "error\_plus": 170, "error\_minus": 69\}, "R\_NSBH": \{"50th\_percentile": 25, "95th\_percentile": 84, "5th\_percentile": 9.1, "error\_plus": 59, "error\_minus": 16\}, "R\_BBH": \{"50th\_percentile": 19, "95th\_percentile": 26, "5th\_percentile": 14, "error\_plus": 7.0, "error\_minus": 5.0\}, "R\_NS{-}Gap": \{"50th\_percentile": 9.7, "95th\_percentile": 61, "5th\_percentile": 1.2, "error\_plus": 51, "error\_minus": 8.5\}, "R\_BH{-}Gap": \{"50th\_percentile": 2.2, "95th\_percentile": 6.3, "5th\_percentile": 0.2, "error\_plus": 4.1, "error\_minus": 2.0\}, "R\_Full": \{"50th\_percentile": 130, "95th\_percentile": 300, "5th\_percentile": 49, "error\_plus": 170, "error\_minus": 81\}\}}\else\ifnum\pdfstrcmp{#1}{R_BNS}=0\let\FullMassSpectrumMerged@out\FullMassSpectrumMerged@I\else\ifnum\pdfstrcmp{#1}{R_NSBH}=0\let\FullMassSpectrumMerged@out\FullMassSpectrumMerged@II\else\ifnum\pdfstrcmp{#1}{R_BBH}=0\let\FullMassSpectrumMerged@out\FullMassSpectrumMerged@III\else\ifnum\pdfstrcmp{#1}{R_NS-Gap}=0\let\FullMassSpectrumMerged@out\FullMassSpectrumMerged@IV\else\ifnum\pdfstrcmp{#1}{R_BH-Gap}=0\let\FullMassSpectrumMerged@out\FullMassSpectrumMerged@V\else\ifnum\pdfstrcmp{#1}{R_Full}=0\let\FullMassSpectrumMerged@out\FullMassSpectrumMerged@VI\else\def\FullMassSpectrumMerged@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumMerged@out}\newcommand\FullMassSpectrumMerged@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumMerged@I@out{\{"50th\_percentile": 77, "95th\_percentile": 250, "5th\_percentile": 7.6, "error\_plus": 170, "error\_minus": 69\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumMerged@I@out{77}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumMerged@I@out{250}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumMerged@I@out{7.6}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumMerged@I@out{170}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumMerged@I@out{69}\else\def\FullMassSpectrumMerged@I@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumMerged@I@out}\newcommand\FullMassSpectrumMerged@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumMerged@II@out{\{"50th\_percentile": 25, "95th\_percentile": 84, "5th\_percentile": 9.1, "error\_plus": 59, "error\_minus": 16\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumMerged@II@out{25}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumMerged@II@out{84}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumMerged@II@out{9.1}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumMerged@II@out{59}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumMerged@II@out{16}\else\def\FullMassSpectrumMerged@II@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumMerged@II@out}\newcommand\FullMassSpectrumMerged@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumMerged@III@out{\{"50th\_percentile": 19, "95th\_percentile": 26, "5th\_percentile": 14, "error\_plus": 7.0, "error\_minus": 5.0\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumMerged@III@out{19}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumMerged@III@out{26}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumMerged@III@out{14}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumMerged@III@out{7.0}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumMerged@III@out{5.0}\else\def\FullMassSpectrumMerged@III@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumMerged@III@out}\newcommand\FullMassSpectrumMerged@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumMerged@IV@out{\{"50th\_percentile": 9.7, "95th\_percentile": 61, "5th\_percentile": 1.2, "error\_plus": 51, "error\_minus": 8.5\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumMerged@IV@out{9.7}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumMerged@IV@out{61}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumMerged@IV@out{1.2}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumMerged@IV@out{51}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumMerged@IV@out{8.5}\else\def\FullMassSpectrumMerged@IV@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumMerged@IV@out}\newcommand\FullMassSpectrumMerged@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumMerged@V@out{\{"50th\_percentile": 2.2, "95th\_percentile": 6.3, "5th\_percentile": 0.2, "error\_plus": 4.1, "error\_minus": 2.0\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumMerged@V@out{2.2}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumMerged@V@out{6.3}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumMerged@V@out{0.2}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumMerged@V@out{4.1}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumMerged@V@out{2.0}\else\def\FullMassSpectrumMerged@V@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumMerged@V@out}\newcommand\FullMassSpectrumMerged@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumMerged@VI@out{\{"50th\_percentile": 130, "95th\_percentile": 300, "5th\_percentile": 49, "error\_plus": 170, "error\_minus": 81\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\FullMassSpectrumMerged@VI@out{130}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\FullMassSpectrumMerged@VI@out{300}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\FullMassSpectrumMerged@VI@out{49}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\FullMassSpectrumMerged@VI@out{170}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\FullMassSpectrumMerged@VI@out{81}\else\def\FullMassSpectrumMerged@VI@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumMerged@VI@out}\makeatother
\makeatletter\newcommand\FullMassSpectrumPDB[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@out{\{"rates": \{"BNS": \{"median": 89, "error plus": 159, "error minus": 67, "5th percentile": 22, "95th percentile": 248\}, "NSBH": \{"median": 23, "error plus": 20, "error minus": 13, "5th percentile": 10, "95th percentile": 42\}, "BBH": \{"median": 19, "error plus": 7, "error minus": 5, "5th percentile": 14, "95th percentile": 26\}, "NS{-}Gap": \{"median": 6.7, "error plus": 9.2, "error minus": 4.6, "5th percentile": 2.2, "95th percentile": 15.9\}, "BH{-}Gap": \{"median": 2.5, "error plus": 3.4, "error minus": 1.6, "5th percentile": 0.9, "95th percentile": 5.9\}, "Full": \{"median": 130, "error plus": 160, "error minus": 80, "5th percentile": 60, "95th percentile": 300\}\}, "pairing\_function\_difference": 100.0\}}\else\ifnum\pdfstrcmp{#1}{rates}=0\let\FullMassSpectrumPDB@out\FullMassSpectrumPDB@I\else\ifnum\pdfstrcmp{#1}{pairing_function_difference}=0\def\FullMassSpectrumPDB@out{100.0}\else\def\FullMassSpectrumPDB@out{??}\fi\fi\fi\FullMassSpectrumPDB@out}\newcommand\FullMassSpectrumPDB@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@I@out{\{"BNS": \{"median": 89, "error plus": 159, "error minus": 67, "5th percentile": 22, "95th percentile": 248\}, "NSBH": \{"median": 23, "error plus": 20, "error minus": 13, "5th percentile": 10, "95th percentile": 42\}, "BBH": \{"median": 19, "error plus": 7, "error minus": 5, "5th percentile": 14, "95th percentile": 26\}, "NS{-}Gap": \{"median": 6.7, "error plus": 9.2, "error minus": 4.6, "5th percentile": 2.2, "95th percentile": 15.9\}, "BH{-}Gap": \{"median": 2.5, "error plus": 3.4, "error minus": 1.6, "5th percentile": 0.9, "95th percentile": 5.9\}, "Full": \{"median": 130, "error plus": 160, "error minus": 80, "5th percentile": 60, "95th percentile": 300\}\}}\else\ifnum\pdfstrcmp{#1}{BNS}=0\let\FullMassSpectrumPDB@I@out\FullMassSpectrumPDB@II\else\ifnum\pdfstrcmp{#1}{NSBH}=0\let\FullMassSpectrumPDB@I@out\FullMassSpectrumPDB@III\else\ifnum\pdfstrcmp{#1}{BBH}=0\let\FullMassSpectrumPDB@I@out\FullMassSpectrumPDB@IV\else\ifnum\pdfstrcmp{#1}{NS-Gap}=0\let\FullMassSpectrumPDB@I@out\FullMassSpectrumPDB@V\else\ifnum\pdfstrcmp{#1}{BH-Gap}=0\let\FullMassSpectrumPDB@I@out\FullMassSpectrumPDB@VI\else\ifnum\pdfstrcmp{#1}{Full}=0\let\FullMassSpectrumPDB@I@out\FullMassSpectrumPDB@VII\else\def\FullMassSpectrumPDB@I@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDB@I@out}\newcommand\FullMassSpectrumPDB@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@II@out{\{"median": 89, "error plus": 159, "error minus": 67, "5th percentile": 22, "95th percentile": 248\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDB@II@out{89}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDB@II@out{159}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDB@II@out{67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDB@II@out{22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDB@II@out{248}\else\def\FullMassSpectrumPDB@II@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDB@II@out}\newcommand\FullMassSpectrumPDB@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@III@out{\{"median": 23, "error plus": 20, "error minus": 13, "5th percentile": 10, "95th percentile": 42\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDB@III@out{23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDB@III@out{20}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDB@III@out{13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDB@III@out{10}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDB@III@out{42}\else\def\FullMassSpectrumPDB@III@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDB@III@out}\newcommand\FullMassSpectrumPDB@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@IV@out{\{"median": 19, "error plus": 7, "error minus": 5, "5th percentile": 14, "95th percentile": 26\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDB@IV@out{19}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDB@IV@out{7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDB@IV@out{5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDB@IV@out{14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDB@IV@out{26}\else\def\FullMassSpectrumPDB@IV@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDB@IV@out}\newcommand\FullMassSpectrumPDB@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@V@out{\{"median": 6.7, "error plus": 9.2, "error minus": 4.6, "5th percentile": 2.2, "95th percentile": 15.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDB@V@out{6.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDB@V@out{9.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDB@V@out{4.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDB@V@out{2.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDB@V@out{15.9}\else\def\FullMassSpectrumPDB@V@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDB@V@out}\newcommand\FullMassSpectrumPDB@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@VI@out{\{"median": 2.5, "error plus": 3.4, "error minus": 1.6, "5th percentile": 0.9, "95th percentile": 5.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDB@VI@out{2.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDB@VI@out{3.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDB@VI@out{1.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDB@VI@out{0.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDB@VI@out{5.9}\else\def\FullMassSpectrumPDB@VI@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDB@VI@out}\newcommand\FullMassSpectrumPDB@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDB@VII@out{\{"median": 130, "error plus": 160, "error minus": 80, "5th percentile": 60, "95th percentile": 300\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDB@VII@out{130}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDB@VII@out{160}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDB@VII@out{80}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDB@VII@out{60}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDB@VII@out{300}\else\def\FullMassSpectrumPDB@VII@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDB@VII@out}\makeatother
\makeatletter\newcommand\FullMassSpectrumPDBNoDip[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@out{\{"rates": \{"BNS": \{"median": 92, "error plus": 159, "error minus": 67, "5th percentile": 25, "95th percentile": 251\}, "NSBH": \{"median": 22, "error plus": 20, "error minus": 12, "5th percentile": 10, "95th percentile": 43\}, "BBH": \{"median": 19, "error plus": 7, "error minus": 5, "5th percentile": 14, "95th percentile": 26\}, "NS{-}Gap": \{"median": 7.4, "error plus": 9.5, "error minus": 4.8, "5th percentile": 2.6, "95th percentile": 16.9\}, "BH{-}Gap": \{"median": 2.7, "error plus": 3.3, "error minus": 1.7, "5th percentile": 1.0, "95th percentile": 6.1\}, "Full": \{"median": 140, "error plus": 170, "error minus": 80, "5th percentile": 60, "95th percentile": 300\}\}, "pairing\_function\_difference": 99.0\}}\else\ifnum\pdfstrcmp{#1}{rates}=0\let\FullMassSpectrumPDBNoDip@out\FullMassSpectrumPDBNoDip@I\else\ifnum\pdfstrcmp{#1}{pairing_function_difference}=0\def\FullMassSpectrumPDBNoDip@out{99.0}\else\def\FullMassSpectrumPDBNoDip@out{??}\fi\fi\fi\FullMassSpectrumPDBNoDip@out}\newcommand\FullMassSpectrumPDBNoDip@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@I@out{\{"BNS": \{"median": 92, "error plus": 159, "error minus": 67, "5th percentile": 25, "95th percentile": 251\}, "NSBH": \{"median": 22, "error plus": 20, "error minus": 12, "5th percentile": 10, "95th percentile": 43\}, "BBH": \{"median": 19, "error plus": 7, "error minus": 5, "5th percentile": 14, "95th percentile": 26\}, "NS{-}Gap": \{"median": 7.4, "error plus": 9.5, "error minus": 4.8, "5th percentile": 2.6, "95th percentile": 16.9\}, "BH{-}Gap": \{"median": 2.7, "error plus": 3.3, "error minus": 1.7, "5th percentile": 1.0, "95th percentile": 6.1\}, "Full": \{"median": 140, "error plus": 170, "error minus": 80, "5th percentile": 60, "95th percentile": 300\}\}}\else\ifnum\pdfstrcmp{#1}{BNS}=0\let\FullMassSpectrumPDBNoDip@I@out\FullMassSpectrumPDBNoDip@II\else\ifnum\pdfstrcmp{#1}{NSBH}=0\let\FullMassSpectrumPDBNoDip@I@out\FullMassSpectrumPDBNoDip@III\else\ifnum\pdfstrcmp{#1}{BBH}=0\let\FullMassSpectrumPDBNoDip@I@out\FullMassSpectrumPDBNoDip@IV\else\ifnum\pdfstrcmp{#1}{NS-Gap}=0\let\FullMassSpectrumPDBNoDip@I@out\FullMassSpectrumPDBNoDip@V\else\ifnum\pdfstrcmp{#1}{BH-Gap}=0\let\FullMassSpectrumPDBNoDip@I@out\FullMassSpectrumPDBNoDip@VI\else\ifnum\pdfstrcmp{#1}{Full}=0\let\FullMassSpectrumPDBNoDip@I@out\FullMassSpectrumPDBNoDip@VII\else\def\FullMassSpectrumPDBNoDip@I@out{??}\fi\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDBNoDip@I@out}\newcommand\FullMassSpectrumPDBNoDip@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@II@out{\{"median": 92, "error plus": 159, "error minus": 67, "5th percentile": 25, "95th percentile": 251\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDBNoDip@II@out{92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDBNoDip@II@out{159}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDBNoDip@II@out{67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDBNoDip@II@out{25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDBNoDip@II@out{251}\else\def\FullMassSpectrumPDBNoDip@II@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDBNoDip@II@out}\newcommand\FullMassSpectrumPDBNoDip@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@III@out{\{"median": 22, "error plus": 20, "error minus": 12, "5th percentile": 10, "95th percentile": 43\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDBNoDip@III@out{22}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDBNoDip@III@out{20}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDBNoDip@III@out{12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDBNoDip@III@out{10}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDBNoDip@III@out{43}\else\def\FullMassSpectrumPDBNoDip@III@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDBNoDip@III@out}\newcommand\FullMassSpectrumPDBNoDip@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@IV@out{\{"median": 19, "error plus": 7, "error minus": 5, "5th percentile": 14, "95th percentile": 26\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDBNoDip@IV@out{19}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDBNoDip@IV@out{7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDBNoDip@IV@out{5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDBNoDip@IV@out{14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDBNoDip@IV@out{26}\else\def\FullMassSpectrumPDBNoDip@IV@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDBNoDip@IV@out}\newcommand\FullMassSpectrumPDBNoDip@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@V@out{\{"median": 7.4, "error plus": 9.5, "error minus": 4.8, "5th percentile": 2.6, "95th percentile": 16.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDBNoDip@V@out{7.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDBNoDip@V@out{9.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDBNoDip@V@out{4.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDBNoDip@V@out{2.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDBNoDip@V@out{16.9}\else\def\FullMassSpectrumPDBNoDip@V@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDBNoDip@V@out}\newcommand\FullMassSpectrumPDBNoDip@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@VI@out{\{"median": 2.7, "error plus": 3.3, "error minus": 1.7, "5th percentile": 1.0, "95th percentile": 6.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDBNoDip@VI@out{2.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDBNoDip@VI@out{3.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDBNoDip@VI@out{1.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDBNoDip@VI@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDBNoDip@VI@out{6.1}\else\def\FullMassSpectrumPDBNoDip@VI@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDBNoDip@VI@out}\newcommand\FullMassSpectrumPDBNoDip@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullMassSpectrumPDBNoDip@VII@out{\{"median": 140, "error plus": 170, "error minus": 80, "5th percentile": 60, "95th percentile": 300\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullMassSpectrumPDBNoDip@VII@out{140}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullMassSpectrumPDBNoDip@VII@out{170}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullMassSpectrumPDBNoDip@VII@out{80}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullMassSpectrumPDBNoDip@VII@out{60}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullMassSpectrumPDBNoDip@VII@out{300}\else\def\FullMassSpectrumPDBNoDip@VII@out{??}\fi\fi\fi\fi\fi\fi\FullMassSpectrumPDBNoDip@VII@out}\makeatother
\makeatletter\newcommand\FullPop[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@out{\{"rates": \{"BNS": \{"median": 89.4, "error plus": 159, "error minus": 66.9, "5th percentile": 22.5, "95th percentile": 248\}, "NSBH": \{"median": 22.8, "error plus": 19.6, "error minus": 12.6, "5th percentile": 10.2, "95th percentile": 42.4\}, "BBH": \{"median": 19, "error plus": 7.16, "error minus": 5.19, "5th percentile": 13.8, "95th percentile": 26.2\}, "NS{-}Gap": \{"median": 6.73, "error plus": 9.17, "error minus": 4.56, "5th percentile": 2.17, "95th percentile": 15.9\}, "BH{-}Gap": \{"median": 2.47, "error plus": 3.39, "error minus": 1.61, "5th percentile": 0.855, "95th percentile": 5.86\}, "Full": \{"median": 134, "error plus": 164, "error minus": 76, "5th percentile": 57.6, "95th percentile": 298\}\}, "pairing\_function\_difference": 1.0, "peak\_locations": \{"OneMsun": \{"median": 1.23, "error plus": 0.14, "error minus": 0.15, "5th percentile": 1.08, "95th percentile": 1.37\}, "TenMsun": \{"median": 9.02, "error plus": 0.41, "error minus": 1.21, "5th percentile": 7.81, "95th percentile": 9.43\}, "ThirtyMsun": \{"median": 26.9, "error plus": 13.1, "error minus": 8.1, "5th percentile": 18.8, "95th percentile": 40\}\}\}}\else\ifnum\pdfstrcmp{#1}{rates}=0\let\FullPop@out\FullPop@I\else\ifnum\pdfstrcmp{#1}{pairing_function_difference}=0\def\FullPop@out{1.0}\else\ifnum\pdfstrcmp{#1}{peak_locations}=0\let\FullPop@out\FullPop@II\else\def\FullPop@out{??}\fi\fi\fi\fi\FullPop@out}\newcommand\FullPop@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@I@out{\{"BNS": \{"median": 89.4, "error plus": 159, "error minus": 66.9, "5th percentile": 22.5, "95th percentile": 248\}, "NSBH": \{"median": 22.8, "error plus": 19.6, "error minus": 12.6, "5th percentile": 10.2, "95th percentile": 42.4\}, "BBH": \{"median": 19, "error plus": 7.16, "error minus": 5.19, "5th percentile": 13.8, "95th percentile": 26.2\}, "NS{-}Gap": \{"median": 6.73, "error plus": 9.17, "error minus": 4.56, "5th percentile": 2.17, "95th percentile": 15.9\}, "BH{-}Gap": \{"median": 2.47, "error plus": 3.39, "error minus": 1.61, "5th percentile": 0.855, "95th percentile": 5.86\}, "Full": \{"median": 134, "error plus": 164, "error minus": 76, "5th percentile": 57.6, "95th percentile": 298\}\}}\else\ifnum\pdfstrcmp{#1}{BNS}=0\let\FullPop@I@out\FullPop@III\else\ifnum\pdfstrcmp{#1}{NSBH}=0\let\FullPop@I@out\FullPop@IV\else\ifnum\pdfstrcmp{#1}{BBH}=0\let\FullPop@I@out\FullPop@V\else\ifnum\pdfstrcmp{#1}{NS-Gap}=0\let\FullPop@I@out\FullPop@VI\else\ifnum\pdfstrcmp{#1}{BH-Gap}=0\let\FullPop@I@out\FullPop@VII\else\ifnum\pdfstrcmp{#1}{Full}=0\let\FullPop@I@out\FullPop@VIII\else\def\FullPop@I@out{??}\fi\fi\fi\fi\fi\fi\fi\FullPop@I@out}\newcommand\FullPop@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@II@out{\{"OneMsun": \{"median": 1.23, "error plus": 0.14, "error minus": 0.15, "5th percentile": 1.08, "95th percentile": 1.37\}, "TenMsun": \{"median": 9.02, "error plus": 0.41, "error minus": 1.21, "5th percentile": 7.81, "95th percentile": 9.43\}, "ThirtyMsun": \{"median": 26.9, "error plus": 13.1, "error minus": 8.1, "5th percentile": 18.8, "95th percentile": 40\}\}}\else\ifnum\pdfstrcmp{#1}{OneMsun}=0\let\FullPop@II@out\FullPop@IX\else\ifnum\pdfstrcmp{#1}{TenMsun}=0\let\FullPop@II@out\FullPop@X\else\ifnum\pdfstrcmp{#1}{ThirtyMsun}=0\let\FullPop@II@out\FullPop@XI\else\def\FullPop@II@out{??}\fi\fi\fi\fi\FullPop@II@out}\newcommand\FullPop@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@III@out{\{"median": 89.4, "error plus": 159, "error minus": 66.9, "5th percentile": 22.5, "95th percentile": 248\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@III@out{89.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@III@out{159}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@III@out{66.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@III@out{22.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@III@out{248}\else\def\FullPop@III@out{??}\fi\fi\fi\fi\fi\fi\FullPop@III@out}\newcommand\FullPop@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@IV@out{\{"median": 22.8, "error plus": 19.6, "error minus": 12.6, "5th percentile": 10.2, "95th percentile": 42.4\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@IV@out{22.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@IV@out{19.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@IV@out{12.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@IV@out{10.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@IV@out{42.4}\else\def\FullPop@IV@out{??}\fi\fi\fi\fi\fi\fi\FullPop@IV@out}\newcommand\FullPop@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@V@out{\{"median": 19, "error plus": 7.16, "error minus": 5.19, "5th percentile": 13.8, "95th percentile": 26.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@V@out{19}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@V@out{7.16}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@V@out{5.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@V@out{13.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@V@out{26.2}\else\def\FullPop@V@out{??}\fi\fi\fi\fi\fi\fi\FullPop@V@out}\newcommand\FullPop@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@VI@out{\{"median": 6.73, "error plus": 9.17, "error minus": 4.56, "5th percentile": 2.17, "95th percentile": 15.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@VI@out{6.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@VI@out{9.17}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@VI@out{4.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@VI@out{2.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@VI@out{15.9}\else\def\FullPop@VI@out{??}\fi\fi\fi\fi\fi\fi\FullPop@VI@out}\newcommand\FullPop@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@VII@out{\{"median": 2.47, "error plus": 3.39, "error minus": 1.61, "5th percentile": 0.855, "95th percentile": 5.86\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@VII@out{2.47}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@VII@out{3.39}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@VII@out{1.61}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@VII@out{0.855}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@VII@out{5.86}\else\def\FullPop@VII@out{??}\fi\fi\fi\fi\fi\fi\FullPop@VII@out}\newcommand\FullPop@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@VIII@out{\{"median": 134, "error plus": 164, "error minus": 76, "5th percentile": 57.6, "95th percentile": 298\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@VIII@out{134}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@VIII@out{164}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@VIII@out{76}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@VIII@out{57.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@VIII@out{298}\else\def\FullPop@VIII@out{??}\fi\fi\fi\fi\fi\fi\FullPop@VIII@out}\newcommand\FullPop@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@IX@out{\{"median": 1.23, "error plus": 0.14, "error minus": 0.15, "5th percentile": 1.08, "95th percentile": 1.37\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@IX@out{1.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@IX@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@IX@out{0.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@IX@out{1.08}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@IX@out{1.37}\else\def\FullPop@IX@out{??}\fi\fi\fi\fi\fi\fi\FullPop@IX@out}\newcommand\FullPop@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@X@out{\{"median": 9.02, "error plus": 0.41, "error minus": 1.21, "5th percentile": 7.81, "95th percentile": 9.43\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@X@out{9.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@X@out{0.41}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@X@out{1.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@X@out{7.81}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@X@out{9.43}\else\def\FullPop@X@out{??}\fi\fi\fi\fi\fi\fi\FullPop@X@out}\newcommand\FullPop@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPop@XI@out{\{"median": 26.9, "error plus": 13.1, "error minus": 8.1, "5th percentile": 18.8, "95th percentile": 40\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPop@XI@out{26.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPop@XI@out{13.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPop@XI@out{8.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPop@XI@out{18.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPop@XI@out{40}\else\def\FullPop@XI@out{??}\fi\fi\fi\fi\fi\fi\FullPop@XI@out}\makeatother
\makeatletter\newcommand\FullPopNoDip[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@out{\{"rates": \{"BNS": \{"median": 91.9, "error plus": 159, "error minus": 66.8, "5th percentile": 25.1, "95th percentile": 251\}, "NSBH": \{"median": 22.4, "error plus": 20.1, "error minus": 12.4, "5th percentile": 9.99, "95th percentile": 42.6\}, "BBH": \{"median": 18.9, "error plus": 6.8, "error minus": 5.49, "5th percentile": 13.5, "95th percentile": 25.7\}, "NS{-}Gap": \{"median": 7.4, "error plus": 9.49, "error minus": 4.8, "5th percentile": 2.6, "95th percentile": 16.9\}, "BH{-}Gap": \{"median": 2.73, "error plus": 3.32, "error minus": 1.69, "5th percentile": 1.04, "95th percentile": 6.06\}, "Full": \{"median": 135, "error plus": 169, "error minus": 75.5, "5th percentile": 59.6, "95th percentile": 304\}\}, "pairing\_function\_difference": 0.99, "peak\_locations": \{"OneMsun": \{"median": 1.23, "error plus": 0.12, "error minus": 0.155, "5th percentile": 1.08, "95th percentile": 1.35\}, "TenMsun": \{"median": 9.18, "error plus": 0.31, "error minus": 0.41, "5th percentile": 8.77, "95th percentile": 9.49\}, "ThirtyMsun": \{"median": 25.9, "error plus": 13.9, "error minus": 7.49, "5th percentile": 18.4, "95th percentile": 39.8\}\}\}}\else\ifnum\pdfstrcmp{#1}{rates}=0\let\FullPopNoDip@out\FullPopNoDip@I\else\ifnum\pdfstrcmp{#1}{pairing_function_difference}=0\def\FullPopNoDip@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak_locations}=0\let\FullPopNoDip@out\FullPopNoDip@II\else\def\FullPopNoDip@out{??}\fi\fi\fi\fi\FullPopNoDip@out}\newcommand\FullPopNoDip@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@I@out{\{"BNS": \{"median": 91.9, "error plus": 159, "error minus": 66.8, "5th percentile": 25.1, "95th percentile": 251\}, "NSBH": \{"median": 22.4, "error plus": 20.1, "error minus": 12.4, "5th percentile": 9.99, "95th percentile": 42.6\}, "BBH": \{"median": 18.9, "error plus": 6.8, "error minus": 5.49, "5th percentile": 13.5, "95th percentile": 25.7\}, "NS{-}Gap": \{"median": 7.4, "error plus": 9.49, "error minus": 4.8, "5th percentile": 2.6, "95th percentile": 16.9\}, "BH{-}Gap": \{"median": 2.73, "error plus": 3.32, "error minus": 1.69, "5th percentile": 1.04, "95th percentile": 6.06\}, "Full": \{"median": 135, "error plus": 169, "error minus": 75.5, "5th percentile": 59.6, "95th percentile": 304\}\}}\else\ifnum\pdfstrcmp{#1}{BNS}=0\let\FullPopNoDip@I@out\FullPopNoDip@III\else\ifnum\pdfstrcmp{#1}{NSBH}=0\let\FullPopNoDip@I@out\FullPopNoDip@IV\else\ifnum\pdfstrcmp{#1}{BBH}=0\let\FullPopNoDip@I@out\FullPopNoDip@V\else\ifnum\pdfstrcmp{#1}{NS-Gap}=0\let\FullPopNoDip@I@out\FullPopNoDip@VI\else\ifnum\pdfstrcmp{#1}{BH-Gap}=0\let\FullPopNoDip@I@out\FullPopNoDip@VII\else\ifnum\pdfstrcmp{#1}{Full}=0\let\FullPopNoDip@I@out\FullPopNoDip@VIII\else\def\FullPopNoDip@I@out{??}\fi\fi\fi\fi\fi\fi\fi\FullPopNoDip@I@out}\newcommand\FullPopNoDip@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@II@out{\{"OneMsun": \{"median": 1.23, "error plus": 0.12, "error minus": 0.155, "5th percentile": 1.08, "95th percentile": 1.35\}, "TenMsun": \{"median": 9.18, "error plus": 0.31, "error minus": 0.41, "5th percentile": 8.77, "95th percentile": 9.49\}, "ThirtyMsun": \{"median": 25.9, "error plus": 13.9, "error minus": 7.49, "5th percentile": 18.4, "95th percentile": 39.8\}\}}\else\ifnum\pdfstrcmp{#1}{OneMsun}=0\let\FullPopNoDip@II@out\FullPopNoDip@IX\else\ifnum\pdfstrcmp{#1}{TenMsun}=0\let\FullPopNoDip@II@out\FullPopNoDip@X\else\ifnum\pdfstrcmp{#1}{ThirtyMsun}=0\let\FullPopNoDip@II@out\FullPopNoDip@XI\else\def\FullPopNoDip@II@out{??}\fi\fi\fi\fi\FullPopNoDip@II@out}\newcommand\FullPopNoDip@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@III@out{\{"median": 91.9, "error plus": 159, "error minus": 66.8, "5th percentile": 25.1, "95th percentile": 251\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@III@out{91.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@III@out{159}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@III@out{66.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@III@out{25.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@III@out{251}\else\def\FullPopNoDip@III@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@III@out}\newcommand\FullPopNoDip@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@IV@out{\{"median": 22.4, "error plus": 20.1, "error minus": 12.4, "5th percentile": 9.99, "95th percentile": 42.6\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@IV@out{22.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@IV@out{20.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@IV@out{12.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@IV@out{9.99}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@IV@out{42.6}\else\def\FullPopNoDip@IV@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@IV@out}\newcommand\FullPopNoDip@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@V@out{\{"median": 18.9, "error plus": 6.8, "error minus": 5.49, "5th percentile": 13.5, "95th percentile": 25.7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@V@out{18.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@V@out{6.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@V@out{5.49}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@V@out{13.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@V@out{25.7}\else\def\FullPopNoDip@V@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@V@out}\newcommand\FullPopNoDip@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@VI@out{\{"median": 7.4, "error plus": 9.49, "error minus": 4.8, "5th percentile": 2.6, "95th percentile": 16.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@VI@out{7.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@VI@out{9.49}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@VI@out{4.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@VI@out{2.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@VI@out{16.9}\else\def\FullPopNoDip@VI@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@VI@out}\newcommand\FullPopNoDip@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@VII@out{\{"median": 2.73, "error plus": 3.32, "error minus": 1.69, "5th percentile": 1.04, "95th percentile": 6.06\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@VII@out{2.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@VII@out{3.32}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@VII@out{1.69}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@VII@out{1.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@VII@out{6.06}\else\def\FullPopNoDip@VII@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@VII@out}\newcommand\FullPopNoDip@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@VIII@out{\{"median": 135, "error plus": 169, "error minus": 75.5, "5th percentile": 59.6, "95th percentile": 304\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@VIII@out{135}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@VIII@out{169}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@VIII@out{75.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@VIII@out{59.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@VIII@out{304}\else\def\FullPopNoDip@VIII@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@VIII@out}\newcommand\FullPopNoDip@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@IX@out{\{"median": 1.23, "error plus": 0.12, "error minus": 0.155, "5th percentile": 1.08, "95th percentile": 1.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@IX@out{1.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@IX@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@IX@out{0.155}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@IX@out{1.08}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@IX@out{1.35}\else\def\FullPopNoDip@IX@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@IX@out}\newcommand\FullPopNoDip@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@X@out{\{"median": 9.18, "error plus": 0.31, "error minus": 0.41, "5th percentile": 8.77, "95th percentile": 9.49\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@X@out{9.18}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@X@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@X@out{0.41}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@X@out{8.77}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@X@out{9.49}\else\def\FullPopNoDip@X@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@X@out}\newcommand\FullPopNoDip@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\FullPopNoDip@XI@out{\{"median": 25.9, "error plus": 13.9, "error minus": 7.49, "5th percentile": 18.4, "95th percentile": 39.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\FullPopNoDip@XI@out{25.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\FullPopNoDip@XI@out{13.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\FullPopNoDip@XI@out{7.49}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\FullPopNoDip@XI@out{18.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\FullPopNoDip@XI@out{39.8}\else\def\FullPopNoDip@XI@out{??}\fi\fi\fi\fi\fi\fi\FullPopNoDip@XI@out}\makeatother
\makeatletter\newcommand\gaussianChiEffChiP[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@out{\{"param": \{"mu\_eff": \{"median": 0.04, "5th percentile": 0.02, "95th percentile": 0.06, "error plus": 0.02, "error minus": 0.02\}, "sig\_eff": \{"median": 0.1, "5th percentile": 0.08, "95th percentile": 0.13, "error plus": 0.03, "error minus": 0.02\}, "mu\_p": \{"median": 0.31, "5th percentile": 0.23, "95th percentile": 0.39, "error plus": 0.08, "error minus": 0.08\}, "sig\_p": \{"median": 0.19, "5th percentile": 0.12, "95th percentile": 0.33, "error plus": 0.15, "error minus": 0.07\}, "cov": \{"median": 0.06, "5th percentile": {-}0.47, "95th percentile": 0.55, "error plus": 0.49, "error minus": 0.53\}, "min\_eff": \{"median": {-}0.2, "5th percentile": {-}0.27, "95th percentile": {-}0.13, "error plus": 0.06, "error minus": 0.07\}, "f\_neg\_eff": \{"median": 0.34, "5th percentile": 0.24, "95th percentile": 0.43, "error plus": 0.09, "error minus": 0.1\}\}, "ppd": \{"chi\_eff": \{"median": 0.04, "5th percentile": {-}0.13, "95th percentile": 0.22, "spin at peak": 0.04\}, "chi\_p": \{"median": 0.33, "5th percentile": 0.07, "95th percentile": 0.66, "spin at peak": 0.31\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\gaussianChiEffChiP@out\gaussianChiEffChiP@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\gaussianChiEffChiP@out\gaussianChiEffChiP@II\else\def\gaussianChiEffChiP@out{??}\fi\fi\fi\gaussianChiEffChiP@out}\newcommand\gaussianChiEffChiP@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@I@out{\{"mu\_eff": \{"median": 0.04, "5th percentile": 0.02, "95th percentile": 0.06, "error plus": 0.02, "error minus": 0.02\}, "sig\_eff": \{"median": 0.1, "5th percentile": 0.08, "95th percentile": 0.13, "error plus": 0.03, "error minus": 0.02\}, "mu\_p": \{"median": 0.31, "5th percentile": 0.23, "95th percentile": 0.39, "error plus": 0.08, "error minus": 0.08\}, "sig\_p": \{"median": 0.19, "5th percentile": 0.12, "95th percentile": 0.33, "error plus": 0.15, "error minus": 0.07\}, "cov": \{"median": 0.06, "5th percentile": {-}0.47, "95th percentile": 0.55, "error plus": 0.49, "error minus": 0.53\}, "min\_eff": \{"median": {-}0.2, "5th percentile": {-}0.27, "95th percentile": {-}0.13, "error plus": 0.06, "error minus": 0.07\}, "f\_neg\_eff": \{"median": 0.34, "5th percentile": 0.24, "95th percentile": 0.43, "error plus": 0.09, "error minus": 0.1\}\}}\else\ifnum\pdfstrcmp{#1}{mu_eff}=0\let\gaussianChiEffChiP@I@out\gaussianChiEffChiP@III\else\ifnum\pdfstrcmp{#1}{sig_eff}=0\let\gaussianChiEffChiP@I@out\gaussianChiEffChiP@IV\else\ifnum\pdfstrcmp{#1}{mu_p}=0\let\gaussianChiEffChiP@I@out\gaussianChiEffChiP@V\else\ifnum\pdfstrcmp{#1}{sig_p}=0\let\gaussianChiEffChiP@I@out\gaussianChiEffChiP@VI\else\ifnum\pdfstrcmp{#1}{cov}=0\let\gaussianChiEffChiP@I@out\gaussianChiEffChiP@VII\else\ifnum\pdfstrcmp{#1}{min_eff}=0\let\gaussianChiEffChiP@I@out\gaussianChiEffChiP@VIII\else\ifnum\pdfstrcmp{#1}{f_neg_eff}=0\let\gaussianChiEffChiP@I@out\gaussianChiEffChiP@IX\else\def\gaussianChiEffChiP@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@I@out}\newcommand\gaussianChiEffChiP@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@II@out{\{"chi\_eff": \{"median": 0.04, "5th percentile": {-}0.13, "95th percentile": 0.22, "spin at peak": 0.04\}, "chi\_p": \{"median": 0.33, "5th percentile": 0.07, "95th percentile": 0.66, "spin at peak": 0.31\}\}}\else\ifnum\pdfstrcmp{#1}{chi_eff}=0\let\gaussianChiEffChiP@II@out\gaussianChiEffChiP@X\else\ifnum\pdfstrcmp{#1}{chi_p}=0\let\gaussianChiEffChiP@II@out\gaussianChiEffChiP@XI\else\def\gaussianChiEffChiP@II@out{??}\fi\fi\fi\gaussianChiEffChiP@II@out}\newcommand\gaussianChiEffChiP@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@III@out{\{"median": 0.04, "5th percentile": 0.02, "95th percentile": 0.06, "error plus": 0.02, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@III@out{0.04}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@III@out{0.02}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@III@out{0.06}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\gaussianChiEffChiP@III@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\gaussianChiEffChiP@III@out{0.02}\else\def\gaussianChiEffChiP@III@out{??}\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@III@out}\newcommand\gaussianChiEffChiP@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@IV@out{\{"median": 0.1, "5th percentile": 0.08, "95th percentile": 0.13, "error plus": 0.03, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@IV@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@IV@out{0.08}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@IV@out{0.13}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\gaussianChiEffChiP@IV@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\gaussianChiEffChiP@IV@out{0.02}\else\def\gaussianChiEffChiP@IV@out{??}\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@IV@out}\newcommand\gaussianChiEffChiP@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@V@out{\{"median": 0.31, "5th percentile": 0.23, "95th percentile": 0.39, "error plus": 0.08, "error minus": 0.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@V@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@V@out{0.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@V@out{0.39}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\gaussianChiEffChiP@V@out{0.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\gaussianChiEffChiP@V@out{0.08}\else\def\gaussianChiEffChiP@V@out{??}\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@V@out}\newcommand\gaussianChiEffChiP@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@VI@out{\{"median": 0.19, "5th percentile": 0.12, "95th percentile": 0.33, "error plus": 0.15, "error minus": 0.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@VI@out{0.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@VI@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@VI@out{0.33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\gaussianChiEffChiP@VI@out{0.15}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\gaussianChiEffChiP@VI@out{0.07}\else\def\gaussianChiEffChiP@VI@out{??}\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@VI@out}\newcommand\gaussianChiEffChiP@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@VII@out{\{"median": 0.06, "5th percentile": {-}0.47, "95th percentile": 0.55, "error plus": 0.49, "error minus": 0.53\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@VII@out{0.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@VII@out{{-}0.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@VII@out{0.55}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\gaussianChiEffChiP@VII@out{0.49}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\gaussianChiEffChiP@VII@out{0.53}\else\def\gaussianChiEffChiP@VII@out{??}\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@VII@out}\newcommand\gaussianChiEffChiP@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@VIII@out{\{"median": {-}0.2, "5th percentile": {-}0.27, "95th percentile": {-}0.13, "error plus": 0.06, "error minus": 0.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@VIII@out{{-}0.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@VIII@out{{-}0.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@VIII@out{{-}0.13}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\gaussianChiEffChiP@VIII@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\gaussianChiEffChiP@VIII@out{0.07}\else\def\gaussianChiEffChiP@VIII@out{??}\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@VIII@out}\newcommand\gaussianChiEffChiP@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@IX@out{\{"median": 0.34, "5th percentile": 0.24, "95th percentile": 0.43, "error plus": 0.09, "error minus": 0.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@IX@out{0.24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@IX@out{0.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\gaussianChiEffChiP@IX@out{0.09}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\gaussianChiEffChiP@IX@out{0.1}\else\def\gaussianChiEffChiP@IX@out{??}\fi\fi\fi\fi\fi\fi\gaussianChiEffChiP@IX@out}\newcommand\gaussianChiEffChiP@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@X@out{\{"median": 0.04, "5th percentile": {-}0.13, "95th percentile": 0.22, "spin at peak": 0.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@X@out{0.04}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@X@out{{-}0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@X@out{0.22}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\gaussianChiEffChiP@X@out{0.04}\else\def\gaussianChiEffChiP@X@out{??}\fi\fi\fi\fi\fi\gaussianChiEffChiP@X@out}\newcommand\gaussianChiEffChiP@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\gaussianChiEffChiP@XI@out{\{"median": 0.33, "5th percentile": 0.07, "95th percentile": 0.66, "spin at peak": 0.31\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\gaussianChiEffChiP@XI@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\gaussianChiEffChiP@XI@out{0.07}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\gaussianChiEffChiP@XI@out{0.66}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\gaussianChiEffChiP@XI@out{0.31}\else\def\gaussianChiEffChiP@XI@out{??}\fi\fi\fi\fi\fi\gaussianChiEffChiP@XI@out}\makeatother
\makeatletter\newcommand\IsoPeakIID[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@out{\{"mass\_1": \{"peak": \{"peak\_mu": \{"median": "10", "error plus": "0.81", "error minus": "0.68", "5th percentile": "9.6", "95th percentile": "11"\}, "peak\_logsigp": \{"median": "0.10", "error plus": "0.051", "error minus": "0.032", "5th percentile": "0.069", "95th percentile": "0.15"\}\}\}, "mass\_ratio": \{"peak": \{"peak\_location": \{"median": "0.74", "error plus": "0.13", "error minus": "0.13", "5th percentile": "0.61", "95th percentile": "0.87"\}\}, "continuum": \{"peak\_location": \{"median": "0.73", "error plus": "0.16", "error minus": "0.21", "5th percentile": "0.52", "95th percentile": "0.89"\}\}\}, "a": \{"peak": \{"peak\_location": \{"median": "0.12", "error plus": "0.18", "error minus": "0.12", "5th percentile": 0, "95th percentile": "0.30"\}\}, "continuum": \{"peak\_location": \{"median": "0.10", "error plus": "0.28", "error minus": "0.10", "5th percentile": 0, "95th percentile": "0.38"\}\}\}, "cos\_tilt": \{"peak": \{"peak\_location": \{"median": "0.32", "error plus": "0.68", "error minus": "0.52", "5th percentile": "{-}0.19", "95th percentile": "1.0"\}\}, "continuum": \{"peak\_location": \{"median": "0.034", "error plus": "0.97", "error minus": "0.48", "5th percentile": "{-}0.44", "95th percentile": "1.0"\}\}\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\IsoPeakIID@out\IsoPeakIID@I\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\IsoPeakIID@out\IsoPeakIID@II\else\ifnum\pdfstrcmp{#1}{a}=0\let\IsoPeakIID@out\IsoPeakIID@III\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\IsoPeakIID@out\IsoPeakIID@IV\else\def\IsoPeakIID@out{??}\fi\fi\fi\fi\fi\IsoPeakIID@out}\newcommand\IsoPeakIID@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@I@out{\{"peak": \{"peak\_mu": \{"median": "10", "error plus": "0.81", "error minus": "0.68", "5th percentile": "9.6", "95th percentile": "11"\}, "peak\_logsigp": \{"median": "0.10", "error plus": "0.051", "error minus": "0.032", "5th percentile": "0.069", "95th percentile": "0.15"\}\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\IsoPeakIID@I@out\IsoPeakIID@V\else\def\IsoPeakIID@I@out{??}\fi\fi\IsoPeakIID@I@out}\newcommand\IsoPeakIID@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@II@out{\{"peak": \{"peak\_location": \{"median": "0.74", "error plus": "0.13", "error minus": "0.13", "5th percentile": "0.61", "95th percentile": "0.87"\}\}, "continuum": \{"peak\_location": \{"median": "0.73", "error plus": "0.16", "error minus": "0.21", "5th percentile": "0.52", "95th percentile": "0.89"\}\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\IsoPeakIID@II@out\IsoPeakIID@VI\else\ifnum\pdfstrcmp{#1}{continuum}=0\let\IsoPeakIID@II@out\IsoPeakIID@VII\else\def\IsoPeakIID@II@out{??}\fi\fi\fi\IsoPeakIID@II@out}\newcommand\IsoPeakIID@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@III@out{\{"peak": \{"peak\_location": \{"median": "0.12", "error plus": "0.18", "error minus": "0.12", "5th percentile": 0, "95th percentile": "0.30"\}\}, "continuum": \{"peak\_location": \{"median": "0.10", "error plus": "0.28", "error minus": "0.10", "5th percentile": 0, "95th percentile": "0.38"\}\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\IsoPeakIID@III@out\IsoPeakIID@VIII\else\ifnum\pdfstrcmp{#1}{continuum}=0\let\IsoPeakIID@III@out\IsoPeakIID@IX\else\def\IsoPeakIID@III@out{??}\fi\fi\fi\IsoPeakIID@III@out}\newcommand\IsoPeakIID@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@IV@out{\{"peak": \{"peak\_location": \{"median": "0.32", "error plus": "0.68", "error minus": "0.52", "5th percentile": "{-}0.19", "95th percentile": "1.0"\}\}, "continuum": \{"peak\_location": \{"median": "0.034", "error plus": "0.97", "error minus": "0.48", "5th percentile": "{-}0.44", "95th percentile": "1.0"\}\}\}}\else\ifnum\pdfstrcmp{#1}{peak}=0\let\IsoPeakIID@IV@out\IsoPeakIID@X\else\ifnum\pdfstrcmp{#1}{continuum}=0\let\IsoPeakIID@IV@out\IsoPeakIID@XI\else\def\IsoPeakIID@IV@out{??}\fi\fi\fi\IsoPeakIID@IV@out}\newcommand\IsoPeakIID@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@V@out{\{"peak\_mu": \{"median": "10", "error plus": "0.81", "error minus": "0.68", "5th percentile": "9.6", "95th percentile": "11"\}, "peak\_logsigp": \{"median": "0.10", "error plus": "0.051", "error minus": "0.032", "5th percentile": "0.069", "95th percentile": "0.15"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_mu}=0\let\IsoPeakIID@V@out\IsoPeakIID@XII\else\ifnum\pdfstrcmp{#1}{peak_logsigp}=0\let\IsoPeakIID@V@out\IsoPeakIID@XIII\else\def\IsoPeakIID@V@out{??}\fi\fi\fi\IsoPeakIID@V@out}\newcommand\IsoPeakIID@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@VI@out{\{"peak\_location": \{"median": "0.74", "error plus": "0.13", "error minus": "0.13", "5th percentile": "0.61", "95th percentile": "0.87"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_location}=0\let\IsoPeakIID@VI@out\IsoPeakIID@XIV\else\def\IsoPeakIID@VI@out{??}\fi\fi\IsoPeakIID@VI@out}\newcommand\IsoPeakIID@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@VII@out{\{"peak\_location": \{"median": "0.73", "error plus": "0.16", "error minus": "0.21", "5th percentile": "0.52", "95th percentile": "0.89"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_location}=0\let\IsoPeakIID@VII@out\IsoPeakIID@XV\else\def\IsoPeakIID@VII@out{??}\fi\fi\IsoPeakIID@VII@out}\newcommand\IsoPeakIID@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@VIII@out{\{"peak\_location": \{"median": "0.12", "error plus": "0.18", "error minus": "0.12", "5th percentile": 0, "95th percentile": "0.30"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_location}=0\let\IsoPeakIID@VIII@out\IsoPeakIID@XVI\else\def\IsoPeakIID@VIII@out{??}\fi\fi\IsoPeakIID@VIII@out}\newcommand\IsoPeakIID@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@IX@out{\{"peak\_location": \{"median": "0.10", "error plus": "0.28", "error minus": "0.10", "5th percentile": 0, "95th percentile": "0.38"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_location}=0\let\IsoPeakIID@IX@out\IsoPeakIID@XVII\else\def\IsoPeakIID@IX@out{??}\fi\fi\IsoPeakIID@IX@out}\newcommand\IsoPeakIID@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@X@out{\{"peak\_location": \{"median": "0.32", "error plus": "0.68", "error minus": "0.52", "5th percentile": "{-}0.19", "95th percentile": "1.0"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_location}=0\let\IsoPeakIID@X@out\IsoPeakIID@XVIII\else\def\IsoPeakIID@X@out{??}\fi\fi\IsoPeakIID@X@out}\newcommand\IsoPeakIID@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XI@out{\{"peak\_location": \{"median": "0.034", "error plus": "0.97", "error minus": "0.48", "5th percentile": "{-}0.44", "95th percentile": "1.0"\}\}}\else\ifnum\pdfstrcmp{#1}{peak_location}=0\let\IsoPeakIID@XI@out\IsoPeakIID@XIX\else\def\IsoPeakIID@XI@out{??}\fi\fi\IsoPeakIID@XI@out}\newcommand\IsoPeakIID@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XII@out{\{"median": "10", "error plus": "0.81", "error minus": "0.68", "5th percentile": "9.6", "95th percentile": "11"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XII@out{10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XII@out{0.81}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XII@out{0.68}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XII@out{9.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XII@out{11}\else\def\IsoPeakIID@XII@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XII@out}\newcommand\IsoPeakIID@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XIII@out{\{"median": "0.10", "error plus": "0.051", "error minus": "0.032", "5th percentile": "0.069", "95th percentile": "0.15"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XIII@out{0.10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XIII@out{0.051}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XIII@out{0.032}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XIII@out{0.069}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XIII@out{0.15}\else\def\IsoPeakIID@XIII@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XIII@out}\newcommand\IsoPeakIID@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XIV@out{\{"median": "0.74", "error plus": "0.13", "error minus": "0.13", "5th percentile": "0.61", "95th percentile": "0.87"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XIV@out{0.74}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XIV@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XIV@out{0.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XIV@out{0.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XIV@out{0.87}\else\def\IsoPeakIID@XIV@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XIV@out}\newcommand\IsoPeakIID@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XV@out{\{"median": "0.73", "error plus": "0.16", "error minus": "0.21", "5th percentile": "0.52", "95th percentile": "0.89"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XV@out{0.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XV@out{0.16}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XV@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XV@out{0.52}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XV@out{0.89}\else\def\IsoPeakIID@XV@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XV@out}\newcommand\IsoPeakIID@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XVI@out{\{"median": "0.12", "error plus": "0.18", "error minus": "0.12", "5th percentile": 0, "95th percentile": "0.30"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XVI@out{0.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XVI@out{0.18}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XVI@out{0.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XVI@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XVI@out{0.30}\else\def\IsoPeakIID@XVI@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XVI@out}\newcommand\IsoPeakIID@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XVII@out{\{"median": "0.10", "error plus": "0.28", "error minus": "0.10", "5th percentile": 0, "95th percentile": "0.38"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XVII@out{0.10}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XVII@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XVII@out{0.10}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XVII@out{0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XVII@out{0.38}\else\def\IsoPeakIID@XVII@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XVII@out}\newcommand\IsoPeakIID@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XVIII@out{\{"median": "0.32", "error plus": "0.68", "error minus": "0.52", "5th percentile": "{-}0.19", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XVIII@out{0.32}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XVIII@out{0.68}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XVIII@out{0.52}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XVIII@out{{-}0.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XVIII@out{1.0}\else\def\IsoPeakIID@XVIII@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XVIII@out}\newcommand\IsoPeakIID@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\IsoPeakIID@XIX@out{\{"median": "0.034", "error plus": "0.97", "error minus": "0.48", "5th percentile": "{-}0.44", "95th percentile": "1.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\IsoPeakIID@XIX@out{0.034}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\IsoPeakIID@XIX@out{0.97}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\IsoPeakIID@XIX@out{0.48}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\IsoPeakIID@XIX@out{{-}0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\IsoPeakIID@XIX@out{1.0}\else\def\IsoPeakIID@XIX@out{??}\fi\fi\fi\fi\fi\fi\IsoPeakIID@XIX@out}\makeatother
\makeatletter\newcommand\LogNormBBH[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@out{\{"s\_continuum": \{"median": "0.83", "error plus": "0.4", "error minus": "0.15", "5th percentile": "0.68", "95th percentile": "1.23"\}, "beta": \{"median": "1.18", "error plus": "1.28", "error minus": "1.02", "5th percentile": "0.16", "95th percentile": "2.46"\}, "mlow\_1": \{"median": "5.81", "error plus": "3.02", "error minus": "2.37", "5th percentile": "3.43", "95th percentile": "8.83"\}, "mlow\_2": \{"median": "3.75", "error plus": "1.44", "error minus": "0.7", "5th percentile": "3.05", "95th percentile": "5.19"\}, "peak\_from\_lo\_1": \{"median": "3.65", "error plus": "2.58", "error minus": "3.34", "5th percentile": "0.31", "95th percentile": "6.23"\}, "mpp\_2": \{"median": "33.95", "error plus": "2.06", "error minus": "6.07", "5th percentile": "27.89", "95th percentile": "36.02"\}, "sigpp\_1": \{"median": "1.14", "error plus": "0.55", "error minus": "0.13", "5th percentile": "1.01", "95th percentile": "1.69"\}, "sigpp\_2": \{"median": "3.31", "error plus": "7.21", "error minus": "1.92", "5th percentile": "1.39", "95th percentile": "10.51"\}, "m\_peak\_from\_lo\_continuum": \{"median": "6.01", "error plus": "3.49", "error minus": "4.94", "5th percentile": "1.07", "95th percentile": "9.5"\}, "delta\_m\_2": \{"median": "4.88", "error plus": "3.28", "error minus": "4.35", "5th percentile": "0.54", "95th percentile": "8.16"\}, "lam\_0": \{"median": "0.2", "error plus": "0.18", "error minus": "0.11", "5th percentile": "0.09", "95th percentile": "0.39"\}, "lam\_1": \{"median": "0.73", "error plus": "0.11", "error minus": "0.19", "5th percentile": "0.54", "95th percentile": "0.84"\}, "mu\_chi": \{"median": "0.09", "error plus": "0.14", "error minus": "0.08", "5th percentile": "0.01", "95th percentile": "0.23"\}, "sigma\_chi": \{"median": "0.29", "error plus": "0.07", "error minus": "0.07", "5th percentile": "0.22", "95th percentile": "0.36"\}, "xi\_spin": \{"median": "0.68", "error plus": "0.29", "error minus": "0.54", "5th percentile": "0.15", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.38", "error plus": "0.55", "error minus": "0.7", "5th percentile": "{-}0.32", "95th percentile": "0.93"\}, "sigma\_spin": \{"median": "1.11", "error plus": "2.36", "error minus": "0.72", "5th percentile": "0.39", "95th percentile": "3.47"\}, "lamb": \{"median": "1.73", "error plus": "1.05", "error minus": "1.02", "5th percentile": "0.71", "95th percentile": "2.78"\}, "rate": \{"median": "28.47", "error plus": "17.88", "error minus": "10.23", "5th percentile": "18.23", "95th percentile": "46.35"\}\}}\else\ifnum\pdfstrcmp{#1}{s_continuum}=0\let\LogNormBBH@out\LogNormBBH@I\else\ifnum\pdfstrcmp{#1}{beta}=0\let\LogNormBBH@out\LogNormBBH@II\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\LogNormBBH@out\LogNormBBH@III\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\LogNormBBH@out\LogNormBBH@IV\else\ifnum\pdfstrcmp{#1}{peak_from_lo_1}=0\let\LogNormBBH@out\LogNormBBH@V\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\LogNormBBH@out\LogNormBBH@VI\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\LogNormBBH@out\LogNormBBH@VII\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\LogNormBBH@out\LogNormBBH@VIII\else\ifnum\pdfstrcmp{#1}{m_peak_from_lo_continuum}=0\let\LogNormBBH@out\LogNormBBH@IX\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\LogNormBBH@out\LogNormBBH@X\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\LogNormBBH@out\LogNormBBH@XI\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\LogNormBBH@out\LogNormBBH@XII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\LogNormBBH@out\LogNormBBH@XIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\LogNormBBH@out\LogNormBBH@XIV\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\LogNormBBH@out\LogNormBBH@XV\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\LogNormBBH@out\LogNormBBH@XVI\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\LogNormBBH@out\LogNormBBH@XVII\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\LogNormBBH@out\LogNormBBH@XVIII\else\ifnum\pdfstrcmp{#1}{rate}=0\let\LogNormBBH@out\LogNormBBH@XIX\else\def\LogNormBBH@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\LogNormBBH@out}\newcommand\LogNormBBH@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@I@out{\{"median": "0.83", "error plus": "0.4", "error minus": "0.15", "5th percentile": "0.68", "95th percentile": "1.23"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@I@out{0.83}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@I@out{0.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@I@out{0.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@I@out{0.68}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@I@out{1.23}\else\def\LogNormBBH@I@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@I@out}\newcommand\LogNormBBH@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@II@out{\{"median": "1.18", "error plus": "1.28", "error minus": "1.02", "5th percentile": "0.16", "95th percentile": "2.46"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@II@out{1.18}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@II@out{1.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@II@out{1.02}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@II@out{0.16}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@II@out{2.46}\else\def\LogNormBBH@II@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@II@out}\newcommand\LogNormBBH@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@III@out{\{"median": "5.81", "error plus": "3.02", "error minus": "2.37", "5th percentile": "3.43", "95th percentile": "8.83"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@III@out{5.81}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@III@out{3.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@III@out{2.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@III@out{3.43}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@III@out{8.83}\else\def\LogNormBBH@III@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@III@out}\newcommand\LogNormBBH@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@IV@out{\{"median": "3.75", "error plus": "1.44", "error minus": "0.7", "5th percentile": "3.05", "95th percentile": "5.19"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@IV@out{3.75}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@IV@out{1.44}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@IV@out{0.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@IV@out{3.05}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@IV@out{5.19}\else\def\LogNormBBH@IV@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@IV@out}\newcommand\LogNormBBH@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@V@out{\{"median": "3.65", "error plus": "2.58", "error minus": "3.34", "5th percentile": "0.31", "95th percentile": "6.23"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@V@out{3.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@V@out{2.58}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@V@out{3.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@V@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@V@out{6.23}\else\def\LogNormBBH@V@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@V@out}\newcommand\LogNormBBH@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@VI@out{\{"median": "33.95", "error plus": "2.06", "error minus": "6.07", "5th percentile": "27.89", "95th percentile": "36.02"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@VI@out{33.95}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@VI@out{2.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@VI@out{6.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@VI@out{27.89}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@VI@out{36.02}\else\def\LogNormBBH@VI@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@VI@out}\newcommand\LogNormBBH@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@VII@out{\{"median": "1.14", "error plus": "0.55", "error minus": "0.13", "5th percentile": "1.01", "95th percentile": "1.69"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@VII@out{1.14}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@VII@out{0.55}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@VII@out{0.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@VII@out{1.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@VII@out{1.69}\else\def\LogNormBBH@VII@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@VII@out}\newcommand\LogNormBBH@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@VIII@out{\{"median": "3.31", "error plus": "7.21", "error minus": "1.92", "5th percentile": "1.39", "95th percentile": "10.51"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@VIII@out{3.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@VIII@out{7.21}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@VIII@out{1.92}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@VIII@out{1.39}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@VIII@out{10.51}\else\def\LogNormBBH@VIII@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@VIII@out}\newcommand\LogNormBBH@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@IX@out{\{"median": "6.01", "error plus": "3.49", "error minus": "4.94", "5th percentile": "1.07", "95th percentile": "9.5"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@IX@out{6.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@IX@out{3.49}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@IX@out{4.94}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@IX@out{1.07}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@IX@out{9.5}\else\def\LogNormBBH@IX@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@IX@out}\newcommand\LogNormBBH@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@X@out{\{"median": "4.88", "error plus": "3.28", "error minus": "4.35", "5th percentile": "0.54", "95th percentile": "8.16"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@X@out{4.88}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@X@out{3.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@X@out{4.35}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@X@out{0.54}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@X@out{8.16}\else\def\LogNormBBH@X@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@X@out}\newcommand\LogNormBBH@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XI@out{\{"median": "0.2", "error plus": "0.18", "error minus": "0.11", "5th percentile": "0.09", "95th percentile": "0.39"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XI@out{0.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XI@out{0.18}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XI@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XI@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XI@out{0.39}\else\def\LogNormBBH@XI@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XI@out}\newcommand\LogNormBBH@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XII@out{\{"median": "0.73", "error plus": "0.11", "error minus": "0.19", "5th percentile": "0.54", "95th percentile": "0.84"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XII@out{0.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XII@out{0.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XII@out{0.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XII@out{0.54}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XII@out{0.84}\else\def\LogNormBBH@XII@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XII@out}\newcommand\LogNormBBH@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XIII@out{\{"median": "0.09", "error plus": "0.14", "error minus": "0.08", "5th percentile": "0.01", "95th percentile": "0.23"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XIII@out{0.09}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XIII@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XIII@out{0.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XIII@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XIII@out{0.23}\else\def\LogNormBBH@XIII@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XIII@out}\newcommand\LogNormBBH@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XIV@out{\{"median": "0.29", "error plus": "0.07", "error minus": "0.07", "5th percentile": "0.22", "95th percentile": "0.36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XIV@out{0.29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XIV@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XIV@out{0.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XIV@out{0.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XIV@out{0.36}\else\def\LogNormBBH@XIV@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XIV@out}\newcommand\LogNormBBH@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XV@out{\{"median": "0.68", "error plus": "0.29", "error minus": "0.54", "5th percentile": "0.15", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XV@out{0.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XV@out{0.29}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XV@out{0.54}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XV@out{0.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XV@out{0.97}\else\def\LogNormBBH@XV@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XV@out}\newcommand\LogNormBBH@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XVI@out{\{"median": "0.38", "error plus": "0.55", "error minus": "0.7", "5th percentile": "{-}0.32", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XVI@out{0.38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XVI@out{0.55}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XVI@out{0.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XVI@out{{-}0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XVI@out{0.93}\else\def\LogNormBBH@XVI@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XVI@out}\newcommand\LogNormBBH@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XVII@out{\{"median": "1.11", "error plus": "2.36", "error minus": "0.72", "5th percentile": "0.39", "95th percentile": "3.47"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XVII@out{1.11}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XVII@out{2.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XVII@out{0.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XVII@out{0.39}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XVII@out{3.47}\else\def\LogNormBBH@XVII@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XVII@out}\newcommand\LogNormBBH@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XVIII@out{\{"median": "1.73", "error plus": "1.05", "error minus": "1.02", "5th percentile": "0.71", "95th percentile": "2.78"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XVIII@out{1.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XVIII@out{1.05}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XVIII@out{1.02}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XVIII@out{0.71}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XVIII@out{2.78}\else\def\LogNormBBH@XVIII@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XVIII@out}\newcommand\LogNormBBH@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\LogNormBBH@XIX@out{\{"median": "28.47", "error plus": "17.88", "error minus": "10.23", "5th percentile": "18.23", "95th percentile": "46.35"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\LogNormBBH@XIX@out{28.47}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\LogNormBBH@XIX@out{17.88}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\LogNormBBH@XIX@out{10.23}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\LogNormBBH@XIX@out{18.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\LogNormBBH@XIX@out{46.35}\else\def\LogNormBBH@XIX@out{??}\fi\fi\fi\fi\fi\fi\LogNormBBH@XIX@out}\makeatother
\makeatletter\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@out{\{"ln\_evidence": {-}1048.66, "ln\_evidence\_error": 0.25, "ln\_bayes\_factor\_over\_new\_default": {-}1.52, "ln\_bayes\_factor\_over\_old\_default": 0.0, "param": \{"alpha\_1": \{"median": 1.77, "5th percentile": {-}0.07, "95th percentile": 3.01, "error plus": 1.24, "error minus": 1.84\}, "alpha\_2": \{"median": 4.41, "5th percentile": 3.13, "95th percentile": 6.02, "error plus": 1.61, "error minus": 1.28\}, "beta": \{"median": 1.23, "5th percentile": 0.19, "95th percentile": 2.58, "error plus": 1.36, "error minus": 1.04\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.23, "95th percentile": 8.23, "error plus": 3.08, "error minus": 1.92\}, "mlow\_2": \{"median": 3.56, "5th percentile": 3.03, "95th percentile": 4.88, "error plus": 1.32, "error minus": 0.53\}, "break\_mass": \{"median": 35.56, "5th percentile": 22.14, "95th percentile": 48.07, "error plus": 12.51, "error minus": 13.42\}, "mpp\_1": \{"median": 9.72, "5th percentile": 8.27, "95th percentile": 10.22, "error plus": 0.5, "error minus": 1.45\}, "mpp\_2": \{"median": 33.12, "5th percentile": 27.2, "95th percentile": 35.76, "error plus": 2.63, "error minus": 5.92\}, "sigpp\_1": \{"median": 0.66, "5th percentile": 0.32, "95th percentile": 1.59, "error plus": 0.93, "error minus": 0.34\}, "sigpp\_2": \{"median": 3.62, "5th percentile": 1.26, "95th percentile": 8.85, "error plus": 5.22, "error minus": 2.36\}, "delta\_m\_1": \{"median": 4.17, "5th percentile": 0.31, "95th percentile": 9.27, "error plus": 5.11, "error minus": 3.86\}, "delta\_m\_2": \{"median": 5.11, "5th percentile": 0.52, "95th percentile": 9.05, "error plus": 3.94, "error minus": 4.59\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.66, "error plus": 0.3, "error minus": 0.21\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.3, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.3\}, "lamb": \{"median": 3.11, "5th percentile": 2.13, "95th percentile": 4.03, "error plus": 0.93, "error minus": 0.98\}, "mu\_chi": \{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.34, "error plus": 0.04, "error minus": 0.03\}, "sigma\_chi": \{"median": 0.2, "5th percentile": 0.18, "95th percentile": 0.22, "error plus": 0.02, "error minus": 0.02\}, "xi\_spin": \{"median": 0.64, "5th percentile": 0.13, "95th percentile": 0.97, "error plus": 0.33, "error minus": 0.51\}, "sigma\_spin": \{"median": 1.72, "5th percentile": 0.92, "95th percentile": 3.53, "error plus": 1.81, "error minus": 0.79\}, "rate": \{"median": 16.45, "5th percentile": 11.96, "95th percentile": 22.27, "error plus": 5.82, "error minus": 4.5\}, "log\_likelihood": \{"median": {-}1024.24, "5th percentile": {-}1030.09, "95th percentile": {-}1019.81, "error plus": 4.43, "error minus": 5.85\}, "variance": \{"median": 0.89, "5th percentile": 0.67, "95th percentile": 0.99, "error plus": 0.1, "error minus": 0.22\}, "min\_neff": \{"median": 54.92, "5th percentile": 31.25, "95th percentile": 90.6, "error plus": 35.68, "error minus": 23.67\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a": \{"median": 0.26, "5th percentile": 0.03, "90th percentile": 0.59, "95th percentile": 0.69, "peak": 0.11\}, "cos\_tilt": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.83, "95th percentile": 0.91, "peak": 1.0\}, "mass\_1": \{"median": 10.1, "5th percentile": 7.96, "90th percentile": 27.92, "95th percentile": 34.48, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.46, "95th percentile": 0.47, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@out{{-}1048.66}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@out{0.25}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@out{{-}1.52}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@out{0.0}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@II\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@out{??}\fi\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out{\{"alpha\_1": \{"median": 1.77, "5th percentile": {-}0.07, "95th percentile": 3.01, "error plus": 1.24, "error minus": 1.84\}, "alpha\_2": \{"median": 4.41, "5th percentile": 3.13, "95th percentile": 6.02, "error plus": 1.61, "error minus": 1.28\}, "beta": \{"median": 1.23, "5th percentile": 0.19, "95th percentile": 2.58, "error plus": 1.36, "error minus": 1.04\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.23, "95th percentile": 8.23, "error plus": 3.08, "error minus": 1.92\}, "mlow\_2": \{"median": 3.56, "5th percentile": 3.03, "95th percentile": 4.88, "error plus": 1.32, "error minus": 0.53\}, "break\_mass": \{"median": 35.56, "5th percentile": 22.14, "95th percentile": 48.07, "error plus": 12.51, "error minus": 13.42\}, "mpp\_1": \{"median": 9.72, "5th percentile": 8.27, "95th percentile": 10.22, "error plus": 0.5, "error minus": 1.45\}, "mpp\_2": \{"median": 33.12, "5th percentile": 27.2, "95th percentile": 35.76, "error plus": 2.63, "error minus": 5.92\}, "sigpp\_1": \{"median": 0.66, "5th percentile": 0.32, "95th percentile": 1.59, "error plus": 0.93, "error minus": 0.34\}, "sigpp\_2": \{"median": 3.62, "5th percentile": 1.26, "95th percentile": 8.85, "error plus": 5.22, "error minus": 2.36\}, "delta\_m\_1": \{"median": 4.17, "5th percentile": 0.31, "95th percentile": 9.27, "error plus": 5.11, "error minus": 3.86\}, "delta\_m\_2": \{"median": 5.11, "5th percentile": 0.52, "95th percentile": 9.05, "error plus": 3.94, "error minus": 4.59\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.66, "error plus": 0.3, "error minus": 0.21\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.3, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.3\}, "lamb": \{"median": 3.11, "5th percentile": 2.13, "95th percentile": 4.03, "error plus": 0.93, "error minus": 0.98\}, "mu\_chi": \{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.34, "error plus": 0.04, "error minus": 0.03\}, "sigma\_chi": \{"median": 0.2, "5th percentile": 0.18, "95th percentile": 0.22, "error plus": 0.02, "error minus": 0.02\}, "xi\_spin": \{"median": 0.64, "5th percentile": 0.13, "95th percentile": 0.97, "error plus": 0.33, "error minus": 0.51\}, "sigma\_spin": \{"median": 1.72, "5th percentile": 0.92, "95th percentile": 3.53, "error plus": 1.81, "error minus": 0.79\}, "rate": \{"median": 16.45, "5th percentile": 11.96, "95th percentile": 22.27, "error plus": 5.82, "error minus": 4.5\}, "log\_likelihood": \{"median": {-}1024.24, "5th percentile": {-}1030.09, "95th percentile": {-}1019.81, "error plus": 4.43, "error minus": 5.85\}, "variance": \{"median": 0.89, "5th percentile": 0.67, "95th percentile": 0.99, "error plus": 0.1, "error minus": 0.22\}, "min\_neff": \{"median": 54.92, "5th percentile": 31.25, "95th percentile": 90.6, "error plus": 35.68, "error minus": 23.67\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@I@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out{\{"a": \{"median": 0.26, "5th percentile": 0.03, "90th percentile": 0.59, "95th percentile": 0.69, "peak": 0.11\}, "cos\_tilt": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.83, "95th percentile": 0.91, "peak": 1.0\}, "mass\_1": \{"median": 10.1, "5th percentile": 7.96, "90th percentile": 27.92, "95th percentile": 34.48, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.46, "95th percentile": 0.47, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@II@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out{\{"median": 1.77, "5th percentile": {-}0.07, "95th percentile": 3.01, "error plus": 1.24, "error minus": 1.84\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out{1.77}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out{{-}0.07}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out{3.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out{1.24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out{1.84}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@III@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out{\{"median": 4.41, "5th percentile": 3.13, "95th percentile": 6.02, "error plus": 1.61, "error minus": 1.28\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out{4.41}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out{3.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out{6.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out{1.61}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out{1.28}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@IV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out{\{"median": 1.23, "5th percentile": 0.19, "95th percentile": 2.58, "error plus": 1.36, "error minus": 1.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out{1.23}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out{0.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out{2.58}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out{1.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out{1.04}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@V@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out{\{"median": 5.15, "5th percentile": 3.23, "95th percentile": 8.23, "error plus": 3.08, "error minus": 1.92\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out{5.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out{3.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out{8.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out{3.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out{1.92}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@VI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out{\{"median": 3.56, "5th percentile": 3.03, "95th percentile": 4.88, "error plus": 1.32, "error minus": 0.53\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out{3.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out{4.88}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out{1.32}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out{0.53}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@VII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out{\{"median": 35.56, "5th percentile": 22.14, "95th percentile": 48.07, "error plus": 12.51, "error minus": 13.42\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out{35.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out{22.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out{48.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out{12.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out{13.42}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@VIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out{\{"median": 9.72, "5th percentile": 8.27, "95th percentile": 10.22, "error plus": 0.5, "error minus": 1.45\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out{9.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out{8.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out{10.22}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out{0.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out{1.45}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@IX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out{\{"median": 33.12, "5th percentile": 27.2, "95th percentile": 35.76, "error plus": 2.63, "error minus": 5.92\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out{33.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out{27.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out{35.76}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out{2.63}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out{5.92}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@X@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out{\{"median": 0.66, "5th percentile": 0.32, "95th percentile": 1.59, "error plus": 0.93, "error minus": 0.34\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out{0.66}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out{1.59}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out{0.93}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out{0.34}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out{\{"median": 3.62, "5th percentile": 1.26, "95th percentile": 8.85, "error plus": 5.22, "error minus": 2.36\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out{3.62}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out{1.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out{8.85}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out{5.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out{2.36}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out{\{"median": 4.17, "5th percentile": 0.31, "95th percentile": 9.27, "error plus": 5.11, "error minus": 3.86\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out{4.17}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out{9.27}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out{5.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out{3.86}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out{\{"median": 5.11, "5th percentile": 0.52, "95th percentile": 9.05, "error plus": 3.94, "error minus": 4.59\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out{5.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out{0.52}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out{9.05}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out{3.94}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out{4.59}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out{\{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.66, "error plus": 0.3, "error minus": 0.21\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out{0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out{0.66}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out{0.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out{0.21}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out{\{"median": 0.59, "5th percentile": 0.3, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out{0.59}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out{0.81}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out{0.3}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out{\{"median": 3.11, "5th percentile": 2.13, "95th percentile": 4.03, "error plus": 0.93, "error minus": 0.98\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out{3.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out{2.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out{4.03}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out{0.93}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out{0.98}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out{\{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.34, "error plus": 0.04, "error minus": 0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out{0.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out{0.34}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out{0.04}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out{0.03}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XVIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out{\{"median": 0.2, "5th percentile": 0.18, "95th percentile": 0.22, "error plus": 0.02, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out{0.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out{0.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out{0.22}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out{0.02}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XIX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out{\{"median": 0.64, "5th percentile": 0.13, "95th percentile": 0.97, "error plus": 0.33, "error minus": 0.51\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out{0.64}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out{0.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out{0.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out{0.51}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out{\{"median": 1.72, "5th percentile": 0.92, "95th percentile": 3.53, "error plus": 1.81, "error minus": 0.79\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out{1.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out{0.92}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out{3.53}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out{1.81}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out{0.79}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out{\{"median": 16.45, "5th percentile": 11.96, "95th percentile": 22.27, "error plus": 5.82, "error minus": 4.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out{16.45}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out{11.96}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out{22.27}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out{5.82}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out{4.5}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out{\{"median": {-}1024.24, "5th percentile": {-}1030.09, "95th percentile": {-}1019.81, "error plus": 4.43, "error minus": 5.85\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out{{-}1024.24}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out{{-}1030.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out{{-}1019.81}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out{4.43}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out{5.85}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out{\{"median": 0.89, "5th percentile": 0.67, "95th percentile": 0.99, "error plus": 0.1, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out{0.89}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out{0.67}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out{0.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out{0.22}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out{\{"median": 54.92, "5th percentile": 31.25, "95th percentile": 90.6, "error plus": 35.68, "error minus": 23.67\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out{54.92}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out{31.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out{90.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out{35.68}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out{23.67}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out{0.0}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out{\{"median": 0.26, "5th percentile": 0.03, "90th percentile": 0.59, "95th percentile": 0.69, "peak": 0.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out{0.26}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out{0.59}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out{0.69}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out{0.11}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out{\{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.83, "95th percentile": 0.91, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out{{-}0.87}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out{0.83}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out{0.91}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out{1.0}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXVIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out{\{"median": 10.1, "5th percentile": 7.96, "90th percentile": 27.92, "95th percentile": 34.48, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out{10.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out{7.96}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out{27.92}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out{34.48}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out{9.91}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXIX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out{\{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out{0.5}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out{1.0}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.46, "95th percentile": 0.47, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out{0.46}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out{0.47}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out{2.0}\else\def\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicAlignedNid@XXXI@out}\makeatother
\makeatletter\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out{\{"ln\_evidence": {-}1048.61, "ln\_evidence\_error": 0.24, "ln\_bayes\_factor\_over\_new\_default": {-}1.47, "ln\_bayes\_factor\_over\_old\_default": 0.05, "param": \{"alpha\_1": \{"median": 1.76, "5th percentile": {-}0.11, "95th percentile": 2.98, "error plus": 1.22, "error minus": 1.87\}, "alpha\_2": \{"median": 4.39, "5th percentile": 3.13, "95th percentile": 6.04, "error plus": 1.64, "error minus": 1.26\}, "beta": \{"median": 1.23, "5th percentile": 0.19, "95th percentile": 2.59, "error plus": 1.36, "error minus": 1.04\}, "mlow\_1": \{"median": 4.99, "5th percentile": 3.22, "95th percentile": 8.01, "error plus": 3.02, "error minus": 1.77\}, "mlow\_2": \{"median": 3.52, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.35, "error minus": 0.49\}, "break\_mass": \{"median": 35.12, "5th percentile": 22.02, "95th percentile": 47.91, "error plus": 12.79, "error minus": 13.09\}, "mpp\_1": \{"median": 9.71, "5th percentile": 8.45, "95th percentile": 10.23, "error plus": 0.52, "error minus": 1.25\}, "mpp\_2": \{"median": 32.95, "5th percentile": 26.74, "95th percentile": 35.92, "error plus": 2.97, "error minus": 6.21\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.32, "95th percentile": 1.61, "error plus": 0.94, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.94, "5th percentile": 1.33, "95th percentile": 9.2, "error plus": 5.26, "error minus": 2.61\}, "delta\_m\_1": \{"median": 4.56, "5th percentile": 0.39, "95th percentile": 9.32, "error plus": 4.75, "error minus": 4.17\}, "delta\_m\_2": \{"median": 5.18, "5th percentile": 0.56, "95th percentile": 9.16, "error plus": 3.98, "error minus": 4.62\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.64, "error plus": 0.28, "error minus": 0.22\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.31, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.28\}, "lamb": \{"median": 3.11, "5th percentile": 2.09, "95th percentile": 4.07, "error plus": 0.95, "error minus": 1.02\}, "mu\_chi": \{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.35, "error plus": 0.04, "error minus": 0.04\}, "sigma\_chi": \{"median": 0.2, "5th percentile": 0.18, "95th percentile": 0.23, "error plus": 0.02, "error minus": 0.02\}, "xi\_spin": \{"median": 0.63, "5th percentile": 0.09, "95th percentile": 0.96, "error plus": 0.33, "error minus": 0.54\}, "mu\_spin": \{"median": 0.4, "5th percentile": {-}0.41, "95th percentile": 0.93, "error plus": 0.53, "error minus": 0.81\}, "sigma\_spin": \{"median": 1.35, "5th percentile": 0.45, "95th percentile": 3.7, "error plus": 2.35, "error minus": 0.9\}, "rate": \{"median": 16.58, "5th percentile": 11.97, "95th percentile": 22.45, "error plus": 5.87, "error minus": 4.62\}, "log\_likelihood": \{"median": {-}1024.57, "5th percentile": {-}1030.61, "95th percentile": {-}1019.8, "error plus": 4.78, "error minus": 6.03\}, "variance": \{"median": 0.87, "5th percentile": 0.65, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}, "min\_neff": \{"median": 56.16, "5th percentile": 31.71, "95th percentile": 93.86, "error plus": 37.7, "error minus": 24.45\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.6, "95th percentile": 0.69, "peak": 0.11\}, "cos\_tilt": \{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.3\}, "mass\_1": \{"median": 10.09, "5th percentile": 7.94, "90th percentile": 27.68, "95th percentile": 34.42, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out{{-}1048.61}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out{0.24}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out{{-}1.47}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out{0.05}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out{??}\fi\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out{\{"alpha\_1": \{"median": 1.76, "5th percentile": {-}0.11, "95th percentile": 2.98, "error plus": 1.22, "error minus": 1.87\}, "alpha\_2": \{"median": 4.39, "5th percentile": 3.13, "95th percentile": 6.04, "error plus": 1.64, "error minus": 1.26\}, "beta": \{"median": 1.23, "5th percentile": 0.19, "95th percentile": 2.59, "error plus": 1.36, "error minus": 1.04\}, "mlow\_1": \{"median": 4.99, "5th percentile": 3.22, "95th percentile": 8.01, "error plus": 3.02, "error minus": 1.77\}, "mlow\_2": \{"median": 3.52, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.35, "error minus": 0.49\}, "break\_mass": \{"median": 35.12, "5th percentile": 22.02, "95th percentile": 47.91, "error plus": 12.79, "error minus": 13.09\}, "mpp\_1": \{"median": 9.71, "5th percentile": 8.45, "95th percentile": 10.23, "error plus": 0.52, "error minus": 1.25\}, "mpp\_2": \{"median": 32.95, "5th percentile": 26.74, "95th percentile": 35.92, "error plus": 2.97, "error minus": 6.21\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.32, "95th percentile": 1.61, "error plus": 0.94, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.94, "5th percentile": 1.33, "95th percentile": 9.2, "error plus": 5.26, "error minus": 2.61\}, "delta\_m\_1": \{"median": 4.56, "5th percentile": 0.39, "95th percentile": 9.32, "error plus": 4.75, "error minus": 4.17\}, "delta\_m\_2": \{"median": 5.18, "5th percentile": 0.56, "95th percentile": 9.16, "error plus": 3.98, "error minus": 4.62\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.64, "error plus": 0.28, "error minus": 0.22\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.31, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.28\}, "lamb": \{"median": 3.11, "5th percentile": 2.09, "95th percentile": 4.07, "error plus": 0.95, "error minus": 1.02\}, "mu\_chi": \{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.35, "error plus": 0.04, "error minus": 0.04\}, "sigma\_chi": \{"median": 0.2, "5th percentile": 0.18, "95th percentile": 0.23, "error plus": 0.02, "error minus": 0.02\}, "xi\_spin": \{"median": 0.63, "5th percentile": 0.09, "95th percentile": 0.96, "error plus": 0.33, "error minus": 0.54\}, "mu\_spin": \{"median": 0.4, "5th percentile": {-}0.41, "95th percentile": 0.93, "error plus": 0.53, "error minus": 0.81\}, "sigma\_spin": \{"median": 1.35, "5th percentile": 0.45, "95th percentile": 3.7, "error plus": 2.35, "error minus": 0.9\}, "rate": \{"median": 16.58, "5th percentile": 11.97, "95th percentile": 22.45, "error plus": 5.87, "error minus": 4.62\}, "log\_likelihood": \{"median": {-}1024.57, "5th percentile": {-}1030.61, "95th percentile": {-}1019.8, "error plus": 4.78, "error minus": 6.03\}, "variance": \{"median": 0.87, "5th percentile": 0.65, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}, "min\_neff": \{"median": 56.16, "5th percentile": 31.71, "95th percentile": 93.86, "error plus": 37.7, "error minus": 24.45\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@I@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out{\{"a": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.6, "95th percentile": 0.69, "peak": 0.11\}, "cos\_tilt": \{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.3\}, "mass\_1": \{"median": 10.09, "5th percentile": 7.94, "90th percentile": 27.68, "95th percentile": 34.42, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@II@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out{\{"median": 1.76, "5th percentile": {-}0.11, "95th percentile": 2.98, "error plus": 1.22, "error minus": 1.87\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out{1.76}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out{{-}0.11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out{2.98}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out{1.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out{1.87}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@III@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out{\{"median": 4.39, "5th percentile": 3.13, "95th percentile": 6.04, "error plus": 1.64, "error minus": 1.26\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out{4.39}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out{3.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out{6.04}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out{1.64}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out{1.26}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out{\{"median": 1.23, "5th percentile": 0.19, "95th percentile": 2.59, "error plus": 1.36, "error minus": 1.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out{1.23}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out{0.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out{2.59}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out{1.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out{1.04}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@V@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out{\{"median": 4.99, "5th percentile": 3.22, "95th percentile": 8.01, "error plus": 3.02, "error minus": 1.77\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out{4.99}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out{3.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out{8.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out{3.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out{1.77}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out{\{"median": 3.52, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.35, "error minus": 0.49\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out{3.52}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out{4.87}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out{1.35}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out{0.49}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out{\{"median": 35.12, "5th percentile": 22.02, "95th percentile": 47.91, "error plus": 12.79, "error minus": 13.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out{35.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out{22.02}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out{47.91}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out{12.79}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out{13.09}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@VIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out{\{"median": 9.71, "5th percentile": 8.45, "95th percentile": 10.23, "error plus": 0.52, "error minus": 1.25\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out{9.71}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out{8.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out{10.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out{0.52}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out{1.25}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@IX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out{\{"median": 32.95, "5th percentile": 26.74, "95th percentile": 35.92, "error plus": 2.97, "error minus": 6.21\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out{32.95}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out{26.74}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out{35.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out{2.97}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out{6.21}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@X@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out{\{"median": 0.67, "5th percentile": 0.32, "95th percentile": 1.61, "error plus": 0.94, "error minus": 0.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out{0.67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out{1.61}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out{0.94}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out{0.35}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out{\{"median": 3.94, "5th percentile": 1.33, "95th percentile": 9.2, "error plus": 5.26, "error minus": 2.61\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out{3.94}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out{1.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out{9.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out{5.26}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out{2.61}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out{\{"median": 4.56, "5th percentile": 0.39, "95th percentile": 9.32, "error plus": 4.75, "error minus": 4.17\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out{4.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out{0.39}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out{9.32}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out{4.75}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out{4.17}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out{\{"median": 5.18, "5th percentile": 0.56, "95th percentile": 9.16, "error plus": 3.98, "error minus": 4.62\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out{5.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out{0.56}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out{9.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out{3.98}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out{4.62}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out{\{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.64, "error plus": 0.28, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out{0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out{0.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out{0.22}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out{\{"median": 0.59, "5th percentile": 0.31, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.28\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.59}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.81}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.28}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out{\{"median": 3.11, "5th percentile": 2.09, "95th percentile": 4.07, "error plus": 0.95, "error minus": 1.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out{3.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out{2.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out{4.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out{0.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out{1.02}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out{\{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.35, "error plus": 0.04, "error minus": 0.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.35}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.04}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.04}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XVIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out{\{"median": 0.2, "5th percentile": 0.18, "95th percentile": 0.23, "error plus": 0.02, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.02}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XIX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out{\{"median": 0.63, "5th percentile": 0.09, "95th percentile": 0.96, "error plus": 0.33, "error minus": 0.54\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out{0.63}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out{0.96}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out{0.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out{0.54}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out{\{"median": 0.4, "5th percentile": {-}0.41, "95th percentile": 0.93, "error plus": 0.53, "error minus": 0.81\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out{{-}0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.93}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.53}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.81}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out{\{"median": 1.35, "5th percentile": 0.45, "95th percentile": 3.7, "error plus": 2.35, "error minus": 0.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out{1.35}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out{3.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out{2.35}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out{0.9}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out{\{"median": 16.58, "5th percentile": 11.97, "95th percentile": 22.45, "error plus": 5.87, "error minus": 4.62\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out{16.58}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out{11.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out{22.45}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out{5.87}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out{4.62}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out{\{"median": {-}1024.57, "5th percentile": {-}1030.61, "95th percentile": {-}1019.8, "error plus": 4.78, "error minus": 6.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out{{-}1024.57}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out{{-}1030.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out{{-}1019.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out{4.78}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out{6.03}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out{\{"median": 0.87, "5th percentile": 0.65, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.65}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.23}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out{\{"median": 56.16, "5th percentile": 31.71, "95th percentile": 93.86, "error plus": 37.7, "error minus": 24.45\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out{56.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out{31.71}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out{93.86}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out{37.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out{24.45}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out{0.0}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{\{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.6, "95th percentile": 0.69, "peak": 0.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.69}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.11}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXVIII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out{\{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out{{-}0.87}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.3}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXIX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out{\{"median": 10.09, "5th percentile": 7.94, "90th percentile": 27.68, "95th percentile": 34.42, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out{10.09}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out{7.94}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out{27.68}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out{34.42}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out{9.91}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXX@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out{\{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.5}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out{1.0}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.47}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out{2.0}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormNid@XXXII@out}\makeatother
\makeatletter\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@out{\{"param": \{"chi\_A\_1st": \{"median": 0.06, "error plus": 0.03, "error minus": 0.02, "5th percentile": 0.04, "95th percentile": 0.09\}, "chi\_A\_99th": \{"median": 0.86, "error plus": 0.06, "error minus": 0.06, "5th percentile": 0.8, "95th percentile": 0.92\}, "chi\_B\_1st": \{"median": 0.0, "error plus": 0.01, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.01\}, "chi\_B\_99th": \{"median": 0.6, "error plus": 0.08, "error minus": 0.06, "5th percentile": 0.54, "95th percentile": 0.67\}\}, "ppd": \{"chi\_A": \{"median": 0.4, "5th percentile": 0.12, "95th percentile": 0.76, "spin at peak": 0.36\}, "chi\_B": \{"median": 0.16, "5th percentile": 0.02, "95th percentile": 0.46, "spin at peak": 0.05\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@II\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@out{??}\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I@out{\{"chi\_A\_1st": \{"median": 0.06, "error plus": 0.03, "error minus": 0.02, "5th percentile": 0.04, "95th percentile": 0.09\}, "chi\_A\_99th": \{"median": 0.86, "error plus": 0.06, "error minus": 0.06, "5th percentile": 0.8, "95th percentile": 0.92\}, "chi\_B\_1st": \{"median": 0.0, "error plus": 0.01, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.01\}, "chi\_B\_99th": \{"median": 0.6, "error plus": 0.08, "error minus": 0.06, "5th percentile": 0.54, "95th percentile": 0.67\}\}}\else\ifnum\pdfstrcmp{#1}{chi_A_1st}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III\else\ifnum\pdfstrcmp{#1}{chi_A_99th}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV\else\ifnum\pdfstrcmp{#1}{chi_B_1st}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V\else\ifnum\pdfstrcmp{#1}{chi_B_99th}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I@out{??}\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@I@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@II@out{\{"chi\_A": \{"median": 0.4, "5th percentile": 0.12, "95th percentile": 0.76, "spin at peak": 0.36\}, "chi\_B": \{"median": 0.16, "5th percentile": 0.02, "95th percentile": 0.46, "spin at peak": 0.05\}\}}\else\ifnum\pdfstrcmp{#1}{chi_A}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@II@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII\else\ifnum\pdfstrcmp{#1}{chi_B}=0\let\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@II@out\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@II@out{??}\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@II@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{\{"median": 0.06, "error plus": 0.03, "error minus": 0.02, "5th percentile": 0.04, "95th percentile": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.06}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.02}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.09}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@III@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{\{"median": 0.86, "error plus": 0.06, "error minus": 0.06, "5th percentile": 0.8, "95th percentile": 0.92\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.86}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.92}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{\{"median": 0.0, "error plus": 0.01, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.01\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.01}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.01}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@V@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{\{"median": 0.6, "error plus": 0.08, "error minus": 0.06, "5th percentile": 0.54, "95th percentile": 0.67\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.54}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.67}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{\{"median": 0.4, "5th percentile": 0.12, "95th percentile": 0.76, "spin at peak": 0.36\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{0.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{0.76}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{0.36}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{??}\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out}\newcommand\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{\{"median": 0.16, "5th percentile": 0.02, "95th percentile": 0.46, "spin at peak": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.02}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.46}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.05}\else\def\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{??}\fi\fi\fi\fi\fi\MagBetaConstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out}\makeatother
\makeatletter\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out{\{"ln\_evidence": {-}1049.41, "ln\_evidence\_error": 0.26, "ln\_bayes\_factor\_over\_new\_default": {-}2.26, "ln\_bayes\_factor\_over\_old\_default": {-}0.74, "param": \{"alpha\_1": \{"median": 1.74, "5th percentile": {-}0.34, "95th percentile": 3.02, "error plus": 1.28, "error minus": 2.08\}, "alpha\_2": \{"median": 4.45, "5th percentile": 3.13, "95th percentile": 6.01, "error plus": 1.56, "error minus": 1.32\}, "beta": \{"median": 1.22, "5th percentile": 0.15, "95th percentile": 2.59, "error plus": 1.37, "error minus": 1.07\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.25, "95th percentile": 8.34, "error plus": 3.2, "error minus": 1.9\}, "mlow\_2": \{"median": 3.54, "5th percentile": 3.03, "95th percentile": 4.9, "error plus": 1.36, "error minus": 0.51\}, "break\_mass": \{"median": 35.23, "5th percentile": 21.82, "95th percentile": 48.03, "error plus": 12.81, "error minus": 13.41\}, "mpp\_1": \{"median": 9.7, "5th percentile": 7.51, "95th percentile": 10.2, "error plus": 0.5, "error minus": 2.19\}, "mpp\_2": \{"median": 33.01, "5th percentile": 26.85, "95th percentile": 35.82, "error plus": 2.81, "error minus": 6.16\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.33, "95th percentile": 1.97, "error plus": 1.3, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.86, "5th percentile": 1.25, "95th percentile": 8.99, "error plus": 5.13, "error minus": 2.61\}, "delta\_m\_1": \{"median": 4.17, "5th percentile": 0.34, "95th percentile": 9.12, "error plus": 4.95, "error minus": 3.83\}, "delta\_m\_2": \{"median": 5.1, "5th percentile": 0.55, "95th percentile": 9.15, "error plus": 4.05, "error minus": 4.55\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.13, "95th percentile": 0.66, "error plus": 0.3, "error minus": 0.22\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.3, "95th percentile": 0.82, "error plus": 0.22, "error minus": 0.29\}, "lamb": \{"median": 3.11, "5th percentile": 2.16, "95th percentile": 4.06, "error plus": 0.95, "error minus": 0.95\}, "mu\_chi": \{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.34, "error plus": 0.04, "error minus": 0.04\}, "sigma\_chi": \{"median": 0.21, "5th percentile": 0.18, "95th percentile": 0.25, "error plus": 0.03, "error minus": 0.03\}, "xi\_spin": \{"median": 0.66, "5th percentile": 0.12, "95th percentile": 0.97, "error plus": 0.31, "error minus": 0.54\}, "mu\_spin": \{"median": 0.41, "5th percentile": {-}0.41, "95th percentile": 0.93, "error plus": 0.51, "error minus": 0.82\}, "sigma\_spin": \{"median": 1.23, "5th percentile": 0.46, "95th percentile": 3.5, "error plus": 2.27, "error minus": 0.77\}, "rate": \{"median": 16.3, "5th percentile": 11.79, "95th percentile": 22.13, "error plus": 5.83, "error minus": 4.51\}, "log\_likelihood": \{"median": {-}1024.37, "5th percentile": {-}1030.35, "95th percentile": {-}1019.63, "error plus": 4.74, "error minus": 5.99\}, "variance": \{"median": 0.88, "5th percentile": 0.65, "95th percentile": 0.99, "error plus": 0.1, "error minus": 0.24\}, "min\_neff": \{"median": 59.78, "5th percentile": 32.59, "95th percentile": 98.02, "error plus": 38.24, "error minus": 27.19\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a": \{"median": 0.0, "5th percentile": 0.0, "90th percentile": 0.0, "95th percentile": 0.0, "peak": 0.0\}, "cos\_tilt": \{"median": 0.09, "5th percentile": {-}0.86, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.32\}, "mass\_1": \{"median": 10.1, "5th percentile": 7.95, "90th percentile": 27.87, "95th percentile": 34.5, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out{{-}1049.41}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out{0.26}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out{{-}2.26}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out{{-}0.74}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out{??}\fi\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out{\{"alpha\_1": \{"median": 1.74, "5th percentile": {-}0.34, "95th percentile": 3.02, "error plus": 1.28, "error minus": 2.08\}, "alpha\_2": \{"median": 4.45, "5th percentile": 3.13, "95th percentile": 6.01, "error plus": 1.56, "error minus": 1.32\}, "beta": \{"median": 1.22, "5th percentile": 0.15, "95th percentile": 2.59, "error plus": 1.37, "error minus": 1.07\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.25, "95th percentile": 8.34, "error plus": 3.2, "error minus": 1.9\}, "mlow\_2": \{"median": 3.54, "5th percentile": 3.03, "95th percentile": 4.9, "error plus": 1.36, "error minus": 0.51\}, "break\_mass": \{"median": 35.23, "5th percentile": 21.82, "95th percentile": 48.03, "error plus": 12.81, "error minus": 13.41\}, "mpp\_1": \{"median": 9.7, "5th percentile": 7.51, "95th percentile": 10.2, "error plus": 0.5, "error minus": 2.19\}, "mpp\_2": \{"median": 33.01, "5th percentile": 26.85, "95th percentile": 35.82, "error plus": 2.81, "error minus": 6.16\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.33, "95th percentile": 1.97, "error plus": 1.3, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.86, "5th percentile": 1.25, "95th percentile": 8.99, "error plus": 5.13, "error minus": 2.61\}, "delta\_m\_1": \{"median": 4.17, "5th percentile": 0.34, "95th percentile": 9.12, "error plus": 4.95, "error minus": 3.83\}, "delta\_m\_2": \{"median": 5.1, "5th percentile": 0.55, "95th percentile": 9.15, "error plus": 4.05, "error minus": 4.55\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.13, "95th percentile": 0.66, "error plus": 0.3, "error minus": 0.22\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.3, "95th percentile": 0.82, "error plus": 0.22, "error minus": 0.29\}, "lamb": \{"median": 3.11, "5th percentile": 2.16, "95th percentile": 4.06, "error plus": 0.95, "error minus": 0.95\}, "mu\_chi": \{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.34, "error plus": 0.04, "error minus": 0.04\}, "sigma\_chi": \{"median": 0.21, "5th percentile": 0.18, "95th percentile": 0.25, "error plus": 0.03, "error minus": 0.03\}, "xi\_spin": \{"median": 0.66, "5th percentile": 0.12, "95th percentile": 0.97, "error plus": 0.31, "error minus": 0.54\}, "mu\_spin": \{"median": 0.41, "5th percentile": {-}0.41, "95th percentile": 0.93, "error plus": 0.51, "error minus": 0.82\}, "sigma\_spin": \{"median": 1.23, "5th percentile": 0.46, "95th percentile": 3.5, "error plus": 2.27, "error minus": 0.77\}, "rate": \{"median": 16.3, "5th percentile": 11.79, "95th percentile": 22.13, "error plus": 5.83, "error minus": 4.51\}, "log\_likelihood": \{"median": {-}1024.37, "5th percentile": {-}1030.35, "95th percentile": {-}1019.63, "error plus": 4.74, "error minus": 5.99\}, "variance": \{"median": 0.88, "5th percentile": 0.65, "95th percentile": 0.99, "error plus": 0.1, "error minus": 0.24\}, "min\_neff": \{"median": 59.78, "5th percentile": 32.59, "95th percentile": 98.02, "error plus": 38.24, "error minus": 27.19\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@I@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out{\{"a": \{"median": 0.0, "5th percentile": 0.0, "90th percentile": 0.0, "95th percentile": 0.0, "peak": 0.0\}, "cos\_tilt": \{"median": 0.09, "5th percentile": {-}0.86, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.32\}, "mass\_1": \{"median": 10.1, "5th percentile": 7.95, "90th percentile": 27.87, "95th percentile": 34.5, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@II@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out{\{"median": 1.74, "5th percentile": {-}0.34, "95th percentile": 3.02, "error plus": 1.28, "error minus": 2.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out{1.74}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out{{-}0.34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out{3.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out{1.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out{2.08}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@III@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out{\{"median": 4.45, "5th percentile": 3.13, "95th percentile": 6.01, "error plus": 1.56, "error minus": 1.32\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out{4.45}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out{3.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out{6.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out{1.56}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out{1.32}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IV@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out{\{"median": 1.22, "5th percentile": 0.15, "95th percentile": 2.59, "error plus": 1.37, "error minus": 1.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out{1.22}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out{0.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out{2.59}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out{1.37}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out{1.07}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@V@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out{\{"median": 5.15, "5th percentile": 3.25, "95th percentile": 8.34, "error plus": 3.2, "error minus": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out{5.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out{3.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out{8.34}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out{3.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out{1.9}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VI@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out{\{"median": 3.54, "5th percentile": 3.03, "95th percentile": 4.9, "error plus": 1.36, "error minus": 0.51\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out{3.54}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out{4.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out{1.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out{0.51}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out{\{"median": 35.23, "5th percentile": 21.82, "95th percentile": 48.03, "error plus": 12.81, "error minus": 13.41\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out{35.23}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out{21.82}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out{48.03}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out{12.81}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out{13.41}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@VIII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out{\{"median": 9.7, "5th percentile": 7.51, "95th percentile": 10.2, "error plus": 0.5, "error minus": 2.19\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out{9.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out{7.51}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out{10.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out{0.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out{2.19}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@IX@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out{\{"median": 33.01, "5th percentile": 26.85, "95th percentile": 35.82, "error plus": 2.81, "error minus": 6.16\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out{33.01}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out{26.85}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out{35.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out{2.81}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out{6.16}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@X@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out{\{"median": 0.67, "5th percentile": 0.33, "95th percentile": 1.97, "error plus": 1.3, "error minus": 0.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out{0.67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out{0.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out{1.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out{1.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out{0.35}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XI@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out{\{"median": 3.86, "5th percentile": 1.25, "95th percentile": 8.99, "error plus": 5.13, "error minus": 2.61\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out{3.86}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out{1.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out{8.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out{5.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out{2.61}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out{\{"median": 4.17, "5th percentile": 0.34, "95th percentile": 9.12, "error plus": 4.95, "error minus": 3.83\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out{4.17}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out{0.34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out{9.12}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out{4.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out{3.83}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out{\{"median": 5.1, "5th percentile": 0.55, "95th percentile": 9.15, "error plus": 4.05, "error minus": 4.55\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out{5.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out{0.55}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out{9.15}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out{4.05}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out{4.55}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIV@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out{\{"median": 0.36, "5th percentile": 0.13, "95th percentile": 0.66, "error plus": 0.3, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out{0.66}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out{0.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out{0.22}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XV@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out{\{"median": 0.59, "5th percentile": 0.3, "95th percentile": 0.82, "error plus": 0.22, "error minus": 0.29\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.59}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out{0.29}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVI@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out{\{"median": 3.11, "5th percentile": 2.16, "95th percentile": 4.06, "error plus": 0.95, "error minus": 0.95\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out{3.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out{2.16}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out{4.06}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out{0.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out{0.95}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out{\{"median": 0.3, "5th percentile": 0.26, "95th percentile": 0.34, "error plus": 0.04, "error minus": 0.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.34}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.04}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out{0.04}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XVIII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out{\{"median": 0.21, "5th percentile": 0.18, "95th percentile": 0.25, "error plus": 0.03, "error minus": 0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out{0.03}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XIX@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out{\{"median": 0.66, "5th percentile": 0.12, "95th percentile": 0.97, "error plus": 0.31, "error minus": 0.54\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out{0.66}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out{0.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out{0.54}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XX@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out{\{"median": 0.41, "5th percentile": {-}0.41, "95th percentile": 0.93, "error plus": 0.51, "error minus": 0.82\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.41}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out{{-}0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.93}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out{0.82}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXI@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out{\{"median": 1.23, "5th percentile": 0.46, "95th percentile": 3.5, "error plus": 2.27, "error minus": 0.77\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out{1.23}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out{0.46}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out{2.27}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out{0.77}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out{\{"median": 16.3, "5th percentile": 11.79, "95th percentile": 22.13, "error plus": 5.83, "error minus": 4.51\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out{16.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out{11.79}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out{22.13}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out{5.83}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out{4.51}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out{\{"median": {-}1024.37, "5th percentile": {-}1030.35, "95th percentile": {-}1019.63, "error plus": 4.74, "error minus": 5.99\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out{{-}1024.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out{{-}1030.35}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out{{-}1019.63}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out{4.74}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out{5.99}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIV@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out{\{"median": 0.88, "5th percentile": 0.65, "95th percentile": 0.99, "error plus": 0.1, "error minus": 0.24\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.88}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.65}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out{0.24}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXV@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out{\{"median": 59.78, "5th percentile": 32.59, "95th percentile": 98.02, "error plus": 38.24, "error minus": 27.19\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out{59.78}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out{32.59}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out{98.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out{38.24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out{27.19}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVI@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out{0.0}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{\{"median": 0.0, "5th percentile": 0.0, "90th percentile": 0.0, "95th percentile": 0.0, "peak": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{0.0}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXVIII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out{\{"median": 0.09, "5th percentile": {-}0.86, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.32\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.09}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out{{-}0.86}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out{0.32}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXIX@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out{\{"median": 10.1, "5th percentile": 7.95, "90th percentile": 27.87, "95th percentile": 34.5, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out{10.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out{7.95}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out{27.87}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out{34.5}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out{9.91}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXX@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out{\{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.5}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out{1.0}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXI@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out{0.47}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out{2.0}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormNid@XXXII@out}\makeatother
\makeatletter\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@out{\{"param": \{"chi\_A\_1st": \{"median": 0.05, "error plus": 0.04, "error minus": 0.02, "5th percentile": 0.02, "95th percentile": 0.09\}, "chi\_A\_99th": \{"median": 0.88, "error plus": 0.06, "error minus": 0.07, "5th percentile": 0.81, "95th percentile": 0.94\}, "chi\_B\_1st": \{"median": 0.0, "error plus": 0.01, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.01\}, "chi\_B\_99th": \{"median": 0.61, "error plus": 0.08, "error minus": 0.07, "5th percentile": 0.55, "95th percentile": 0.7\}\}, "ppd": \{"chi\_A": \{"median": NaN, "5th percentile": NaN, "95th percentile": NaN, "spin at peak": 0.35\}, "chi\_B": \{"median": NaN, "5th percentile": NaN, "95th percentile": NaN, "spin at peak": 0.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@II\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@out{??}\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I@out{\{"chi\_A\_1st": \{"median": 0.05, "error plus": 0.04, "error minus": 0.02, "5th percentile": 0.02, "95th percentile": 0.09\}, "chi\_A\_99th": \{"median": 0.88, "error plus": 0.06, "error minus": 0.07, "5th percentile": 0.81, "95th percentile": 0.94\}, "chi\_B\_1st": \{"median": 0.0, "error plus": 0.01, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.01\}, "chi\_B\_99th": \{"median": 0.61, "error plus": 0.08, "error minus": 0.07, "5th percentile": 0.55, "95th percentile": 0.7\}\}}\else\ifnum\pdfstrcmp{#1}{chi_A_1st}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III\else\ifnum\pdfstrcmp{#1}{chi_A_99th}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV\else\ifnum\pdfstrcmp{#1}{chi_B_1st}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V\else\ifnum\pdfstrcmp{#1}{chi_B_99th}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I@out{??}\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@I@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@II@out{\{"chi\_A": \{"median": NaN, "5th percentile": NaN, "95th percentile": NaN, "spin at peak": 0.35\}, "chi\_B": \{"median": NaN, "5th percentile": NaN, "95th percentile": NaN, "spin at peak": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{chi_A}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@II@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII\else\ifnum\pdfstrcmp{#1}{chi_B}=0\let\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@II@out\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@II@out{??}\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@II@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{\{"median": 0.05, "error plus": 0.04, "error minus": 0.02, "5th percentile": 0.02, "95th percentile": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.05}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.04}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.02}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.02}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{0.09}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@III@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{\{"median": 0.88, "error plus": 0.06, "error minus": 0.07, "5th percentile": 0.81, "95th percentile": 0.94\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.88}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.81}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{0.94}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@IV@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{\{"median": 0.0, "error plus": 0.01, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.01\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.01}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{0.01}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@V@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{\{"median": 0.61, "error plus": 0.08, "error minus": 0.07, "5th percentile": 0.55, "95th percentile": 0.7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.61}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.55}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{0.7}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out{??}\fi\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VI@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{\{"median": NaN, "5th percentile": NaN, "95th percentile": NaN, "spin at peak": 0.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{nan}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{nan}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{nan}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{0.35}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out{??}\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VII@out}\newcommand\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{\{"median": NaN, "5th percentile": NaN, "95th percentile": NaN, "spin at peak": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{nan}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{nan}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{nan}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.0}\else\def\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out{??}\fi\fi\fi\fi\fi\MagBetaUnconstrainedIidTiltIsotropicTruncnormSpinSorting@VIII@out}\makeatother
\makeatletter\newcommand\MagTruncnormIidTiltIsotropicAlignedNid[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@out{\{"ln\_evidence": {-}1047.34, "ln\_evidence\_error": 0.24, "ln\_bayes\_factor\_over\_new\_default": {-}0.19, "ln\_bayes\_factor\_over\_old\_default": 1.32, "param": \{"alpha\_1": \{"median": 1.83, "5th percentile": {-}0.07, "95th percentile": 3.02, "error plus": 1.18, "error minus": 1.9\}, "alpha\_2": \{"median": 4.49, "5th percentile": 3.19, "95th percentile": 6.04, "error plus": 1.56, "error minus": 1.3\}, "beta": \{"median": 1.32, "5th percentile": 0.26, "95th percentile": 2.66, "error plus": 1.35, "error minus": 1.06\}, "mlow\_1": \{"median": 5.09, "5th percentile": 3.24, "95th percentile": 8.31, "error plus": 3.23, "error minus": 1.84\}, "mlow\_2": \{"median": 3.54, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.33, "error minus": 0.51\}, "break\_mass": \{"median": 35.86, "5th percentile": 22.19, "95th percentile": 48.48, "error plus": 12.62, "error minus": 13.67\}, "mpp\_1": \{"median": 9.74, "5th percentile": 8.19, "95th percentile": 10.24, "error plus": 0.5, "error minus": 1.55\}, "mpp\_2": \{"median": 33.06, "5th percentile": 27.28, "95th percentile": 35.71, "error plus": 2.65, "error minus": 5.77\}, "sigpp\_1": \{"median": 0.65, "5th percentile": 0.31, "95th percentile": 1.69, "error plus": 1.03, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.56, "5th percentile": 1.2, "95th percentile": 8.8, "error plus": 5.24, "error minus": 2.36\}, "delta\_m\_1": \{"median": 4.27, "5th percentile": 0.28, "95th percentile": 9.16, "error plus": 4.89, "error minus": 3.99\}, "delta\_m\_2": \{"median": 4.9, "5th percentile": 0.47, "95th percentile": 9.0, "error plus": 4.1, "error minus": 4.43\}, "lam\_0": \{"median": 0.37, "5th percentile": 0.14, "95th percentile": 0.65, "error plus": 0.28, "error minus": 0.23\}, "lam\_1": \{"median": 0.58, "5th percentile": 0.3, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.28\}, "lamb": \{"median": 3.1, "5th percentile": 2.15, "95th percentile": 3.99, "error plus": 0.89, "error minus": 0.95\}, "mu\_chi": \{"median": 0.09, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.14, "error minus": 0.08\}, "sigma\_chi": \{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.08, "error minus": 0.08\}, "xi\_spin": \{"median": 0.64, "5th percentile": 0.14, "95th percentile": 0.96, "error plus": 0.32, "error minus": 0.51\}, "sigma\_spin": \{"median": 1.73, "5th percentile": 0.95, "95th percentile": 3.5, "error plus": 1.76, "error minus": 0.79\}, "rate": \{"median": 16.39, "5th percentile": 12.04, "95th percentile": 22.27, "error plus": 5.87, "error minus": 4.35\}, "log\_likelihood": \{"median": {-}1023.88, "5th percentile": {-}1029.48, "95th percentile": {-}1019.88, "error plus": 4.0, "error minus": 5.6\}, "variance": \{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}, "min\_neff": \{"median": 56.21, "5th percentile": 31.29, "95th percentile": 94.86, "error plus": 38.66, "error minus": 24.92\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a": \{"median": 0.26, "5th percentile": 0.03, "90th percentile": 0.6, "95th percentile": 0.7, "peak": 0.11\}, "cos\_tilt": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.83, "95th percentile": 0.91, "peak": 1.0\}, "mass\_1": \{"median": 10.11, "5th percentile": 7.95, "90th percentile": 27.61, "95th percentile": 34.33, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.46, "95th percentile": 0.47, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@out{{-}1047.34}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@out{0.24}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@out{{-}0.19}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@out{1.32}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@out\MagTruncnormIidTiltIsotropicAlignedNid@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@out\MagTruncnormIidTiltIsotropicAlignedNid@II\else\def\MagTruncnormIidTiltIsotropicAlignedNid@out{??}\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@I@out{\{"alpha\_1": \{"median": 1.83, "5th percentile": {-}0.07, "95th percentile": 3.02, "error plus": 1.18, "error minus": 1.9\}, "alpha\_2": \{"median": 4.49, "5th percentile": 3.19, "95th percentile": 6.04, "error plus": 1.56, "error minus": 1.3\}, "beta": \{"median": 1.32, "5th percentile": 0.26, "95th percentile": 2.66, "error plus": 1.35, "error minus": 1.06\}, "mlow\_1": \{"median": 5.09, "5th percentile": 3.24, "95th percentile": 8.31, "error plus": 3.23, "error minus": 1.84\}, "mlow\_2": \{"median": 3.54, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.33, "error minus": 0.51\}, "break\_mass": \{"median": 35.86, "5th percentile": 22.19, "95th percentile": 48.48, "error plus": 12.62, "error minus": 13.67\}, "mpp\_1": \{"median": 9.74, "5th percentile": 8.19, "95th percentile": 10.24, "error plus": 0.5, "error minus": 1.55\}, "mpp\_2": \{"median": 33.06, "5th percentile": 27.28, "95th percentile": 35.71, "error plus": 2.65, "error minus": 5.77\}, "sigpp\_1": \{"median": 0.65, "5th percentile": 0.31, "95th percentile": 1.69, "error plus": 1.03, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.56, "5th percentile": 1.2, "95th percentile": 8.8, "error plus": 5.24, "error minus": 2.36\}, "delta\_m\_1": \{"median": 4.27, "5th percentile": 0.28, "95th percentile": 9.16, "error plus": 4.89, "error minus": 3.99\}, "delta\_m\_2": \{"median": 4.9, "5th percentile": 0.47, "95th percentile": 9.0, "error plus": 4.1, "error minus": 4.43\}, "lam\_0": \{"median": 0.37, "5th percentile": 0.14, "95th percentile": 0.65, "error plus": 0.28, "error minus": 0.23\}, "lam\_1": \{"median": 0.58, "5th percentile": 0.3, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.28\}, "lamb": \{"median": 3.1, "5th percentile": 2.15, "95th percentile": 3.99, "error plus": 0.89, "error minus": 0.95\}, "mu\_chi": \{"median": 0.09, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.14, "error minus": 0.08\}, "sigma\_chi": \{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.08, "error minus": 0.08\}, "xi\_spin": \{"median": 0.64, "5th percentile": 0.14, "95th percentile": 0.96, "error plus": 0.32, "error minus": 0.51\}, "sigma\_spin": \{"median": 1.73, "5th percentile": 0.95, "95th percentile": 3.5, "error plus": 1.76, "error minus": 0.79\}, "rate": \{"median": 16.39, "5th percentile": 12.04, "95th percentile": 22.27, "error plus": 5.87, "error minus": 4.35\}, "log\_likelihood": \{"median": {-}1023.88, "5th percentile": {-}1029.48, "95th percentile": {-}1019.88, "error plus": 4.0, "error minus": 5.6\}, "variance": \{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}, "min\_neff": \{"median": 56.21, "5th percentile": 31.29, "95th percentile": 94.86, "error plus": 38.66, "error minus": 24.92\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XIX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XX\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XXI\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XXII\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XXIII\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XXIV\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XXV\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@I@out\MagTruncnormIidTiltIsotropicAlignedNid@XXVI\else\def\MagTruncnormIidTiltIsotropicAlignedNid@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@I@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@II@out{\{"a": \{"median": 0.26, "5th percentile": 0.03, "90th percentile": 0.6, "95th percentile": 0.7, "peak": 0.11\}, "cos\_tilt": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.83, "95th percentile": 0.91, "peak": 1.0\}, "mass\_1": \{"median": 10.11, "5th percentile": 7.95, "90th percentile": 27.61, "95th percentile": 34.33, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.46, "95th percentile": 0.47, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@II@out\MagTruncnormIidTiltIsotropicAlignedNid@XXVII\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@II@out\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@II@out\MagTruncnormIidTiltIsotropicAlignedNid@XXIX\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@II@out\MagTruncnormIidTiltIsotropicAlignedNid@XXX\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagTruncnormIidTiltIsotropicAlignedNid@II@out\MagTruncnormIidTiltIsotropicAlignedNid@XXXI\else\def\MagTruncnormIidTiltIsotropicAlignedNid@II@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@II@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@III@out{\{"median": 1.83, "5th percentile": {-}0.07, "95th percentile": 3.02, "error plus": 1.18, "error minus": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@III@out{1.83}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@III@out{{-}0.07}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@III@out{3.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@III@out{1.18}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@III@out{1.9}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@III@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@III@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IV@out{\{"median": 4.49, "5th percentile": 3.19, "95th percentile": 6.04, "error plus": 1.56, "error minus": 1.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IV@out{4.49}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IV@out{3.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IV@out{6.04}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IV@out{1.56}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IV@out{1.3}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@IV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@IV@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@V@out{\{"median": 1.32, "5th percentile": 0.26, "95th percentile": 2.66, "error plus": 1.35, "error minus": 1.06\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@V@out{1.32}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@V@out{0.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@V@out{2.66}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@V@out{1.35}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@V@out{1.06}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@V@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@V@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VI@out{\{"median": 5.09, "5th percentile": 3.24, "95th percentile": 8.31, "error plus": 3.23, "error minus": 1.84\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VI@out{5.09}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VI@out{3.24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VI@out{8.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VI@out{3.23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VI@out{1.84}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@VI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@VI@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VII@out{\{"median": 3.54, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.33, "error minus": 0.51\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VII@out{3.54}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VII@out{4.87}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VII@out{1.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VII@out{0.51}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@VII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@VII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out{\{"median": 35.86, "5th percentile": 22.19, "95th percentile": 48.48, "error plus": 12.62, "error minus": 13.67\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out{35.86}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out{22.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out{48.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out{12.62}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out{13.67}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@VIII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IX@out{\{"median": 9.74, "5th percentile": 8.19, "95th percentile": 10.24, "error plus": 0.5, "error minus": 1.55\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IX@out{9.74}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IX@out{8.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IX@out{10.24}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IX@out{0.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@IX@out{1.55}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@IX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@IX@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@X@out{\{"median": 33.06, "5th percentile": 27.28, "95th percentile": 35.71, "error plus": 2.65, "error minus": 5.77\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@X@out{33.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@X@out{27.28}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@X@out{35.71}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@X@out{2.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@X@out{5.77}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@X@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@X@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XI@out{\{"median": 0.65, "5th percentile": 0.31, "95th percentile": 1.69, "error plus": 1.03, "error minus": 0.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XI@out{0.65}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XI@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XI@out{1.69}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XI@out{1.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XI@out{0.35}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XI@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XII@out{\{"median": 3.56, "5th percentile": 1.2, "95th percentile": 8.8, "error plus": 5.24, "error minus": 2.36\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XII@out{3.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XII@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XII@out{8.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XII@out{5.24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XII@out{2.36}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out{\{"median": 4.27, "5th percentile": 0.28, "95th percentile": 9.16, "error plus": 4.89, "error minus": 3.99\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out{4.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out{0.28}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out{9.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out{4.89}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out{3.99}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XIII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out{\{"median": 4.9, "5th percentile": 0.47, "95th percentile": 9.0, "error plus": 4.1, "error minus": 4.43\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out{4.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out{0.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out{9.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out{4.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out{4.43}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XIV@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XV@out{\{"median": 0.37, "5th percentile": 0.14, "95th percentile": 0.65, "error plus": 0.28, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XV@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XV@out{0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XV@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XV@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XV@out{0.23}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XV@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out{\{"median": 0.58, "5th percentile": 0.3, "95th percentile": 0.81, "error plus": 0.22, "error minus": 0.28\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out{0.58}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out{0.81}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out{0.28}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XVI@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out{\{"median": 3.1, "5th percentile": 2.15, "95th percentile": 3.99, "error plus": 0.89, "error minus": 0.95\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out{3.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out{2.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out{3.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out{0.89}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out{0.95}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XVII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out{\{"median": 0.09, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.14, "error minus": 0.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out{0.09}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out{0.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out{0.08}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XVIII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out{\{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.08, "error minus": 0.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out{0.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out{0.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out{0.08}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XIX@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XX@out{\{"median": 0.64, "5th percentile": 0.14, "95th percentile": 0.96, "error plus": 0.32, "error minus": 0.51\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XX@out{0.64}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XX@out{0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XX@out{0.96}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XX@out{0.32}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XX@out{0.51}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XX@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out{\{"median": 1.73, "5th percentile": 0.95, "95th percentile": 3.5, "error plus": 1.76, "error minus": 0.79\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out{1.73}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out{0.95}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out{1.76}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out{0.79}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXI@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out{\{"median": 16.39, "5th percentile": 12.04, "95th percentile": 22.27, "error plus": 5.87, "error minus": 4.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out{16.39}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out{12.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out{22.27}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out{5.87}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out{4.35}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out{\{"median": {-}1023.88, "5th percentile": {-}1029.48, "95th percentile": {-}1019.88, "error plus": 4.0, "error minus": 5.6\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out{{-}1023.88}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out{{-}1029.48}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out{{-}1019.88}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out{4.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out{5.6}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXIII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out{\{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out{0.64}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out{0.23}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXIV@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out{\{"median": 56.21, "5th percentile": 31.29, "95th percentile": 94.86, "error plus": 38.66, "error minus": 24.92\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out{56.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out{31.29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out{94.86}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out{38.66}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out{24.92}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXV@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out{0.0}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXVI@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out{\{"median": 0.26, "5th percentile": 0.03, "90th percentile": 0.6, "95th percentile": 0.7, "peak": 0.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out{0.26}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out{0.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out{0.7}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out{0.11}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXVII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out{\{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.83, "95th percentile": 0.91, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out{{-}0.87}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out{0.83}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out{0.91}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out{1.0}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXVIII@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out{\{"median": 10.11, "5th percentile": 7.95, "90th percentile": 27.61, "95th percentile": 34.33, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out{10.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out{7.95}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out{27.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out{34.33}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out{9.91}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXIX@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out{\{"median": 0.84, "5th percentile": 0.5, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out{0.5}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out{1.0}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXX@out}\newcommand\MagTruncnormIidTiltIsotropicAlignedNid@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.46, "95th percentile": 0.47, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out{0.46}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out{0.47}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out{2.0}\else\def\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicAlignedNid@XXXI@out}\makeatother
\makeatletter\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@out{\{"ln\_evidence": {-}1029.55, "ln\_evidence\_error": 0.24, "ln\_bayes\_factor\_over\_new\_default": 17.6, "ln\_bayes\_factor\_over\_old\_default": 19.11, "param": \{"alpha\_1": \{"median": 1.63, "5th percentile": {-}0.17, "95th percentile": 2.73, "error plus": 1.09, "error minus": 1.81\}, "alpha\_2": \{"median": 5.17, "5th percentile": 3.6, "95th percentile": 6.97, "error plus": 1.8, "error minus": 1.57\}, "beta": \{"median": 1.1, "5th percentile": 0.09, "95th percentile": 2.43, "error plus": 1.33, "error minus": 1.01\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.27, "95th percentile": 8.16, "error plus": 3.01, "error minus": 1.87\}, "mlow\_2": \{"median": 3.56, "5th percentile": 3.04, "95th percentile": 4.91, "error plus": 1.36, "error minus": 0.52\}, "break\_mass": \{"median": 37.07, "5th percentile": 26.17, "95th percentile": 48.58, "error plus": 11.5, "error minus": 10.91\}, "mpp\_1": \{"median": 9.75, "5th percentile": 8.48, "95th percentile": 10.23, "error plus": 0.48, "error minus": 1.27\}, "mpp\_2": \{"median": 32.84, "5th percentile": 26.68, "95th percentile": 36.62, "error plus": 3.78, "error minus": 6.16\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.33, "95th percentile": 1.54, "error plus": 0.87, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.86, "5th percentile": 1.24, "95th percentile": 9.11, "error plus": 5.25, "error minus": 2.62\}, "delta\_m\_1": \{"median": 4.14, "5th percentile": 0.32, "95th percentile": 9.09, "error plus": 4.95, "error minus": 3.83\}, "delta\_m\_2": \{"median": 5.01, "5th percentile": 0.55, "95th percentile": 9.09, "error plus": 4.09, "error minus": 4.46\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.63, "error plus": 0.27, "error minus": 0.23\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.23, "error minus": 0.27\}, "lamb": \{"median": 3.18, "5th percentile": 2.23, "95th percentile": 4.1, "error plus": 0.92, "error minus": 0.95\}, "mu\_chi": \{"median": 0.1, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.13, "error minus": 0.09\}, "sigma\_chi": \{"median": 0.31, "5th percentile": 0.23, "95th percentile": 0.38, "error plus": 0.07, "error minus": 0.08\}, "xi\_spin": \{"median": 0.62, "5th percentile": 0.08, "95th percentile": 0.97, "error plus": 0.34, "error minus": 0.54\}, "mu\_spin": \{"median": 0.46, "5th percentile": {-}0.41, "95th percentile": 0.95, "error plus": 0.48, "error minus": 0.87\}, "sigma\_spin": \{"median": 1.38, "5th percentile": 0.5, "95th percentile": 3.58, "error plus": 2.2, "error minus": 0.88\}, "rate": \{"median": 16.01, "5th percentile": 11.63, "95th percentile": 22.01, "error plus": 6.0, "error minus": 4.37\}, "log\_likelihood": \{"median": {-}1006.0, "5th percentile": {-}1011.94, "95th percentile": {-}1001.88, "error plus": 4.12, "error minus": 5.95\}, "variance": \{"median": 0.9, "5th percentile": 0.7, "95th percentile": 0.99, "error plus": 0.09, "error minus": 0.2\}, "min\_neff": \{"median": 56.51, "5th percentile": 33.25, "95th percentile": 87.51, "error plus": 31.0, "error minus": 23.26\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a": \{"median": 0.25, "5th percentile": 0.03, "90th percentile": 0.57, "95th percentile": 0.67, "peak": 0.12\}, "cos\_tilt": \{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.37\}, "mass\_1": \{"median": 10.13, "5th percentile": 7.97, "90th percentile": 28.0, "95th percentile": 34.54, "peak": 9.91\}, "mass\_ratio": \{"median": 0.83, "5th percentile": 0.49, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.46, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@out{{-}1029.55}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@out{0.24}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@out{17.6}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@out{19.11}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@out\MagTruncnormIidTiltIsotropicTruncnormNid@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@out\MagTruncnormIidTiltIsotropicTruncnormNid@II\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@out{??}\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@I@out{\{"alpha\_1": \{"median": 1.63, "5th percentile": {-}0.17, "95th percentile": 2.73, "error plus": 1.09, "error minus": 1.81\}, "alpha\_2": \{"median": 5.17, "5th percentile": 3.6, "95th percentile": 6.97, "error plus": 1.8, "error minus": 1.57\}, "beta": \{"median": 1.1, "5th percentile": 0.09, "95th percentile": 2.43, "error plus": 1.33, "error minus": 1.01\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.27, "95th percentile": 8.16, "error plus": 3.01, "error minus": 1.87\}, "mlow\_2": \{"median": 3.56, "5th percentile": 3.04, "95th percentile": 4.91, "error plus": 1.36, "error minus": 0.52\}, "break\_mass": \{"median": 37.07, "5th percentile": 26.17, "95th percentile": 48.58, "error plus": 11.5, "error minus": 10.91\}, "mpp\_1": \{"median": 9.75, "5th percentile": 8.48, "95th percentile": 10.23, "error plus": 0.48, "error minus": 1.27\}, "mpp\_2": \{"median": 32.84, "5th percentile": 26.68, "95th percentile": 36.62, "error plus": 3.78, "error minus": 6.16\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.33, "95th percentile": 1.54, "error plus": 0.87, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.86, "5th percentile": 1.24, "95th percentile": 9.11, "error plus": 5.25, "error minus": 2.62\}, "delta\_m\_1": \{"median": 4.14, "5th percentile": 0.32, "95th percentile": 9.09, "error plus": 4.95, "error minus": 3.83\}, "delta\_m\_2": \{"median": 5.01, "5th percentile": 0.55, "95th percentile": 9.09, "error plus": 4.09, "error minus": 4.46\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.63, "error plus": 0.27, "error minus": 0.23\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.23, "error minus": 0.27\}, "lamb": \{"median": 3.18, "5th percentile": 2.23, "95th percentile": 4.1, "error plus": 0.92, "error minus": 0.95\}, "mu\_chi": \{"median": 0.1, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.13, "error minus": 0.09\}, "sigma\_chi": \{"median": 0.31, "5th percentile": 0.23, "95th percentile": 0.38, "error plus": 0.07, "error minus": 0.08\}, "xi\_spin": \{"median": 0.62, "5th percentile": 0.08, "95th percentile": 0.97, "error plus": 0.34, "error minus": 0.54\}, "mu\_spin": \{"median": 0.46, "5th percentile": {-}0.41, "95th percentile": 0.95, "error plus": 0.48, "error minus": 0.87\}, "sigma\_spin": \{"median": 1.38, "5th percentile": 0.5, "95th percentile": 3.58, "error plus": 2.2, "error minus": 0.88\}, "rate": \{"median": 16.01, "5th percentile": 11.63, "95th percentile": 22.01, "error plus": 6.0, "error minus": 4.37\}, "log\_likelihood": \{"median": {-}1006.0, "5th percentile": {-}1011.94, "95th percentile": {-}1001.88, "error plus": 4.12, "error minus": 5.95\}, "variance": \{"median": 0.9, "5th percentile": 0.7, "95th percentile": 0.99, "error plus": 0.09, "error minus": 0.2\}, "min\_neff": \{"median": 56.51, "5th percentile": 33.25, "95th percentile": 87.51, "error plus": 31.0, "error minus": 23.26\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XIX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XX\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXI\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXII\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXV\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@I@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@I@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@II@out{\{"a": \{"median": 0.25, "5th percentile": 0.03, "90th percentile": 0.57, "95th percentile": 0.67, "peak": 0.12\}, "cos\_tilt": \{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.37\}, "mass\_1": \{"median": 10.13, "5th percentile": 7.97, "90th percentile": 28.0, "95th percentile": 34.54, "peak": 9.91\}, "mass\_ratio": \{"median": 0.83, "5th percentile": 0.49, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.46, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@II@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@II@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@II@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXX\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@II@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagTruncnormIidTiltIsotropicTruncnormNid@II@out\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@II@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@II@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@III@out{\{"median": 1.63, "5th percentile": {-}0.17, "95th percentile": 2.73, "error plus": 1.09, "error minus": 1.81\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@III@out{1.63}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@III@out{{-}0.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@III@out{2.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@III@out{1.09}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@III@out{1.81}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@III@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@III@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out{\{"median": 5.17, "5th percentile": 3.6, "95th percentile": 6.97, "error plus": 1.8, "error minus": 1.57\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out{5.17}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out{3.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out{6.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out{1.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out{1.57}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@IV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@V@out{\{"median": 1.1, "5th percentile": 0.09, "95th percentile": 2.43, "error plus": 1.33, "error minus": 1.01\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@V@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@V@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@V@out{2.43}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@V@out{1.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@V@out{1.01}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@V@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@V@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out{\{"median": 5.15, "5th percentile": 3.27, "95th percentile": 8.16, "error plus": 3.01, "error minus": 1.87\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out{5.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out{3.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out{8.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out{3.01}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out{1.87}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@VI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out{\{"median": 3.56, "5th percentile": 3.04, "95th percentile": 4.91, "error plus": 1.36, "error minus": 0.52\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out{3.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out{3.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out{4.91}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out{1.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out{0.52}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@VII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out{\{"median": 37.07, "5th percentile": 26.17, "95th percentile": 48.58, "error plus": 11.5, "error minus": 10.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out{37.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out{26.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out{48.58}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out{11.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out{10.91}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@VIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out{\{"median": 9.75, "5th percentile": 8.48, "95th percentile": 10.23, "error plus": 0.48, "error minus": 1.27\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out{9.75}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out{8.48}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out{10.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out{0.48}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out{1.27}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@IX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@X@out{\{"median": 32.84, "5th percentile": 26.68, "95th percentile": 36.62, "error plus": 3.78, "error minus": 6.16\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@X@out{32.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@X@out{26.68}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@X@out{36.62}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@X@out{3.78}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@X@out{6.16}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@X@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@X@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out{\{"median": 0.67, "5th percentile": 0.33, "95th percentile": 1.54, "error plus": 0.87, "error minus": 0.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out{0.67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out{0.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out{1.54}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out{0.87}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out{0.35}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out{\{"median": 3.86, "5th percentile": 1.24, "95th percentile": 9.11, "error plus": 5.25, "error minus": 2.62\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out{3.86}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out{1.24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out{9.11}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out{5.25}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out{2.62}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out{\{"median": 4.14, "5th percentile": 0.32, "95th percentile": 9.09, "error plus": 4.95, "error minus": 3.83\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out{4.14}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out{9.09}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out{4.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out{3.83}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out{\{"median": 5.01, "5th percentile": 0.55, "95th percentile": 9.09, "error plus": 4.09, "error minus": 4.46\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out{5.01}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out{0.55}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out{9.09}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out{4.09}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out{4.46}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XIV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out{\{"median": 0.36, "5th percentile": 0.14, "95th percentile": 0.63, "error plus": 0.27, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out{0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out{0.63}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out{0.27}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out{0.23}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out{\{"median": 0.59, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.23, "error minus": 0.27\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out{0.59}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out{0.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out{0.23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out{0.27}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XVI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out{\{"median": 3.18, "5th percentile": 2.23, "95th percentile": 4.1, "error plus": 0.92, "error minus": 0.95\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out{3.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out{2.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out{4.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out{0.92}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out{0.95}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XVII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out{\{"median": 0.1, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.13, "error minus": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out{0.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out{0.09}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XVIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out{\{"median": 0.31, "5th percentile": 0.23, "95th percentile": 0.38, "error plus": 0.07, "error minus": 0.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out{0.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out{0.38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out{0.08}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XIX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out{\{"median": 0.62, "5th percentile": 0.08, "95th percentile": 0.97, "error plus": 0.34, "error minus": 0.54\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out{0.62}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out{0.08}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out{0.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out{0.34}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out{0.54}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out{\{"median": 0.46, "5th percentile": {-}0.41, "95th percentile": 0.95, "error plus": 0.48, "error minus": 0.87\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out{0.46}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out{{-}0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out{0.95}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out{0.48}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out{0.87}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out{\{"median": 1.38, "5th percentile": 0.5, "95th percentile": 3.58, "error plus": 2.2, "error minus": 0.88\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out{1.38}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out{0.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out{3.58}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out{2.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out{0.88}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out{\{"median": 16.01, "5th percentile": 11.63, "95th percentile": 22.01, "error plus": 6.0, "error minus": 4.37\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out{16.01}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out{11.63}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out{22.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out{6.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out{4.37}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out{\{"median": {-}1006.0, "5th percentile": {-}1011.94, "95th percentile": {-}1001.88, "error plus": 4.12, "error minus": 5.95\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out{{-}1006.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out{{-}1011.94}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out{{-}1001.88}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out{4.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out{5.95}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXIV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out{\{"median": 0.9, "5th percentile": 0.7, "95th percentile": 0.99, "error plus": 0.09, "error minus": 0.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out{0.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out{0.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out{0.09}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out{0.2}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out{\{"median": 56.51, "5th percentile": 33.25, "95th percentile": 87.51, "error plus": 31.0, "error minus": 23.26\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out{56.51}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out{33.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out{87.51}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out{31.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out{23.26}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXVI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out{0.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXVII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out{\{"median": 0.25, "5th percentile": 0.03, "90th percentile": 0.57, "95th percentile": 0.67, "peak": 0.12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out{0.25}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out{0.57}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out{0.67}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out{0.12}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXVIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out{\{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.37\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out{0.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out{{-}0.87}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out{0.81}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out{0.37}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXIX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out{\{"median": 10.13, "5th percentile": 7.97, "90th percentile": 28.0, "95th percentile": 34.54, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out{10.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out{7.97}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out{28.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out{34.54}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out{9.91}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out{\{"median": 0.83, "5th percentile": 0.49, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out{0.83}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out{0.49}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out{1.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXXI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.46, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out{0.46}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out{2.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNid@XXXII@out}\makeatother
\makeatletter\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@out{\{"ln\_evidence": {-}1047.54, "ln\_evidence\_error": 0.24, "ln\_bayes\_factor\_over\_new\_default": {-}0.39, "ln\_bayes\_factor\_over\_old\_default": 1.12, "param": \{"alpha\_1": \{"median": 1.83, "5th percentile": {-}0.02, "95th percentile": 3.02, "error plus": 1.19, "error minus": 1.85\}, "alpha\_2": \{"median": 4.43, "5th percentile": 3.16, "95th percentile": 5.94, "error plus": 1.51, "error minus": 1.28\}, "beta": \{"median": 1.25, "5th percentile": 0.16, "95th percentile": 2.6, "error plus": 1.35, "error minus": 1.09\}, "mlow\_1": \{"median": 5.03, "5th percentile": 3.23, "95th percentile": 7.87, "error plus": 2.84, "error minus": 1.8\}, "mlow\_2": \{"median": 3.58, "5th percentile": 3.03, "95th percentile": 4.96, "error plus": 1.38, "error minus": 0.55\}, "break\_mass": \{"median": 35.57, "5th percentile": 22.2, "95th percentile": 48.19, "error plus": 12.62, "error minus": 13.37\}, "mpp\_1": \{"median": 9.72, "5th percentile": 8.62, "95th percentile": 10.2, "error plus": 0.48, "error minus": 1.1\}, "mpp\_2": \{"median": 33.02, "5th percentile": 27.33, "95th percentile": 35.59, "error plus": 2.57, "error minus": 5.69\}, "sigpp\_1": \{"median": 0.64, "5th percentile": 0.3, "95th percentile": 1.5, "error plus": 0.86, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.58, "5th percentile": 1.2, "95th percentile": 8.78, "error plus": 5.2, "error minus": 2.39\}, "delta\_m\_1": \{"median": 4.67, "5th percentile": 0.42, "95th percentile": 9.32, "error plus": 4.65, "error minus": 4.25\}, "delta\_m\_2": \{"median": 5.24, "5th percentile": 0.54, "95th percentile": 9.13, "error plus": 3.89, "error minus": 4.7\}, "lam\_0": \{"median": 0.38, "5th percentile": 0.15, "95th percentile": 0.67, "error plus": 0.29, "error minus": 0.22\}, "lam\_1": \{"median": 0.57, "5th percentile": 0.29, "95th percentile": 0.8, "error plus": 0.23, "error minus": 0.28\}, "lamb": \{"median": 3.12, "5th percentile": 2.18, "95th percentile": 4.07, "error plus": 0.95, "error minus": 0.94\}, "mu\_chi": \{"median": 0.09, "5th percentile": 0.01, "95th percentile": 0.24, "error plus": 0.14, "error minus": 0.09\}, "sigma\_chi": \{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.41, "error plus": 0.08, "error minus": 0.08\}, "xi\_spin": \{"median": 0.62, "5th percentile": 0.11, "95th percentile": 0.96, "error plus": 0.34, "error minus": 0.5\}, "mu\_1": \{"median": 0.32, "5th percentile": {-}0.76, "95th percentile": 0.92, "error plus": 0.6, "error minus": 1.09\}, "sigma\_1": \{"median": 1.76, "5th percentile": 0.44, "95th percentile": 3.74, "error plus": 1.99, "error minus": 1.32\}, "mu\_2": \{"median": 0.37, "5th percentile": {-}0.71, "95th percentile": 0.93, "error plus": 0.56, "error minus": 1.08\}, "sigma\_2": \{"median": 1.58, "5th percentile": 0.34, "95th percentile": 3.71, "error plus": 2.13, "error minus": 1.24\}, "rate": \{"median": 16.4, "5th percentile": 12.06, "95th percentile": 22.24, "error plus": 5.84, "error minus": 4.34\}, "log\_likelihood": \{"median": {-}1024.07, "5th percentile": {-}1029.91, "95th percentile": {-}1019.48, "error plus": 4.59, "error minus": 5.84\}, "variance": \{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.11, "error minus": 0.23\}, "min\_neff": \{"median": 56.43, "5th percentile": 31.56, "95th percentile": 95.56, "error plus": 39.13, "error minus": 24.87\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.71, "peak": 0.12\}, "cos\_tilt\_1": \{"median": 0.07, "5th percentile": {-}0.88, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.34\}, "cos\_tilt\_2": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.4\}, "mass\_1": \{"median": 10.08, "5th percentile": 7.92, "90th percentile": 27.67, "95th percentile": 34.34, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@out{{-}1047.54}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@out{0.24}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@out{{-}0.39}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@out{1.12}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@out\MagTruncnormIidTiltIsotropicTruncnormNnd@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@out\MagTruncnormIidTiltIsotropicTruncnormNnd@II\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@out{??}\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out{\{"alpha\_1": \{"median": 1.83, "5th percentile": {-}0.02, "95th percentile": 3.02, "error plus": 1.19, "error minus": 1.85\}, "alpha\_2": \{"median": 4.43, "5th percentile": 3.16, "95th percentile": 5.94, "error plus": 1.51, "error minus": 1.28\}, "beta": \{"median": 1.25, "5th percentile": 0.16, "95th percentile": 2.6, "error plus": 1.35, "error minus": 1.09\}, "mlow\_1": \{"median": 5.03, "5th percentile": 3.23, "95th percentile": 7.87, "error plus": 2.84, "error minus": 1.8\}, "mlow\_2": \{"median": 3.58, "5th percentile": 3.03, "95th percentile": 4.96, "error plus": 1.38, "error minus": 0.55\}, "break\_mass": \{"median": 35.57, "5th percentile": 22.2, "95th percentile": 48.19, "error plus": 12.62, "error minus": 13.37\}, "mpp\_1": \{"median": 9.72, "5th percentile": 8.62, "95th percentile": 10.2, "error plus": 0.48, "error minus": 1.1\}, "mpp\_2": \{"median": 33.02, "5th percentile": 27.33, "95th percentile": 35.59, "error plus": 2.57, "error minus": 5.69\}, "sigpp\_1": \{"median": 0.64, "5th percentile": 0.3, "95th percentile": 1.5, "error plus": 0.86, "error minus": 0.35\}, "sigpp\_2": \{"median": 3.58, "5th percentile": 1.2, "95th percentile": 8.78, "error plus": 5.2, "error minus": 2.39\}, "delta\_m\_1": \{"median": 4.67, "5th percentile": 0.42, "95th percentile": 9.32, "error plus": 4.65, "error minus": 4.25\}, "delta\_m\_2": \{"median": 5.24, "5th percentile": 0.54, "95th percentile": 9.13, "error plus": 3.89, "error minus": 4.7\}, "lam\_0": \{"median": 0.38, "5th percentile": 0.15, "95th percentile": 0.67, "error plus": 0.29, "error minus": 0.22\}, "lam\_1": \{"median": 0.57, "5th percentile": 0.29, "95th percentile": 0.8, "error plus": 0.23, "error minus": 0.28\}, "lamb": \{"median": 3.12, "5th percentile": 2.18, "95th percentile": 4.07, "error plus": 0.95, "error minus": 0.94\}, "mu\_chi": \{"median": 0.09, "5th percentile": 0.01, "95th percentile": 0.24, "error plus": 0.14, "error minus": 0.09\}, "sigma\_chi": \{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.41, "error plus": 0.08, "error minus": 0.08\}, "xi\_spin": \{"median": 0.62, "5th percentile": 0.11, "95th percentile": 0.96, "error plus": 0.34, "error minus": 0.5\}, "mu\_1": \{"median": 0.32, "5th percentile": {-}0.76, "95th percentile": 0.92, "error plus": 0.6, "error minus": 1.09\}, "sigma\_1": \{"median": 1.76, "5th percentile": 0.44, "95th percentile": 3.74, "error plus": 1.99, "error minus": 1.32\}, "mu\_2": \{"median": 0.37, "5th percentile": {-}0.71, "95th percentile": 0.93, "error plus": 0.56, "error minus": 1.08\}, "sigma\_2": \{"median": 1.58, "5th percentile": 0.34, "95th percentile": 3.71, "error plus": 2.13, "error minus": 1.24\}, "rate": \{"median": 16.4, "5th percentile": 12.06, "95th percentile": 22.24, "error plus": 5.84, "error minus": 4.34\}, "log\_likelihood": \{"median": {-}1024.07, "5th percentile": {-}1029.91, "95th percentile": {-}1019.48, "error plus": 4.59, "error minus": 5.84\}, "variance": \{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.11, "error minus": 0.23\}, "min\_neff": \{"median": 56.43, "5th percentile": 31.56, "95th percentile": 95.56, "error plus": 39.13, "error minus": 24.87\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XX\else\ifnum\pdfstrcmp{#1}{mu_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI\else\ifnum\pdfstrcmp{#1}{sigma_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII\else\ifnum\pdfstrcmp{#1}{mu_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII\else\ifnum\pdfstrcmp{#1}{sigma_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@I@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out{\{"a": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.71, "peak": 0.12\}, "cos\_tilt\_1": \{"median": 0.07, "5th percentile": {-}0.88, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.34\}, "cos\_tilt\_2": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.4\}, "mass\_1": \{"median": 10.08, "5th percentile": 7.92, "90th percentile": 27.67, "95th percentile": 34.34, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out{??}\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@II@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out{\{"median": 1.83, "5th percentile": {-}0.02, "95th percentile": 3.02, "error plus": 1.19, "error minus": 1.85\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out{1.83}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out{{-}0.02}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out{3.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out{1.19}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out{1.85}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@III@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out{\{"median": 4.43, "5th percentile": 3.16, "95th percentile": 5.94, "error plus": 1.51, "error minus": 1.28\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out{4.43}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out{3.16}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out{5.94}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out{1.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out{1.28}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@IV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out{\{"median": 1.25, "5th percentile": 0.16, "95th percentile": 2.6, "error plus": 1.35, "error minus": 1.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out{1.25}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out{0.16}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out{2.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out{1.35}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out{1.09}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@V@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out{\{"median": 5.03, "5th percentile": 3.23, "95th percentile": 7.87, "error plus": 2.84, "error minus": 1.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out{5.03}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out{3.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out{7.87}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out{2.84}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out{1.8}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@VI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out{\{"median": 3.58, "5th percentile": 3.03, "95th percentile": 4.96, "error plus": 1.38, "error minus": 0.55\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out{3.58}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out{4.96}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out{1.38}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out{0.55}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@VII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out{\{"median": 35.57, "5th percentile": 22.2, "95th percentile": 48.19, "error plus": 12.62, "error minus": 13.37\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out{35.57}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out{22.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out{48.19}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out{12.62}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out{13.37}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@VIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out{\{"median": 9.72, "5th percentile": 8.62, "95th percentile": 10.2, "error plus": 0.48, "error minus": 1.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out{9.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out{8.62}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out{10.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out{0.48}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out{1.1}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@IX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out{\{"median": 33.02, "5th percentile": 27.33, "95th percentile": 35.59, "error plus": 2.57, "error minus": 5.69\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out{33.02}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out{27.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out{35.59}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out{2.57}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out{5.69}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@X@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out{\{"median": 0.64, "5th percentile": 0.3, "95th percentile": 1.5, "error plus": 0.86, "error minus": 0.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out{0.64}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out{0.86}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out{0.35}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out{\{"median": 3.58, "5th percentile": 1.2, "95th percentile": 8.78, "error plus": 5.2, "error minus": 2.39\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out{3.58}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out{8.78}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out{5.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out{2.39}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out{\{"median": 4.67, "5th percentile": 0.42, "95th percentile": 9.32, "error plus": 4.65, "error minus": 4.25\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out{4.67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out{0.42}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out{9.32}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out{4.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out{4.25}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out{\{"median": 5.24, "5th percentile": 0.54, "95th percentile": 9.13, "error plus": 3.89, "error minus": 4.7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out{5.24}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out{0.54}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out{9.13}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out{3.89}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out{4.7}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XIV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out{\{"median": 0.38, "5th percentile": 0.15, "95th percentile": 0.67, "error plus": 0.29, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out{0.38}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out{0.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out{0.67}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out{0.29}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out{0.22}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out{\{"median": 0.57, "5th percentile": 0.29, "95th percentile": 0.8, "error plus": 0.23, "error minus": 0.28\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out{0.57}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out{0.29}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out{0.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out{0.23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out{0.28}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XVI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out{\{"median": 3.12, "5th percentile": 2.18, "95th percentile": 4.07, "error plus": 0.95, "error minus": 0.94\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out{3.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out{2.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out{4.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out{0.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out{0.94}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XVII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out{\{"median": 0.09, "5th percentile": 0.01, "95th percentile": 0.24, "error plus": 0.14, "error minus": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out{0.09}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out{0.24}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out{0.09}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XVIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out{\{"median": 0.33, "5th percentile": 0.25, "95th percentile": 0.41, "error plus": 0.08, "error minus": 0.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out{0.41}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out{0.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out{0.08}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XIX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out{\{"median": 0.62, "5th percentile": 0.11, "95th percentile": 0.96, "error plus": 0.34, "error minus": 0.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out{0.62}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out{0.11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out{0.96}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out{0.34}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out{0.5}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out{\{"median": 0.32, "5th percentile": {-}0.76, "95th percentile": 0.92, "error plus": 0.6, "error minus": 1.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out{0.32}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out{{-}0.76}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out{0.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out{0.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out{1.09}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out{\{"median": 1.76, "5th percentile": 0.44, "95th percentile": 3.74, "error plus": 1.99, "error minus": 1.32\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out{1.76}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out{3.74}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out{1.99}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out{1.32}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out{\{"median": 0.37, "5th percentile": {-}0.71, "95th percentile": 0.93, "error plus": 0.56, "error minus": 1.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out{{-}0.71}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out{0.93}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out{0.56}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out{1.08}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out{\{"median": 1.58, "5th percentile": 0.34, "95th percentile": 3.71, "error plus": 2.13, "error minus": 1.24\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out{1.58}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out{0.34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out{3.71}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out{2.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out{1.24}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out{\{"median": 16.4, "5th percentile": 12.06, "95th percentile": 22.24, "error plus": 5.84, "error minus": 4.34\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out{16.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out{12.06}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out{22.24}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out{5.84}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out{4.34}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out{\{"median": {-}1024.07, "5th percentile": {-}1029.91, "95th percentile": {-}1019.48, "error plus": 4.59, "error minus": 5.84\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out{{-}1024.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out{{-}1029.91}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out{{-}1019.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out{4.59}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out{5.84}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out{\{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.11, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out{0.64}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out{0.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out{0.23}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out{\{"median": 56.43, "5th percentile": 31.56, "95th percentile": 95.56, "error plus": 39.13, "error minus": 24.87\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out{56.43}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out{31.56}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out{95.56}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out{39.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out{24.87}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXVIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out{0.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXIX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out{\{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.71, "peak": 0.12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out{0.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out{0.71}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out{0.12}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXX@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out{\{"median": 0.07, "5th percentile": {-}0.88, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.34\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out{0.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out{{-}0.88}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out{0.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out{0.34}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out{\{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.4\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out{{-}0.87}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out{0.81}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out{0.4}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out{\{"median": 10.08, "5th percentile": 7.92, "90th percentile": 27.67, "95th percentile": 34.34, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out{10.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out{7.92}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out{27.67}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out{34.34}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out{9.91}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out{\{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out{0.51}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out{1.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXIV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out{0.47}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out{2.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormNnd@XXXV@out}\makeatother
\makeatletter\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@out{\{"param": \{"chi\_A\_1st": \{"median": 0.05, "error plus": 0.02, "error minus": 0.01, "5th percentile": 0.04, "95th percentile": 0.07\}, "chi\_A\_99th": \{"median": 0.92, "error plus": 0.04, "error minus": 0.08, "5th percentile": 0.85, "95th percentile": 0.97\}, "chi\_B\_1st": \{"median": 0.0, "error plus": 0.0, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.0\}, "chi\_B\_99th": \{"median": 0.6, "error plus": 0.09, "error minus": 0.07, "5th percentile": 0.53, "95th percentile": 0.69\}\}, "ppd": \{"chi\_A": \{"median": 0.4, "5th percentile": 0.12, "95th percentile": 0.79, "spin at peak": 0.35\}, "chi\_B": \{"median": 0.15, "5th percentile": 0.01, "95th percentile": 0.46, "spin at peak": 0.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@II\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@out{??}\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I@out{\{"chi\_A\_1st": \{"median": 0.05, "error plus": 0.02, "error minus": 0.01, "5th percentile": 0.04, "95th percentile": 0.07\}, "chi\_A\_99th": \{"median": 0.92, "error plus": 0.04, "error minus": 0.08, "5th percentile": 0.85, "95th percentile": 0.97\}, "chi\_B\_1st": \{"median": 0.0, "error plus": 0.0, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.0\}, "chi\_B\_99th": \{"median": 0.6, "error plus": 0.09, "error minus": 0.07, "5th percentile": 0.53, "95th percentile": 0.69\}\}}\else\ifnum\pdfstrcmp{#1}{chi_A_1st}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III\else\ifnum\pdfstrcmp{#1}{chi_A_99th}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV\else\ifnum\pdfstrcmp{#1}{chi_B_1st}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V\else\ifnum\pdfstrcmp{#1}{chi_B_99th}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I@out{??}\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@I@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@II@out{\{"chi\_A": \{"median": 0.4, "5th percentile": 0.12, "95th percentile": 0.79, "spin at peak": 0.35\}, "chi\_B": \{"median": 0.15, "5th percentile": 0.01, "95th percentile": 0.46, "spin at peak": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{chi_A}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@II@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII\else\ifnum\pdfstrcmp{#1}{chi_B}=0\let\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@II@out\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@II@out{??}\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@II@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out{\{"median": 0.05, "error plus": 0.02, "error minus": 0.01, "5th percentile": 0.04, "95th percentile": 0.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out{0.05}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out{0.01}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out{0.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out{0.07}\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@III@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out{\{"median": 0.92, "error plus": 0.04, "error minus": 0.08, "5th percentile": 0.85, "95th percentile": 0.97\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out{0.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out{0.04}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out{0.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out{0.85}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out{0.97}\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@IV@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out{\{"median": 0.0, "error plus": 0.0, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out{0.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@V@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out{\{"median": 0.6, "error plus": 0.09, "error minus": 0.07, "5th percentile": 0.53, "95th percentile": 0.69\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out{0.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out{0.09}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out{0.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out{0.53}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out{0.69}\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VI@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII@out{\{"median": 0.4, "5th percentile": 0.12, "95th percentile": 0.79, "spin at peak": 0.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII@out{0.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII@out{0.79}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII@out{0.35}\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII@out{??}\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VII@out}\newcommand\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII@out{\{"median": 0.15, "5th percentile": 0.01, "95th percentile": 0.46, "spin at peak": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.46}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII@out{0.0}\else\def\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII@out{??}\fi\fi\fi\fi\fi\MagTruncnormIidTiltIsotropicTruncnormSpinSorting@VIII@out}\makeatother
\makeatletter\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@out{\{"ln\_evidence": {-}1049.67, "ln\_evidence\_error": 0.25, "ln\_bayes\_factor\_over\_new\_default": {-}2.52, "ln\_bayes\_factor\_over\_old\_default": {-}1.0, "param": \{"alpha\_1": \{"median": 1.81, "5th percentile": {-}0.14, "95th percentile": 3.0, "error plus": 1.18, "error minus": 1.95\}, "alpha\_2": \{"median": 4.5, "5th percentile": 3.18, "95th percentile": 6.01, "error plus": 1.51, "error minus": 1.32\}, "beta": \{"median": 1.28, "5th percentile": 0.2, "95th percentile": 2.74, "error plus": 1.46, "error minus": 1.08\}, "mlow\_1": \{"median": 5.11, "5th percentile": 3.25, "95th percentile": 8.0, "error plus": 2.89, "error minus": 1.85\}, "mlow\_2": \{"median": 3.56, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.3, "error minus": 0.53\}, "break\_mass": \{"median": 35.7, "5th percentile": 22.11, "95th percentile": 48.05, "error plus": 12.35, "error minus": 13.59\}, "mpp\_1": \{"median": 9.71, "5th percentile": 8.48, "95th percentile": 10.2, "error plus": 0.48, "error minus": 1.23\}, "mpp\_2": \{"median": 32.94, "5th percentile": 26.95, "95th percentile": 35.73, "error plus": 2.79, "error minus": 5.99\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.3, "95th percentile": 1.49, "error plus": 0.83, "error minus": 0.36\}, "sigpp\_2": \{"median": 3.76, "5th percentile": 1.21, "95th percentile": 9.0, "error plus": 5.24, "error minus": 2.55\}, "delta\_m\_1": \{"median": 4.49, "5th percentile": 0.41, "95th percentile": 9.23, "error plus": 4.74, "error minus": 4.08\}, "delta\_m\_2": \{"median": 5.03, "5th percentile": 0.5, "95th percentile": 9.08, "error plus": 4.05, "error minus": 4.54\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.13, "95th percentile": 0.64, "error plus": 0.28, "error minus": 0.23\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.24, "error minus": 0.27\}, "lamb": \{"median": 3.11, "5th percentile": 2.21, "95th percentile": 4.02, "error plus": 0.91, "error minus": 0.9\}, "mu\_chi\_1": \{"median": 0.11, "5th percentile": 0.01, "95th percentile": 0.27, "error plus": 0.16, "error minus": 0.1\}, "sigma\_chi\_1": \{"median": 0.33, "5th percentile": 0.22, "95th percentile": 0.45, "error plus": 0.13, "error minus": 0.11\}, "mu\_chi\_2": \{"median": 0.13, "5th percentile": 0.01, "95th percentile": 0.31, "error plus": 0.17, "error minus": 0.12\}, "sigma\_chi\_2": \{"median": 0.32, "5th percentile": 0.19, "95th percentile": 0.54, "error plus": 0.22, "error minus": 0.13\}, "xi\_spin": \{"median": 0.64, "5th percentile": 0.1, "95th percentile": 0.97, "error plus": 0.32, "error minus": 0.54\}, "mu\_spin": \{"median": 0.37, "5th percentile": {-}0.46, "95th percentile": 0.93, "error plus": 0.56, "error minus": 0.82\}, "sigma\_spin": \{"median": 1.3, "5th percentile": 0.44, "95th percentile": 3.63, "error plus": 2.34, "error minus": 0.86\}, "rate": \{"median": 16.54, "5th percentile": 12.06, "95th percentile": 22.25, "error plus": 5.71, "error minus": 4.48\}, "log\_likelihood": \{"median": {-}1024.99, "5th percentile": {-}1031.16, "95th percentile": {-}1020.14, "error plus": 4.85, "error minus": 6.17\}, "variance": \{"median": 0.86, "5th percentile": 0.63, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}, "min\_neff": \{"median": 53.6, "5th percentile": 29.47, "95th percentile": 92.17, "error plus": 38.57, "error minus": 24.14\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a\_1": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.72, "peak": 0.13\}, "a\_2": \{"median": 0.28, "5th percentile": 0.03, "90th percentile": 0.63, "95th percentile": 0.75, "peak": 0.16\}, "cos\_tilt": \{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.27\}, "mass\_1": \{"median": 10.09, "5th percentile": 7.95, "90th percentile": 27.63, "95th percentile": 34.34, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@out{{-}1049.67}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@out{0.25}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@out{{-}2.52}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@out{{-}1.0}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@out\MagTruncnormIndTiltIsotropicTruncnormNid@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@out\MagTruncnormIndTiltIsotropicTruncnormNid@II\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@out{??}\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@I@out{\{"alpha\_1": \{"median": 1.81, "5th percentile": {-}0.14, "95th percentile": 3.0, "error plus": 1.18, "error minus": 1.95\}, "alpha\_2": \{"median": 4.5, "5th percentile": 3.18, "95th percentile": 6.01, "error plus": 1.51, "error minus": 1.32\}, "beta": \{"median": 1.28, "5th percentile": 0.2, "95th percentile": 2.74, "error plus": 1.46, "error minus": 1.08\}, "mlow\_1": \{"median": 5.11, "5th percentile": 3.25, "95th percentile": 8.0, "error plus": 2.89, "error minus": 1.85\}, "mlow\_2": \{"median": 3.56, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.3, "error minus": 0.53\}, "break\_mass": \{"median": 35.7, "5th percentile": 22.11, "95th percentile": 48.05, "error plus": 12.35, "error minus": 13.59\}, "mpp\_1": \{"median": 9.71, "5th percentile": 8.48, "95th percentile": 10.2, "error plus": 0.48, "error minus": 1.23\}, "mpp\_2": \{"median": 32.94, "5th percentile": 26.95, "95th percentile": 35.73, "error plus": 2.79, "error minus": 5.99\}, "sigpp\_1": \{"median": 0.67, "5th percentile": 0.3, "95th percentile": 1.49, "error plus": 0.83, "error minus": 0.36\}, "sigpp\_2": \{"median": 3.76, "5th percentile": 1.21, "95th percentile": 9.0, "error plus": 5.24, "error minus": 2.55\}, "delta\_m\_1": \{"median": 4.49, "5th percentile": 0.41, "95th percentile": 9.23, "error plus": 4.74, "error minus": 4.08\}, "delta\_m\_2": \{"median": 5.03, "5th percentile": 0.5, "95th percentile": 9.08, "error plus": 4.05, "error minus": 4.54\}, "lam\_0": \{"median": 0.36, "5th percentile": 0.13, "95th percentile": 0.64, "error plus": 0.28, "error minus": 0.23\}, "lam\_1": \{"median": 0.59, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.24, "error minus": 0.27\}, "lamb": \{"median": 3.11, "5th percentile": 2.21, "95th percentile": 4.02, "error plus": 0.91, "error minus": 0.9\}, "mu\_chi\_1": \{"median": 0.11, "5th percentile": 0.01, "95th percentile": 0.27, "error plus": 0.16, "error minus": 0.1\}, "sigma\_chi\_1": \{"median": 0.33, "5th percentile": 0.22, "95th percentile": 0.45, "error plus": 0.13, "error minus": 0.11\}, "mu\_chi\_2": \{"median": 0.13, "5th percentile": 0.01, "95th percentile": 0.31, "error plus": 0.17, "error minus": 0.12\}, "sigma\_chi\_2": \{"median": 0.32, "5th percentile": 0.19, "95th percentile": 0.54, "error plus": 0.22, "error minus": 0.13\}, "xi\_spin": \{"median": 0.64, "5th percentile": 0.1, "95th percentile": 0.97, "error plus": 0.32, "error minus": 0.54\}, "mu\_spin": \{"median": 0.37, "5th percentile": {-}0.46, "95th percentile": 0.93, "error plus": 0.56, "error minus": 0.82\}, "sigma\_spin": \{"median": 1.3, "5th percentile": 0.44, "95th percentile": 3.63, "error plus": 2.34, "error minus": 0.86\}, "rate": \{"median": 16.54, "5th percentile": 12.06, "95th percentile": 22.25, "error plus": 5.71, "error minus": 4.48\}, "log\_likelihood": \{"median": {-}1024.99, "5th percentile": {-}1031.16, "95th percentile": {-}1020.14, "error plus": 4.85, "error minus": 6.17\}, "variance": \{"median": 0.86, "5th percentile": 0.63, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}, "min\_neff": \{"median": 53.6, "5th percentile": 29.47, "95th percentile": 92.17, "error plus": 38.57, "error minus": 24.14\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XIX\else\ifnum\pdfstrcmp{#1}{mu_chi_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XX\else\ifnum\pdfstrcmp{#1}{sigma_chi_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXI\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXII\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXV\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@I@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@I@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@II@out{\{"a\_1": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.72, "peak": 0.13\}, "a\_2": \{"median": 0.28, "5th percentile": 0.03, "90th percentile": 0.63, "95th percentile": 0.75, "peak": 0.16\}, "cos\_tilt": \{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.27\}, "mass\_1": \{"median": 10.09, "5th percentile": 7.95, "90th percentile": 27.63, "95th percentile": 34.34, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@II@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXX\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@II@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI\else\ifnum\pdfstrcmp{#1}{cos_tilt}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@II@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@II@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@II@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagTruncnormIndTiltIsotropicTruncnormNid@II@out\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@II@out{??}\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@II@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@III@out{\{"median": 1.81, "5th percentile": {-}0.14, "95th percentile": 3.0, "error plus": 1.18, "error minus": 1.95\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@III@out{1.81}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@III@out{{-}0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@III@out{3.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@III@out{1.18}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@III@out{1.95}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@III@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@III@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out{\{"median": 4.5, "5th percentile": 3.18, "95th percentile": 6.01, "error plus": 1.51, "error minus": 1.32\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out{4.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out{3.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out{6.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out{1.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out{1.32}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@IV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@V@out{\{"median": 1.28, "5th percentile": 0.2, "95th percentile": 2.74, "error plus": 1.46, "error minus": 1.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@V@out{1.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@V@out{0.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@V@out{2.74}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@V@out{1.46}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@V@out{1.08}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@V@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@V@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out{\{"median": 5.11, "5th percentile": 3.25, "95th percentile": 8.0, "error plus": 2.89, "error minus": 1.85\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out{5.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out{3.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out{8.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out{2.89}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out{1.85}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@VI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out{\{"median": 3.56, "5th percentile": 3.03, "95th percentile": 4.87, "error plus": 1.3, "error minus": 0.53\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out{3.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out{4.87}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out{1.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out{0.53}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@VII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out{\{"median": 35.7, "5th percentile": 22.11, "95th percentile": 48.05, "error plus": 12.35, "error minus": 13.59\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out{35.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out{22.11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out{48.05}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out{12.35}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out{13.59}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@VIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out{\{"median": 9.71, "5th percentile": 8.48, "95th percentile": 10.2, "error plus": 0.48, "error minus": 1.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out{9.71}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out{8.48}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out{10.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out{0.48}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out{1.23}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@IX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@X@out{\{"median": 32.94, "5th percentile": 26.95, "95th percentile": 35.73, "error plus": 2.79, "error minus": 5.99\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@X@out{32.94}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@X@out{26.95}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@X@out{35.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@X@out{2.79}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@X@out{5.99}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@X@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@X@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out{\{"median": 0.67, "5th percentile": 0.3, "95th percentile": 1.49, "error plus": 0.83, "error minus": 0.36\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out{0.67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out{1.49}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out{0.83}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out{0.36}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out{\{"median": 3.76, "5th percentile": 1.21, "95th percentile": 9.0, "error plus": 5.24, "error minus": 2.55\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out{3.76}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out{1.21}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out{9.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out{5.24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out{2.55}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out{\{"median": 4.49, "5th percentile": 0.41, "95th percentile": 9.23, "error plus": 4.74, "error minus": 4.08\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out{4.49}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out{0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out{9.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out{4.74}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out{4.08}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out{\{"median": 5.03, "5th percentile": 0.5, "95th percentile": 9.08, "error plus": 4.05, "error minus": 4.54\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out{5.03}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out{0.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out{9.08}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out{4.05}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out{4.54}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XIV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out{\{"median": 0.36, "5th percentile": 0.13, "95th percentile": 0.64, "error plus": 0.28, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out{0.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out{0.23}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out{\{"median": 0.59, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.24, "error minus": 0.27\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out{0.59}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out{0.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out{0.24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out{0.27}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XVI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out{\{"median": 3.11, "5th percentile": 2.21, "95th percentile": 4.02, "error plus": 0.91, "error minus": 0.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out{3.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out{2.21}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out{4.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out{0.91}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out{0.9}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XVII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out{\{"median": 0.11, "5th percentile": 0.01, "95th percentile": 0.27, "error plus": 0.16, "error minus": 0.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out{0.27}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out{0.16}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out{0.1}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XVIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out{\{"median": 0.33, "5th percentile": 0.22, "95th percentile": 0.45, "error plus": 0.13, "error minus": 0.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out{0.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out{0.45}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out{0.11}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XIX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out{\{"median": 0.13, "5th percentile": 0.01, "95th percentile": 0.31, "error plus": 0.17, "error minus": 0.12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out{0.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out{0.17}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out{0.12}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out{\{"median": 0.32, "5th percentile": 0.19, "95th percentile": 0.54, "error plus": 0.22, "error minus": 0.13\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out{0.32}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out{0.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out{0.54}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out{0.13}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out{\{"median": 0.64, "5th percentile": 0.1, "95th percentile": 0.97, "error plus": 0.32, "error minus": 0.54\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out{0.64}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out{0.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out{0.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out{0.32}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out{0.54}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out{\{"median": 0.37, "5th percentile": {-}0.46, "95th percentile": 0.93, "error plus": 0.56, "error minus": 0.82\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out{{-}0.46}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out{0.93}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out{0.56}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out{0.82}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out{\{"median": 1.3, "5th percentile": 0.44, "95th percentile": 3.63, "error plus": 2.34, "error minus": 0.86\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out{3.63}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out{2.34}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out{0.86}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXIV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out{\{"median": 16.54, "5th percentile": 12.06, "95th percentile": 22.25, "error plus": 5.71, "error minus": 4.48\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out{16.54}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out{12.06}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out{22.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out{5.71}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out{4.48}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out{\{"median": {-}1024.99, "5th percentile": {-}1031.16, "95th percentile": {-}1020.14, "error plus": 4.85, "error minus": 6.17\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out{{-}1024.99}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out{{-}1031.16}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out{{-}1020.14}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out{4.85}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out{6.17}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXVI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out{\{"median": 0.86, "5th percentile": 0.63, "95th percentile": 0.99, "error plus": 0.12, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out{0.86}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out{0.63}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out{0.23}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXVII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out{\{"median": 53.6, "5th percentile": 29.47, "95th percentile": 92.17, "error plus": 38.57, "error minus": 24.14\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out{53.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out{29.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out{92.17}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out{38.57}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out{24.14}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXVIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out{0.0}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXIX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out{\{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.72, "peak": 0.13\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out{0.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out{0.72}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out{0.13}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out{\{"median": 0.28, "5th percentile": 0.03, "90th percentile": 0.63, "95th percentile": 0.75, "peak": 0.16\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out{0.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out{0.63}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out{0.75}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out{0.16}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXXI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out{\{"median": 0.08, "5th percentile": {-}0.87, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.27\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out{0.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out{{-}0.87}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out{0.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out{0.27}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXXII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out{\{"median": 10.09, "5th percentile": 7.95, "90th percentile": 27.63, "95th percentile": 34.34, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out{10.09}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out{7.95}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out{27.63}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out{34.34}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out{9.91}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out{\{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out{0.51}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out{1.0}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXXIV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out{0.47}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out{2.0}\else\def\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNid@XXXV@out}\makeatother
\makeatletter\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@out{\{"ln\_evidence": {-}1049.24, "ln\_evidence\_error": 0.24, "ln\_bayes\_factor\_over\_new\_default": {-}2.09, "ln\_bayes\_factor\_over\_old\_default": {-}0.58, "param": \{"alpha\_1": \{"median": 1.82, "5th percentile": {-}0.01, "95th percentile": 2.95, "error plus": 1.13, "error minus": 1.83\}, "alpha\_2": \{"median": 4.46, "5th percentile": 3.25, "95th percentile": 6.01, "error plus": 1.55, "error minus": 1.22\}, "beta": \{"median": 1.29, "5th percentile": 0.26, "95th percentile": 2.7, "error plus": 1.41, "error minus": 1.03\}, "mlow\_1": \{"median": 5.06, "5th percentile": 3.25, "95th percentile": 8.16, "error plus": 3.1, "error minus": 1.81\}, "mlow\_2": \{"median": 3.55, "5th percentile": 3.03, "95th percentile": 4.89, "error plus": 1.34, "error minus": 0.51\}, "break\_mass": \{"median": 35.69, "5th percentile": 22.14, "95th percentile": 48.38, "error plus": 12.69, "error minus": 13.55\}, "mpp\_1": \{"median": 9.72, "5th percentile": 8.5, "95th percentile": 10.22, "error plus": 0.49, "error minus": 1.22\}, "mpp\_2": \{"median": 33.08, "5th percentile": 27.28, "95th percentile": 35.71, "error plus": 2.63, "error minus": 5.8\}, "sigpp\_1": \{"median": 0.65, "5th percentile": 0.31, "95th percentile": 1.5, "error plus": 0.85, "error minus": 0.34\}, "sigpp\_2": \{"median": 3.65, "5th percentile": 1.23, "95th percentile": 8.97, "error plus": 5.31, "error minus": 2.43\}, "delta\_m\_1": \{"median": 4.39, "5th percentile": 0.36, "95th percentile": 9.16, "error plus": 4.77, "error minus": 4.03\}, "delta\_m\_2": \{"median": 5.14, "5th percentile": 0.47, "95th percentile": 9.13, "error plus": 4.0, "error minus": 4.66\}, "lam\_0": \{"median": 0.37, "5th percentile": 0.15, "95th percentile": 0.65, "error plus": 0.27, "error minus": 0.22\}, "lam\_1": \{"median": 0.58, "5th percentile": 0.31, "95th percentile": 0.8, "error plus": 0.22, "error minus": 0.27\}, "lamb": \{"median": 3.12, "5th percentile": 2.21, "95th percentile": 4.02, "error plus": 0.91, "error minus": 0.91\}, "mu\_chi\_1": \{"median": 0.1, "5th percentile": 0.01, "95th percentile": 0.26, "error plus": 0.15, "error minus": 0.09\}, "sigma\_chi\_1": \{"median": 0.33, "5th percentile": 0.22, "95th percentile": 0.45, "error plus": 0.12, "error minus": 0.11\}, "mu\_chi\_2": \{"median": 0.13, "5th percentile": 0.01, "95th percentile": 0.3, "error plus": 0.17, "error minus": 0.11\}, "sigma\_chi\_2": \{"median": 0.33, "5th percentile": 0.19, "95th percentile": 0.55, "error plus": 0.22, "error minus": 0.13\}, "xi\_spin": \{"median": 0.6, "5th percentile": 0.11, "95th percentile": 0.96, "error plus": 0.36, "error minus": 0.49\}, "mu\_1": \{"median": 0.29, "5th percentile": {-}0.75, "95th percentile": 0.92, "error plus": 0.63, "error minus": 1.04\}, "sigma\_1": \{"median": 1.73, "5th percentile": 0.39, "95th percentile": 3.75, "error plus": 2.03, "error minus": 1.33\}, "mu\_2": \{"median": 0.33, "5th percentile": {-}0.77, "95th percentile": 0.92, "error plus": 0.59, "error minus": 1.09\}, "sigma\_2": \{"median": 1.44, "5th percentile": 0.33, "95th percentile": 3.69, "error plus": 2.25, "error minus": 1.11\}, "rate": \{"median": 16.36, "5th percentile": 11.94, "95th percentile": 22.29, "error plus": 5.92, "error minus": 4.42\}, "log\_likelihood": \{"median": {-}1024.69, "5th percentile": {-}1030.93, "95th percentile": {-}1019.99, "error plus": 4.7, "error minus": 6.23\}, "variance": \{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.11, "error minus": 0.23\}, "min\_neff": \{"median": 53.1, "5th percentile": 29.3, "95th percentile": 89.97, "error plus": 36.87, "error minus": 23.8\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}, "ppd": \{"a\_1": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.72, "peak": 0.13\}, "a\_2": \{"median": 0.28, "5th percentile": 0.03, "90th percentile": 0.64, "95th percentile": 0.75, "peak": 0.16\}, "cos\_tilt\_1": \{"median": 0.06, "5th percentile": {-}0.88, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.3\}, "cos\_tilt\_2": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.37\}, "mass\_1": \{"median": 10.09, "5th percentile": 7.96, "90th percentile": 27.75, "95th percentile": 34.39, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{ln_evidence}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@out{{-}1049.24}\else\ifnum\pdfstrcmp{#1}{ln_evidence_error}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@out{0.24}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_new_default}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@out{{-}2.09}\else\ifnum\pdfstrcmp{#1}{ln_bayes_factor_over_old_default}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@out{{-}0.58}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@out\MagTruncnormIndTiltIsotropicTruncnormNnd@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@out\MagTruncnormIndTiltIsotropicTruncnormNnd@II\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@out{??}\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out{\{"alpha\_1": \{"median": 1.82, "5th percentile": {-}0.01, "95th percentile": 2.95, "error plus": 1.13, "error minus": 1.83\}, "alpha\_2": \{"median": 4.46, "5th percentile": 3.25, "95th percentile": 6.01, "error plus": 1.55, "error minus": 1.22\}, "beta": \{"median": 1.29, "5th percentile": 0.26, "95th percentile": 2.7, "error plus": 1.41, "error minus": 1.03\}, "mlow\_1": \{"median": 5.06, "5th percentile": 3.25, "95th percentile": 8.16, "error plus": 3.1, "error minus": 1.81\}, "mlow\_2": \{"median": 3.55, "5th percentile": 3.03, "95th percentile": 4.89, "error plus": 1.34, "error minus": 0.51\}, "break\_mass": \{"median": 35.69, "5th percentile": 22.14, "95th percentile": 48.38, "error plus": 12.69, "error minus": 13.55\}, "mpp\_1": \{"median": 9.72, "5th percentile": 8.5, "95th percentile": 10.22, "error plus": 0.49, "error minus": 1.22\}, "mpp\_2": \{"median": 33.08, "5th percentile": 27.28, "95th percentile": 35.71, "error plus": 2.63, "error minus": 5.8\}, "sigpp\_1": \{"median": 0.65, "5th percentile": 0.31, "95th percentile": 1.5, "error plus": 0.85, "error minus": 0.34\}, "sigpp\_2": \{"median": 3.65, "5th percentile": 1.23, "95th percentile": 8.97, "error plus": 5.31, "error minus": 2.43\}, "delta\_m\_1": \{"median": 4.39, "5th percentile": 0.36, "95th percentile": 9.16, "error plus": 4.77, "error minus": 4.03\}, "delta\_m\_2": \{"median": 5.14, "5th percentile": 0.47, "95th percentile": 9.13, "error plus": 4.0, "error minus": 4.66\}, "lam\_0": \{"median": 0.37, "5th percentile": 0.15, "95th percentile": 0.65, "error plus": 0.27, "error minus": 0.22\}, "lam\_1": \{"median": 0.58, "5th percentile": 0.31, "95th percentile": 0.8, "error plus": 0.22, "error minus": 0.27\}, "lamb": \{"median": 3.12, "5th percentile": 2.21, "95th percentile": 4.02, "error plus": 0.91, "error minus": 0.91\}, "mu\_chi\_1": \{"median": 0.1, "5th percentile": 0.01, "95th percentile": 0.26, "error plus": 0.15, "error minus": 0.09\}, "sigma\_chi\_1": \{"median": 0.33, "5th percentile": 0.22, "95th percentile": 0.45, "error plus": 0.12, "error minus": 0.11\}, "mu\_chi\_2": \{"median": 0.13, "5th percentile": 0.01, "95th percentile": 0.3, "error plus": 0.17, "error minus": 0.11\}, "sigma\_chi\_2": \{"median": 0.33, "5th percentile": 0.19, "95th percentile": 0.55, "error plus": 0.22, "error minus": 0.13\}, "xi\_spin": \{"median": 0.6, "5th percentile": 0.11, "95th percentile": 0.96, "error plus": 0.36, "error minus": 0.49\}, "mu\_1": \{"median": 0.29, "5th percentile": {-}0.75, "95th percentile": 0.92, "error plus": 0.63, "error minus": 1.04\}, "sigma\_1": \{"median": 1.73, "5th percentile": 0.39, "95th percentile": 3.75, "error plus": 2.03, "error minus": 1.33\}, "mu\_2": \{"median": 0.33, "5th percentile": {-}0.77, "95th percentile": 0.92, "error plus": 0.59, "error minus": 1.09\}, "sigma\_2": \{"median": 1.44, "5th percentile": 0.33, "95th percentile": 3.69, "error plus": 2.25, "error minus": 1.11\}, "rate": \{"median": 16.36, "5th percentile": 11.94, "95th percentile": 22.29, "error plus": 5.92, "error minus": 4.42\}, "log\_likelihood": \{"median": {-}1024.69, "5th percentile": {-}1030.93, "95th percentile": {-}1019.99, "error plus": 4.7, "error minus": 6.23\}, "variance": \{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.11, "error minus": 0.23\}, "min\_neff": \{"median": 53.1, "5th percentile": 29.3, "95th percentile": 89.97, "error plus": 36.87, "error minus": 23.8\}, "selection\_neff": \{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@V\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@VI\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@IX\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@X\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XI\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX\else\ifnum\pdfstrcmp{#1}{mu_chi_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XX\else\ifnum\pdfstrcmp{#1}{sigma_chi_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII\else\ifnum\pdfstrcmp{#1}{mu_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII\else\ifnum\pdfstrcmp{#1}{sigma_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV\else\ifnum\pdfstrcmp{#1}{mu_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV\else\ifnum\pdfstrcmp{#1}{sigma_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI\else\ifnum\pdfstrcmp{#1}{rate}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII\else\ifnum\pdfstrcmp{#1}{log_likelihood}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII\else\ifnum\pdfstrcmp{#1}{variance}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX\else\ifnum\pdfstrcmp{#1}{min_neff}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX\else\ifnum\pdfstrcmp{#1}{selection_neff}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@I@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out{\{"a\_1": \{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.72, "peak": 0.13\}, "a\_2": \{"median": 0.28, "5th percentile": 0.03, "90th percentile": 0.64, "95th percentile": 0.75, "peak": 0.16\}, "cos\_tilt\_1": \{"median": 0.06, "5th percentile": {-}0.88, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.3\}, "cos\_tilt\_2": \{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.37\}, "mass\_1": \{"median": 10.09, "5th percentile": 7.96, "90th percentile": 27.75, "95th percentile": 34.39, "peak": 9.91\}, "mass\_ratio": \{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}, "redshift": \{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV\else\ifnum\pdfstrcmp{#1}{mass_1}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI\else\ifnum\pdfstrcmp{#1}{mass_ratio}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII\else\ifnum\pdfstrcmp{#1}{redshift}=0\let\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@II@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out{\{"median": 1.82, "5th percentile": {-}0.01, "95th percentile": 2.95, "error plus": 1.13, "error minus": 1.83\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out{1.82}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out{{-}0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out{2.95}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out{1.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out{1.83}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@III@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out{\{"median": 4.46, "5th percentile": 3.25, "95th percentile": 6.01, "error plus": 1.55, "error minus": 1.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out{4.46}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out{3.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out{6.01}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out{1.55}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out{1.22}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@IV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out{\{"median": 1.29, "5th percentile": 0.26, "95th percentile": 2.7, "error plus": 1.41, "error minus": 1.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out{1.29}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out{0.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out{2.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out{1.41}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out{1.03}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@V@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out{\{"median": 5.06, "5th percentile": 3.25, "95th percentile": 8.16, "error plus": 3.1, "error minus": 1.81\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out{5.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out{3.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out{8.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out{3.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out{1.81}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@VI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out{\{"median": 3.55, "5th percentile": 3.03, "95th percentile": 4.89, "error plus": 1.34, "error minus": 0.51\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out{3.55}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out{4.89}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out{1.34}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out{0.51}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@VII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out{\{"median": 35.69, "5th percentile": 22.14, "95th percentile": 48.38, "error plus": 12.69, "error minus": 13.55\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out{35.69}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out{22.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out{48.38}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out{12.69}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out{13.55}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@VIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out{\{"median": 9.72, "5th percentile": 8.5, "95th percentile": 10.22, "error plus": 0.49, "error minus": 1.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out{9.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out{8.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out{10.22}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out{0.49}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out{1.22}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@IX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out{\{"median": 33.08, "5th percentile": 27.28, "95th percentile": 35.71, "error plus": 2.63, "error minus": 5.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out{33.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out{27.28}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out{35.71}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out{2.63}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out{5.8}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@X@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out{\{"median": 0.65, "5th percentile": 0.31, "95th percentile": 1.5, "error plus": 0.85, "error minus": 0.34\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out{0.65}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out{0.85}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out{0.34}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out{\{"median": 3.65, "5th percentile": 1.23, "95th percentile": 8.97, "error plus": 5.31, "error minus": 2.43\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out{3.65}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out{1.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out{8.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out{5.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out{2.43}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out{\{"median": 4.39, "5th percentile": 0.36, "95th percentile": 9.16, "error plus": 4.77, "error minus": 4.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out{4.39}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out{0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out{9.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out{4.77}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out{4.03}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out{\{"median": 5.14, "5th percentile": 0.47, "95th percentile": 9.13, "error plus": 4.0, "error minus": 4.66\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out{5.14}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out{0.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out{9.13}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out{4.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out{4.66}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XIV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out{\{"median": 0.37, "5th percentile": 0.15, "95th percentile": 0.65, "error plus": 0.27, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out{0.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out{0.27}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out{0.22}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out{\{"median": 0.58, "5th percentile": 0.31, "95th percentile": 0.8, "error plus": 0.22, "error minus": 0.27\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out{0.58}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out{0.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out{0.27}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XVI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out{\{"median": 3.12, "5th percentile": 2.21, "95th percentile": 4.02, "error plus": 0.91, "error minus": 0.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out{3.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out{2.21}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out{4.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out{0.91}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out{0.91}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XVII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out{\{"median": 0.1, "5th percentile": 0.01, "95th percentile": 0.26, "error plus": 0.15, "error minus": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out{0.26}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out{0.15}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out{0.09}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XVIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out{\{"median": 0.33, "5th percentile": 0.22, "95th percentile": 0.45, "error plus": 0.12, "error minus": 0.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out{0.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out{0.45}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out{0.11}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XIX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out{\{"median": 0.13, "5th percentile": 0.01, "95th percentile": 0.3, "error plus": 0.17, "error minus": 0.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out{0.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out{0.17}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out{0.11}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out{\{"median": 0.33, "5th percentile": 0.19, "95th percentile": 0.55, "error plus": 0.22, "error minus": 0.13\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out{0.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out{0.55}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out{0.13}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out{\{"median": 0.6, "5th percentile": 0.11, "95th percentile": 0.96, "error plus": 0.36, "error minus": 0.49\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out{0.11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out{0.96}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out{0.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out{0.49}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out{\{"median": 0.29, "5th percentile": {-}0.75, "95th percentile": 0.92, "error plus": 0.63, "error minus": 1.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out{0.29}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out{{-}0.75}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out{0.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out{0.63}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out{1.04}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out{\{"median": 1.73, "5th percentile": 0.39, "95th percentile": 3.75, "error plus": 2.03, "error minus": 1.33\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out{1.73}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out{0.39}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out{3.75}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out{2.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out{1.33}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out{\{"median": 0.33, "5th percentile": {-}0.77, "95th percentile": 0.92, "error plus": 0.59, "error minus": 1.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out{{-}0.77}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out{0.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out{0.59}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out{1.09}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out{\{"median": 1.44, "5th percentile": 0.33, "95th percentile": 3.69, "error plus": 2.25, "error minus": 1.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out{1.44}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out{0.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out{3.69}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out{2.25}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out{1.11}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out{\{"median": 16.36, "5th percentile": 11.94, "95th percentile": 22.29, "error plus": 5.92, "error minus": 4.42\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out{16.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out{11.94}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out{22.29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out{5.92}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out{4.42}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out{\{"median": {-}1024.69, "5th percentile": {-}1030.93, "95th percentile": {-}1019.99, "error plus": 4.7, "error minus": 6.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out{{-}1024.69}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out{{-}1030.93}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out{{-}1019.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out{4.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out{6.23}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXVIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out{\{"median": 0.87, "5th percentile": 0.64, "95th percentile": 0.99, "error plus": 0.11, "error minus": 0.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out{0.64}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out{0.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out{0.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out{0.23}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXIX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out{\{"median": 53.1, "5th percentile": 29.3, "95th percentile": 89.97, "error plus": 36.87, "error minus": 23.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out{53.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out{29.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out{89.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out{36.87}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out{23.8}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXX@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out{\{"median": 1993.0, "5th percentile": 1993.0, "95th percentile": 1993.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out{1993.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out{0.0}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out{\{"median": 0.27, "5th percentile": 0.03, "90th percentile": 0.61, "95th percentile": 0.72, "peak": 0.13\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out{0.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out{0.72}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out{0.13}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out{\{"median": 0.28, "5th percentile": 0.03, "90th percentile": 0.64, "95th percentile": 0.75, "peak": 0.16\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out{0.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out{0.03}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out{0.64}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out{0.75}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out{0.16}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out{\{"median": 0.06, "5th percentile": {-}0.88, "90th percentile": 0.8, "95th percentile": 0.9, "peak": 0.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out{0.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out{{-}0.88}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out{0.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out{0.3}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXIV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out{\{"median": 0.1, "5th percentile": {-}0.87, "90th percentile": 0.81, "95th percentile": 0.9, "peak": 0.37\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out{0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out{{-}0.87}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out{0.81}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out{0.37}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXV@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out{\{"median": 10.09, "5th percentile": 7.96, "90th percentile": 27.75, "95th percentile": 34.39, "peak": 9.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out{10.09}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out{7.96}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out{27.75}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out{34.39}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out{9.91}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVI@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out{\{"median": 0.84, "5th percentile": 0.51, "90th percentile": 0.97, "95th percentile": 0.99, "peak": 1.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out{0.51}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out{0.97}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out{0.99}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out{1.0}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVII@out}\newcommand\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out{\{"median": 0.31, "5th percentile": 0.05, "90th percentile": 0.45, "95th percentile": 0.47, "peak": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out{0.05}\else\ifnum\pdfstrcmp{#1}{90th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out{0.47}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out{2.0}\else\def\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out{??}\fi\fi\fi\fi\fi\fi\MagTruncnormIndTiltIsotropicTruncnormNnd@XXXVIII@out}\makeatother
\makeatletter\newcommand\MassSpinCorrelatedBGPModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MassSpinCorrelatedBGPModel@out{\{"param": \{"positive{-}to{-}negative chi\_eff ratio for m in 30{-}40": \{"median": 1.9, "5th percentile": 0.7, "95th percentile": 6.7, "error plus": 4.8, "error minus": 1.2\}, "positive{-}to{-}negative chi\_eff ratio for m outside 30{-}40": \{"median": 6.6, "5th percentile": 2.4, "95th percentile": 20.7, "error plus": 14.1, "error minus": 4.2\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MassSpinCorrelatedBGPModel@out\MassSpinCorrelatedBGPModel@I\else\def\MassSpinCorrelatedBGPModel@out{??}\fi\fi\MassSpinCorrelatedBGPModel@out}\newcommand\MassSpinCorrelatedBGPModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MassSpinCorrelatedBGPModel@I@out{\{"positive{-}to{-}negative chi\_eff ratio for m in 30{-}40": \{"median": 1.9, "5th percentile": 0.7, "95th percentile": 6.7, "error plus": 4.8, "error minus": 1.2\}, "positive{-}to{-}negative chi\_eff ratio for m outside 30{-}40": \{"median": 6.6, "5th percentile": 2.4, "95th percentile": 20.7, "error plus": 14.1, "error minus": 4.2\}\}}\else\ifnum\pdfstrcmp{#1}{positive-to-negative chi_eff ratio for m in 30-40}=0\let\MassSpinCorrelatedBGPModel@I@out\MassSpinCorrelatedBGPModel@II\else\ifnum\pdfstrcmp{#1}{positive-to-negative chi_eff ratio for m outside 30-40}=0\let\MassSpinCorrelatedBGPModel@I@out\MassSpinCorrelatedBGPModel@III\else\def\MassSpinCorrelatedBGPModel@I@out{??}\fi\fi\fi\MassSpinCorrelatedBGPModel@I@out}\newcommand\MassSpinCorrelatedBGPModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MassSpinCorrelatedBGPModel@II@out{\{"median": 1.9, "5th percentile": 0.7, "95th percentile": 6.7, "error plus": 4.8, "error minus": 1.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MassSpinCorrelatedBGPModel@II@out{1.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MassSpinCorrelatedBGPModel@II@out{0.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MassSpinCorrelatedBGPModel@II@out{6.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MassSpinCorrelatedBGPModel@II@out{4.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MassSpinCorrelatedBGPModel@II@out{1.2}\else\def\MassSpinCorrelatedBGPModel@II@out{??}\fi\fi\fi\fi\fi\fi\MassSpinCorrelatedBGPModel@II@out}\newcommand\MassSpinCorrelatedBGPModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MassSpinCorrelatedBGPModel@III@out{\{"median": 6.6, "5th percentile": 2.4, "95th percentile": 20.7, "error plus": 14.1, "error minus": 4.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MassSpinCorrelatedBGPModel@III@out{6.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MassSpinCorrelatedBGPModel@III@out{2.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MassSpinCorrelatedBGPModel@III@out{20.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MassSpinCorrelatedBGPModel@III@out{14.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MassSpinCorrelatedBGPModel@III@out{4.2}\else\def\MassSpinCorrelatedBGPModel@III@out{??}\fi\fi\fi\fi\fi\fi\MassSpinCorrelatedBGPModel@III@out}\makeatother
\makeatletter\newcommand\mchieffCopulaCorrelationModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@out{\{"param": \{"alpha\_1": \{"median": 1.85, "5th percentile": {-}0.04, "95th percentile": 3.09, "error plus": 1.24, "error minus": 1.89\}, "alpha\_2": \{"median": 4.38, "5th percentile": 3.1, "95th percentile": 5.85, "error plus": 1.47, "error minus": 1.28\}, "beta": \{"median": 0.89, "5th percentile": {-}0.08, "95th percentile": 2.06, "error plus": 1.17, "error minus": 0.97\}, "break\_mass": \{"median": 35.51, "5th percentile": 22.47, "95th percentile": 48.21, "error plus": 12.69, "error minus": 13.04\}, "delta\_m\_1": \{"median": 4.64, "5th percentile": 0.44, "95th percentile": 9.19, "error plus": 4.56, "error minus": 4.19\}, "delta\_m\_2": \{"median": 4.28, "5th percentile": 0.45, "95th percentile": 7.73, "error plus": 3.44, "error minus": 3.83\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.65, "error plus": 0.31, "error minus": 0.22\}, "lam\_1": \{"median": 0.61, "5th percentile": 0.31, "95th percentile": 0.83, "error plus": 0.22, "error minus": 0.3\}, "lamb": \{"median": 3.03, "5th percentile": 2.12, "95th percentile": 3.96, "error plus": 0.93, "error minus": 0.9\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.27, "95th percentile": 7.64, "error plus": 2.49, "error minus": 1.89\}, "mlow\_2": \{"median": 3.59, "5th percentile": 3.03, "95th percentile": 4.97, "error plus": 1.37, "error minus": 0.56\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.76, "5th percentile": 8.5, "95th percentile": 10.25, "error plus": 0.5, "error minus": 1.25\}, "mpp\_2": \{"median": 32.79, "5th percentile": 26.44, "95th percentile": 36.08, "error plus": 3.29, "error minus": 6.35\}, "mu\_chi\_eff": \{"median": 0.04, "5th percentile": {-}0.0, "95th percentile": 0.07, "error plus": 0.03, "error minus": 0.04\}, "mu\_chi\_p": \{"median": 0.36, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.06\}, "sigma\_chi\_eff": \{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.03, "error minus": 0.02\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.26, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": 0.4, "5th percentile": {-}1.0, "95th percentile": 2.0, "error plus": 1.6, "error minus": 1.4, "correlated percentile": 68\}\}, "ppd": \{\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\mchieffCopulaCorrelationModel@out\mchieffCopulaCorrelationModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\mchieffCopulaCorrelationModel@out\mchieffCopulaCorrelationModel@II\else\def\mchieffCopulaCorrelationModel@out{??}\fi\fi\fi\mchieffCopulaCorrelationModel@out}\newcommand\mchieffCopulaCorrelationModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@I@out{\{"alpha\_1": \{"median": 1.85, "5th percentile": {-}0.04, "95th percentile": 3.09, "error plus": 1.24, "error minus": 1.89\}, "alpha\_2": \{"median": 4.38, "5th percentile": 3.1, "95th percentile": 5.85, "error plus": 1.47, "error minus": 1.28\}, "beta": \{"median": 0.89, "5th percentile": {-}0.08, "95th percentile": 2.06, "error plus": 1.17, "error minus": 0.97\}, "break\_mass": \{"median": 35.51, "5th percentile": 22.47, "95th percentile": 48.21, "error plus": 12.69, "error minus": 13.04\}, "delta\_m\_1": \{"median": 4.64, "5th percentile": 0.44, "95th percentile": 9.19, "error plus": 4.56, "error minus": 4.19\}, "delta\_m\_2": \{"median": 4.28, "5th percentile": 0.45, "95th percentile": 7.73, "error plus": 3.44, "error minus": 3.83\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.65, "error plus": 0.31, "error minus": 0.22\}, "lam\_1": \{"median": 0.61, "5th percentile": 0.31, "95th percentile": 0.83, "error plus": 0.22, "error minus": 0.3\}, "lamb": \{"median": 3.03, "5th percentile": 2.12, "95th percentile": 3.96, "error plus": 0.93, "error minus": 0.9\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.27, "95th percentile": 7.64, "error plus": 2.49, "error minus": 1.89\}, "mlow\_2": \{"median": 3.59, "5th percentile": 3.03, "95th percentile": 4.97, "error plus": 1.37, "error minus": 0.56\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.76, "5th percentile": 8.5, "95th percentile": 10.25, "error plus": 0.5, "error minus": 1.25\}, "mpp\_2": \{"median": 32.79, "5th percentile": 26.44, "95th percentile": 36.08, "error plus": 3.29, "error minus": 6.35\}, "mu\_chi\_eff": \{"median": 0.04, "5th percentile": {-}0.0, "95th percentile": 0.07, "error plus": 0.03, "error minus": 0.04\}, "mu\_chi\_p": \{"median": 0.36, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.06\}, "sigma\_chi\_eff": \{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.03, "error minus": 0.02\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.26, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": 0.4, "5th percentile": {-}1.0, "95th percentile": 2.0, "error plus": 1.6, "error minus": 1.4, "correlated percentile": 68\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@VI\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@VII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@VIII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@IX\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@X\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XI\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XII\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XIII\else\ifnum\pdfstrcmp{#1}{mmax}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XIV\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XV\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XVI\else\ifnum\pdfstrcmp{#1}{mu_chi_eff}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi_p}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi_eff}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XIX\else\ifnum\pdfstrcmp{#1}{sigma_chi_p}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XX\else\ifnum\pdfstrcmp{#1}{kappa}=0\let\mchieffCopulaCorrelationModel@I@out\mchieffCopulaCorrelationModel@XXI\else\def\mchieffCopulaCorrelationModel@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@I@out}\newcommand\mchieffCopulaCorrelationModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@II@out{\{\}}\else\def\mchieffCopulaCorrelationModel@II@out{??}\fi\mchieffCopulaCorrelationModel@II@out}\newcommand\mchieffCopulaCorrelationModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@III@out{\{"median": 1.85, "5th percentile": {-}0.04, "95th percentile": 3.09, "error plus": 1.24, "error minus": 1.89\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@III@out{1.85}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@III@out{{-}0.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@III@out{3.09}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@III@out{1.24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@III@out{1.89}\else\def\mchieffCopulaCorrelationModel@III@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@III@out}\newcommand\mchieffCopulaCorrelationModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@IV@out{\{"median": 4.38, "5th percentile": 3.1, "95th percentile": 5.85, "error plus": 1.47, "error minus": 1.28\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@IV@out{4.38}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@IV@out{3.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@IV@out{5.85}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@IV@out{1.47}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@IV@out{1.28}\else\def\mchieffCopulaCorrelationModel@IV@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@IV@out}\newcommand\mchieffCopulaCorrelationModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@V@out{\{"median": 0.89, "5th percentile": {-}0.08, "95th percentile": 2.06, "error plus": 1.17, "error minus": 0.97\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@V@out{0.89}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@V@out{{-}0.08}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@V@out{2.06}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@V@out{1.17}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@V@out{0.97}\else\def\mchieffCopulaCorrelationModel@V@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@V@out}\newcommand\mchieffCopulaCorrelationModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@VI@out{\{"median": 35.51, "5th percentile": 22.47, "95th percentile": 48.21, "error plus": 12.69, "error minus": 13.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@VI@out{35.51}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@VI@out{22.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@VI@out{48.21}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@VI@out{12.69}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@VI@out{13.04}\else\def\mchieffCopulaCorrelationModel@VI@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@VI@out}\newcommand\mchieffCopulaCorrelationModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@VII@out{\{"median": 4.64, "5th percentile": 0.44, "95th percentile": 9.19, "error plus": 4.56, "error minus": 4.19\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@VII@out{4.64}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@VII@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@VII@out{9.19}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@VII@out{4.56}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@VII@out{4.19}\else\def\mchieffCopulaCorrelationModel@VII@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@VII@out}\newcommand\mchieffCopulaCorrelationModel@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@VIII@out{\{"median": 4.28, "5th percentile": 0.45, "95th percentile": 7.73, "error plus": 3.44, "error minus": 3.83\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@VIII@out{4.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@VIII@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@VIII@out{7.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@VIII@out{3.44}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@VIII@out{3.83}\else\def\mchieffCopulaCorrelationModel@VIII@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@VIII@out}\newcommand\mchieffCopulaCorrelationModel@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@IX@out{\{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.65, "error plus": 0.31, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@IX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@IX@out{0.65}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@IX@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@IX@out{0.22}\else\def\mchieffCopulaCorrelationModel@IX@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@IX@out}\newcommand\mchieffCopulaCorrelationModel@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@X@out{\{"median": 0.61, "5th percentile": 0.31, "95th percentile": 0.83, "error plus": 0.22, "error minus": 0.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@X@out{0.61}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@X@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@X@out{0.83}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@X@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@X@out{0.3}\else\def\mchieffCopulaCorrelationModel@X@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@X@out}\newcommand\mchieffCopulaCorrelationModel@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XI@out{\{"median": 3.03, "5th percentile": 2.12, "95th percentile": 3.96, "error plus": 0.93, "error minus": 0.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XI@out{3.03}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XI@out{2.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XI@out{3.96}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XI@out{0.93}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XI@out{0.9}\else\def\mchieffCopulaCorrelationModel@XI@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XI@out}\newcommand\mchieffCopulaCorrelationModel@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XII@out{\{"median": 5.15, "5th percentile": 3.27, "95th percentile": 7.64, "error plus": 2.49, "error minus": 1.89\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XII@out{5.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XII@out{3.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XII@out{7.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XII@out{2.49}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XII@out{1.89}\else\def\mchieffCopulaCorrelationModel@XII@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XII@out}\newcommand\mchieffCopulaCorrelationModel@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XIII@out{\{"median": 3.59, "5th percentile": 3.03, "95th percentile": 4.97, "error plus": 1.37, "error minus": 0.56\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XIII@out{3.59}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XIII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XIII@out{4.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XIII@out{1.37}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XIII@out{0.56}\else\def\mchieffCopulaCorrelationModel@XIII@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XIII@out}\newcommand\mchieffCopulaCorrelationModel@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XIV@out{\{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XIV@out{0.0}\else\def\mchieffCopulaCorrelationModel@XIV@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XIV@out}\newcommand\mchieffCopulaCorrelationModel@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XV@out{\{"median": 9.76, "5th percentile": 8.5, "95th percentile": 10.25, "error plus": 0.5, "error minus": 1.25\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XV@out{9.76}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XV@out{8.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XV@out{10.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XV@out{0.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XV@out{1.25}\else\def\mchieffCopulaCorrelationModel@XV@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XV@out}\newcommand\mchieffCopulaCorrelationModel@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XVI@out{\{"median": 32.79, "5th percentile": 26.44, "95th percentile": 36.08, "error plus": 3.29, "error minus": 6.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XVI@out{32.79}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XVI@out{26.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XVI@out{36.08}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XVI@out{3.29}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XVI@out{6.35}\else\def\mchieffCopulaCorrelationModel@XVI@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XVI@out}\newcommand\mchieffCopulaCorrelationModel@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XVII@out{\{"median": 0.04, "5th percentile": {-}0.0, "95th percentile": 0.07, "error plus": 0.03, "error minus": 0.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XVII@out{0.04}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XVII@out{{-}0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XVII@out{0.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XVII@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XVII@out{0.04}\else\def\mchieffCopulaCorrelationModel@XVII@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XVII@out}\newcommand\mchieffCopulaCorrelationModel@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XVIII@out{\{"median": 0.36, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.06\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XVIII@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XVIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XVIII@out{0.42}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XVIII@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XVIII@out{0.06}\else\def\mchieffCopulaCorrelationModel@XVIII@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XVIII@out}\newcommand\mchieffCopulaCorrelationModel@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XIX@out{\{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.03, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XIX@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XIX@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XIX@out{0.14}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XIX@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XIX@out{0.02}\else\def\mchieffCopulaCorrelationModel@XIX@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XIX@out}\newcommand\mchieffCopulaCorrelationModel@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XX@out{\{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.26, "error plus": 0.07, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XX@out{0.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XX@out{0.26}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XX@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XX@out{0.05}\else\def\mchieffCopulaCorrelationModel@XX@out{??}\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XX@out}\newcommand\mchieffCopulaCorrelationModel@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mchieffCopulaCorrelationModel@XXI@out{\{"median": 0.4, "5th percentile": {-}1.0, "95th percentile": 2.0, "error plus": 1.6, "error minus": 1.4, "correlated percentile": 68\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mchieffCopulaCorrelationModel@XXI@out{0.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mchieffCopulaCorrelationModel@XXI@out{{-}1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mchieffCopulaCorrelationModel@XXI@out{2.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mchieffCopulaCorrelationModel@XXI@out{1.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mchieffCopulaCorrelationModel@XXI@out{1.4}\else\ifnum\pdfstrcmp{#1}{correlated percentile}=0\def\mchieffCopulaCorrelationModel@XXI@out{68}\else\def\mchieffCopulaCorrelationModel@XXI@out{??}\fi\fi\fi\fi\fi\fi\fi\mchieffCopulaCorrelationModel@XXI@out}\makeatother
\makeatletter\newcommand\MinimumTiltModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@out{\{"param": \{"alpha\_1": \{"median": 1.77, "5th percentile": {-}0.32, "95th percentile": 2.97, "error plus": 1.2, "error minus": 2.09\}, "alpha\_2": \{"median": 4.48, "5th percentile": 3.3, "95th percentile": 5.94, "error plus": 1.46, "error minus": 1.19\}, "amax": \{"median": 1.0, "5th percentile": 1.0, "95th percentile": 1.0, "error plus": 0.0, "error minus": 0.0\}, "beta": \{"median": 1.16, "5th percentile": 0.2, "95th percentile": 2.25, "error plus": 1.09, "error minus": 0.96\}, "break\_mass": \{"median": 35.61, "5th percentile": 21.95, "95th percentile": 48.03, "error plus": 12.42, "error minus": 13.66\}, "delta\_m\_1": \{"median": 4.72, "5th percentile": 0.54, "95th percentile": 9.3, "error plus": 4.57, "error minus": 4.18\}, "delta\_m\_2": \{"median": 3.38, "5th percentile": 0.36, "95th percentile": 7.28, "error plus": 3.9, "error minus": 3.02\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.64, "error plus": 0.29, "error minus": 0.21\}, "lam\_1": \{"median": 0.62, "5th percentile": 0.33, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.29\}, "lamb": \{"median": 3.03, "5th percentile": 2.1, "95th percentile": 3.92, "error plus": 0.89, "error minus": 0.93\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.27, "95th percentile": 7.8, "error plus": 2.65, "error minus": 1.88\}, "mlow\_2": \{"median": 3.58, "5th percentile": 3.04, "95th percentile": 4.85, "error plus": 1.26, "error minus": 0.55\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.8, "5th percentile": 8.74, "95th percentile": 10.29, "error plus": 0.48, "error minus": 1.07\}, "mpp\_2": \{"median": 33.08, "5th percentile": 26.87, "95th percentile": 35.93, "error plus": 2.85, "error minus": 6.22\}, "mu\_chi": \{"median": 0.11, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.12, "error minus": 0.09\}, "mu\_spin": \{"median": {-}0.0, "5th percentile": {-}0.88, "95th percentile": 0.88, "error plus": 0.88, "error minus": 0.87\}, "sigma\_chi": \{"median": 0.34, "5th percentile": 0.27, "95th percentile": 0.39, "error plus": 0.05, "error minus": 0.07\}, "sigma\_spin": \{"median": 2.21, "5th percentile": 0.7, "95th percentile": 3.8, "error plus": 1.59, "error minus": 1.52\}, "sigpp\_1": \{"median": 0.7, "5th percentile": 0.34, "95th percentile": 1.54, "error plus": 0.84, "error minus": 0.37\}, "sigpp\_2": \{"median": 3.9, "5th percentile": 1.34, "95th percentile": 8.82, "error plus": 4.92, "error minus": 2.56\}, "tmin": \{"median": {-}0.71, "5th percentile": {-}0.89, "95th percentile": {-}0.56, "error plus": 0.15, "error minus": 0.19\}, "xi\_spin": \{"median": 0.51, "5th percentile": 0.05, "95th percentile": 0.95, "error plus": 0.45, "error minus": 0.46\}\}, "ppd": \{"a\_1": \{"median": 0.27, "5th percentile": 0.03, "95th percentile": 0.73, "peak": 0.12\}, "a\_2": \{"median": 0.27, "5th percentile": 0.03, "95th percentile": 0.71, "peak": 0.12\}, "cos\_tilt\_1": \{"median": 0.14, "5th percentile": {-}0.64, "95th percentile": 0.91, "peak": 0.02\}, "cos\_tilt\_2": \{"median": 0.13, "5th percentile": {-}0.63, "95th percentile": 0.9, "peak": 0.02\}\}, "fraction negative cos theta": \{"median": 0.41, "5th percentile": 0.36, "95th percentile": 0.47, "error plus": 0.05, "error minus": 0.05\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\MinimumTiltModel@out\MinimumTiltModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\MinimumTiltModel@out\MinimumTiltModel@II\else\ifnum\pdfstrcmp{#1}{fraction negative cos theta}=0\let\MinimumTiltModel@out\MinimumTiltModel@III\else\def\MinimumTiltModel@out{??}\fi\fi\fi\fi\MinimumTiltModel@out}\newcommand\MinimumTiltModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@I@out{\{"alpha\_1": \{"median": 1.77, "5th percentile": {-}0.32, "95th percentile": 2.97, "error plus": 1.2, "error minus": 2.09\}, "alpha\_2": \{"median": 4.48, "5th percentile": 3.3, "95th percentile": 5.94, "error plus": 1.46, "error minus": 1.19\}, "amax": \{"median": 1.0, "5th percentile": 1.0, "95th percentile": 1.0, "error plus": 0.0, "error minus": 0.0\}, "beta": \{"median": 1.16, "5th percentile": 0.2, "95th percentile": 2.25, "error plus": 1.09, "error minus": 0.96\}, "break\_mass": \{"median": 35.61, "5th percentile": 21.95, "95th percentile": 48.03, "error plus": 12.42, "error minus": 13.66\}, "delta\_m\_1": \{"median": 4.72, "5th percentile": 0.54, "95th percentile": 9.3, "error plus": 4.57, "error minus": 4.18\}, "delta\_m\_2": \{"median": 3.38, "5th percentile": 0.36, "95th percentile": 7.28, "error plus": 3.9, "error minus": 3.02\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.64, "error plus": 0.29, "error minus": 0.21\}, "lam\_1": \{"median": 0.62, "5th percentile": 0.33, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.29\}, "lamb": \{"median": 3.03, "5th percentile": 2.1, "95th percentile": 3.92, "error plus": 0.89, "error minus": 0.93\}, "mlow\_1": \{"median": 5.15, "5th percentile": 3.27, "95th percentile": 7.8, "error plus": 2.65, "error minus": 1.88\}, "mlow\_2": \{"median": 3.58, "5th percentile": 3.04, "95th percentile": 4.85, "error plus": 1.26, "error minus": 0.55\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.8, "5th percentile": 8.74, "95th percentile": 10.29, "error plus": 0.48, "error minus": 1.07\}, "mpp\_2": \{"median": 33.08, "5th percentile": 26.87, "95th percentile": 35.93, "error plus": 2.85, "error minus": 6.22\}, "mu\_chi": \{"median": 0.11, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.12, "error minus": 0.09\}, "mu\_spin": \{"median": {-}0.0, "5th percentile": {-}0.88, "95th percentile": 0.88, "error plus": 0.88, "error minus": 0.87\}, "sigma\_chi": \{"median": 0.34, "5th percentile": 0.27, "95th percentile": 0.39, "error plus": 0.05, "error minus": 0.07\}, "sigma\_spin": \{"median": 2.21, "5th percentile": 0.7, "95th percentile": 3.8, "error plus": 1.59, "error minus": 1.52\}, "sigpp\_1": \{"median": 0.7, "5th percentile": 0.34, "95th percentile": 1.54, "error plus": 0.84, "error minus": 0.37\}, "sigpp\_2": \{"median": 3.9, "5th percentile": 1.34, "95th percentile": 8.82, "error plus": 4.92, "error minus": 2.56\}, "tmin": \{"median": {-}0.71, "5th percentile": {-}0.89, "95th percentile": {-}0.56, "error plus": 0.15, "error minus": 0.19\}, "xi\_spin": \{"median": 0.51, "5th percentile": 0.05, "95th percentile": 0.95, "error plus": 0.45, "error minus": 0.46\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@IV\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@V\else\ifnum\pdfstrcmp{#1}{amax}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@VI\else\ifnum\pdfstrcmp{#1}{beta}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@VII\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@VIII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@IX\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@X\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XI\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XII\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XIII\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XIV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XV\else\ifnum\pdfstrcmp{#1}{mmax}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XVI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XVII\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XVIII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XIX\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XX\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XXI\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XXII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XXIII\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XXIV\else\ifnum\pdfstrcmp{#1}{tmin}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XXV\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\MinimumTiltModel@I@out\MinimumTiltModel@XXVI\else\def\MinimumTiltModel@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\MinimumTiltModel@I@out}\newcommand\MinimumTiltModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@II@out{\{"a\_1": \{"median": 0.27, "5th percentile": 0.03, "95th percentile": 0.73, "peak": 0.12\}, "a\_2": \{"median": 0.27, "5th percentile": 0.03, "95th percentile": 0.71, "peak": 0.12\}, "cos\_tilt\_1": \{"median": 0.14, "5th percentile": {-}0.64, "95th percentile": 0.91, "peak": 0.02\}, "cos\_tilt\_2": \{"median": 0.13, "5th percentile": {-}0.63, "95th percentile": 0.9, "peak": 0.02\}\}}\else\ifnum\pdfstrcmp{#1}{a_1}=0\let\MinimumTiltModel@II@out\MinimumTiltModel@XXVII\else\ifnum\pdfstrcmp{#1}{a_2}=0\let\MinimumTiltModel@II@out\MinimumTiltModel@XXVIII\else\ifnum\pdfstrcmp{#1}{cos_tilt_1}=0\let\MinimumTiltModel@II@out\MinimumTiltModel@XXIX\else\ifnum\pdfstrcmp{#1}{cos_tilt_2}=0\let\MinimumTiltModel@II@out\MinimumTiltModel@XXX\else\def\MinimumTiltModel@II@out{??}\fi\fi\fi\fi\fi\MinimumTiltModel@II@out}\newcommand\MinimumTiltModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@III@out{\{"median": 0.41, "5th percentile": 0.36, "95th percentile": 0.47, "error plus": 0.05, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@III@out{0.41}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@III@out{0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@III@out{0.47}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@III@out{0.05}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@III@out{0.05}\else\def\MinimumTiltModel@III@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@III@out}\newcommand\MinimumTiltModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@IV@out{\{"median": 1.77, "5th percentile": {-}0.32, "95th percentile": 2.97, "error plus": 1.2, "error minus": 2.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@IV@out{1.77}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@IV@out{{-}0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@IV@out{2.97}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@IV@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@IV@out{2.09}\else\def\MinimumTiltModel@IV@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@IV@out}\newcommand\MinimumTiltModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@V@out{\{"median": 4.48, "5th percentile": 3.3, "95th percentile": 5.94, "error plus": 1.46, "error minus": 1.19\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@V@out{4.48}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@V@out{3.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@V@out{5.94}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@V@out{1.46}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@V@out{1.19}\else\def\MinimumTiltModel@V@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@V@out}\newcommand\MinimumTiltModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@VI@out{\{"median": 1.0, "5th percentile": 1.0, "95th percentile": 1.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@VI@out{1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@VI@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@VI@out{1.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@VI@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@VI@out{0.0}\else\def\MinimumTiltModel@VI@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@VI@out}\newcommand\MinimumTiltModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@VII@out{\{"median": 1.16, "5th percentile": 0.2, "95th percentile": 2.25, "error plus": 1.09, "error minus": 0.96\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@VII@out{1.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@VII@out{0.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@VII@out{2.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@VII@out{1.09}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@VII@out{0.96}\else\def\MinimumTiltModel@VII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@VII@out}\newcommand\MinimumTiltModel@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@VIII@out{\{"median": 35.61, "5th percentile": 21.95, "95th percentile": 48.03, "error plus": 12.42, "error minus": 13.66\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@VIII@out{35.61}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@VIII@out{21.95}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@VIII@out{48.03}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@VIII@out{12.42}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@VIII@out{13.66}\else\def\MinimumTiltModel@VIII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@VIII@out}\newcommand\MinimumTiltModel@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@IX@out{\{"median": 4.72, "5th percentile": 0.54, "95th percentile": 9.3, "error plus": 4.57, "error minus": 4.18\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@IX@out{4.72}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@IX@out{0.54}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@IX@out{9.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@IX@out{4.57}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@IX@out{4.18}\else\def\MinimumTiltModel@IX@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@IX@out}\newcommand\MinimumTiltModel@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@X@out{\{"median": 3.38, "5th percentile": 0.36, "95th percentile": 7.28, "error plus": 3.9, "error minus": 3.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@X@out{3.38}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@X@out{0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@X@out{7.28}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@X@out{3.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@X@out{3.02}\else\def\MinimumTiltModel@X@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@X@out}\newcommand\MinimumTiltModel@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XI@out{\{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.64, "error plus": 0.29, "error minus": 0.21\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XI@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XI@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XI@out{0.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XI@out{0.29}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XI@out{0.21}\else\def\MinimumTiltModel@XI@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XI@out}\newcommand\MinimumTiltModel@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XII@out{\{"median": 0.62, "5th percentile": 0.33, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.29\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XII@out{0.62}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XII@out{0.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XII@out{0.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XII@out{0.21}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XII@out{0.29}\else\def\MinimumTiltModel@XII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XII@out}\newcommand\MinimumTiltModel@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XIII@out{\{"median": 3.03, "5th percentile": 2.1, "95th percentile": 3.92, "error plus": 0.89, "error minus": 0.93\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XIII@out{3.03}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XIII@out{2.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XIII@out{3.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XIII@out{0.89}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XIII@out{0.93}\else\def\MinimumTiltModel@XIII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XIII@out}\newcommand\MinimumTiltModel@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XIV@out{\{"median": 5.15, "5th percentile": 3.27, "95th percentile": 7.8, "error plus": 2.65, "error minus": 1.88\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XIV@out{5.15}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XIV@out{3.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XIV@out{7.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XIV@out{2.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XIV@out{1.88}\else\def\MinimumTiltModel@XIV@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XIV@out}\newcommand\MinimumTiltModel@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XV@out{\{"median": 3.58, "5th percentile": 3.04, "95th percentile": 4.85, "error plus": 1.26, "error minus": 0.55\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XV@out{3.58}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XV@out{3.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XV@out{4.85}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XV@out{1.26}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XV@out{0.55}\else\def\MinimumTiltModel@XV@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XV@out}\newcommand\MinimumTiltModel@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XVI@out{\{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XVI@out{300.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XVI@out{300.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XVI@out{300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XVI@out{0.0}\else\def\MinimumTiltModel@XVI@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XVI@out}\newcommand\MinimumTiltModel@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XVII@out{\{"median": 9.8, "5th percentile": 8.74, "95th percentile": 10.29, "error plus": 0.48, "error minus": 1.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XVII@out{9.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XVII@out{8.74}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XVII@out{10.29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XVII@out{0.48}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XVII@out{1.07}\else\def\MinimumTiltModel@XVII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XVII@out}\newcommand\MinimumTiltModel@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XVIII@out{\{"median": 33.08, "5th percentile": 26.87, "95th percentile": 35.93, "error plus": 2.85, "error minus": 6.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XVIII@out{33.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XVIII@out{26.87}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XVIII@out{35.93}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XVIII@out{2.85}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XVIII@out{6.22}\else\def\MinimumTiltModel@XVIII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XVIII@out}\newcommand\MinimumTiltModel@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XIX@out{\{"median": 0.11, "5th percentile": 0.01, "95th percentile": 0.23, "error plus": 0.12, "error minus": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XIX@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XIX@out{0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XIX@out{0.23}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XIX@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XIX@out{0.09}\else\def\MinimumTiltModel@XIX@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XIX@out}\newcommand\MinimumTiltModel@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XX@out{\{"median": {-}0.0, "5th percentile": {-}0.88, "95th percentile": 0.88, "error plus": 0.88, "error minus": 0.87\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XX@out{{-}0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XX@out{{-}0.88}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XX@out{0.88}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XX@out{0.88}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XX@out{0.87}\else\def\MinimumTiltModel@XX@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XX@out}\newcommand\MinimumTiltModel@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXI@out{\{"median": 0.34, "5th percentile": 0.27, "95th percentile": 0.39, "error plus": 0.05, "error minus": 0.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXI@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXI@out{0.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXI@out{0.39}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XXI@out{0.05}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XXI@out{0.07}\else\def\MinimumTiltModel@XXI@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XXI@out}\newcommand\MinimumTiltModel@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXII@out{\{"median": 2.21, "5th percentile": 0.7, "95th percentile": 3.8, "error plus": 1.59, "error minus": 1.52\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXII@out{2.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXII@out{0.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXII@out{3.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XXII@out{1.59}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XXII@out{1.52}\else\def\MinimumTiltModel@XXII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XXII@out}\newcommand\MinimumTiltModel@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXIII@out{\{"median": 0.7, "5th percentile": 0.34, "95th percentile": 1.54, "error plus": 0.84, "error minus": 0.37\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXIII@out{0.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXIII@out{0.34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXIII@out{1.54}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XXIII@out{0.84}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XXIII@out{0.37}\else\def\MinimumTiltModel@XXIII@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XXIII@out}\newcommand\MinimumTiltModel@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXIV@out{\{"median": 3.9, "5th percentile": 1.34, "95th percentile": 8.82, "error plus": 4.92, "error minus": 2.56\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXIV@out{3.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXIV@out{1.34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXIV@out{8.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XXIV@out{4.92}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XXIV@out{2.56}\else\def\MinimumTiltModel@XXIV@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XXIV@out}\newcommand\MinimumTiltModel@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXV@out{\{"median": {-}0.71, "5th percentile": {-}0.89, "95th percentile": {-}0.56, "error plus": 0.15, "error minus": 0.19\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXV@out{{-}0.71}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXV@out{{-}0.89}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXV@out{{-}0.56}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XXV@out{0.15}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XXV@out{0.19}\else\def\MinimumTiltModel@XXV@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XXV@out}\newcommand\MinimumTiltModel@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXVI@out{\{"median": 0.51, "5th percentile": 0.05, "95th percentile": 0.95, "error plus": 0.45, "error minus": 0.46\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXVI@out{0.51}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXVI@out{0.05}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXVI@out{0.95}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\MinimumTiltModel@XXVI@out{0.45}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\MinimumTiltModel@XXVI@out{0.46}\else\def\MinimumTiltModel@XXVI@out{??}\fi\fi\fi\fi\fi\fi\MinimumTiltModel@XXVI@out}\newcommand\MinimumTiltModel@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXVII@out{\{"median": 0.27, "5th percentile": 0.03, "95th percentile": 0.73, "peak": 0.12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXVII@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXVII@out{0.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXVII@out{0.73}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MinimumTiltModel@XXVII@out{0.12}\else\def\MinimumTiltModel@XXVII@out{??}\fi\fi\fi\fi\fi\MinimumTiltModel@XXVII@out}\newcommand\MinimumTiltModel@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXVIII@out{\{"median": 0.27, "5th percentile": 0.03, "95th percentile": 0.71, "peak": 0.12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXVIII@out{0.27}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXVIII@out{0.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXVIII@out{0.71}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MinimumTiltModel@XXVIII@out{0.12}\else\def\MinimumTiltModel@XXVIII@out{??}\fi\fi\fi\fi\fi\MinimumTiltModel@XXVIII@out}\newcommand\MinimumTiltModel@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXIX@out{\{"median": 0.14, "5th percentile": {-}0.64, "95th percentile": 0.91, "peak": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXIX@out{0.14}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXIX@out{{-}0.64}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXIX@out{0.91}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MinimumTiltModel@XXIX@out{0.02}\else\def\MinimumTiltModel@XXIX@out{??}\fi\fi\fi\fi\fi\MinimumTiltModel@XXIX@out}\newcommand\MinimumTiltModel@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\MinimumTiltModel@XXX@out{\{"median": 0.13, "5th percentile": {-}0.63, "95th percentile": 0.9, "peak": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\MinimumTiltModel@XXX@out{0.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\MinimumTiltModel@XXX@out{{-}0.63}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\MinimumTiltModel@XXX@out{0.9}\else\ifnum\pdfstrcmp{#1}{peak}=0\def\MinimumTiltModel@XXX@out{0.02}\else\def\MinimumTiltModel@XXX@out{??}\fi\fi\fi\fi\fi\MinimumTiltModel@XXX@out}\makeatother
\makeatletter\newcommand\mzCopulaCorrelationModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@out{\{"param": \{"alpha\_1": \{"median": 1.51, "5th percentile": {-}1.06, "95th percentile": 3.03, "error plus": 1.52, "error minus": 2.57\}, "alpha\_2": \{"median": 4.34, "5th percentile": 3.0, "95th percentile": 5.75, "error plus": 1.42, "error minus": 1.33\}, "beta": \{"median": 0.91, "5th percentile": {-}0.01, "95th percentile": 2.0, "error plus": 1.09, "error minus": 0.92\}, "break\_mass": \{"median": 36.25, "5th percentile": 22.61, "95th percentile": 48.19, "error plus": 11.95, "error minus": 13.63\}, "delta\_m\_1": \{"median": 4.51, "5th percentile": 0.48, "95th percentile": 9.31, "error plus": 4.8, "error minus": 4.03\}, "delta\_m\_2": \{"median": 4.57, "5th percentile": 0.47, "95th percentile": 8.48, "error plus": 3.9, "error minus": 4.1\}, "lam\_0": \{"median": 0.37, "5th percentile": 0.11, "95th percentile": 0.66, "error plus": 0.29, "error minus": 0.27\}, "lam\_1": \{"median": 0.56, "5th percentile": 0.27, "95th percentile": 0.86, "error plus": 0.29, "error minus": 0.3\}, "lamb": \{"median": 2.7, "5th percentile": 0.58, "95th percentile": 4.1, "error plus": 1.41, "error minus": 2.12\}, "mlow\_1": \{"median": 4.89, "5th percentile": 3.2, "95th percentile": 7.68, "error plus": 2.8, "error minus": 1.68\}, "mlow\_2": \{"median": 3.49, "5th percentile": 3.03, "95th percentile": 4.76, "error plus": 1.26, "error minus": 0.47\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.76, "5th percentile": 8.09, "95th percentile": 10.32, "error plus": 0.56, "error minus": 1.67\}, "mpp\_2": \{"median": 33.13, "5th percentile": 26.76, "95th percentile": 37.39, "error plus": 4.25, "error minus": 6.37\}, "mu\_chi\_eff": \{"median": 0.04, "5th percentile": 0.02, "95th percentile": 0.06, "error plus": 0.02, "error minus": 0.02\}, "mu\_chi\_p": \{"median": 0.35, "5th percentile": 0.3, "95th percentile": 0.41, "error plus": 0.06, "error minus": 0.05\}, "sigma\_chi\_eff": \{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.02, "error minus": 0.02\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": 0.6, "5th percentile": {-}2.0, "95th percentile": 3.5, "error plus": 2.8, "error minus": 2.6, "correlated percentile": 66\}\}, "ppd": \{\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\mzCopulaCorrelationModel@out\mzCopulaCorrelationModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\mzCopulaCorrelationModel@out\mzCopulaCorrelationModel@II\else\def\mzCopulaCorrelationModel@out{??}\fi\fi\fi\mzCopulaCorrelationModel@out}\newcommand\mzCopulaCorrelationModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@I@out{\{"alpha\_1": \{"median": 1.51, "5th percentile": {-}1.06, "95th percentile": 3.03, "error plus": 1.52, "error minus": 2.57\}, "alpha\_2": \{"median": 4.34, "5th percentile": 3.0, "95th percentile": 5.75, "error plus": 1.42, "error minus": 1.33\}, "beta": \{"median": 0.91, "5th percentile": {-}0.01, "95th percentile": 2.0, "error plus": 1.09, "error minus": 0.92\}, "break\_mass": \{"median": 36.25, "5th percentile": 22.61, "95th percentile": 48.19, "error plus": 11.95, "error minus": 13.63\}, "delta\_m\_1": \{"median": 4.51, "5th percentile": 0.48, "95th percentile": 9.31, "error plus": 4.8, "error minus": 4.03\}, "delta\_m\_2": \{"median": 4.57, "5th percentile": 0.47, "95th percentile": 8.48, "error plus": 3.9, "error minus": 4.1\}, "lam\_0": \{"median": 0.37, "5th percentile": 0.11, "95th percentile": 0.66, "error plus": 0.29, "error minus": 0.27\}, "lam\_1": \{"median": 0.56, "5th percentile": 0.27, "95th percentile": 0.86, "error plus": 0.29, "error minus": 0.3\}, "lamb": \{"median": 2.7, "5th percentile": 0.58, "95th percentile": 4.1, "error plus": 1.41, "error minus": 2.12\}, "mlow\_1": \{"median": 4.89, "5th percentile": 3.2, "95th percentile": 7.68, "error plus": 2.8, "error minus": 1.68\}, "mlow\_2": \{"median": 3.49, "5th percentile": 3.03, "95th percentile": 4.76, "error plus": 1.26, "error minus": 0.47\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.76, "5th percentile": 8.09, "95th percentile": 10.32, "error plus": 0.56, "error minus": 1.67\}, "mpp\_2": \{"median": 33.13, "5th percentile": 26.76, "95th percentile": 37.39, "error plus": 4.25, "error minus": 6.37\}, "mu\_chi\_eff": \{"median": 0.04, "5th percentile": 0.02, "95th percentile": 0.06, "error plus": 0.02, "error minus": 0.02\}, "mu\_chi\_p": \{"median": 0.35, "5th percentile": 0.3, "95th percentile": 0.41, "error plus": 0.06, "error minus": 0.05\}, "sigma\_chi\_eff": \{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.02, "error minus": 0.02\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": 0.6, "5th percentile": {-}2.0, "95th percentile": 3.5, "error plus": 2.8, "error minus": 2.6, "correlated percentile": 66\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@VI\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@VII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@VIII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@IX\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@X\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XI\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XII\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XIII\else\ifnum\pdfstrcmp{#1}{mmax}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XIV\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XV\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XVI\else\ifnum\pdfstrcmp{#1}{mu_chi_eff}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi_p}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi_eff}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XIX\else\ifnum\pdfstrcmp{#1}{sigma_chi_p}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XX\else\ifnum\pdfstrcmp{#1}{kappa}=0\let\mzCopulaCorrelationModel@I@out\mzCopulaCorrelationModel@XXI\else\def\mzCopulaCorrelationModel@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@I@out}\newcommand\mzCopulaCorrelationModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@II@out{\{\}}\else\def\mzCopulaCorrelationModel@II@out{??}\fi\mzCopulaCorrelationModel@II@out}\newcommand\mzCopulaCorrelationModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@III@out{\{"median": 1.51, "5th percentile": {-}1.06, "95th percentile": 3.03, "error plus": 1.52, "error minus": 2.57\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@III@out{1.51}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@III@out{{-}1.06}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@III@out{3.03}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@III@out{1.52}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@III@out{2.57}\else\def\mzCopulaCorrelationModel@III@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@III@out}\newcommand\mzCopulaCorrelationModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@IV@out{\{"median": 4.34, "5th percentile": 3.0, "95th percentile": 5.75, "error plus": 1.42, "error minus": 1.33\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@IV@out{4.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@IV@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@IV@out{5.75}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@IV@out{1.42}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@IV@out{1.33}\else\def\mzCopulaCorrelationModel@IV@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@IV@out}\newcommand\mzCopulaCorrelationModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@V@out{\{"median": 0.91, "5th percentile": {-}0.01, "95th percentile": 2.0, "error plus": 1.09, "error minus": 0.92\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@V@out{0.91}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@V@out{{-}0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@V@out{2.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@V@out{1.09}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@V@out{0.92}\else\def\mzCopulaCorrelationModel@V@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@V@out}\newcommand\mzCopulaCorrelationModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@VI@out{\{"median": 36.25, "5th percentile": 22.61, "95th percentile": 48.19, "error plus": 11.95, "error minus": 13.63\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@VI@out{36.25}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@VI@out{22.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@VI@out{48.19}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@VI@out{11.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@VI@out{13.63}\else\def\mzCopulaCorrelationModel@VI@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@VI@out}\newcommand\mzCopulaCorrelationModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@VII@out{\{"median": 4.51, "5th percentile": 0.48, "95th percentile": 9.31, "error plus": 4.8, "error minus": 4.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@VII@out{4.51}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@VII@out{0.48}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@VII@out{9.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@VII@out{4.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@VII@out{4.03}\else\def\mzCopulaCorrelationModel@VII@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@VII@out}\newcommand\mzCopulaCorrelationModel@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@VIII@out{\{"median": 4.57, "5th percentile": 0.47, "95th percentile": 8.48, "error plus": 3.9, "error minus": 4.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@VIII@out{4.57}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@VIII@out{0.47}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@VIII@out{8.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@VIII@out{3.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@VIII@out{4.1}\else\def\mzCopulaCorrelationModel@VIII@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@VIII@out}\newcommand\mzCopulaCorrelationModel@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@IX@out{\{"median": 0.37, "5th percentile": 0.11, "95th percentile": 0.66, "error plus": 0.29, "error minus": 0.27\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@IX@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@IX@out{0.11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@IX@out{0.66}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@IX@out{0.29}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@IX@out{0.27}\else\def\mzCopulaCorrelationModel@IX@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@IX@out}\newcommand\mzCopulaCorrelationModel@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@X@out{\{"median": 0.56, "5th percentile": 0.27, "95th percentile": 0.86, "error plus": 0.29, "error minus": 0.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@X@out{0.56}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@X@out{0.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@X@out{0.86}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@X@out{0.29}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@X@out{0.3}\else\def\mzCopulaCorrelationModel@X@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@X@out}\newcommand\mzCopulaCorrelationModel@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XI@out{\{"median": 2.7, "5th percentile": 0.58, "95th percentile": 4.1, "error plus": 1.41, "error minus": 2.12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XI@out{2.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XI@out{0.58}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XI@out{4.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XI@out{1.41}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XI@out{2.12}\else\def\mzCopulaCorrelationModel@XI@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XI@out}\newcommand\mzCopulaCorrelationModel@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XII@out{\{"median": 4.89, "5th percentile": 3.2, "95th percentile": 7.68, "error plus": 2.8, "error minus": 1.68\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XII@out{4.89}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XII@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XII@out{7.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XII@out{2.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XII@out{1.68}\else\def\mzCopulaCorrelationModel@XII@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XII@out}\newcommand\mzCopulaCorrelationModel@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XIII@out{\{"median": 3.49, "5th percentile": 3.03, "95th percentile": 4.76, "error plus": 1.26, "error minus": 0.47\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XIII@out{3.49}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XIII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XIII@out{4.76}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XIII@out{1.26}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XIII@out{0.47}\else\def\mzCopulaCorrelationModel@XIII@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XIII@out}\newcommand\mzCopulaCorrelationModel@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XIV@out{\{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XIV@out{0.0}\else\def\mzCopulaCorrelationModel@XIV@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XIV@out}\newcommand\mzCopulaCorrelationModel@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XV@out{\{"median": 9.76, "5th percentile": 8.09, "95th percentile": 10.32, "error plus": 0.56, "error minus": 1.67\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XV@out{9.76}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XV@out{8.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XV@out{10.32}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XV@out{0.56}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XV@out{1.67}\else\def\mzCopulaCorrelationModel@XV@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XV@out}\newcommand\mzCopulaCorrelationModel@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XVI@out{\{"median": 33.13, "5th percentile": 26.76, "95th percentile": 37.39, "error plus": 4.25, "error minus": 6.37\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XVI@out{33.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XVI@out{26.76}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XVI@out{37.39}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XVI@out{4.25}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XVI@out{6.37}\else\def\mzCopulaCorrelationModel@XVI@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XVI@out}\newcommand\mzCopulaCorrelationModel@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XVII@out{\{"median": 0.04, "5th percentile": 0.02, "95th percentile": 0.06, "error plus": 0.02, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XVII@out{0.04}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XVII@out{0.02}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XVII@out{0.06}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XVII@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XVII@out{0.02}\else\def\mzCopulaCorrelationModel@XVII@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XVII@out}\newcommand\mzCopulaCorrelationModel@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XVIII@out{\{"median": 0.35, "5th percentile": 0.3, "95th percentile": 0.41, "error plus": 0.06, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XVIII@out{0.35}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XVIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XVIII@out{0.41}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XVIII@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XVIII@out{0.05}\else\def\mzCopulaCorrelationModel@XVIII@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XVIII@out}\newcommand\mzCopulaCorrelationModel@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XIX@out{\{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.02, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XIX@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XIX@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XIX@out{0.14}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XIX@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XIX@out{0.02}\else\def\mzCopulaCorrelationModel@XIX@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XIX@out}\newcommand\mzCopulaCorrelationModel@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XX@out{\{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XX@out{0.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XX@out{0.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XX@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XX@out{0.05}\else\def\mzCopulaCorrelationModel@XX@out{??}\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XX@out}\newcommand\mzCopulaCorrelationModel@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\mzCopulaCorrelationModel@XXI@out{\{"median": 0.6, "5th percentile": {-}2.0, "95th percentile": 3.5, "error plus": 2.8, "error minus": 2.6, "correlated percentile": 66\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\mzCopulaCorrelationModel@XXI@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\mzCopulaCorrelationModel@XXI@out{{-}2.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\mzCopulaCorrelationModel@XXI@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\mzCopulaCorrelationModel@XXI@out{2.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\mzCopulaCorrelationModel@XXI@out{2.6}\else\ifnum\pdfstrcmp{#1}{correlated percentile}=0\def\mzCopulaCorrelationModel@XXI@out{66}\else\def\mzCopulaCorrelationModel@XXI@out{??}\fi\fi\fi\fi\fi\fi\fi\mzCopulaCorrelationModel@XXI@out}\makeatother
\makeatletter\newcommand\OriginalFullMassSpectrumBGPRate[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumBGPRate@out{\{"R\_BNS": \{"50th\_percentile": 49.23959431655902, "5th\_percentile": 7.63870789460828, "95th\_percentile": 170.3250260991897, "error\_plus": 121.08543178263068, "error\_minus": 41.60088642195074, "mean": 63.83278679172662\}, "R\_NSBH": \{"50th\_percentile": 30.32940457330811, "5th\_percentile": 9.07526509046296, "95th\_percentile": 83.94604323753286, "error\_plus": 53.61663866422475, "error\_minus": 21.25413948284515, "mean": 36.45956698365504\}, "R\_BBH": \{"50th\_percentile": 19.414850041762822, "5th\_percentile": 14.582011780531317, "95th\_percentile": 26.188227956973606, "error\_plus": 6.773377915210784, "error\_minus": 4.832838261231505, "mean": 19.83182217256504\}, "R\_NS{-}Gap": \{"50th\_percentile": 15.071382002475659, "5th\_percentile": 1.1738486176884464, "95th\_percentile": 61.157050253184785, "error\_plus": 46.085668250709126, "error\_minus": 13.897533384787213, "mean": 21.135299049905807\}, "R\_BH{-}Gap": \{"50th\_percentile": 1.4853440799062816, "5th\_percentile": 0.21880998459277184, "95th\_percentile": 6.341950502253728, "error\_plus": 4.856606422347447, "error\_minus": 1.2665340953135098, "mean": 2.1710767640642694\}, "R\_Full": \{"50th\_percentile": 107.01394328339877, "5th\_percentile": 49.29117790588764, "95th\_percentile": 235.93969518355047, "error\_plus": 128.92575190015168, "error\_minus": 57.72276537751113, "mean": 120.1241759479467\}\}}\else\ifnum\pdfstrcmp{#1}{R_BNS}=0\let\OriginalFullMassSpectrumBGPRate@out\OriginalFullMassSpectrumBGPRate@I\else\ifnum\pdfstrcmp{#1}{R_NSBH}=0\let\OriginalFullMassSpectrumBGPRate@out\OriginalFullMassSpectrumBGPRate@II\else\ifnum\pdfstrcmp{#1}{R_BBH}=0\let\OriginalFullMassSpectrumBGPRate@out\OriginalFullMassSpectrumBGPRate@III\else\ifnum\pdfstrcmp{#1}{R_NS-Gap}=0\let\OriginalFullMassSpectrumBGPRate@out\OriginalFullMassSpectrumBGPRate@IV\else\ifnum\pdfstrcmp{#1}{R_BH-Gap}=0\let\OriginalFullMassSpectrumBGPRate@out\OriginalFullMassSpectrumBGPRate@V\else\ifnum\pdfstrcmp{#1}{R_Full}=0\let\OriginalFullMassSpectrumBGPRate@out\OriginalFullMassSpectrumBGPRate@VI\else\def\OriginalFullMassSpectrumBGPRate@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumBGPRate@out}\newcommand\OriginalFullMassSpectrumBGPRate@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumBGPRate@I@out{\{"50th\_percentile": 49.23959431655902, "5th\_percentile": 7.63870789460828, "95th\_percentile": 170.3250260991897, "error\_plus": 121.08543178263068, "error\_minus": 41.60088642195074, "mean": 63.83278679172662\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@I@out{49.23959431655902}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@I@out{7.63870789460828}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@I@out{170.3250260991897}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\OriginalFullMassSpectrumBGPRate@I@out{121.08543178263068}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\OriginalFullMassSpectrumBGPRate@I@out{41.60088642195074}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\OriginalFullMassSpectrumBGPRate@I@out{63.83278679172662}\else\def\OriginalFullMassSpectrumBGPRate@I@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumBGPRate@I@out}\newcommand\OriginalFullMassSpectrumBGPRate@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumBGPRate@II@out{\{"50th\_percentile": 30.32940457330811, "5th\_percentile": 9.07526509046296, "95th\_percentile": 83.94604323753286, "error\_plus": 53.61663866422475, "error\_minus": 21.25413948284515, "mean": 36.45956698365504\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@II@out{30.32940457330811}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@II@out{9.07526509046296}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@II@out{83.94604323753286}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\OriginalFullMassSpectrumBGPRate@II@out{53.61663866422475}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\OriginalFullMassSpectrumBGPRate@II@out{21.25413948284515}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\OriginalFullMassSpectrumBGPRate@II@out{36.45956698365504}\else\def\OriginalFullMassSpectrumBGPRate@II@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumBGPRate@II@out}\newcommand\OriginalFullMassSpectrumBGPRate@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumBGPRate@III@out{\{"50th\_percentile": 19.414850041762822, "5th\_percentile": 14.582011780531317, "95th\_percentile": 26.188227956973606, "error\_plus": 6.773377915210784, "error\_minus": 4.832838261231505, "mean": 19.83182217256504\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@III@out{19.414850041762822}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@III@out{14.582011780531317}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@III@out{26.188227956973606}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\OriginalFullMassSpectrumBGPRate@III@out{6.773377915210784}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\OriginalFullMassSpectrumBGPRate@III@out{4.832838261231505}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\OriginalFullMassSpectrumBGPRate@III@out{19.83182217256504}\else\def\OriginalFullMassSpectrumBGPRate@III@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumBGPRate@III@out}\newcommand\OriginalFullMassSpectrumBGPRate@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumBGPRate@IV@out{\{"50th\_percentile": 15.071382002475659, "5th\_percentile": 1.1738486176884464, "95th\_percentile": 61.157050253184785, "error\_plus": 46.085668250709126, "error\_minus": 13.897533384787213, "mean": 21.135299049905807\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@IV@out{15.071382002475659}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@IV@out{1.1738486176884464}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@IV@out{61.157050253184785}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\OriginalFullMassSpectrumBGPRate@IV@out{46.085668250709126}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\OriginalFullMassSpectrumBGPRate@IV@out{13.897533384787213}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\OriginalFullMassSpectrumBGPRate@IV@out{21.135299049905807}\else\def\OriginalFullMassSpectrumBGPRate@IV@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumBGPRate@IV@out}\newcommand\OriginalFullMassSpectrumBGPRate@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumBGPRate@V@out{\{"50th\_percentile": 1.4853440799062816, "5th\_percentile": 0.21880998459277184, "95th\_percentile": 6.341950502253728, "error\_plus": 4.856606422347447, "error\_minus": 1.2665340953135098, "mean": 2.1710767640642694\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@V@out{1.4853440799062816}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@V@out{0.21880998459277184}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@V@out{6.341950502253728}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\OriginalFullMassSpectrumBGPRate@V@out{4.856606422347447}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\OriginalFullMassSpectrumBGPRate@V@out{1.2665340953135098}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\OriginalFullMassSpectrumBGPRate@V@out{2.1710767640642694}\else\def\OriginalFullMassSpectrumBGPRate@V@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumBGPRate@V@out}\newcommand\OriginalFullMassSpectrumBGPRate@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumBGPRate@VI@out{\{"50th\_percentile": 107.01394328339877, "5th\_percentile": 49.29117790588764, "95th\_percentile": 235.93969518355047, "error\_plus": 128.92575190015168, "error\_minus": 57.72276537751113, "mean": 120.1241759479467\}}\else\ifnum\pdfstrcmp{#1}{50th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@VI@out{107.01394328339877}\else\ifnum\pdfstrcmp{#1}{5th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@VI@out{49.29117790588764}\else\ifnum\pdfstrcmp{#1}{95th_percentile}=0\def\OriginalFullMassSpectrumBGPRate@VI@out{235.93969518355047}\else\ifnum\pdfstrcmp{#1}{error_plus}=0\def\OriginalFullMassSpectrumBGPRate@VI@out{128.92575190015168}\else\ifnum\pdfstrcmp{#1}{error_minus}=0\def\OriginalFullMassSpectrumBGPRate@VI@out{57.72276537751113}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\OriginalFullMassSpectrumBGPRate@VI@out{120.1241759479467}\else\def\OriginalFullMassSpectrumBGPRate@VI@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumBGPRate@VI@out}\makeatother
\makeatletter\newcommand\OriginalFullMassSpectrumPDB[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@out{\{"ppd": \{"rates": \{"BNS": \{"median": 13.18, "error plus": 122.51, "error minus": 11.91, "5th percentile": 1.27, "95th percentile": 135.69\}, "NSBH": \{"median": 2.92, "error plus": 34.19, "error minus": 2.68, "5th percentile": 0.24, "95th percentile": 37.11\}, "BBH": \{"median": 2.27, "error plus": 24.88, "error minus": 2.04, "5th percentile": 0.23, "95th percentile": 27.15\}, "NS{-}Gap": \{"median": 0.07, "error plus": 1.2, "error minus": 0.07, "5th percentile": 0.0, "95th percentile": 1.27\}, "BH{-}Gap": \{"median": 0.0, "error plus": 0.0, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.0\}, "Full": \{"median": 19.7, "error plus": 178.42, "error minus": 17.75, "5th percentile": 1.96, "95th percentile": 198.12\}\}\}\}}\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\OriginalFullMassSpectrumPDB@out\OriginalFullMassSpectrumPDB@I\else\def\OriginalFullMassSpectrumPDB@out{??}\fi\fi\OriginalFullMassSpectrumPDB@out}\newcommand\OriginalFullMassSpectrumPDB@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@I@out{\{"rates": \{"BNS": \{"median": 13.18, "error plus": 122.51, "error minus": 11.91, "5th percentile": 1.27, "95th percentile": 135.69\}, "NSBH": \{"median": 2.92, "error plus": 34.19, "error minus": 2.68, "5th percentile": 0.24, "95th percentile": 37.11\}, "BBH": \{"median": 2.27, "error plus": 24.88, "error minus": 2.04, "5th percentile": 0.23, "95th percentile": 27.15\}, "NS{-}Gap": \{"median": 0.07, "error plus": 1.2, "error minus": 0.07, "5th percentile": 0.0, "95th percentile": 1.27\}, "BH{-}Gap": \{"median": 0.0, "error plus": 0.0, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.0\}, "Full": \{"median": 19.7, "error plus": 178.42, "error minus": 17.75, "5th percentile": 1.96, "95th percentile": 198.12\}\}\}}\else\ifnum\pdfstrcmp{#1}{rates}=0\let\OriginalFullMassSpectrumPDB@I@out\OriginalFullMassSpectrumPDB@II\else\def\OriginalFullMassSpectrumPDB@I@out{??}\fi\fi\OriginalFullMassSpectrumPDB@I@out}\newcommand\OriginalFullMassSpectrumPDB@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@II@out{\{"BNS": \{"median": 13.18, "error plus": 122.51, "error minus": 11.91, "5th percentile": 1.27, "95th percentile": 135.69\}, "NSBH": \{"median": 2.92, "error plus": 34.19, "error minus": 2.68, "5th percentile": 0.24, "95th percentile": 37.11\}, "BBH": \{"median": 2.27, "error plus": 24.88, "error minus": 2.04, "5th percentile": 0.23, "95th percentile": 27.15\}, "NS{-}Gap": \{"median": 0.07, "error plus": 1.2, "error minus": 0.07, "5th percentile": 0.0, "95th percentile": 1.27\}, "BH{-}Gap": \{"median": 0.0, "error plus": 0.0, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.0\}, "Full": \{"median": 19.7, "error plus": 178.42, "error minus": 17.75, "5th percentile": 1.96, "95th percentile": 198.12\}\}}\else\ifnum\pdfstrcmp{#1}{BNS}=0\let\OriginalFullMassSpectrumPDB@II@out\OriginalFullMassSpectrumPDB@III\else\ifnum\pdfstrcmp{#1}{NSBH}=0\let\OriginalFullMassSpectrumPDB@II@out\OriginalFullMassSpectrumPDB@IV\else\ifnum\pdfstrcmp{#1}{BBH}=0\let\OriginalFullMassSpectrumPDB@II@out\OriginalFullMassSpectrumPDB@V\else\ifnum\pdfstrcmp{#1}{NS-Gap}=0\let\OriginalFullMassSpectrumPDB@II@out\OriginalFullMassSpectrumPDB@VI\else\ifnum\pdfstrcmp{#1}{BH-Gap}=0\let\OriginalFullMassSpectrumPDB@II@out\OriginalFullMassSpectrumPDB@VII\else\ifnum\pdfstrcmp{#1}{Full}=0\let\OriginalFullMassSpectrumPDB@II@out\OriginalFullMassSpectrumPDB@VIII\else\def\OriginalFullMassSpectrumPDB@II@out{??}\fi\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumPDB@II@out}\newcommand\OriginalFullMassSpectrumPDB@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@III@out{\{"median": 13.18, "error plus": 122.51, "error minus": 11.91, "5th percentile": 1.27, "95th percentile": 135.69\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OriginalFullMassSpectrumPDB@III@out{13.18}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OriginalFullMassSpectrumPDB@III@out{122.51}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OriginalFullMassSpectrumPDB@III@out{11.91}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\OriginalFullMassSpectrumPDB@III@out{1.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\OriginalFullMassSpectrumPDB@III@out{135.69}\else\def\OriginalFullMassSpectrumPDB@III@out{??}\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumPDB@III@out}\newcommand\OriginalFullMassSpectrumPDB@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@IV@out{\{"median": 2.92, "error plus": 34.19, "error minus": 2.68, "5th percentile": 0.24, "95th percentile": 37.11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OriginalFullMassSpectrumPDB@IV@out{2.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OriginalFullMassSpectrumPDB@IV@out{34.19}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OriginalFullMassSpectrumPDB@IV@out{2.68}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\OriginalFullMassSpectrumPDB@IV@out{0.24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\OriginalFullMassSpectrumPDB@IV@out{37.11}\else\def\OriginalFullMassSpectrumPDB@IV@out{??}\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumPDB@IV@out}\newcommand\OriginalFullMassSpectrumPDB@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@V@out{\{"median": 2.27, "error plus": 24.88, "error minus": 2.04, "5th percentile": 0.23, "95th percentile": 27.15\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OriginalFullMassSpectrumPDB@V@out{2.27}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OriginalFullMassSpectrumPDB@V@out{24.88}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OriginalFullMassSpectrumPDB@V@out{2.04}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\OriginalFullMassSpectrumPDB@V@out{0.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\OriginalFullMassSpectrumPDB@V@out{27.15}\else\def\OriginalFullMassSpectrumPDB@V@out{??}\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumPDB@V@out}\newcommand\OriginalFullMassSpectrumPDB@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@VI@out{\{"median": 0.07, "error plus": 1.2, "error minus": 0.07, "5th percentile": 0.0, "95th percentile": 1.27\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OriginalFullMassSpectrumPDB@VI@out{0.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OriginalFullMassSpectrumPDB@VI@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OriginalFullMassSpectrumPDB@VI@out{0.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\OriginalFullMassSpectrumPDB@VI@out{0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\OriginalFullMassSpectrumPDB@VI@out{1.27}\else\def\OriginalFullMassSpectrumPDB@VI@out{??}\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumPDB@VI@out}\newcommand\OriginalFullMassSpectrumPDB@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@VII@out{\{"median": 0.0, "error plus": 0.0, "error minus": 0.0, "5th percentile": 0.0, "95th percentile": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OriginalFullMassSpectrumPDB@VII@out{0.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OriginalFullMassSpectrumPDB@VII@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OriginalFullMassSpectrumPDB@VII@out{0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\OriginalFullMassSpectrumPDB@VII@out{0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\OriginalFullMassSpectrumPDB@VII@out{0.0}\else\def\OriginalFullMassSpectrumPDB@VII@out{??}\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumPDB@VII@out}\newcommand\OriginalFullMassSpectrumPDB@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OriginalFullMassSpectrumPDB@VIII@out{\{"median": 19.7, "error plus": 178.42, "error minus": 17.75, "5th percentile": 1.96, "95th percentile": 198.12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OriginalFullMassSpectrumPDB@VIII@out{19.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OriginalFullMassSpectrumPDB@VIII@out{178.42}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OriginalFullMassSpectrumPDB@VIII@out{17.75}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\OriginalFullMassSpectrumPDB@VIII@out{1.96}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\OriginalFullMassSpectrumPDB@VIII@out{198.12}\else\def\OriginalFullMassSpectrumPDB@VIII@out{??}\fi\fi\fi\fi\fi\fi\OriginalFullMassSpectrumPDB@VIII@out}\makeatother
\makeatletter\newcommand\OutlierTestMassiveEvent[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@out{\{"percentilemmax300": \{"total\_mass\_source": \{"median": 87, "error plus": 6, "error minus": 10\}, "mass\_1\_source": \{"median": 82, "error plus": 9, "error minus": 11\}, "mass\_2\_source": \{"median": 87, "error plus": 8, "error minus": 12\}\}, "percentilemmaxlessthan300": \{"total\_mass\_source": \{"median": 94, "error plus": 4, "error minus": 5\}, "mass\_1\_source": \{"median": 92, "error plus": 5, "error minus": 7\}, "mass\_2\_source": \{"median": 94, "error plus": 4, "error minus": 9\}\}\}}\else\ifnum\pdfstrcmp{#1}{percentilemmax300}=0\let\OutlierTestMassiveEvent@out\OutlierTestMassiveEvent@I\else\ifnum\pdfstrcmp{#1}{percentilemmaxlessthan300}=0\let\OutlierTestMassiveEvent@out\OutlierTestMassiveEvent@II\else\def\OutlierTestMassiveEvent@out{??}\fi\fi\fi\OutlierTestMassiveEvent@out}\newcommand\OutlierTestMassiveEvent@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@I@out{\{"total\_mass\_source": \{"median": 87, "error plus": 6, "error minus": 10\}, "mass\_1\_source": \{"median": 82, "error plus": 9, "error minus": 11\}, "mass\_2\_source": \{"median": 87, "error plus": 8, "error minus": 12\}\}}\else\ifnum\pdfstrcmp{#1}{total_mass_source}=0\let\OutlierTestMassiveEvent@I@out\OutlierTestMassiveEvent@III\else\ifnum\pdfstrcmp{#1}{mass_1_source}=0\let\OutlierTestMassiveEvent@I@out\OutlierTestMassiveEvent@IV\else\ifnum\pdfstrcmp{#1}{mass_2_source}=0\let\OutlierTestMassiveEvent@I@out\OutlierTestMassiveEvent@V\else\def\OutlierTestMassiveEvent@I@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@I@out}\newcommand\OutlierTestMassiveEvent@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@II@out{\{"total\_mass\_source": \{"median": 94, "error plus": 4, "error minus": 5\}, "mass\_1\_source": \{"median": 92, "error plus": 5, "error minus": 7\}, "mass\_2\_source": \{"median": 94, "error plus": 4, "error minus": 9\}\}}\else\ifnum\pdfstrcmp{#1}{total_mass_source}=0\let\OutlierTestMassiveEvent@II@out\OutlierTestMassiveEvent@VI\else\ifnum\pdfstrcmp{#1}{mass_1_source}=0\let\OutlierTestMassiveEvent@II@out\OutlierTestMassiveEvent@VII\else\ifnum\pdfstrcmp{#1}{mass_2_source}=0\let\OutlierTestMassiveEvent@II@out\OutlierTestMassiveEvent@VIII\else\def\OutlierTestMassiveEvent@II@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@II@out}\newcommand\OutlierTestMassiveEvent@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@III@out{\{"median": 87, "error plus": 6, "error minus": 10\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OutlierTestMassiveEvent@III@out{87}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OutlierTestMassiveEvent@III@out{6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OutlierTestMassiveEvent@III@out{10}\else\def\OutlierTestMassiveEvent@III@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@III@out}\newcommand\OutlierTestMassiveEvent@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@IV@out{\{"median": 82, "error plus": 9, "error minus": 11\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OutlierTestMassiveEvent@IV@out{82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OutlierTestMassiveEvent@IV@out{9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OutlierTestMassiveEvent@IV@out{11}\else\def\OutlierTestMassiveEvent@IV@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@IV@out}\newcommand\OutlierTestMassiveEvent@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@V@out{\{"median": 87, "error plus": 8, "error minus": 12\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OutlierTestMassiveEvent@V@out{87}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OutlierTestMassiveEvent@V@out{8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OutlierTestMassiveEvent@V@out{12}\else\def\OutlierTestMassiveEvent@V@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@V@out}\newcommand\OutlierTestMassiveEvent@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@VI@out{\{"median": 94, "error plus": 4, "error minus": 5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OutlierTestMassiveEvent@VI@out{94}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OutlierTestMassiveEvent@VI@out{4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OutlierTestMassiveEvent@VI@out{5}\else\def\OutlierTestMassiveEvent@VI@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@VI@out}\newcommand\OutlierTestMassiveEvent@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@VII@out{\{"median": 92, "error plus": 5, "error minus": 7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OutlierTestMassiveEvent@VII@out{92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OutlierTestMassiveEvent@VII@out{5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OutlierTestMassiveEvent@VII@out{7}\else\def\OutlierTestMassiveEvent@VII@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@VII@out}\newcommand\OutlierTestMassiveEvent@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\OutlierTestMassiveEvent@VIII@out{\{"median": 94, "error plus": 4, "error minus": 9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\OutlierTestMassiveEvent@VIII@out{94}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\OutlierTestMassiveEvent@VIII@out{4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\OutlierTestMassiveEvent@VIII@out{9}\else\def\OutlierTestMassiveEvent@VIII@out{??}\fi\fi\fi\fi\OutlierTestMassiveEvent@VIII@out}\makeatother
\makeatletter\newcommand\peakcutsodapop[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@out{\{"woGW190814": \{"param": \{"mu": \{"median": 1.4, "error plus": 0.48, "error minus": 0.25, "5th percentile": 1.1, "95th percentile": 1.8\}, "sigma": \{"median": 0.68, "error plus": 1.2, "error minus": 0.45, "5th percentile": 0.23, "95th percentile": 1.9\}, "m\_min": \{"median": 1.1, "error plus": 0.14, "error minus": 0.092, "5th percentile": 1.0, "95th percentile": 1.2\}, "m\_max": \{"median": 2.0, "error plus": 0.86, "error minus": 0.13, "5th percentile": 1.8, "95th percentile": 2.8\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.6, "5th percentile": 1.3, "95th percentile": 1.9\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.1, "95th percentile": 1.7\}, "mass\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 1.9\}\}\}, "wGW190814": \{"param": \{"mu": \{"median": 1.3, "error plus": 0.47, "error minus": 0.21, "5th percentile": 1.1, "95th percentile": 1.7\}, "sigma": \{"median": 0.54, "error plus": 1.0, "error minus": 0.18, "5th percentile": 0.36, "95th percentile": 1.5\}, "m\_min": \{"median": 1.1, "error plus": 0.15, "error minus": 0.081, "5th percentile": 1.0, "95th percentile": 1.2\}, "m\_max": \{"median": 2.8, "error plus": 0.22, "error minus": 0.19, "5th percentile": 2.6, "95th percentile": 3.0\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.8, "5th percentile": 1.3, "95th percentile": 2.4\}, "mass\_2\_source": \{"median": 1.4, "5th percentile": 1.1, "95th percentile": 1.9\}, "mass\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.3\}\}\}\}}\else\ifnum\pdfstrcmp{#1}{woGW190814}=0\let\peakcutsodapop@out\peakcutsodapop@I\else\ifnum\pdfstrcmp{#1}{wGW190814}=0\let\peakcutsodapop@out\peakcutsodapop@II\else\def\peakcutsodapop@out{??}\fi\fi\fi\peakcutsodapop@out}\newcommand\peakcutsodapop@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@I@out{\{"param": \{"mu": \{"median": 1.4, "error plus": 0.48, "error minus": 0.25, "5th percentile": 1.1, "95th percentile": 1.8\}, "sigma": \{"median": 0.68, "error plus": 1.2, "error minus": 0.45, "5th percentile": 0.23, "95th percentile": 1.9\}, "m\_min": \{"median": 1.1, "error plus": 0.14, "error minus": 0.092, "5th percentile": 1.0, "95th percentile": 1.2\}, "m\_max": \{"median": 2.0, "error plus": 0.86, "error minus": 0.13, "5th percentile": 1.8, "95th percentile": 2.8\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.6, "5th percentile": 1.3, "95th percentile": 1.9\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.1, "95th percentile": 1.7\}, "mass\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 1.9\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\peakcutsodapop@I@out\peakcutsodapop@III\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\peakcutsodapop@I@out\peakcutsodapop@IV\else\def\peakcutsodapop@I@out{??}\fi\fi\fi\peakcutsodapop@I@out}\newcommand\peakcutsodapop@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@II@out{\{"param": \{"mu": \{"median": 1.3, "error plus": 0.47, "error minus": 0.21, "5th percentile": 1.1, "95th percentile": 1.7\}, "sigma": \{"median": 0.54, "error plus": 1.0, "error minus": 0.18, "5th percentile": 0.36, "95th percentile": 1.5\}, "m\_min": \{"median": 1.1, "error plus": 0.15, "error minus": 0.081, "5th percentile": 1.0, "95th percentile": 1.2\}, "m\_max": \{"median": 2.8, "error plus": 0.22, "error minus": 0.19, "5th percentile": 2.6, "95th percentile": 3.0\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.8, "5th percentile": 1.3, "95th percentile": 2.4\}, "mass\_2\_source": \{"median": 1.4, "5th percentile": 1.1, "95th percentile": 1.9\}, "mass\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.3\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\peakcutsodapop@II@out\peakcutsodapop@V\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\peakcutsodapop@II@out\peakcutsodapop@VI\else\def\peakcutsodapop@II@out{??}\fi\fi\fi\peakcutsodapop@II@out}\newcommand\peakcutsodapop@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@III@out{\{"mu": \{"median": 1.4, "error plus": 0.48, "error minus": 0.25, "5th percentile": 1.1, "95th percentile": 1.8\}, "sigma": \{"median": 0.68, "error plus": 1.2, "error minus": 0.45, "5th percentile": 0.23, "95th percentile": 1.9\}, "m\_min": \{"median": 1.1, "error plus": 0.14, "error minus": 0.092, "5th percentile": 1.0, "95th percentile": 1.2\}, "m\_max": \{"median": 2.0, "error plus": 0.86, "error minus": 0.13, "5th percentile": 1.8, "95th percentile": 2.8\}\}}\else\ifnum\pdfstrcmp{#1}{mu}=0\let\peakcutsodapop@III@out\peakcutsodapop@VII\else\ifnum\pdfstrcmp{#1}{sigma}=0\let\peakcutsodapop@III@out\peakcutsodapop@VIII\else\ifnum\pdfstrcmp{#1}{m_min}=0\let\peakcutsodapop@III@out\peakcutsodapop@IX\else\ifnum\pdfstrcmp{#1}{m_max}=0\let\peakcutsodapop@III@out\peakcutsodapop@X\else\def\peakcutsodapop@III@out{??}\fi\fi\fi\fi\fi\peakcutsodapop@III@out}\newcommand\peakcutsodapop@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@IV@out{\{"mass\_1\_source": \{"median": 1.6, "5th percentile": 1.3, "95th percentile": 1.9\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.1, "95th percentile": 1.7\}, "mass\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 1.9\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1_source}=0\let\peakcutsodapop@IV@out\peakcutsodapop@XI\else\ifnum\pdfstrcmp{#1}{mass_2_source}=0\let\peakcutsodapop@IV@out\peakcutsodapop@XII\else\ifnum\pdfstrcmp{#1}{mass_source}=0\let\peakcutsodapop@IV@out\peakcutsodapop@XIII\else\def\peakcutsodapop@IV@out{??}\fi\fi\fi\fi\peakcutsodapop@IV@out}\newcommand\peakcutsodapop@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@V@out{\{"mu": \{"median": 1.3, "error plus": 0.47, "error minus": 0.21, "5th percentile": 1.1, "95th percentile": 1.7\}, "sigma": \{"median": 0.54, "error plus": 1.0, "error minus": 0.18, "5th percentile": 0.36, "95th percentile": 1.5\}, "m\_min": \{"median": 1.1, "error plus": 0.15, "error minus": 0.081, "5th percentile": 1.0, "95th percentile": 1.2\}, "m\_max": \{"median": 2.8, "error plus": 0.22, "error minus": 0.19, "5th percentile": 2.6, "95th percentile": 3.0\}\}}\else\ifnum\pdfstrcmp{#1}{mu}=0\let\peakcutsodapop@V@out\peakcutsodapop@XIV\else\ifnum\pdfstrcmp{#1}{sigma}=0\let\peakcutsodapop@V@out\peakcutsodapop@XV\else\ifnum\pdfstrcmp{#1}{m_min}=0\let\peakcutsodapop@V@out\peakcutsodapop@XVI\else\ifnum\pdfstrcmp{#1}{m_max}=0\let\peakcutsodapop@V@out\peakcutsodapop@XVII\else\def\peakcutsodapop@V@out{??}\fi\fi\fi\fi\fi\peakcutsodapop@V@out}\newcommand\peakcutsodapop@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@VI@out{\{"mass\_1\_source": \{"median": 1.8, "5th percentile": 1.3, "95th percentile": 2.4\}, "mass\_2\_source": \{"median": 1.4, "5th percentile": 1.1, "95th percentile": 1.9\}, "mass\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.3\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1_source}=0\let\peakcutsodapop@VI@out\peakcutsodapop@XVIII\else\ifnum\pdfstrcmp{#1}{mass_2_source}=0\let\peakcutsodapop@VI@out\peakcutsodapop@XIX\else\ifnum\pdfstrcmp{#1}{mass_source}=0\let\peakcutsodapop@VI@out\peakcutsodapop@XX\else\def\peakcutsodapop@VI@out{??}\fi\fi\fi\fi\peakcutsodapop@VI@out}\newcommand\peakcutsodapop@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@VII@out{\{"median": 1.4, "error plus": 0.48, "error minus": 0.25, "5th percentile": 1.1, "95th percentile": 1.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@VII@out{1.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@VII@out{0.48}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@VII@out{0.25}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@VII@out{1.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@VII@out{1.8}\else\def\peakcutsodapop@VII@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@VII@out}\newcommand\peakcutsodapop@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@VIII@out{\{"median": 0.68, "error plus": 1.2, "error minus": 0.45, "5th percentile": 0.23, "95th percentile": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@VIII@out{0.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@VIII@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@VIII@out{0.45}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@VIII@out{0.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@VIII@out{1.9}\else\def\peakcutsodapop@VIII@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@VIII@out}\newcommand\peakcutsodapop@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@IX@out{\{"median": 1.1, "error plus": 0.14, "error minus": 0.092, "5th percentile": 1.0, "95th percentile": 1.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@IX@out{1.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@IX@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@IX@out{0.092}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@IX@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@IX@out{1.2}\else\def\peakcutsodapop@IX@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@IX@out}\newcommand\peakcutsodapop@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@X@out{\{"median": 2.0, "error plus": 0.86, "error minus": 0.13, "5th percentile": 1.8, "95th percentile": 2.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@X@out{2.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@X@out{0.86}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@X@out{0.13}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@X@out{1.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@X@out{2.8}\else\def\peakcutsodapop@X@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@X@out}\newcommand\peakcutsodapop@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XI@out{\{"median": 1.6, "5th percentile": 1.3, "95th percentile": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XI@out{1.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XI@out{1.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XI@out{1.9}\else\def\peakcutsodapop@XI@out{??}\fi\fi\fi\fi\peakcutsodapop@XI@out}\newcommand\peakcutsodapop@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XII@out{\{"median": 1.3, "5th percentile": 1.1, "95th percentile": 1.7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XII@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XII@out{1.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XII@out{1.7}\else\def\peakcutsodapop@XII@out{??}\fi\fi\fi\fi\peakcutsodapop@XII@out}\newcommand\peakcutsodapop@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XIII@out{\{"median": 1.5, "5th percentile": 1.2, "95th percentile": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XIII@out{1.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XIII@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XIII@out{1.9}\else\def\peakcutsodapop@XIII@out{??}\fi\fi\fi\fi\peakcutsodapop@XIII@out}\newcommand\peakcutsodapop@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XIV@out{\{"median": 1.3, "error plus": 0.47, "error minus": 0.21, "5th percentile": 1.1, "95th percentile": 1.7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XIV@out{1.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@XIV@out{0.47}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@XIV@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XIV@out{1.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XIV@out{1.7}\else\def\peakcutsodapop@XIV@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@XIV@out}\newcommand\peakcutsodapop@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XV@out{\{"median": 0.54, "error plus": 1.0, "error minus": 0.18, "5th percentile": 0.36, "95th percentile": 1.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XV@out{0.54}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@XV@out{1.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@XV@out{0.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XV@out{0.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XV@out{1.5}\else\def\peakcutsodapop@XV@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@XV@out}\newcommand\peakcutsodapop@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XVI@out{\{"median": 1.1, "error plus": 0.15, "error minus": 0.081, "5th percentile": 1.0, "95th percentile": 1.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XVI@out{1.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@XVI@out{0.15}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@XVI@out{0.081}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XVI@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XVI@out{1.2}\else\def\peakcutsodapop@XVI@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@XVI@out}\newcommand\peakcutsodapop@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XVII@out{\{"median": 2.8, "error plus": 0.22, "error minus": 0.19, "5th percentile": 2.6, "95th percentile": 3.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XVII@out{2.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\peakcutsodapop@XVII@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\peakcutsodapop@XVII@out{0.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XVII@out{2.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XVII@out{3.0}\else\def\peakcutsodapop@XVII@out{??}\fi\fi\fi\fi\fi\fi\peakcutsodapop@XVII@out}\newcommand\peakcutsodapop@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XVIII@out{\{"median": 1.8, "5th percentile": 1.3, "95th percentile": 2.4\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XVIII@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XVIII@out{1.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XVIII@out{2.4}\else\def\peakcutsodapop@XVIII@out{??}\fi\fi\fi\fi\peakcutsodapop@XVIII@out}\newcommand\peakcutsodapop@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XIX@out{\{"median": 1.4, "5th percentile": 1.1, "95th percentile": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XIX@out{1.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XIX@out{1.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XIX@out{1.9}\else\def\peakcutsodapop@XIX@out{??}\fi\fi\fi\fi\peakcutsodapop@XIX@out}\newcommand\peakcutsodapop@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\peakcutsodapop@XX@out{\{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\peakcutsodapop@XX@out{1.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\peakcutsodapop@XX@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\peakcutsodapop@XX@out{2.3}\else\def\peakcutsodapop@XX@out{??}\fi\fi\fi\fi\peakcutsodapop@XX@out}\makeatother
\makeatletter\newcommand\PowerLawPeak[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@out{\{"alpha": \{"median": "3.5", "error plus": "0.35", "error minus": "0.31", "5th percentile": "3.2", "95th percentile": "3.8"\}, "beta": \{"median": "1.1", "error plus": "1.2", "error minus": "1.00", "5th percentile": "0.095", "95th percentile": "2.3"\}, "delta\_m": \{"median": "4.7", "error plus": "2.5", "error minus": "2.3", "5th percentile": "2.4", "95th percentile": "7.2"\}, "mmin": \{"median": "5.2", "error plus": "0.75", "error minus": "1.2", "5th percentile": "4.0", "95th percentile": "5.9"\}, "lam": \{"median": "0.029", "error plus": "0.029", "error minus": "0.017", "5th percentile": "0.012", "95th percentile": "0.058"\}, "mpp": \{"median": "34", "error plus": "1.9", "error minus": "2.9", "5th percentile": "31", "95th percentile": "35"\}, "sigpp": \{"median": "3.8", "error plus": "4.0", "error minus": "1.8", "5th percentile": "1.9", "95th percentile": "7.8"\}, "mu\_chi": \{"median": "0.083", "error plus": "0.14", "error minus": "0.076", "5th percentile": "0.0070", "95th percentile": "0.22"\}, "sigma\_chi": \{"median": "0.33", "error plus": "0.074", "error minus": "0.078", "5th percentile": "0.25", "95th percentile": "0.40"\}, "xi\_spin": \{"median": "0.64", "error plus": "0.33", "error minus": "0.54", "5th percentile": "0.10", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.40", "error plus": "0.55", "error minus": "0.84", "5th percentile": "{-}0.45", "95th percentile": "0.94"\}, "sigma\_spin": \{"median": "1.3", "error plus": "2.3", "error minus": "0.87", "5th percentile": "0.43", "95th percentile": "3.6"\}, "lamb": \{"median": "3.3", "error plus": "0.95", "error minus": "0.97", "5th percentile": "2.4", "95th percentile": "4.3"\}, "rate": \{"median": "15", "error plus": "5.9", "error minus": "4.5", "5th percentile": "11", "95th percentile": "21"\}\}}\else\ifnum\pdfstrcmp{#1}{alpha}=0\let\PowerLawPeak@out\PowerLawPeak@I\else\ifnum\pdfstrcmp{#1}{beta}=0\let\PowerLawPeak@out\PowerLawPeak@II\else\ifnum\pdfstrcmp{#1}{delta_m}=0\let\PowerLawPeak@out\PowerLawPeak@III\else\ifnum\pdfstrcmp{#1}{mmin}=0\let\PowerLawPeak@out\PowerLawPeak@IV\else\ifnum\pdfstrcmp{#1}{lam}=0\let\PowerLawPeak@out\PowerLawPeak@V\else\ifnum\pdfstrcmp{#1}{mpp}=0\let\PowerLawPeak@out\PowerLawPeak@VI\else\ifnum\pdfstrcmp{#1}{sigpp}=0\let\PowerLawPeak@out\PowerLawPeak@VII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\PowerLawPeak@out\PowerLawPeak@VIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\PowerLawPeak@out\PowerLawPeak@IX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\PowerLawPeak@out\PowerLawPeak@X\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\PowerLawPeak@out\PowerLawPeak@XI\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\PowerLawPeak@out\PowerLawPeak@XII\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\PowerLawPeak@out\PowerLawPeak@XIII\else\ifnum\pdfstrcmp{#1}{rate}=0\let\PowerLawPeak@out\PowerLawPeak@XIV\else\def\PowerLawPeak@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\PowerLawPeak@out}\newcommand\PowerLawPeak@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@I@out{\{"median": "3.5", "error plus": "0.35", "error minus": "0.31", "5th percentile": "3.2", "95th percentile": "3.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@I@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@I@out{0.35}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@I@out{0.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@I@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@I@out{3.8}\else\def\PowerLawPeak@I@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@I@out}\newcommand\PowerLawPeak@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@II@out{\{"median": "1.1", "error plus": "1.2", "error minus": "1.00", "5th percentile": "0.095", "95th percentile": "2.3"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@II@out{1.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@II@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@II@out{1.00}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@II@out{0.095}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@II@out{2.3}\else\def\PowerLawPeak@II@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@II@out}\newcommand\PowerLawPeak@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@III@out{\{"median": "4.7", "error plus": "2.5", "error minus": "2.3", "5th percentile": "2.4", "95th percentile": "7.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@III@out{4.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@III@out{2.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@III@out{2.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@III@out{2.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@III@out{7.2}\else\def\PowerLawPeak@III@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@III@out}\newcommand\PowerLawPeak@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@IV@out{\{"median": "5.2", "error plus": "0.75", "error minus": "1.2", "5th percentile": "4.0", "95th percentile": "5.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@IV@out{5.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@IV@out{0.75}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@IV@out{1.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@IV@out{4.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@IV@out{5.9}\else\def\PowerLawPeak@IV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@IV@out}\newcommand\PowerLawPeak@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@V@out{\{"median": "0.029", "error plus": "0.029", "error minus": "0.017", "5th percentile": "0.012", "95th percentile": "0.058"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@V@out{0.029}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@V@out{0.029}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@V@out{0.017}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@V@out{0.012}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@V@out{0.058}\else\def\PowerLawPeak@V@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@V@out}\newcommand\PowerLawPeak@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@VI@out{\{"median": "34", "error plus": "1.9", "error minus": "2.9", "5th percentile": "31", "95th percentile": "35"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@VI@out{34}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@VI@out{1.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@VI@out{2.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@VI@out{31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@VI@out{35}\else\def\PowerLawPeak@VI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@VI@out}\newcommand\PowerLawPeak@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@VII@out{\{"median": "3.8", "error plus": "4.0", "error minus": "1.8", "5th percentile": "1.9", "95th percentile": "7.8"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@VII@out{3.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@VII@out{4.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@VII@out{1.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@VII@out{1.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@VII@out{7.8}\else\def\PowerLawPeak@VII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@VII@out}\newcommand\PowerLawPeak@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@VIII@out{\{"median": "0.083", "error plus": "0.14", "error minus": "0.076", "5th percentile": "0.0070", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@VIII@out{0.083}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@VIII@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@VIII@out{0.076}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@VIII@out{0.0070}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@VIII@out{0.22}\else\def\PowerLawPeak@VIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@VIII@out}\newcommand\PowerLawPeak@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@IX@out{\{"median": "0.33", "error plus": "0.074", "error minus": "0.078", "5th percentile": "0.25", "95th percentile": "0.40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@IX@out{0.33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@IX@out{0.074}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@IX@out{0.078}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@IX@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@IX@out{0.40}\else\def\PowerLawPeak@IX@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@IX@out}\newcommand\PowerLawPeak@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@X@out{\{"median": "0.64", "error plus": "0.33", "error minus": "0.54", "5th percentile": "0.10", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@X@out{0.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@X@out{0.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@X@out{0.54}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@X@out{0.10}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@X@out{0.97}\else\def\PowerLawPeak@X@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@X@out}\newcommand\PowerLawPeak@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@XI@out{\{"median": "0.40", "error plus": "0.55", "error minus": "0.84", "5th percentile": "{-}0.45", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@XI@out{0.40}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@XI@out{0.55}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@XI@out{0.84}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@XI@out{{-}0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@XI@out{0.94}\else\def\PowerLawPeak@XI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@XI@out}\newcommand\PowerLawPeak@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@XII@out{\{"median": "1.3", "error plus": "2.3", "error minus": "0.87", "5th percentile": "0.43", "95th percentile": "3.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@XII@out{1.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@XII@out{2.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@XII@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@XII@out{0.43}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@XII@out{3.6}\else\def\PowerLawPeak@XII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@XII@out}\newcommand\PowerLawPeak@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@XIII@out{\{"median": "3.3", "error plus": "0.95", "error minus": "0.97", "5th percentile": "2.4", "95th percentile": "4.3"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@XIII@out{3.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@XIII@out{0.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@XIII@out{0.97}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@XIII@out{2.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@XIII@out{4.3}\else\def\PowerLawPeak@XIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@XIII@out}\newcommand\PowerLawPeak@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawPeak@XIV@out{\{"median": "15", "error plus": "5.9", "error minus": "4.5", "5th percentile": "11", "95th percentile": "21"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawPeak@XIV@out{15}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawPeak@XIV@out{5.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawPeak@XIV@out{4.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawPeak@XIV@out{11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawPeak@XIV@out{21}\else\def\PowerLawPeak@XIV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawPeak@XIV@out}\makeatother
\makeatletter\newcommand\PowerLawTwoPeakOneBBH[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@out{\{"alpha\_1": \{"median": "0.54", "error plus": "0.96", "error minus": "1.2", "5th percentile": "{-}0.70", "95th percentile": "1.5"\}, "alpha\_2": \{"median": "5.6", "error plus": "1.0", "error minus": "0.79", "5th percentile": "4.8", "95th percentile": "6.6"\}, "beta": \{"median": "1.3", "error plus": "1.3", "error minus": "1.1", "5th percentile": "0.19", "95th percentile": "2.6"\}, "mlow\_1": \{"median": "4.9", "error plus": "3.3", "error minus": "1.7", "5th percentile": "3.2", "95th percentile": "8.2"\}, "mlow\_2": \{"median": "3.5", "error plus": "1.2", "error minus": "0.44", "5th percentile": "3.0", "95th percentile": "4.7"\}, "break\_mass": \{"median": "34.1", "error plus": "3.8", "error minus": "3.3", "5th percentile": "31", "95th percentile": "38"\}, "mpp\_1": \{"median": "9.7", "error plus": "0.49", "error minus": "2.0", "5th percentile": "7.7", "95th percentile": "10"\}, "sigpp\_1": \{"median": "0.71", "error plus": "1.2", "error minus": "0.37", "5th percentile": "0.34", "95th percentile": "1.9"\}, "delta\_m\_1": \{"median": "4.8", "error plus": "4.7", "error minus": "4.4", "5th percentile": "0.44", "95th percentile": "9.5"\}, "delta\_m\_2": \{"median": "4.6", "error plus": "4.3", "error minus": "4.2", "5th percentile": "0.38", "95th percentile": "8.9"\}, "lam\_0": \{"median": "0.29", "error plus": "0.22", "error minus": "0.19", "5th percentile": "0.093", "95th percentile": "0.51"\}, "mu\_chi": \{"median": "0.081", "error plus": "0.14", "error minus": "0.074", "5th percentile": "0.0069", "95th percentile": "0.22"\}, "sigma\_chi": \{"median": "0.33", "error plus": "0.072", "error minus": "0.076", "5th percentile": "0.25", "95th percentile": "0.40"\}, "xi\_spin": \{"median": "0.68", "error plus": "0.29", "error minus": "0.55", "5th percentile": "0.13", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.42", "error plus": "0.52", "error minus": "0.65", "5th percentile": "{-}0.23", "95th percentile": "0.94"\}, "sigma\_spin": \{"median": "1.1", "error plus": "2.5", "error minus": "0.68", "5th percentile": "0.44", "95th percentile": "3.6"\}, "lamb": \{"median": "3.1", "error plus": "0.93", "error minus": "0.97", "5th percentile": "2.2", "95th percentile": "4.1"\}, "rate": \{"median": "16", "error plus": "5.9", "error minus": "4.7", "5th percentile": "12", "95th percentile": "22"\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@I\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@II\else\ifnum\pdfstrcmp{#1}{beta}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@III\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@IV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@VI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@VII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@VIII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@IX\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@X\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XI\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XIII\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XIV\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XV\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XVI\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XVII\else\ifnum\pdfstrcmp{#1}{rate}=0\let\PowerLawTwoPeakOneBBH@out\PowerLawTwoPeakOneBBH@XVIII\else\def\PowerLawTwoPeakOneBBH@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@out}\newcommand\PowerLawTwoPeakOneBBH@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@I@out{\{"median": "0.54", "error plus": "0.96", "error minus": "1.2", "5th percentile": "{-}0.70", "95th percentile": "1.5"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@I@out{0.54}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@I@out{0.96}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@I@out{1.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@I@out{{-}0.70}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@I@out{1.5}\else\def\PowerLawTwoPeakOneBBH@I@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@I@out}\newcommand\PowerLawTwoPeakOneBBH@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@II@out{\{"median": "5.6", "error plus": "1.0", "error minus": "0.79", "5th percentile": "4.8", "95th percentile": "6.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@II@out{5.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@II@out{1.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@II@out{0.79}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@II@out{4.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@II@out{6.6}\else\def\PowerLawTwoPeakOneBBH@II@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@II@out}\newcommand\PowerLawTwoPeakOneBBH@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@III@out{\{"median": "1.3", "error plus": "1.3", "error minus": "1.1", "5th percentile": "0.19", "95th percentile": "2.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@III@out{1.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@III@out{1.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@III@out{1.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@III@out{0.19}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@III@out{2.6}\else\def\PowerLawTwoPeakOneBBH@III@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@III@out}\newcommand\PowerLawTwoPeakOneBBH@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@IV@out{\{"median": "4.9", "error plus": "3.3", "error minus": "1.7", "5th percentile": "3.2", "95th percentile": "8.2"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@IV@out{4.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@IV@out{3.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@IV@out{1.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@IV@out{8.2}\else\def\PowerLawTwoPeakOneBBH@IV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@IV@out}\newcommand\PowerLawTwoPeakOneBBH@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@V@out{\{"median": "3.5", "error plus": "1.2", "error minus": "0.44", "5th percentile": "3.0", "95th percentile": "4.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@V@out{3.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@V@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@V@out{0.44}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@V@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@V@out{4.7}\else\def\PowerLawTwoPeakOneBBH@V@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@V@out}\newcommand\PowerLawTwoPeakOneBBH@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@VI@out{\{"median": "34.1", "error plus": "3.8", "error minus": "3.3", "5th percentile": "31", "95th percentile": "38"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@VI@out{34.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@VI@out{3.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@VI@out{3.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@VI@out{31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@VI@out{38}\else\def\PowerLawTwoPeakOneBBH@VI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@VI@out}\newcommand\PowerLawTwoPeakOneBBH@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@VII@out{\{"median": "9.7", "error plus": "0.49", "error minus": "2.0", "5th percentile": "7.7", "95th percentile": "10"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@VII@out{9.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@VII@out{0.49}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@VII@out{2.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@VII@out{7.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@VII@out{10}\else\def\PowerLawTwoPeakOneBBH@VII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@VII@out}\newcommand\PowerLawTwoPeakOneBBH@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@VIII@out{\{"median": "0.71", "error plus": "1.2", "error minus": "0.37", "5th percentile": "0.34", "95th percentile": "1.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@VIII@out{0.71}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@VIII@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@VIII@out{0.37}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@VIII@out{0.34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@VIII@out{1.9}\else\def\PowerLawTwoPeakOneBBH@VIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@VIII@out}\newcommand\PowerLawTwoPeakOneBBH@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@IX@out{\{"median": "4.8", "error plus": "4.7", "error minus": "4.4", "5th percentile": "0.44", "95th percentile": "9.5"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@IX@out{4.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@IX@out{4.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@IX@out{4.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@IX@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@IX@out{9.5}\else\def\PowerLawTwoPeakOneBBH@IX@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@IX@out}\newcommand\PowerLawTwoPeakOneBBH@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@X@out{\{"median": "4.6", "error plus": "4.3", "error minus": "4.2", "5th percentile": "0.38", "95th percentile": "8.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@X@out{4.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@X@out{4.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@X@out{4.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@X@out{0.38}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@X@out{8.9}\else\def\PowerLawTwoPeakOneBBH@X@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@X@out}\newcommand\PowerLawTwoPeakOneBBH@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XI@out{\{"median": "0.29", "error plus": "0.22", "error minus": "0.19", "5th percentile": "0.093", "95th percentile": "0.51"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XI@out{0.29}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XI@out{0.22}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XI@out{0.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XI@out{0.093}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XI@out{0.51}\else\def\PowerLawTwoPeakOneBBH@XI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XI@out}\newcommand\PowerLawTwoPeakOneBBH@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XII@out{\{"median": "0.081", "error plus": "0.14", "error minus": "0.074", "5th percentile": "0.0069", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XII@out{0.081}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XII@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XII@out{0.074}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XII@out{0.0069}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XII@out{0.22}\else\def\PowerLawTwoPeakOneBBH@XII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XII@out}\newcommand\PowerLawTwoPeakOneBBH@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XIII@out{\{"median": "0.33", "error plus": "0.072", "error minus": "0.076", "5th percentile": "0.25", "95th percentile": "0.40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XIII@out{0.33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XIII@out{0.072}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XIII@out{0.076}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XIII@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XIII@out{0.40}\else\def\PowerLawTwoPeakOneBBH@XIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XIII@out}\newcommand\PowerLawTwoPeakOneBBH@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XIV@out{\{"median": "0.68", "error plus": "0.29", "error minus": "0.55", "5th percentile": "0.13", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XIV@out{0.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XIV@out{0.29}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XIV@out{0.55}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XIV@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XIV@out{0.97}\else\def\PowerLawTwoPeakOneBBH@XIV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XIV@out}\newcommand\PowerLawTwoPeakOneBBH@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XV@out{\{"median": "0.42", "error plus": "0.52", "error minus": "0.65", "5th percentile": "{-}0.23", "95th percentile": "0.94"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XV@out{0.42}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XV@out{0.52}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XV@out{0.65}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XV@out{{-}0.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XV@out{0.94}\else\def\PowerLawTwoPeakOneBBH@XV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XV@out}\newcommand\PowerLawTwoPeakOneBBH@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XVI@out{\{"median": "1.1", "error plus": "2.5", "error minus": "0.68", "5th percentile": "0.44", "95th percentile": "3.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XVI@out{1.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XVI@out{2.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XVI@out{0.68}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XVI@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XVI@out{3.6}\else\def\PowerLawTwoPeakOneBBH@XVI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XVI@out}\newcommand\PowerLawTwoPeakOneBBH@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XVII@out{\{"median": "3.1", "error plus": "0.93", "error minus": "0.97", "5th percentile": "2.2", "95th percentile": "4.1"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XVII@out{3.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XVII@out{0.93}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XVII@out{0.97}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XVII@out{2.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XVII@out{4.1}\else\def\PowerLawTwoPeakOneBBH@XVII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XVII@out}\newcommand\PowerLawTwoPeakOneBBH@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakOneBBH@XVIII@out{\{"median": "16", "error plus": "5.9", "error minus": "4.7", "5th percentile": "12", "95th percentile": "22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakOneBBH@XVIII@out{16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakOneBBH@XVIII@out{5.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakOneBBH@XVIII@out{4.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakOneBBH@XVIII@out{12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakOneBBH@XVIII@out{22}\else\def\PowerLawTwoPeakOneBBH@XVIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakOneBBH@XVIII@out}\makeatother
\makeatletter\newcommand\PowerLawTwoPeakThreeBBH[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@out{\{"alpha\_1": \{"median": "0.78", "error plus": "1.8", "error minus": "3.9", "5th percentile": "{-}3.1", "95th percentile": "2.6"\}, "alpha\_2": \{"median": "4.5", "error plus": "1.5", "error minus": "1.4", "5th percentile": "3.1", "95th percentile": "6.0"\}, "beta": \{"median": "1.2", "error plus": "1.2", "error minus": "0.97", "5th percentile": "0.18", "95th percentile": "2.4"\}, "mlow\_1": \{"median": "4.8", "error plus": "3.2", "error minus": "1.6", "5th percentile": "3.2", "95th percentile": "7.9"\}, "mlow\_2": \{"median": "3.4", "error plus": "1.3", "error minus": "0.42", "5th percentile": "3.0", "95th percentile": "4.7"\}, "break\_mass": \{"median": "37", "error plus": "12", "error minus": "11", "5th percentile": "26", "95th percentile": "49"\}, "mpp\_1": \{"median": "9.8", "error plus": "0.45", "error minus": "0.76", "5th percentile": "9.0", "95th percentile": "10"\}, "sigpp\_1": \{"median": "0.68", "error plus": "0.67", "error minus": "0.35", "5th percentile": "0.33", "95th percentile": "1.4"\}, "mpp\_2": \{"median": "18", "error plus": "5.3", "error minus": "2.7", "5th percentile": "15", "95th percentile": "23"\}, "sigpp\_2": \{"median": "4.4", "error plus": "5.0", "error minus": "3.5", "5th percentile": "0.91", "95th percentile": "9.4"\}, "mpp\_3": \{"median": "33", "error plus": "3.0", "error minus": "5.2", "5th percentile": "28", "95th percentile": "36"\}, "sigpp\_3": \{"median": "3.8", "error plus": "5.0", "error minus": "2.5", "5th percentile": "1.3", "95th percentile": "8.7"\}, "delta\_m\_1": \{"median": "4.0", "error plus": "4.9", "error minus": "3.7", "5th percentile": "0.31", "95th percentile": "8.9"\}, "delta\_m\_2": \{"median": "5.0", "error plus": "3.9", "error minus": "4.4", "5th percentile": "0.58", "95th percentile": "8.9"\}, "lam\_0": \{"median": "0.16", "error plus": "0.33", "error minus": "0.12", "5th percentile": "0.038", "95th percentile": "0.49"\}, "lam\_1": \{"median": "0.69", "error plus": "0.13", "error minus": "0.28", "5th percentile": "0.41", "95th percentile": "0.82"\}, "lam\_2": \{"median": "0.071", "error plus": "0.10", "error minus": "0.062", "5th percentile": "0.0088", "95th percentile": "0.17"\}, "mu\_chi": \{"median": "0.089", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0090", "95th percentile": "0.22"\}, "sigma\_chi": \{"median": "0.33", "error plus": "0.075", "error minus": "0.076", "5th percentile": "0.25", "95th percentile": "0.40"\}, "xi\_spin": \{"median": "0.67", "error plus": "0.30", "error minus": "0.54", "5th percentile": "0.13", "95th percentile": "0.97"\}, "mu\_spin": \{"median": "0.41", "error plus": "0.53", "error minus": "0.65", "5th percentile": "{-}0.25", "95th percentile": "0.93"\}, "sigma\_spin": \{"median": "1.2", "error plus": "2.3", "error minus": "0.73", "5th percentile": "0.44", "95th percentile": "3.5"\}, "lamb": \{"median": "3.1", "error plus": "0.92", "error minus": "0.94", "5th percentile": "2.2", "95th percentile": "4.0"\}, "rate": \{"median": "16", "error plus": "5.9", "error minus": "4.4", "5th percentile": "11", "95th percentile": "22"\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@I\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@II\else\ifnum\pdfstrcmp{#1}{beta}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@III\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@IV\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@VI\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@VII\else\ifnum\pdfstrcmp{#1}{sigpp_1}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@VIII\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@IX\else\ifnum\pdfstrcmp{#1}{sigpp_2}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@X\else\ifnum\pdfstrcmp{#1}{mpp_3}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XI\else\ifnum\pdfstrcmp{#1}{sigpp_3}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XII\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XIII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XIV\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XV\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XVI\else\ifnum\pdfstrcmp{#1}{lam_2}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XIX\else\ifnum\pdfstrcmp{#1}{xi_spin}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XX\else\ifnum\pdfstrcmp{#1}{mu_spin}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XXI\else\ifnum\pdfstrcmp{#1}{sigma_spin}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XXII\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XXIII\else\ifnum\pdfstrcmp{#1}{rate}=0\let\PowerLawTwoPeakThreeBBH@out\PowerLawTwoPeakThreeBBH@XXIV\else\def\PowerLawTwoPeakThreeBBH@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@out}\newcommand\PowerLawTwoPeakThreeBBH@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@I@out{\{"median": "0.78", "error plus": "1.8", "error minus": "3.9", "5th percentile": "{-}3.1", "95th percentile": "2.6"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@I@out{0.78}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@I@out{1.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@I@out{3.9}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@I@out{{-}3.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@I@out{2.6}\else\def\PowerLawTwoPeakThreeBBH@I@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@I@out}\newcommand\PowerLawTwoPeakThreeBBH@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@II@out{\{"median": "4.5", "error plus": "1.5", "error minus": "1.4", "5th percentile": "3.1", "95th percentile": "6.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@II@out{4.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@II@out{1.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@II@out{1.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@II@out{3.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@II@out{6.0}\else\def\PowerLawTwoPeakThreeBBH@II@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@II@out}\newcommand\PowerLawTwoPeakThreeBBH@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@III@out{\{"median": "1.2", "error plus": "1.2", "error minus": "0.97", "5th percentile": "0.18", "95th percentile": "2.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@III@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@III@out{0.97}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@III@out{0.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@III@out{2.4}\else\def\PowerLawTwoPeakThreeBBH@III@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@III@out}\newcommand\PowerLawTwoPeakThreeBBH@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@IV@out{\{"median": "4.8", "error plus": "3.2", "error minus": "1.6", "5th percentile": "3.2", "95th percentile": "7.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@IV@out{4.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@IV@out{1.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@IV@out{3.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@IV@out{7.9}\else\def\PowerLawTwoPeakThreeBBH@IV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@IV@out}\newcommand\PowerLawTwoPeakThreeBBH@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@V@out{\{"median": "3.4", "error plus": "1.3", "error minus": "0.42", "5th percentile": "3.0", "95th percentile": "4.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@V@out{3.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@V@out{1.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@V@out{0.42}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@V@out{3.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@V@out{4.7}\else\def\PowerLawTwoPeakThreeBBH@V@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@V@out}\newcommand\PowerLawTwoPeakThreeBBH@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@VI@out{\{"median": "37", "error plus": "12", "error minus": "11", "5th percentile": "26", "95th percentile": "49"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@VI@out{37}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@VI@out{12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@VI@out{11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@VI@out{26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@VI@out{49}\else\def\PowerLawTwoPeakThreeBBH@VI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@VI@out}\newcommand\PowerLawTwoPeakThreeBBH@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@VII@out{\{"median": "9.8", "error plus": "0.45", "error minus": "0.76", "5th percentile": "9.0", "95th percentile": "10"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@VII@out{9.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@VII@out{0.45}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@VII@out{0.76}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@VII@out{9.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@VII@out{10}\else\def\PowerLawTwoPeakThreeBBH@VII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@VII@out}\newcommand\PowerLawTwoPeakThreeBBH@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@VIII@out{\{"median": "0.68", "error plus": "0.67", "error minus": "0.35", "5th percentile": "0.33", "95th percentile": "1.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@VIII@out{0.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@VIII@out{0.67}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@VIII@out{0.35}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@VIII@out{0.33}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@VIII@out{1.4}\else\def\PowerLawTwoPeakThreeBBH@VIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@VIII@out}\newcommand\PowerLawTwoPeakThreeBBH@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@IX@out{\{"median": "18", "error plus": "5.3", "error minus": "2.7", "5th percentile": "15", "95th percentile": "23"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@IX@out{18}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@IX@out{5.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@IX@out{2.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@IX@out{15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@IX@out{23}\else\def\PowerLawTwoPeakThreeBBH@IX@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@IX@out}\newcommand\PowerLawTwoPeakThreeBBH@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@X@out{\{"median": "4.4", "error plus": "5.0", "error minus": "3.5", "5th percentile": "0.91", "95th percentile": "9.4"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@X@out{4.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@X@out{5.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@X@out{3.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@X@out{0.91}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@X@out{9.4}\else\def\PowerLawTwoPeakThreeBBH@X@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@X@out}\newcommand\PowerLawTwoPeakThreeBBH@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XI@out{\{"median": "33", "error plus": "3.0", "error minus": "5.2", "5th percentile": "28", "95th percentile": "36"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XI@out{33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XI@out{3.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XI@out{5.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XI@out{28}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XI@out{36}\else\def\PowerLawTwoPeakThreeBBH@XI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XI@out}\newcommand\PowerLawTwoPeakThreeBBH@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XII@out{\{"median": "3.8", "error plus": "5.0", "error minus": "2.5", "5th percentile": "1.3", "95th percentile": "8.7"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XII@out{3.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XII@out{5.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XII@out{2.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XII@out{1.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XII@out{8.7}\else\def\PowerLawTwoPeakThreeBBH@XII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XII@out}\newcommand\PowerLawTwoPeakThreeBBH@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XIII@out{\{"median": "4.0", "error plus": "4.9", "error minus": "3.7", "5th percentile": "0.31", "95th percentile": "8.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XIII@out{4.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XIII@out{4.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XIII@out{3.7}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XIII@out{0.31}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XIII@out{8.9}\else\def\PowerLawTwoPeakThreeBBH@XIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XIII@out}\newcommand\PowerLawTwoPeakThreeBBH@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XIV@out{\{"median": "5.0", "error plus": "3.9", "error minus": "4.4", "5th percentile": "0.58", "95th percentile": "8.9"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XIV@out{3.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XIV@out{4.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XIV@out{0.58}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XIV@out{8.9}\else\def\PowerLawTwoPeakThreeBBH@XIV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XIV@out}\newcommand\PowerLawTwoPeakThreeBBH@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XV@out{\{"median": "0.16", "error plus": "0.33", "error minus": "0.12", "5th percentile": "0.038", "95th percentile": "0.49"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XV@out{0.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XV@out{0.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XV@out{0.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XV@out{0.038}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XV@out{0.49}\else\def\PowerLawTwoPeakThreeBBH@XV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XV@out}\newcommand\PowerLawTwoPeakThreeBBH@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XVI@out{\{"median": "0.69", "error plus": "0.13", "error minus": "0.28", "5th percentile": "0.41", "95th percentile": "0.82"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XVI@out{0.69}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XVI@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XVI@out{0.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XVI@out{0.41}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XVI@out{0.82}\else\def\PowerLawTwoPeakThreeBBH@XVI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XVI@out}\newcommand\PowerLawTwoPeakThreeBBH@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XVII@out{\{"median": "0.071", "error plus": "0.10", "error minus": "0.062", "5th percentile": "0.0088", "95th percentile": "0.17"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XVII@out{0.071}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XVII@out{0.10}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XVII@out{0.062}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XVII@out{0.0088}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XVII@out{0.17}\else\def\PowerLawTwoPeakThreeBBH@XVII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XVII@out}\newcommand\PowerLawTwoPeakThreeBBH@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XVIII@out{\{"median": "0.089", "error plus": "0.13", "error minus": "0.080", "5th percentile": "0.0090", "95th percentile": "0.22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XVIII@out{0.089}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XVIII@out{0.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XVIII@out{0.080}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XVIII@out{0.0090}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XVIII@out{0.22}\else\def\PowerLawTwoPeakThreeBBH@XVIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XVIII@out}\newcommand\PowerLawTwoPeakThreeBBH@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XIX@out{\{"median": "0.33", "error plus": "0.075", "error minus": "0.076", "5th percentile": "0.25", "95th percentile": "0.40"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XIX@out{0.33}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XIX@out{0.075}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XIX@out{0.076}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XIX@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XIX@out{0.40}\else\def\PowerLawTwoPeakThreeBBH@XIX@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XIX@out}\newcommand\PowerLawTwoPeakThreeBBH@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XX@out{\{"median": "0.67", "error plus": "0.30", "error minus": "0.54", "5th percentile": "0.13", "95th percentile": "0.97"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XX@out{0.67}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XX@out{0.30}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XX@out{0.54}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XX@out{0.97}\else\def\PowerLawTwoPeakThreeBBH@XX@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XX@out}\newcommand\PowerLawTwoPeakThreeBBH@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XXI@out{\{"median": "0.41", "error plus": "0.53", "error minus": "0.65", "5th percentile": "{-}0.25", "95th percentile": "0.93"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XXI@out{0.41}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XXI@out{0.53}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XXI@out{0.65}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXI@out{{-}0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXI@out{0.93}\else\def\PowerLawTwoPeakThreeBBH@XXI@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XXI@out}\newcommand\PowerLawTwoPeakThreeBBH@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XXII@out{\{"median": "1.2", "error plus": "2.3", "error minus": "0.73", "5th percentile": "0.44", "95th percentile": "3.5"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XXII@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XXII@out{2.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XXII@out{0.73}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXII@out{0.44}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXII@out{3.5}\else\def\PowerLawTwoPeakThreeBBH@XXII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XXII@out}\newcommand\PowerLawTwoPeakThreeBBH@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XXIII@out{\{"median": "3.1", "error plus": "0.92", "error minus": "0.94", "5th percentile": "2.2", "95th percentile": "4.0"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XXIII@out{3.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XXIII@out{0.92}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XXIII@out{0.94}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXIII@out{2.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXIII@out{4.0}\else\def\PowerLawTwoPeakThreeBBH@XXIII@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XXIII@out}\newcommand\PowerLawTwoPeakThreeBBH@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\PowerLawTwoPeakThreeBBH@XXIV@out{\{"median": "16", "error plus": "5.9", "error minus": "4.4", "5th percentile": "11", "95th percentile": "22"\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\PowerLawTwoPeakThreeBBH@XXIV@out{16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\PowerLawTwoPeakThreeBBH@XXIV@out{5.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\PowerLawTwoPeakThreeBBH@XXIV@out{4.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXIV@out{11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\PowerLawTwoPeakThreeBBH@XXIV@out{22}\else\def\PowerLawTwoPeakThreeBBH@XXIV@out{??}\fi\fi\fi\fi\fi\fi\PowerLawTwoPeakThreeBBH@XXIV@out}\makeatother
\makeatletter\newcommand\powersodapop[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@out{\{"woGW190814": \{"param": \{"alpha": \{"median": 7.7, "error plus": 5.1, "error minus": 5.5, "5th percentile": 2.2, "95th percentile": 13.0\}, "m\_min": \{"median": 1.2, "error plus": 0.093, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}, "m\_max": \{"median": 2.3, "error plus": 0.65, "error minus": 0.39, "5th percentile": 1.9, "95th percentile": 2.9\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.4, "5th percentile": 1.3, "95th percentile": 1.9\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.5\}, "mass\_source": \{"median": 1.4, "5th percentile": 1.2, "95th percentile": 1.8\}\}\}, "wGW190814": \{"param": \{"alpha": \{"median": 6.7, "error plus": 3.5, "error minus": 3.1, "5th percentile": 3.6, "95th percentile": 10.0\}, "m\_min": \{"median": 1.2, "error plus": 0.094, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}, "m\_max": \{"median": 2.8, "error plus": 0.2, "error minus": 0.21, "5th percentile": 2.6, "95th percentile": 3.0\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.1\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.6\}, "mass\_source": \{"median": 1.4, "5th percentile": 1.2, "95th percentile": 2.0\}\}\}\}}\else\ifnum\pdfstrcmp{#1}{woGW190814}=0\let\powersodapop@out\powersodapop@I\else\ifnum\pdfstrcmp{#1}{wGW190814}=0\let\powersodapop@out\powersodapop@II\else\def\powersodapop@out{??}\fi\fi\fi\powersodapop@out}\newcommand\powersodapop@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@I@out{\{"param": \{"alpha": \{"median": 7.7, "error plus": 5.1, "error minus": 5.5, "5th percentile": 2.2, "95th percentile": 13.0\}, "m\_min": \{"median": 1.2, "error plus": 0.093, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}, "m\_max": \{"median": 2.3, "error plus": 0.65, "error minus": 0.39, "5th percentile": 1.9, "95th percentile": 2.9\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.4, "5th percentile": 1.3, "95th percentile": 1.9\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.5\}, "mass\_source": \{"median": 1.4, "5th percentile": 1.2, "95th percentile": 1.8\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\powersodapop@I@out\powersodapop@III\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\powersodapop@I@out\powersodapop@IV\else\def\powersodapop@I@out{??}\fi\fi\fi\powersodapop@I@out}\newcommand\powersodapop@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@II@out{\{"param": \{"alpha": \{"median": 6.7, "error plus": 3.5, "error minus": 3.1, "5th percentile": 3.6, "95th percentile": 10.0\}, "m\_min": \{"median": 1.2, "error plus": 0.094, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}, "m\_max": \{"median": 2.8, "error plus": 0.2, "error minus": 0.21, "5th percentile": 2.6, "95th percentile": 3.0\}\}, "ppd": \{"mass\_1\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.1\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.6\}, "mass\_source": \{"median": 1.4, "5th percentile": 1.2, "95th percentile": 2.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\powersodapop@II@out\powersodapop@V\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\powersodapop@II@out\powersodapop@VI\else\def\powersodapop@II@out{??}\fi\fi\fi\powersodapop@II@out}\newcommand\powersodapop@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@III@out{\{"alpha": \{"median": 7.7, "error plus": 5.1, "error minus": 5.5, "5th percentile": 2.2, "95th percentile": 13.0\}, "m\_min": \{"median": 1.2, "error plus": 0.093, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}, "m\_max": \{"median": 2.3, "error plus": 0.65, "error minus": 0.39, "5th percentile": 1.9, "95th percentile": 2.9\}\}}\else\ifnum\pdfstrcmp{#1}{alpha}=0\let\powersodapop@III@out\powersodapop@VII\else\ifnum\pdfstrcmp{#1}{m_min}=0\let\powersodapop@III@out\powersodapop@VIII\else\ifnum\pdfstrcmp{#1}{m_max}=0\let\powersodapop@III@out\powersodapop@IX\else\def\powersodapop@III@out{??}\fi\fi\fi\fi\powersodapop@III@out}\newcommand\powersodapop@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@IV@out{\{"mass\_1\_source": \{"median": 1.4, "5th percentile": 1.3, "95th percentile": 1.9\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.5\}, "mass\_source": \{"median": 1.4, "5th percentile": 1.2, "95th percentile": 1.8\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1_source}=0\let\powersodapop@IV@out\powersodapop@X\else\ifnum\pdfstrcmp{#1}{mass_2_source}=0\let\powersodapop@IV@out\powersodapop@XI\else\ifnum\pdfstrcmp{#1}{mass_source}=0\let\powersodapop@IV@out\powersodapop@XII\else\def\powersodapop@IV@out{??}\fi\fi\fi\fi\powersodapop@IV@out}\newcommand\powersodapop@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@V@out{\{"alpha": \{"median": 6.7, "error plus": 3.5, "error minus": 3.1, "5th percentile": 3.6, "95th percentile": 10.0\}, "m\_min": \{"median": 1.2, "error plus": 0.094, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}, "m\_max": \{"median": 2.8, "error plus": 0.2, "error minus": 0.21, "5th percentile": 2.6, "95th percentile": 3.0\}\}}\else\ifnum\pdfstrcmp{#1}{alpha}=0\let\powersodapop@V@out\powersodapop@XIII\else\ifnum\pdfstrcmp{#1}{m_min}=0\let\powersodapop@V@out\powersodapop@XIV\else\ifnum\pdfstrcmp{#1}{m_max}=0\let\powersodapop@V@out\powersodapop@XV\else\def\powersodapop@V@out{??}\fi\fi\fi\fi\powersodapop@V@out}\newcommand\powersodapop@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@VI@out{\{"mass\_1\_source": \{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.1\}, "mass\_2\_source": \{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.6\}, "mass\_source": \{"median": 1.4, "5th percentile": 1.2, "95th percentile": 2.0\}\}}\else\ifnum\pdfstrcmp{#1}{mass_1_source}=0\let\powersodapop@VI@out\powersodapop@XVI\else\ifnum\pdfstrcmp{#1}{mass_2_source}=0\let\powersodapop@VI@out\powersodapop@XVII\else\ifnum\pdfstrcmp{#1}{mass_source}=0\let\powersodapop@VI@out\powersodapop@XVIII\else\def\powersodapop@VI@out{??}\fi\fi\fi\fi\powersodapop@VI@out}\newcommand\powersodapop@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@VII@out{\{"median": 7.7, "error plus": 5.1, "error minus": 5.5, "5th percentile": 2.2, "95th percentile": 13.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@VII@out{7.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\powersodapop@VII@out{5.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\powersodapop@VII@out{5.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@VII@out{2.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@VII@out{13.0}\else\def\powersodapop@VII@out{??}\fi\fi\fi\fi\fi\fi\powersodapop@VII@out}\newcommand\powersodapop@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@VIII@out{\{"median": 1.2, "error plus": 0.093, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@VIII@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\powersodapop@VIII@out{0.093}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\powersodapop@VIII@out{0.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@VIII@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@VIII@out{1.3}\else\def\powersodapop@VIII@out{??}\fi\fi\fi\fi\fi\fi\powersodapop@VIII@out}\newcommand\powersodapop@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@IX@out{\{"median": 2.3, "error plus": 0.65, "error minus": 0.39, "5th percentile": 1.9, "95th percentile": 2.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@IX@out{2.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\powersodapop@IX@out{0.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\powersodapop@IX@out{0.39}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@IX@out{1.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@IX@out{2.9}\else\def\powersodapop@IX@out{??}\fi\fi\fi\fi\fi\fi\powersodapop@IX@out}\newcommand\powersodapop@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@X@out{\{"median": 1.4, "5th percentile": 1.3, "95th percentile": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@X@out{1.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@X@out{1.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@X@out{1.9}\else\def\powersodapop@X@out{??}\fi\fi\fi\fi\powersodapop@X@out}\newcommand\powersodapop@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XI@out{\{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XI@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XI@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XI@out{1.5}\else\def\powersodapop@XI@out{??}\fi\fi\fi\fi\powersodapop@XI@out}\newcommand\powersodapop@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XII@out{\{"median": 1.4, "5th percentile": 1.2, "95th percentile": 1.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XII@out{1.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XII@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XII@out{1.8}\else\def\powersodapop@XII@out{??}\fi\fi\fi\fi\powersodapop@XII@out}\newcommand\powersodapop@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XIII@out{\{"median": 6.7, "error plus": 3.5, "error minus": 3.1, "5th percentile": 3.6, "95th percentile": 10.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XIII@out{6.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\powersodapop@XIII@out{3.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\powersodapop@XIII@out{3.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XIII@out{3.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XIII@out{10.0}\else\def\powersodapop@XIII@out{??}\fi\fi\fi\fi\fi\fi\powersodapop@XIII@out}\newcommand\powersodapop@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XIV@out{\{"median": 1.2, "error plus": 0.094, "error minus": 0.16, "5th percentile": 1.0, "95th percentile": 1.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XIV@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\powersodapop@XIV@out{0.094}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\powersodapop@XIV@out{0.16}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XIV@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XIV@out{1.3}\else\def\powersodapop@XIV@out{??}\fi\fi\fi\fi\fi\fi\powersodapop@XIV@out}\newcommand\powersodapop@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XV@out{\{"median": 2.8, "error plus": 0.2, "error minus": 0.21, "5th percentile": 2.6, "95th percentile": 3.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XV@out{2.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\powersodapop@XV@out{0.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\powersodapop@XV@out{0.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XV@out{2.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XV@out{3.0}\else\def\powersodapop@XV@out{??}\fi\fi\fi\fi\fi\fi\powersodapop@XV@out}\newcommand\powersodapop@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XVI@out{\{"median": 1.5, "5th percentile": 1.2, "95th percentile": 2.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XVI@out{1.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XVI@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XVI@out{2.1}\else\def\powersodapop@XVI@out{??}\fi\fi\fi\fi\powersodapop@XVI@out}\newcommand\powersodapop@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XVII@out{\{"median": 1.3, "5th percentile": 1.2, "95th percentile": 1.6\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XVII@out{1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XVII@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XVII@out{1.6}\else\def\powersodapop@XVII@out{??}\fi\fi\fi\fi\powersodapop@XVII@out}\newcommand\powersodapop@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\powersodapop@XVIII@out{\{"median": 1.4, "5th percentile": 1.2, "95th percentile": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\powersodapop@XVIII@out{1.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\powersodapop@XVIII@out{1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\powersodapop@XVIII@out{2.0}\else\def\powersodapop@XVIII@out{??}\fi\fi\fi\fi\powersodapop@XVIII@out}\makeatother
\makeatletter\newcommand\qchieffCopulaCorrelationModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@out{\{"param": \{"alpha\_1": \{"median": 1.81, "5th percentile": {-}0.53, "95th percentile": 3.16, "error plus": 1.34, "error minus": 2.35\}, "alpha\_2": \{"median": 4.32, "5th percentile": 3.17, "95th percentile": 5.73, "error plus": 1.42, "error minus": 1.14\}, "beta": \{"median": 0.82, "5th percentile": {-}0.04, "95th percentile": 1.92, "error plus": 1.1, "error minus": 0.85\}, "break\_mass": \{"median": 34.98, "5th percentile": 21.66, "95th percentile": 47.64, "error plus": 12.65, "error minus": 13.33\}, "delta\_m\_1": \{"median": 4.44, "5th percentile": 0.45, "95th percentile": 9.22, "error plus": 4.78, "error minus": 3.99\}, "delta\_m\_2": \{"median": 3.36, "5th percentile": 0.3, "95th percentile": 7.02, "error plus": 3.65, "error minus": 3.07\}, "lam\_0": \{"median": 0.35, "5th percentile": 0.12, "95th percentile": 0.68, "error plus": 0.33, "error minus": 0.24\}, "lam\_1": \{"median": 0.6, "5th percentile": 0.28, "95th percentile": 0.83, "error plus": 0.23, "error minus": 0.32\}, "lamb": \{"median": 3.14, "5th percentile": 2.15, "95th percentile": 4.07, "error plus": 0.93, "error minus": 0.98\}, "mlow\_1": \{"median": 5.28, "5th percentile": 3.28, "95th percentile": 7.91, "error plus": 2.62, "error minus": 2.0\}, "mlow\_2": \{"median": 3.6, "5th percentile": 3.03, "95th percentile": 4.93, "error plus": 1.33, "error minus": 0.57\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.71, "5th percentile": 7.03, "95th percentile": 10.3, "error plus": 0.59, "error minus": 2.68\}, "mpp\_2": \{"median": 32.69, "5th percentile": 26.46, "95th percentile": 35.91, "error plus": 3.21, "error minus": 6.23\}, "mu\_chi\_eff": \{"median": 0.05, "5th percentile": 0.02, "95th percentile": 0.08, "error plus": 0.03, "error minus": 0.03\}, "mu\_chi\_p": \{"median": 0.35, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.05\}, "sigma\_chi\_eff": \{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.02, "error minus": 0.02\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": {-}2.1, "5th percentile": {-}5.0, "95th percentile": 0.3, "error plus": 2.4, "error minus": 2.9, "correlated percentile": 92\}\}, "ppd": \{\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\qchieffCopulaCorrelationModel@out\qchieffCopulaCorrelationModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\qchieffCopulaCorrelationModel@out\qchieffCopulaCorrelationModel@II\else\def\qchieffCopulaCorrelationModel@out{??}\fi\fi\fi\qchieffCopulaCorrelationModel@out}\newcommand\qchieffCopulaCorrelationModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@I@out{\{"alpha\_1": \{"median": 1.81, "5th percentile": {-}0.53, "95th percentile": 3.16, "error plus": 1.34, "error minus": 2.35\}, "alpha\_2": \{"median": 4.32, "5th percentile": 3.17, "95th percentile": 5.73, "error plus": 1.42, "error minus": 1.14\}, "beta": \{"median": 0.82, "5th percentile": {-}0.04, "95th percentile": 1.92, "error plus": 1.1, "error minus": 0.85\}, "break\_mass": \{"median": 34.98, "5th percentile": 21.66, "95th percentile": 47.64, "error plus": 12.65, "error minus": 13.33\}, "delta\_m\_1": \{"median": 4.44, "5th percentile": 0.45, "95th percentile": 9.22, "error plus": 4.78, "error minus": 3.99\}, "delta\_m\_2": \{"median": 3.36, "5th percentile": 0.3, "95th percentile": 7.02, "error plus": 3.65, "error minus": 3.07\}, "lam\_0": \{"median": 0.35, "5th percentile": 0.12, "95th percentile": 0.68, "error plus": 0.33, "error minus": 0.24\}, "lam\_1": \{"median": 0.6, "5th percentile": 0.28, "95th percentile": 0.83, "error plus": 0.23, "error minus": 0.32\}, "lamb": \{"median": 3.14, "5th percentile": 2.15, "95th percentile": 4.07, "error plus": 0.93, "error minus": 0.98\}, "mlow\_1": \{"median": 5.28, "5th percentile": 3.28, "95th percentile": 7.91, "error plus": 2.62, "error minus": 2.0\}, "mlow\_2": \{"median": 3.6, "5th percentile": 3.03, "95th percentile": 4.93, "error plus": 1.33, "error minus": 0.57\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.71, "5th percentile": 7.03, "95th percentile": 10.3, "error plus": 0.59, "error minus": 2.68\}, "mpp\_2": \{"median": 32.69, "5th percentile": 26.46, "95th percentile": 35.91, "error plus": 3.21, "error minus": 6.23\}, "mu\_chi\_eff": \{"median": 0.05, "5th percentile": 0.02, "95th percentile": 0.08, "error plus": 0.03, "error minus": 0.03\}, "mu\_chi\_p": \{"median": 0.35, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.05\}, "sigma\_chi\_eff": \{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.02, "error minus": 0.02\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": {-}2.1, "5th percentile": {-}5.0, "95th percentile": 0.3, "error plus": 2.4, "error minus": 2.9, "correlated percentile": 92\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@VI\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@VII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@VIII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@IX\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@X\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XI\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XII\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XIII\else\ifnum\pdfstrcmp{#1}{mmax}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XIV\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XV\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XVI\else\ifnum\pdfstrcmp{#1}{mu_chi_eff}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi_p}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi_eff}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XIX\else\ifnum\pdfstrcmp{#1}{sigma_chi_p}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XX\else\ifnum\pdfstrcmp{#1}{kappa}=0\let\qchieffCopulaCorrelationModel@I@out\qchieffCopulaCorrelationModel@XXI\else\def\qchieffCopulaCorrelationModel@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@I@out}\newcommand\qchieffCopulaCorrelationModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@II@out{\{\}}\else\def\qchieffCopulaCorrelationModel@II@out{??}\fi\qchieffCopulaCorrelationModel@II@out}\newcommand\qchieffCopulaCorrelationModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@III@out{\{"median": 1.81, "5th percentile": {-}0.53, "95th percentile": 3.16, "error plus": 1.34, "error minus": 2.35\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@III@out{1.81}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@III@out{{-}0.53}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@III@out{3.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@III@out{1.34}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@III@out{2.35}\else\def\qchieffCopulaCorrelationModel@III@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@III@out}\newcommand\qchieffCopulaCorrelationModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@IV@out{\{"median": 4.32, "5th percentile": 3.17, "95th percentile": 5.73, "error plus": 1.42, "error minus": 1.14\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@IV@out{4.32}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@IV@out{3.17}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@IV@out{5.73}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@IV@out{1.42}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@IV@out{1.14}\else\def\qchieffCopulaCorrelationModel@IV@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@IV@out}\newcommand\qchieffCopulaCorrelationModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@V@out{\{"median": 0.82, "5th percentile": {-}0.04, "95th percentile": 1.92, "error plus": 1.1, "error minus": 0.85\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@V@out{0.82}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@V@out{{-}0.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@V@out{1.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@V@out{1.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@V@out{0.85}\else\def\qchieffCopulaCorrelationModel@V@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@V@out}\newcommand\qchieffCopulaCorrelationModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@VI@out{\{"median": 34.98, "5th percentile": 21.66, "95th percentile": 47.64, "error plus": 12.65, "error minus": 13.33\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@VI@out{34.98}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@VI@out{21.66}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@VI@out{47.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@VI@out{12.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@VI@out{13.33}\else\def\qchieffCopulaCorrelationModel@VI@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@VI@out}\newcommand\qchieffCopulaCorrelationModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@VII@out{\{"median": 4.44, "5th percentile": 0.45, "95th percentile": 9.22, "error plus": 4.78, "error minus": 3.99\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@VII@out{4.44}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@VII@out{0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@VII@out{9.22}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@VII@out{4.78}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@VII@out{3.99}\else\def\qchieffCopulaCorrelationModel@VII@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@VII@out}\newcommand\qchieffCopulaCorrelationModel@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@VIII@out{\{"median": 3.36, "5th percentile": 0.3, "95th percentile": 7.02, "error plus": 3.65, "error minus": 3.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@VIII@out{3.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@VIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@VIII@out{7.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@VIII@out{3.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@VIII@out{3.07}\else\def\qchieffCopulaCorrelationModel@VIII@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@VIII@out}\newcommand\qchieffCopulaCorrelationModel@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@IX@out{\{"median": 0.35, "5th percentile": 0.12, "95th percentile": 0.68, "error plus": 0.33, "error minus": 0.24\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@IX@out{0.35}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@IX@out{0.12}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@IX@out{0.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@IX@out{0.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@IX@out{0.24}\else\def\qchieffCopulaCorrelationModel@IX@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@IX@out}\newcommand\qchieffCopulaCorrelationModel@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@X@out{\{"median": 0.6, "5th percentile": 0.28, "95th percentile": 0.83, "error plus": 0.23, "error minus": 0.32\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@X@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@X@out{0.28}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@X@out{0.83}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@X@out{0.23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@X@out{0.32}\else\def\qchieffCopulaCorrelationModel@X@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@X@out}\newcommand\qchieffCopulaCorrelationModel@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XI@out{\{"median": 3.14, "5th percentile": 2.15, "95th percentile": 4.07, "error plus": 0.93, "error minus": 0.98\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XI@out{3.14}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XI@out{2.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XI@out{4.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XI@out{0.93}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XI@out{0.98}\else\def\qchieffCopulaCorrelationModel@XI@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XI@out}\newcommand\qchieffCopulaCorrelationModel@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XII@out{\{"median": 5.28, "5th percentile": 3.28, "95th percentile": 7.91, "error plus": 2.62, "error minus": 2.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XII@out{5.28}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XII@out{3.28}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XII@out{7.91}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XII@out{2.62}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XII@out{2.0}\else\def\qchieffCopulaCorrelationModel@XII@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XII@out}\newcommand\qchieffCopulaCorrelationModel@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XIII@out{\{"median": 3.6, "5th percentile": 3.03, "95th percentile": 4.93, "error plus": 1.33, "error minus": 0.57\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XIII@out{3.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XIII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XIII@out{4.93}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XIII@out{1.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XIII@out{0.57}\else\def\qchieffCopulaCorrelationModel@XIII@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XIII@out}\newcommand\qchieffCopulaCorrelationModel@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XIV@out{\{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XIV@out{0.0}\else\def\qchieffCopulaCorrelationModel@XIV@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XIV@out}\newcommand\qchieffCopulaCorrelationModel@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XV@out{\{"median": 9.71, "5th percentile": 7.03, "95th percentile": 10.3, "error plus": 0.59, "error minus": 2.68\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XV@out{9.71}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XV@out{7.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XV@out{10.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XV@out{0.59}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XV@out{2.68}\else\def\qchieffCopulaCorrelationModel@XV@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XV@out}\newcommand\qchieffCopulaCorrelationModel@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XVI@out{\{"median": 32.69, "5th percentile": 26.46, "95th percentile": 35.91, "error plus": 3.21, "error minus": 6.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XVI@out{32.69}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XVI@out{26.46}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XVI@out{35.91}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XVI@out{3.21}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XVI@out{6.23}\else\def\qchieffCopulaCorrelationModel@XVI@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XVI@out}\newcommand\qchieffCopulaCorrelationModel@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XVII@out{\{"median": 0.05, "5th percentile": 0.02, "95th percentile": 0.08, "error plus": 0.03, "error minus": 0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XVII@out{0.05}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XVII@out{0.02}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XVII@out{0.08}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XVII@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XVII@out{0.03}\else\def\qchieffCopulaCorrelationModel@XVII@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XVII@out}\newcommand\qchieffCopulaCorrelationModel@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XVIII@out{\{"median": 0.35, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XVIII@out{0.35}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XVIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XVIII@out{0.42}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XVIII@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XVIII@out{0.05}\else\def\qchieffCopulaCorrelationModel@XVIII@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XVIII@out}\newcommand\qchieffCopulaCorrelationModel@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XIX@out{\{"median": 0.11, "5th percentile": 0.09, "95th percentile": 0.14, "error plus": 0.02, "error minus": 0.02\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XIX@out{0.11}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XIX@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XIX@out{0.14}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XIX@out{0.02}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XIX@out{0.02}\else\def\qchieffCopulaCorrelationModel@XIX@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XIX@out}\newcommand\qchieffCopulaCorrelationModel@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XX@out{\{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XX@out{0.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XX@out{0.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XX@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XX@out{0.05}\else\def\qchieffCopulaCorrelationModel@XX@out{??}\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XX@out}\newcommand\qchieffCopulaCorrelationModel@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffCopulaCorrelationModel@XXI@out{\{"median": {-}2.1, "5th percentile": {-}5.0, "95th percentile": 0.3, "error plus": 2.4, "error minus": 2.9, "correlated percentile": 92\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffCopulaCorrelationModel@XXI@out{{-}2.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffCopulaCorrelationModel@XXI@out{{-}5.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffCopulaCorrelationModel@XXI@out{0.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffCopulaCorrelationModel@XXI@out{2.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffCopulaCorrelationModel@XXI@out{2.9}\else\ifnum\pdfstrcmp{#1}{correlated percentile}=0\def\qchieffCopulaCorrelationModel@XXI@out{92}\else\def\qchieffCopulaCorrelationModel@XXI@out{??}\fi\fi\fi\fi\fi\fi\fi\qchieffCopulaCorrelationModel@XXI@out}\makeatother
\makeatletter\newcommand\qchieffLinearCorrelationModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@out{\{"param": \{"alpha\_1": \{"median": 1.82, "5th percentile": {-}0.49, "95th percentile": 2.95, "error plus": 1.13, "error minus": 2.31\}, "alpha\_2": \{"median": 4.36, "5th percentile": 3.22, "95th percentile": 5.85, "error plus": 1.5, "error minus": 1.13\}, "beta": \{"median": 0.87, "5th percentile": {-}0.09, "95th percentile": 2.11, "error plus": 1.23, "error minus": 0.96\}, "break\_mass": \{"median": 35.34, "5th percentile": 21.75, "95th percentile": 48.48, "error plus": 13.14, "error minus": 13.59\}, "delta\_m\_1": \{"median": 3.93, "5th percentile": 0.28, "95th percentile": 9.13, "error plus": 5.2, "error minus": 3.65\}, "delta\_m\_2": \{"median": 5.19, "5th percentile": 0.67, "95th percentile": 9.1, "error plus": 3.91, "error minus": 4.52\}, "lam\_0": \{"median": 0.38, "5th percentile": 0.14, "95th percentile": 0.68, "error plus": 0.31, "error minus": 0.24\}, "lam\_1": \{"median": 0.57, "5th percentile": 0.27, "95th percentile": 0.81, "error plus": 0.24, "error minus": 0.29\}, "lamb": \{"median": 3.21, "5th percentile": 2.22, "95th percentile": 4.16, "error plus": 0.95, "error minus": 0.99\}, "mlow\_1": \{"median": 5.12, "5th percentile": 3.26, "95th percentile": 8.2, "error plus": 3.08, "error minus": 1.86\}, "mlow\_2": \{"median": 3.66, "5th percentile": 3.04, "95th percentile": 5.32, "error plus": 1.66, "error minus": 0.62\}, "mpp\_1": \{"median": 9.75, "5th percentile": 7.75, "95th percentile": 10.3, "error plus": 0.55, "error minus": 1.99\}, "mpp\_2": \{"median": 33.07, "5th percentile": 27.36, "95th percentile": 35.89, "error plus": 2.81, "error minus": 5.71\}, "mu\_chieff\_0": \{"median": 0.0, "5th percentile": {-}0.05, "95th percentile": 0.05, "error plus": 0.05, "error minus": 0.06\}, "ln\_sigma\_chieff\_0": \{"median": {-}2.91, "5th percentile": {-}3.37, "95th percentile": {-}2.46, "error plus": 0.45, "error minus": 0.46\}, "mu\_chieff\_1": \{"median": {-}0.17, "5th percentile": {-}0.45, "95th percentile": 0.14, "error plus": 0.31, "error minus": 0.28, "percentile exclude zero": 82\}, "ln\_sigma\_chieff\_1": \{"median": {-}1.94, "5th percentile": {-}3.61, "95th percentile": 0.07, "error plus": 2.01, "error minus": 1.66, "percentile exclude zero": 95\}\}, "ppd": \{\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\qchieffLinearCorrelationModel@out\qchieffLinearCorrelationModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\qchieffLinearCorrelationModel@out\qchieffLinearCorrelationModel@II\else\def\qchieffLinearCorrelationModel@out{??}\fi\fi\fi\qchieffLinearCorrelationModel@out}\newcommand\qchieffLinearCorrelationModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@I@out{\{"alpha\_1": \{"median": 1.82, "5th percentile": {-}0.49, "95th percentile": 2.95, "error plus": 1.13, "error minus": 2.31\}, "alpha\_2": \{"median": 4.36, "5th percentile": 3.22, "95th percentile": 5.85, "error plus": 1.5, "error minus": 1.13\}, "beta": \{"median": 0.87, "5th percentile": {-}0.09, "95th percentile": 2.11, "error plus": 1.23, "error minus": 0.96\}, "break\_mass": \{"median": 35.34, "5th percentile": 21.75, "95th percentile": 48.48, "error plus": 13.14, "error minus": 13.59\}, "delta\_m\_1": \{"median": 3.93, "5th percentile": 0.28, "95th percentile": 9.13, "error plus": 5.2, "error minus": 3.65\}, "delta\_m\_2": \{"median": 5.19, "5th percentile": 0.67, "95th percentile": 9.1, "error plus": 3.91, "error minus": 4.52\}, "lam\_0": \{"median": 0.38, "5th percentile": 0.14, "95th percentile": 0.68, "error plus": 0.31, "error minus": 0.24\}, "lam\_1": \{"median": 0.57, "5th percentile": 0.27, "95th percentile": 0.81, "error plus": 0.24, "error minus": 0.29\}, "lamb": \{"median": 3.21, "5th percentile": 2.22, "95th percentile": 4.16, "error plus": 0.95, "error minus": 0.99\}, "mlow\_1": \{"median": 5.12, "5th percentile": 3.26, "95th percentile": 8.2, "error plus": 3.08, "error minus": 1.86\}, "mlow\_2": \{"median": 3.66, "5th percentile": 3.04, "95th percentile": 5.32, "error plus": 1.66, "error minus": 0.62\}, "mpp\_1": \{"median": 9.75, "5th percentile": 7.75, "95th percentile": 10.3, "error plus": 0.55, "error minus": 1.99\}, "mpp\_2": \{"median": 33.07, "5th percentile": 27.36, "95th percentile": 35.89, "error plus": 2.81, "error minus": 5.71\}, "mu\_chieff\_0": \{"median": 0.0, "5th percentile": {-}0.05, "95th percentile": 0.05, "error plus": 0.05, "error minus": 0.06\}, "ln\_sigma\_chieff\_0": \{"median": {-}2.91, "5th percentile": {-}3.37, "95th percentile": {-}2.46, "error plus": 0.45, "error minus": 0.46\}, "mu\_chieff\_1": \{"median": {-}0.17, "5th percentile": {-}0.45, "95th percentile": 0.14, "error plus": 0.31, "error minus": 0.28, "percentile exclude zero": 82\}, "ln\_sigma\_chieff\_1": \{"median": {-}1.94, "5th percentile": {-}3.61, "95th percentile": 0.07, "error plus": 2.01, "error minus": 1.66, "percentile exclude zero": 95\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@VI\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@VII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@VIII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@IX\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@X\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XI\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XII\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XIV\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XV\else\ifnum\pdfstrcmp{#1}{mu_chieff_0}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XVI\else\ifnum\pdfstrcmp{#1}{ln_sigma_chieff_0}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XVII\else\ifnum\pdfstrcmp{#1}{mu_chieff_1}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XVIII\else\ifnum\pdfstrcmp{#1}{ln_sigma_chieff_1}=0\let\qchieffLinearCorrelationModel@I@out\qchieffLinearCorrelationModel@XIX\else\def\qchieffLinearCorrelationModel@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@I@out}\newcommand\qchieffLinearCorrelationModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@II@out{\{\}}\else\def\qchieffLinearCorrelationModel@II@out{??}\fi\qchieffLinearCorrelationModel@II@out}\newcommand\qchieffLinearCorrelationModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@III@out{\{"median": 1.82, "5th percentile": {-}0.49, "95th percentile": 2.95, "error plus": 1.13, "error minus": 2.31\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@III@out{1.82}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@III@out{{-}0.49}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@III@out{2.95}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@III@out{1.13}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@III@out{2.31}\else\def\qchieffLinearCorrelationModel@III@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@III@out}\newcommand\qchieffLinearCorrelationModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@IV@out{\{"median": 4.36, "5th percentile": 3.22, "95th percentile": 5.85, "error plus": 1.5, "error minus": 1.13\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@IV@out{4.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@IV@out{3.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@IV@out{5.85}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@IV@out{1.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@IV@out{1.13}\else\def\qchieffLinearCorrelationModel@IV@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@IV@out}\newcommand\qchieffLinearCorrelationModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@V@out{\{"median": 0.87, "5th percentile": {-}0.09, "95th percentile": 2.11, "error plus": 1.23, "error minus": 0.96\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@V@out{0.87}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@V@out{{-}0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@V@out{2.11}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@V@out{1.23}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@V@out{0.96}\else\def\qchieffLinearCorrelationModel@V@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@V@out}\newcommand\qchieffLinearCorrelationModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@VI@out{\{"median": 35.34, "5th percentile": 21.75, "95th percentile": 48.48, "error plus": 13.14, "error minus": 13.59\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@VI@out{35.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@VI@out{21.75}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@VI@out{48.48}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@VI@out{13.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@VI@out{13.59}\else\def\qchieffLinearCorrelationModel@VI@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@VI@out}\newcommand\qchieffLinearCorrelationModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@VII@out{\{"median": 3.93, "5th percentile": 0.28, "95th percentile": 9.13, "error plus": 5.2, "error minus": 3.65\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@VII@out{3.93}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@VII@out{0.28}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@VII@out{9.13}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@VII@out{5.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@VII@out{3.65}\else\def\qchieffLinearCorrelationModel@VII@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@VII@out}\newcommand\qchieffLinearCorrelationModel@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@VIII@out{\{"median": 5.19, "5th percentile": 0.67, "95th percentile": 9.1, "error plus": 3.91, "error minus": 4.52\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@VIII@out{5.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@VIII@out{0.67}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@VIII@out{9.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@VIII@out{3.91}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@VIII@out{4.52}\else\def\qchieffLinearCorrelationModel@VIII@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@VIII@out}\newcommand\qchieffLinearCorrelationModel@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@IX@out{\{"median": 0.38, "5th percentile": 0.14, "95th percentile": 0.68, "error plus": 0.31, "error minus": 0.24\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@IX@out{0.38}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@IX@out{0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@IX@out{0.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@IX@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@IX@out{0.24}\else\def\qchieffLinearCorrelationModel@IX@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@IX@out}\newcommand\qchieffLinearCorrelationModel@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@X@out{\{"median": 0.57, "5th percentile": 0.27, "95th percentile": 0.81, "error plus": 0.24, "error minus": 0.29\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@X@out{0.57}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@X@out{0.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@X@out{0.81}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@X@out{0.24}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@X@out{0.29}\else\def\qchieffLinearCorrelationModel@X@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@X@out}\newcommand\qchieffLinearCorrelationModel@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XI@out{\{"median": 3.21, "5th percentile": 2.22, "95th percentile": 4.16, "error plus": 0.95, "error minus": 0.99\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XI@out{3.21}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XI@out{2.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XI@out{4.16}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XI@out{0.95}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XI@out{0.99}\else\def\qchieffLinearCorrelationModel@XI@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XI@out}\newcommand\qchieffLinearCorrelationModel@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XII@out{\{"median": 5.12, "5th percentile": 3.26, "95th percentile": 8.2, "error plus": 3.08, "error minus": 1.86\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XII@out{5.12}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XII@out{3.26}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XII@out{8.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XII@out{3.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XII@out{1.86}\else\def\qchieffLinearCorrelationModel@XII@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XII@out}\newcommand\qchieffLinearCorrelationModel@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XIII@out{\{"median": 3.66, "5th percentile": 3.04, "95th percentile": 5.32, "error plus": 1.66, "error minus": 0.62\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XIII@out{3.66}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XIII@out{3.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XIII@out{5.32}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XIII@out{1.66}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XIII@out{0.62}\else\def\qchieffLinearCorrelationModel@XIII@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XIII@out}\newcommand\qchieffLinearCorrelationModel@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XIV@out{\{"median": 9.75, "5th percentile": 7.75, "95th percentile": 10.3, "error plus": 0.55, "error minus": 1.99\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XIV@out{9.75}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XIV@out{7.75}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XIV@out{10.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XIV@out{0.55}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XIV@out{1.99}\else\def\qchieffLinearCorrelationModel@XIV@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XIV@out}\newcommand\qchieffLinearCorrelationModel@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XV@out{\{"median": 33.07, "5th percentile": 27.36, "95th percentile": 35.89, "error plus": 2.81, "error minus": 5.71\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XV@out{33.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XV@out{27.36}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XV@out{35.89}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XV@out{2.81}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XV@out{5.71}\else\def\qchieffLinearCorrelationModel@XV@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XV@out}\newcommand\qchieffLinearCorrelationModel@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XVI@out{\{"median": 0.0, "5th percentile": {-}0.05, "95th percentile": 0.05, "error plus": 0.05, "error minus": 0.06\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XVI@out{{-}0.05}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XVI@out{0.05}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XVI@out{0.05}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XVI@out{0.06}\else\def\qchieffLinearCorrelationModel@XVI@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XVI@out}\newcommand\qchieffLinearCorrelationModel@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XVII@out{\{"median": {-}2.91, "5th percentile": {-}3.37, "95th percentile": {-}2.46, "error plus": 0.45, "error minus": 0.46\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XVII@out{{-}2.91}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XVII@out{{-}3.37}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XVII@out{{-}2.46}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XVII@out{0.45}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XVII@out{0.46}\else\def\qchieffLinearCorrelationModel@XVII@out{??}\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XVII@out}\newcommand\qchieffLinearCorrelationModel@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XVIII@out{\{"median": {-}0.17, "5th percentile": {-}0.45, "95th percentile": 0.14, "error plus": 0.31, "error minus": 0.28, "percentile exclude zero": 82\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XVIII@out{{-}0.17}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XVIII@out{{-}0.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XVIII@out{0.14}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XVIII@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XVIII@out{0.28}\else\ifnum\pdfstrcmp{#1}{percentile exclude zero}=0\def\qchieffLinearCorrelationModel@XVIII@out{82}\else\def\qchieffLinearCorrelationModel@XVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XVIII@out}\newcommand\qchieffLinearCorrelationModel@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\qchieffLinearCorrelationModel@XIX@out{\{"median": {-}1.94, "5th percentile": {-}3.61, "95th percentile": 0.07, "error plus": 2.01, "error minus": 1.66, "percentile exclude zero": 95\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\qchieffLinearCorrelationModel@XIX@out{{-}1.94}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\qchieffLinearCorrelationModel@XIX@out{{-}3.61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\qchieffLinearCorrelationModel@XIX@out{0.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\qchieffLinearCorrelationModel@XIX@out{2.01}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\qchieffLinearCorrelationModel@XIX@out{1.66}\else\ifnum\pdfstrcmp{#1}{percentile exclude zero}=0\def\qchieffLinearCorrelationModel@XIX@out{95}\else\def\qchieffLinearCorrelationModel@XIX@out{??}\fi\fi\fi\fi\fi\fi\fi\qchieffLinearCorrelationModel@XIX@out}\makeatother
\makeatletter\newcommand\samplePurityEstimate[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\samplePurityEstimate@out{\{"totalNumEvents": 161, "numEventsFAROnePerFourYear": 144, "expectedNumFalseTrialsFactor": \{"full": 6.721301493142698, "rounded": 6.7\}, "expectedNumFalseSimple": \{"full": 1.9103253732856744, "rounded": 1.9\}, "percentFalseTrialsFactor": \{"full": 4.174721424312235, "rounded": 4.17\}, "percentFalseSimple": \{"full": 1.1865374989352013, "rounded": 1.19\}, "totalAnalysisTimeYears": \{"full": 1.9103253732856744, "rounded": 1.91\}, "totalNumEventsO4aOnly": 85, "totalNumEventsGWTC3": 76\}}\else\ifnum\pdfstrcmp{#1}{totalNumEvents}=0\def\samplePurityEstimate@out{161}\else\ifnum\pdfstrcmp{#1}{numEventsFAROnePerFourYear}=0\def\samplePurityEstimate@out{144}\else\ifnum\pdfstrcmp{#1}{expectedNumFalseTrialsFactor}=0\let\samplePurityEstimate@out\samplePurityEstimate@I\else\ifnum\pdfstrcmp{#1}{expectedNumFalseSimple}=0\let\samplePurityEstimate@out\samplePurityEstimate@II\else\ifnum\pdfstrcmp{#1}{percentFalseTrialsFactor}=0\let\samplePurityEstimate@out\samplePurityEstimate@III\else\ifnum\pdfstrcmp{#1}{percentFalseSimple}=0\let\samplePurityEstimate@out\samplePurityEstimate@IV\else\ifnum\pdfstrcmp{#1}{totalAnalysisTimeYears}=0\let\samplePurityEstimate@out\samplePurityEstimate@V\else\ifnum\pdfstrcmp{#1}{totalNumEventsO4aOnly}=0\def\samplePurityEstimate@out{85}\else\ifnum\pdfstrcmp{#1}{totalNumEventsGWTC3}=0\def\samplePurityEstimate@out{76}\else\def\samplePurityEstimate@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\samplePurityEstimate@out}\newcommand\samplePurityEstimate@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\samplePurityEstimate@I@out{\{"full": 6.721301493142698, "rounded": 6.7\}}\else\ifnum\pdfstrcmp{#1}{full}=0\def\samplePurityEstimate@I@out{6.721301493142698}\else\ifnum\pdfstrcmp{#1}{rounded}=0\def\samplePurityEstimate@I@out{6.7}\else\def\samplePurityEstimate@I@out{??}\fi\fi\fi\samplePurityEstimate@I@out}\newcommand\samplePurityEstimate@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\samplePurityEstimate@II@out{\{"full": 1.9103253732856744, "rounded": 1.9\}}\else\ifnum\pdfstrcmp{#1}{full}=0\def\samplePurityEstimate@II@out{1.9103253732856744}\else\ifnum\pdfstrcmp{#1}{rounded}=0\def\samplePurityEstimate@II@out{1.9}\else\def\samplePurityEstimate@II@out{??}\fi\fi\fi\samplePurityEstimate@II@out}\newcommand\samplePurityEstimate@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\samplePurityEstimate@III@out{\{"full": 4.174721424312235, "rounded": 4.17\}}\else\ifnum\pdfstrcmp{#1}{full}=0\def\samplePurityEstimate@III@out{4.174721424312235}\else\ifnum\pdfstrcmp{#1}{rounded}=0\def\samplePurityEstimate@III@out{4.17}\else\def\samplePurityEstimate@III@out{??}\fi\fi\fi\samplePurityEstimate@III@out}\newcommand\samplePurityEstimate@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\samplePurityEstimate@IV@out{\{"full": 1.1865374989352013, "rounded": 1.19\}}\else\ifnum\pdfstrcmp{#1}{full}=0\def\samplePurityEstimate@IV@out{1.1865374989352013}\else\ifnum\pdfstrcmp{#1}{rounded}=0\def\samplePurityEstimate@IV@out{1.19}\else\def\samplePurityEstimate@IV@out{??}\fi\fi\fi\samplePurityEstimate@IV@out}\newcommand\samplePurityEstimate@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\samplePurityEstimate@V@out{\{"full": 1.9103253732856744, "rounded": 1.91\}}\else\ifnum\pdfstrcmp{#1}{full}=0\def\samplePurityEstimate@V@out{1.9103253732856744}\else\ifnum\pdfstrcmp{#1}{rounded}=0\def\samplePurityEstimate@V@out{1.91}\else\def\samplePurityEstimate@V@out{??}\fi\fi\fi\samplePurityEstimate@V@out}\makeatother
\makeatletter\newcommand\simplerates[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\simplerates@out{\{"RBNS": \{"5th percentile": 13, "median": 61, "95th percentile": 170\}, "RNSBH3Msun": \{"5th percentile": 11, "median": 30, "95th percentile": 63\}, "RNSBH5Msun": \{"5th percentile": 10, "median": 27, "95th percentile": 58\}\}}\else\ifnum\pdfstrcmp{#1}{RBNS}=0\let\simplerates@out\simplerates@I\else\ifnum\pdfstrcmp{#1}{RNSBH3Msun}=0\let\simplerates@out\simplerates@II\else\ifnum\pdfstrcmp{#1}{RNSBH5Msun}=0\let\simplerates@out\simplerates@III\else\def\simplerates@out{??}\fi\fi\fi\fi\simplerates@out}\newcommand\simplerates@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\simplerates@I@out{\{"5th percentile": 13, "median": 61, "95th percentile": 170\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\simplerates@I@out{13}\else\ifnum\pdfstrcmp{#1}{median}=0\def\simplerates@I@out{61}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\simplerates@I@out{170}\else\def\simplerates@I@out{??}\fi\fi\fi\fi\simplerates@I@out}\newcommand\simplerates@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\simplerates@II@out{\{"5th percentile": 11, "median": 30, "95th percentile": 63\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\simplerates@II@out{11}\else\ifnum\pdfstrcmp{#1}{median}=0\def\simplerates@II@out{30}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\simplerates@II@out{63}\else\def\simplerates@II@out{??}\fi\fi\fi\fi\simplerates@II@out}\newcommand\simplerates@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\simplerates@III@out{\{"5th percentile": 10, "median": 27, "95th percentile": 58\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\simplerates@III@out{10}\else\ifnum\pdfstrcmp{#1}{median}=0\def\simplerates@III@out{27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\simplerates@III@out{58}\else\def\simplerates@III@out{??}\fi\fi\fi\fi\simplerates@III@out}\makeatother
\makeatletter\newcommand\SkewNormalChiEff[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@out{\{"param": \{"mu\_chi\_eff": \{"median": {-}0.08, "5th percentile": {-}0.11, "95th percentile": {-}0.06, "error plus": 0.03, "error minus": 0.03\}, "sigma\_chi\_eff": \{"median": 0.17, "5th percentile": 0.14, "95th percentile": 0.21, "error plus": 0.03, "error minus": 0.03\}, "mu\_chi\_p": \{"median": 0.32, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.07, "error minus": 0.07\}, "sigma\_chi\_p": \{"median": 0.19, "5th percentile": 0.13, "95th percentile": 0.31, "error plus": 0.12, "error minus": 0.06\}, "eta\_chi\_eff": \{"median": 11.31, "5th percentile": 3.53, "95th percentile": 19.13, "error plus": 7.82, "error minus": 7.78\}, "min\_chi\_eff": \{"median": {-}0.1, "5th percentile": {-}0.15, "95th percentile": {-}0.07, "error plus": 0.03, "error minus": 0.05\}, "f\_neg\_chi\_eff": \{"median": 0.33, "5th percentile": 0.24, "95th percentile": 0.41, "error plus": 0.08, "error minus": 0.09\}\}, "ppd": \{"chi\_eff": \{"median": 0.03, "5th percentile": {-}0.08, "95th percentile": 0.26, "spin at peak": {-}0.03\}, "chi\_p": \{"median": 0.34, "5th percentile": 0.07, "95th percentile": 0.67, "spin at peak": 0.33\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\SkewNormalChiEff@out\SkewNormalChiEff@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\SkewNormalChiEff@out\SkewNormalChiEff@II\else\def\SkewNormalChiEff@out{??}\fi\fi\fi\SkewNormalChiEff@out}\newcommand\SkewNormalChiEff@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@I@out{\{"mu\_chi\_eff": \{"median": {-}0.08, "5th percentile": {-}0.11, "95th percentile": {-}0.06, "error plus": 0.03, "error minus": 0.03\}, "sigma\_chi\_eff": \{"median": 0.17, "5th percentile": 0.14, "95th percentile": 0.21, "error plus": 0.03, "error minus": 0.03\}, "mu\_chi\_p": \{"median": 0.32, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.07, "error minus": 0.07\}, "sigma\_chi\_p": \{"median": 0.19, "5th percentile": 0.13, "95th percentile": 0.31, "error plus": 0.12, "error minus": 0.06\}, "eta\_chi\_eff": \{"median": 11.31, "5th percentile": 3.53, "95th percentile": 19.13, "error plus": 7.82, "error minus": 7.78\}, "min\_chi\_eff": \{"median": {-}0.1, "5th percentile": {-}0.15, "95th percentile": {-}0.07, "error plus": 0.03, "error minus": 0.05\}, "f\_neg\_chi\_eff": \{"median": 0.33, "5th percentile": 0.24, "95th percentile": 0.41, "error plus": 0.08, "error minus": 0.09\}\}}\else\ifnum\pdfstrcmp{#1}{mu_chi_eff}=0\let\SkewNormalChiEff@I@out\SkewNormalChiEff@III\else\ifnum\pdfstrcmp{#1}{sigma_chi_eff}=0\let\SkewNormalChiEff@I@out\SkewNormalChiEff@IV\else\ifnum\pdfstrcmp{#1}{mu_chi_p}=0\let\SkewNormalChiEff@I@out\SkewNormalChiEff@V\else\ifnum\pdfstrcmp{#1}{sigma_chi_p}=0\let\SkewNormalChiEff@I@out\SkewNormalChiEff@VI\else\ifnum\pdfstrcmp{#1}{eta_chi_eff}=0\let\SkewNormalChiEff@I@out\SkewNormalChiEff@VII\else\ifnum\pdfstrcmp{#1}{min_chi_eff}=0\let\SkewNormalChiEff@I@out\SkewNormalChiEff@VIII\else\ifnum\pdfstrcmp{#1}{f_neg_chi_eff}=0\let\SkewNormalChiEff@I@out\SkewNormalChiEff@IX\else\def\SkewNormalChiEff@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@I@out}\newcommand\SkewNormalChiEff@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@II@out{\{"chi\_eff": \{"median": 0.03, "5th percentile": {-}0.08, "95th percentile": 0.26, "spin at peak": {-}0.03\}, "chi\_p": \{"median": 0.34, "5th percentile": 0.07, "95th percentile": 0.67, "spin at peak": 0.33\}\}}\else\ifnum\pdfstrcmp{#1}{chi_eff}=0\let\SkewNormalChiEff@II@out\SkewNormalChiEff@X\else\ifnum\pdfstrcmp{#1}{chi_p}=0\let\SkewNormalChiEff@II@out\SkewNormalChiEff@XI\else\def\SkewNormalChiEff@II@out{??}\fi\fi\fi\SkewNormalChiEff@II@out}\newcommand\SkewNormalChiEff@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@III@out{\{"median": {-}0.08, "5th percentile": {-}0.11, "95th percentile": {-}0.06, "error plus": 0.03, "error minus": 0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@III@out{{-}0.08}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@III@out{{-}0.11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@III@out{{-}0.06}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\SkewNormalChiEff@III@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\SkewNormalChiEff@III@out{0.03}\else\def\SkewNormalChiEff@III@out{??}\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@III@out}\newcommand\SkewNormalChiEff@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@IV@out{\{"median": 0.17, "5th percentile": 0.14, "95th percentile": 0.21, "error plus": 0.03, "error minus": 0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@IV@out{0.17}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@IV@out{0.14}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@IV@out{0.21}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\SkewNormalChiEff@IV@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\SkewNormalChiEff@IV@out{0.03}\else\def\SkewNormalChiEff@IV@out{??}\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@IV@out}\newcommand\SkewNormalChiEff@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@V@out{\{"median": 0.32, "5th percentile": 0.25, "95th percentile": 0.4, "error plus": 0.07, "error minus": 0.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@V@out{0.32}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@V@out{0.25}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@V@out{0.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\SkewNormalChiEff@V@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\SkewNormalChiEff@V@out{0.07}\else\def\SkewNormalChiEff@V@out{??}\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@V@out}\newcommand\SkewNormalChiEff@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@VI@out{\{"median": 0.19, "5th percentile": 0.13, "95th percentile": 0.31, "error plus": 0.12, "error minus": 0.06\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@VI@out{0.19}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@VI@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@VI@out{0.31}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\SkewNormalChiEff@VI@out{0.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\SkewNormalChiEff@VI@out{0.06}\else\def\SkewNormalChiEff@VI@out{??}\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@VI@out}\newcommand\SkewNormalChiEff@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@VII@out{\{"median": 11.31, "5th percentile": 3.53, "95th percentile": 19.13, "error plus": 7.82, "error minus": 7.78\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@VII@out{11.31}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@VII@out{3.53}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@VII@out{19.13}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\SkewNormalChiEff@VII@out{7.82}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\SkewNormalChiEff@VII@out{7.78}\else\def\SkewNormalChiEff@VII@out{??}\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@VII@out}\newcommand\SkewNormalChiEff@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@VIII@out{\{"median": {-}0.1, "5th percentile": {-}0.15, "95th percentile": {-}0.07, "error plus": 0.03, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@VIII@out{{-}0.1}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@VIII@out{{-}0.15}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@VIII@out{{-}0.07}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\SkewNormalChiEff@VIII@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\SkewNormalChiEff@VIII@out{0.05}\else\def\SkewNormalChiEff@VIII@out{??}\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@VIII@out}\newcommand\SkewNormalChiEff@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@IX@out{\{"median": 0.33, "5th percentile": 0.24, "95th percentile": 0.41, "error plus": 0.08, "error minus": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@IX@out{0.33}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@IX@out{0.24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@IX@out{0.41}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\SkewNormalChiEff@IX@out{0.08}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\SkewNormalChiEff@IX@out{0.09}\else\def\SkewNormalChiEff@IX@out{??}\fi\fi\fi\fi\fi\fi\SkewNormalChiEff@IX@out}\newcommand\SkewNormalChiEff@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@X@out{\{"median": 0.03, "5th percentile": {-}0.08, "95th percentile": 0.26, "spin at peak": {-}0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@X@out{0.03}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@X@out{{-}0.08}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@X@out{0.26}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\SkewNormalChiEff@X@out{{-}0.03}\else\def\SkewNormalChiEff@X@out{??}\fi\fi\fi\fi\fi\SkewNormalChiEff@X@out}\newcommand\SkewNormalChiEff@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\SkewNormalChiEff@XI@out{\{"median": 0.34, "5th percentile": 0.07, "95th percentile": 0.67, "spin at peak": 0.33\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\SkewNormalChiEff@XI@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\SkewNormalChiEff@XI@out{0.07}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\SkewNormalChiEff@XI@out{0.67}\else\ifnum\pdfstrcmp{#1}{spin at peak}=0\def\SkewNormalChiEff@XI@out{0.33}\else\def\SkewNormalChiEff@XI@out{??}\fi\fi\fi\fi\fi\SkewNormalChiEff@XI@out}\makeatother
\makeatletter\newcommand\spinModelComparisonLogTenBayesFactors[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@out{\{"MagBetaConstrainedIidTiltIsotropicTruncnormNid": \{"log10\_bayes\_factor\_over\_new\_default": {-}0.64, "log10\_bayes\_factor\_over\_old\_default": 0.02\}, "MagTruncnormIndTiltIsotropicTruncnormNnd": \{"log10\_bayes\_factor\_over\_new\_default": {-}0.91, "log10\_bayes\_factor\_over\_old\_default": {-}0.25\}, "MagTruncnormIidTiltIsotropicTruncnormNid": \{"log10\_bayes\_factor\_over\_new\_default": 0.0, "log10\_bayes\_factor\_over\_old\_default": 0.66\}, "MagTruncnormIidTiltIsotropicAlignedNid": \{"log10\_bayes\_factor\_over\_new\_default": {-}0.08, "log10\_bayes\_factor\_over\_old\_default": 0.57\}, "MagTruncnormIidTiltIsotropicTruncnormNnd": \{"log10\_bayes\_factor\_over\_new\_default": {-}0.17, "log10\_bayes\_factor\_over\_old\_default": 0.49\}, "MagBetaConstrainedIidTiltIsotropicAlignedNid": \{"log10\_bayes\_factor\_over\_new\_default": {-}0.66, "log10\_bayes\_factor\_over\_old\_default": 0.0\}, "MagTruncnormIndTiltIsotropicTruncnormNid": \{"log10\_bayes\_factor\_over\_new\_default": {-}1.09, "log10\_bayes\_factor\_over\_old\_default": {-}0.43\}, "MagBetaUnconstrainedIidTiltIsotropicTruncnormNid": \{"log10\_bayes\_factor\_over\_new\_default": {-}0.98, "log10\_bayes\_factor\_over\_old\_default": {-}0.32\}\}}\else\ifnum\pdfstrcmp{#1}{MagBetaConstrainedIidTiltIsotropicTruncnormNid}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@I\else\ifnum\pdfstrcmp{#1}{MagTruncnormIndTiltIsotropicTruncnormNnd}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@II\else\ifnum\pdfstrcmp{#1}{MagTruncnormIidTiltIsotropicTruncnormNid}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@III\else\ifnum\pdfstrcmp{#1}{MagTruncnormIidTiltIsotropicAlignedNid}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@IV\else\ifnum\pdfstrcmp{#1}{MagTruncnormIidTiltIsotropicTruncnormNnd}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@V\else\ifnum\pdfstrcmp{#1}{MagBetaConstrainedIidTiltIsotropicAlignedNid}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@VI\else\ifnum\pdfstrcmp{#1}{MagTruncnormIndTiltIsotropicTruncnormNid}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@VII\else\ifnum\pdfstrcmp{#1}{MagBetaUnconstrainedIidTiltIsotropicTruncnormNid}=0\let\spinModelComparisonLogTenBayesFactors@out\spinModelComparisonLogTenBayesFactors@VIII\else\def\spinModelComparisonLogTenBayesFactors@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\spinModelComparisonLogTenBayesFactors@out}\newcommand\spinModelComparisonLogTenBayesFactors@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@I@out{\{"log10\_bayes\_factor\_over\_new\_default": {-}0.64, "log10\_bayes\_factor\_over\_old\_default": 0.02\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@I@out{{-}0.64}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@I@out{0.02}\else\def\spinModelComparisonLogTenBayesFactors@I@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@I@out}\newcommand\spinModelComparisonLogTenBayesFactors@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@II@out{\{"log10\_bayes\_factor\_over\_new\_default": {-}0.91, "log10\_bayes\_factor\_over\_old\_default": {-}0.25\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@II@out{{-}0.91}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@II@out{{-}0.25}\else\def\spinModelComparisonLogTenBayesFactors@II@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@II@out}\newcommand\spinModelComparisonLogTenBayesFactors@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@III@out{\{"log10\_bayes\_factor\_over\_new\_default": 0.0, "log10\_bayes\_factor\_over\_old\_default": 0.66\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@III@out{0.0}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@III@out{0.66}\else\def\spinModelComparisonLogTenBayesFactors@III@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@III@out}\newcommand\spinModelComparisonLogTenBayesFactors@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@IV@out{\{"log10\_bayes\_factor\_over\_new\_default": {-}0.08, "log10\_bayes\_factor\_over\_old\_default": 0.57\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@IV@out{{-}0.08}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@IV@out{0.57}\else\def\spinModelComparisonLogTenBayesFactors@IV@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@IV@out}\newcommand\spinModelComparisonLogTenBayesFactors@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@V@out{\{"log10\_bayes\_factor\_over\_new\_default": {-}0.17, "log10\_bayes\_factor\_over\_old\_default": 0.49\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@V@out{{-}0.17}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@V@out{0.49}\else\def\spinModelComparisonLogTenBayesFactors@V@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@V@out}\newcommand\spinModelComparisonLogTenBayesFactors@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@VI@out{\{"log10\_bayes\_factor\_over\_new\_default": {-}0.66, "log10\_bayes\_factor\_over\_old\_default": 0.0\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@VI@out{{-}0.66}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@VI@out{0.0}\else\def\spinModelComparisonLogTenBayesFactors@VI@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@VI@out}\newcommand\spinModelComparisonLogTenBayesFactors@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@VII@out{\{"log10\_bayes\_factor\_over\_new\_default": {-}1.09, "log10\_bayes\_factor\_over\_old\_default": {-}0.43\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@VII@out{{-}1.09}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@VII@out{{-}0.43}\else\def\spinModelComparisonLogTenBayesFactors@VII@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@VII@out}\newcommand\spinModelComparisonLogTenBayesFactors@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\spinModelComparisonLogTenBayesFactors@VIII@out{\{"log10\_bayes\_factor\_over\_new\_default": {-}0.98, "log10\_bayes\_factor\_over\_old\_default": {-}0.32\}}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_new_default}=0\def\spinModelComparisonLogTenBayesFactors@VIII@out{{-}0.98}\else\ifnum\pdfstrcmp{#1}{log10_bayes_factor_over_old_default}=0\def\spinModelComparisonLogTenBayesFactors@VIII@out{{-}0.32}\else\def\spinModelComparisonLogTenBayesFactors@VIII@out{??}\fi\fi\fi\spinModelComparisonLogTenBayesFactors@VIII@out}\makeatother
\makeatletter\newcommand\VaryingBetaQsDominantMode[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsDominantMode@out{\{"param": \{"beta\_q\_high\_mass\_peak": \{"5th percentile": 2.7, "95th percentile": 12.2, "error minus": 4.8, "error plus": 4.7, "median": 7.5\}, "beta\_q\_high\_mass\_peak\_minus\_beta\_q\_power\_law": \{"5th percentile": 2.4, "95th percentile": 12.3, "error minus": 5.0, "error plus": 4.9, "median": 7.4\}, "beta\_q\_low\_mass\_peak": \{"5th percentile": {-}6.5, "95th percentile": 11.2, "error minus": 8.1, "error plus": 9.6, "median": 1.6\}, "beta\_q\_power\_law": \{"5th percentile": {-}1.2, "95th percentile": 1.6, "error minus": 1.2, "error plus": 1.6, "median": 0.0\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\VaryingBetaQsDominantMode@out\VaryingBetaQsDominantMode@I\else\def\VaryingBetaQsDominantMode@out{??}\fi\fi\VaryingBetaQsDominantMode@out}\newcommand\VaryingBetaQsDominantMode@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsDominantMode@I@out{\{"beta\_q\_high\_mass\_peak": \{"5th percentile": 2.7, "95th percentile": 12.2, "error minus": 4.8, "error plus": 4.7, "median": 7.5\}, "beta\_q\_high\_mass\_peak\_minus\_beta\_q\_power\_law": \{"5th percentile": 2.4, "95th percentile": 12.3, "error minus": 5.0, "error plus": 4.9, "median": 7.4\}, "beta\_q\_low\_mass\_peak": \{"5th percentile": {-}6.5, "95th percentile": 11.2, "error minus": 8.1, "error plus": 9.6, "median": 1.6\}, "beta\_q\_power\_law": \{"5th percentile": {-}1.2, "95th percentile": 1.6, "error minus": 1.2, "error plus": 1.6, "median": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{beta_q_high_mass_peak}=0\let\VaryingBetaQsDominantMode@I@out\VaryingBetaQsDominantMode@II\else\ifnum\pdfstrcmp{#1}{beta_q_high_mass_peak_minus_beta_q_power_law}=0\let\VaryingBetaQsDominantMode@I@out\VaryingBetaQsDominantMode@III\else\ifnum\pdfstrcmp{#1}{beta_q_low_mass_peak}=0\let\VaryingBetaQsDominantMode@I@out\VaryingBetaQsDominantMode@IV\else\ifnum\pdfstrcmp{#1}{beta_q_power_law}=0\let\VaryingBetaQsDominantMode@I@out\VaryingBetaQsDominantMode@V\else\def\VaryingBetaQsDominantMode@I@out{??}\fi\fi\fi\fi\fi\VaryingBetaQsDominantMode@I@out}\newcommand\VaryingBetaQsDominantMode@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsDominantMode@II@out{\{"5th percentile": 2.7, "95th percentile": 12.2, "error minus": 4.8, "error plus": 4.7, "median": 7.5\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsDominantMode@II@out{2.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsDominantMode@II@out{12.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsDominantMode@II@out{4.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsDominantMode@II@out{4.7}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsDominantMode@II@out{7.5}\else\def\VaryingBetaQsDominantMode@II@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsDominantMode@II@out}\newcommand\VaryingBetaQsDominantMode@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsDominantMode@III@out{\{"5th percentile": 2.4, "95th percentile": 12.3, "error minus": 5.0, "error plus": 4.9, "median": 7.4\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsDominantMode@III@out{2.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsDominantMode@III@out{12.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsDominantMode@III@out{5.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsDominantMode@III@out{4.9}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsDominantMode@III@out{7.4}\else\def\VaryingBetaQsDominantMode@III@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsDominantMode@III@out}\newcommand\VaryingBetaQsDominantMode@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsDominantMode@IV@out{\{"5th percentile": {-}6.5, "95th percentile": 11.2, "error minus": 8.1, "error plus": 9.6, "median": 1.6\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsDominantMode@IV@out{{-}6.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsDominantMode@IV@out{11.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsDominantMode@IV@out{8.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsDominantMode@IV@out{9.6}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsDominantMode@IV@out{1.6}\else\def\VaryingBetaQsDominantMode@IV@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsDominantMode@IV@out}\newcommand\VaryingBetaQsDominantMode@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsDominantMode@V@out{\{"5th percentile": {-}1.2, "95th percentile": 1.6, "error minus": 1.2, "error plus": 1.6, "median": 0.0\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsDominantMode@V@out{{-}1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsDominantMode@V@out{1.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsDominantMode@V@out{1.2}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsDominantMode@V@out{1.6}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsDominantMode@V@out{0.0}\else\def\VaryingBetaQsDominantMode@V@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsDominantMode@V@out}\makeatother
\makeatletter\newcommand\VaryingBetaQsTwoModesBetaDiffPerc[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsTwoModesBetaDiffPerc@out{\{"beta\_peak\_pl\_diff\_perc": 97.3\}}\else\ifnum\pdfstrcmp{#1}{beta_peak_pl_diff_perc}=0\def\VaryingBetaQsTwoModesBetaDiffPerc@out{97.3}\else\def\VaryingBetaQsTwoModesBetaDiffPerc@out{??}\fi\fi\VaryingBetaQsTwoModesBetaDiffPerc@out}\makeatother
\makeatletter\newcommand\VaryingBetaQsTwoModes[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsTwoModes@out{\{"param": \{"beta\_q\_high\_mass\_peak": \{"5th percentile": 2.3, "95th percentile": 12.2, "error minus": 5.1, "error plus": 4.8, "median": 7.4\}, "beta\_q\_high\_mass\_peak\_minus\_beta\_q\_power\_law": \{"5th percentile": 1.8, "95th percentile": 12.3, "error minus": 5.5, "error plus": 5.0, "median": 7.3\}, "beta\_q\_low\_mass\_peak": \{"5th percentile": {-}6.5, "95th percentile": 11.2, "error minus": 8.1, "error plus": 9.6, "median": 1.6\}, "beta\_q\_power\_law": \{"5th percentile": {-}1.2, "95th percentile": 1.8, "error minus": 1.3, "error plus": 1.7, "median": 0.1\}\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\VaryingBetaQsTwoModes@out\VaryingBetaQsTwoModes@I\else\def\VaryingBetaQsTwoModes@out{??}\fi\fi\VaryingBetaQsTwoModes@out}\newcommand\VaryingBetaQsTwoModes@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsTwoModes@I@out{\{"beta\_q\_high\_mass\_peak": \{"5th percentile": 2.3, "95th percentile": 12.2, "error minus": 5.1, "error plus": 4.8, "median": 7.4\}, "beta\_q\_high\_mass\_peak\_minus\_beta\_q\_power\_law": \{"5th percentile": 1.8, "95th percentile": 12.3, "error minus": 5.5, "error plus": 5.0, "median": 7.3\}, "beta\_q\_low\_mass\_peak": \{"5th percentile": {-}6.5, "95th percentile": 11.2, "error minus": 8.1, "error plus": 9.6, "median": 1.6\}, "beta\_q\_power\_law": \{"5th percentile": {-}1.2, "95th percentile": 1.8, "error minus": 1.3, "error plus": 1.7, "median": 0.1\}\}}\else\ifnum\pdfstrcmp{#1}{beta_q_high_mass_peak}=0\let\VaryingBetaQsTwoModes@I@out\VaryingBetaQsTwoModes@II\else\ifnum\pdfstrcmp{#1}{beta_q_high_mass_peak_minus_beta_q_power_law}=0\let\VaryingBetaQsTwoModes@I@out\VaryingBetaQsTwoModes@III\else\ifnum\pdfstrcmp{#1}{beta_q_low_mass_peak}=0\let\VaryingBetaQsTwoModes@I@out\VaryingBetaQsTwoModes@IV\else\ifnum\pdfstrcmp{#1}{beta_q_power_law}=0\let\VaryingBetaQsTwoModes@I@out\VaryingBetaQsTwoModes@V\else\def\VaryingBetaQsTwoModes@I@out{??}\fi\fi\fi\fi\fi\VaryingBetaQsTwoModes@I@out}\newcommand\VaryingBetaQsTwoModes@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsTwoModes@II@out{\{"5th percentile": 2.3, "95th percentile": 12.2, "error minus": 5.1, "error plus": 4.8, "median": 7.4\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsTwoModes@II@out{2.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsTwoModes@II@out{12.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsTwoModes@II@out{5.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsTwoModes@II@out{4.8}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsTwoModes@II@out{7.4}\else\def\VaryingBetaQsTwoModes@II@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsTwoModes@II@out}\newcommand\VaryingBetaQsTwoModes@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsTwoModes@III@out{\{"5th percentile": 1.8, "95th percentile": 12.3, "error minus": 5.5, "error plus": 5.0, "median": 7.3\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsTwoModes@III@out{1.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsTwoModes@III@out{12.3}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsTwoModes@III@out{5.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsTwoModes@III@out{5.0}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsTwoModes@III@out{7.3}\else\def\VaryingBetaQsTwoModes@III@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsTwoModes@III@out}\newcommand\VaryingBetaQsTwoModes@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsTwoModes@IV@out{\{"5th percentile": {-}6.5, "95th percentile": 11.2, "error minus": 8.1, "error plus": 9.6, "median": 1.6\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsTwoModes@IV@out{{-}6.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsTwoModes@IV@out{11.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsTwoModes@IV@out{8.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsTwoModes@IV@out{9.6}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsTwoModes@IV@out{1.6}\else\def\VaryingBetaQsTwoModes@IV@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsTwoModes@IV@out}\newcommand\VaryingBetaQsTwoModes@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\VaryingBetaQsTwoModes@V@out{\{"5th percentile": {-}1.2, "95th percentile": 1.8, "error minus": 1.3, "error plus": 1.7, "median": 0.1\}}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\VaryingBetaQsTwoModes@V@out{{-}1.2}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\VaryingBetaQsTwoModes@V@out{1.8}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\VaryingBetaQsTwoModes@V@out{1.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\VaryingBetaQsTwoModes@V@out{1.7}\else\ifnum\pdfstrcmp{#1}{median}=0\def\VaryingBetaQsTwoModes@V@out{0.1}\else\def\VaryingBetaQsTwoModes@V@out{??}\fi\fi\fi\fi\fi\fi\VaryingBetaQsTwoModes@V@out}\makeatother
\makeatletter\newcommand\zchieffCopulaCorrelationModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@out{\{"param": \{"alpha\_1": \{"median": 1.71, "5th percentile": {-}0.18, "95th percentile": 2.9, "error plus": 1.19, "error minus": 1.89\}, "alpha\_2": \{"median": 4.57, "5th percentile": 3.27, "95th percentile": 5.99, "error plus": 1.42, "error minus": 1.29\}, "beta": \{"median": 1.05, "5th percentile": 0.09, "95th percentile": 2.17, "error plus": 1.12, "error minus": 0.96\}, "break\_mass": \{"median": 35.68, "5th percentile": 22.75, "95th percentile": 48.08, "error plus": 12.4, "error minus": 12.93\}, "delta\_m\_1": \{"median": 4.75, "5th percentile": 0.52, "95th percentile": 9.4, "error plus": 4.65, "error minus": 4.23\}, "delta\_m\_2": \{"median": 3.94, "5th percentile": 0.4, "95th percentile": 7.64, "error plus": 3.7, "error minus": 3.54\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.63, "error plus": 0.28, "error minus": 0.21\}, "lam\_1": \{"median": 0.61, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.29\}, "lamb": \{"median": 2.69, "5th percentile": 1.78, "95th percentile": 3.62, "error plus": 0.93, "error minus": 0.91\}, "mlow\_1": \{"median": 5.07, "5th percentile": 3.3, "95th percentile": 7.67, "error plus": 2.6, "error minus": 1.77\}, "mlow\_2": \{"median": 3.59, "5th percentile": 3.04, "95th percentile": 5.02, "error plus": 1.42, "error minus": 0.55\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.8, "5th percentile": 8.75, "95th percentile": 10.28, "error plus": 0.48, "error minus": 1.05\}, "mpp\_2": \{"median": 32.74, "5th percentile": 26.91, "95th percentile": 36.24, "error plus": 3.5, "error minus": 5.83\}, "mu\_chi\_eff": \{"median": 0.18, "5th percentile": 0.09, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.09\}, "mu\_chi\_p": \{"median": 0.36, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.06\}, "sigma\_chi\_eff": \{"median": 0.14, "5th percentile": 0.11, "95th percentile": 0.18, "error plus": 0.04, "error minus": 0.03\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": 4.6, "5th percentile": 1.5, "95th percentile": 7.5, "error plus": 3.0, "error minus": 3.1, "correlated percentile": 98\}\}, "ppd": \{\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\zchieffCopulaCorrelationModel@out\zchieffCopulaCorrelationModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\zchieffCopulaCorrelationModel@out\zchieffCopulaCorrelationModel@II\else\def\zchieffCopulaCorrelationModel@out{??}\fi\fi\fi\zchieffCopulaCorrelationModel@out}\newcommand\zchieffCopulaCorrelationModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@I@out{\{"alpha\_1": \{"median": 1.71, "5th percentile": {-}0.18, "95th percentile": 2.9, "error plus": 1.19, "error minus": 1.89\}, "alpha\_2": \{"median": 4.57, "5th percentile": 3.27, "95th percentile": 5.99, "error plus": 1.42, "error minus": 1.29\}, "beta": \{"median": 1.05, "5th percentile": 0.09, "95th percentile": 2.17, "error plus": 1.12, "error minus": 0.96\}, "break\_mass": \{"median": 35.68, "5th percentile": 22.75, "95th percentile": 48.08, "error plus": 12.4, "error minus": 12.93\}, "delta\_m\_1": \{"median": 4.75, "5th percentile": 0.52, "95th percentile": 9.4, "error plus": 4.65, "error minus": 4.23\}, "delta\_m\_2": \{"median": 3.94, "5th percentile": 0.4, "95th percentile": 7.64, "error plus": 3.7, "error minus": 3.54\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.63, "error plus": 0.28, "error minus": 0.21\}, "lam\_1": \{"median": 0.61, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.29\}, "lamb": \{"median": 2.69, "5th percentile": 1.78, "95th percentile": 3.62, "error plus": 0.93, "error minus": 0.91\}, "mlow\_1": \{"median": 5.07, "5th percentile": 3.3, "95th percentile": 7.67, "error plus": 2.6, "error minus": 1.77\}, "mlow\_2": \{"median": 3.59, "5th percentile": 3.04, "95th percentile": 5.02, "error plus": 1.42, "error minus": 0.55\}, "mmax": \{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}, "mpp\_1": \{"median": 9.8, "5th percentile": 8.75, "95th percentile": 10.28, "error plus": 0.48, "error minus": 1.05\}, "mpp\_2": \{"median": 32.74, "5th percentile": 26.91, "95th percentile": 36.24, "error plus": 3.5, "error minus": 5.83\}, "mu\_chi\_eff": \{"median": 0.18, "5th percentile": 0.09, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.09\}, "mu\_chi\_p": \{"median": 0.36, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.06\}, "sigma\_chi\_eff": \{"median": 0.14, "5th percentile": 0.11, "95th percentile": 0.18, "error plus": 0.04, "error minus": 0.03\}, "sigma\_chi\_p": \{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}, "kappa": \{"median": 4.6, "5th percentile": 1.5, "95th percentile": 7.5, "error plus": 3.0, "error minus": 3.1, "correlated percentile": 98\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@VI\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@VII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@VIII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@IX\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@X\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XI\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XII\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XIII\else\ifnum\pdfstrcmp{#1}{mmax}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XIV\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XV\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XVI\else\ifnum\pdfstrcmp{#1}{mu_chi_eff}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XVII\else\ifnum\pdfstrcmp{#1}{mu_chi_p}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XVIII\else\ifnum\pdfstrcmp{#1}{sigma_chi_eff}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XIX\else\ifnum\pdfstrcmp{#1}{sigma_chi_p}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XX\else\ifnum\pdfstrcmp{#1}{kappa}=0\let\zchieffCopulaCorrelationModel@I@out\zchieffCopulaCorrelationModel@XXI\else\def\zchieffCopulaCorrelationModel@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@I@out}\newcommand\zchieffCopulaCorrelationModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@II@out{\{\}}\else\def\zchieffCopulaCorrelationModel@II@out{??}\fi\zchieffCopulaCorrelationModel@II@out}\newcommand\zchieffCopulaCorrelationModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@III@out{\{"median": 1.71, "5th percentile": {-}0.18, "95th percentile": 2.9, "error plus": 1.19, "error minus": 1.89\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@III@out{1.71}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@III@out{{-}0.18}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@III@out{2.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@III@out{1.19}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@III@out{1.89}\else\def\zchieffCopulaCorrelationModel@III@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@III@out}\newcommand\zchieffCopulaCorrelationModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@IV@out{\{"median": 4.57, "5th percentile": 3.27, "95th percentile": 5.99, "error plus": 1.42, "error minus": 1.29\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@IV@out{4.57}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@IV@out{3.27}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@IV@out{5.99}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@IV@out{1.42}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@IV@out{1.29}\else\def\zchieffCopulaCorrelationModel@IV@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@IV@out}\newcommand\zchieffCopulaCorrelationModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@V@out{\{"median": 1.05, "5th percentile": 0.09, "95th percentile": 2.17, "error plus": 1.12, "error minus": 0.96\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@V@out{1.05}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@V@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@V@out{2.17}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@V@out{1.12}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@V@out{0.96}\else\def\zchieffCopulaCorrelationModel@V@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@V@out}\newcommand\zchieffCopulaCorrelationModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@VI@out{\{"median": 35.68, "5th percentile": 22.75, "95th percentile": 48.08, "error plus": 12.4, "error minus": 12.93\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@VI@out{35.68}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@VI@out{22.75}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@VI@out{48.08}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@VI@out{12.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@VI@out{12.93}\else\def\zchieffCopulaCorrelationModel@VI@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@VI@out}\newcommand\zchieffCopulaCorrelationModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@VII@out{\{"median": 4.75, "5th percentile": 0.52, "95th percentile": 9.4, "error plus": 4.65, "error minus": 4.23\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@VII@out{4.75}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@VII@out{0.52}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@VII@out{9.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@VII@out{4.65}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@VII@out{4.23}\else\def\zchieffCopulaCorrelationModel@VII@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@VII@out}\newcommand\zchieffCopulaCorrelationModel@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@VIII@out{\{"median": 3.94, "5th percentile": 0.4, "95th percentile": 7.64, "error plus": 3.7, "error minus": 3.54\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@VIII@out{3.94}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@VIII@out{0.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@VIII@out{7.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@VIII@out{3.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@VIII@out{3.54}\else\def\zchieffCopulaCorrelationModel@VIII@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@VIII@out}\newcommand\zchieffCopulaCorrelationModel@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@IX@out{\{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.63, "error plus": 0.28, "error minus": 0.21\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@IX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@IX@out{0.63}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@IX@out{0.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@IX@out{0.21}\else\def\zchieffCopulaCorrelationModel@IX@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@IX@out}\newcommand\zchieffCopulaCorrelationModel@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@X@out{\{"median": 0.61, "5th percentile": 0.32, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.29\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@X@out{0.61}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@X@out{0.32}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@X@out{0.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@X@out{0.21}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@X@out{0.29}\else\def\zchieffCopulaCorrelationModel@X@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@X@out}\newcommand\zchieffCopulaCorrelationModel@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XI@out{\{"median": 2.69, "5th percentile": 1.78, "95th percentile": 3.62, "error plus": 0.93, "error minus": 0.91\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XI@out{2.69}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XI@out{1.78}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XI@out{3.62}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XI@out{0.93}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XI@out{0.91}\else\def\zchieffCopulaCorrelationModel@XI@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XI@out}\newcommand\zchieffCopulaCorrelationModel@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XII@out{\{"median": 5.07, "5th percentile": 3.3, "95th percentile": 7.67, "error plus": 2.6, "error minus": 1.77\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XII@out{5.07}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XII@out{3.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XII@out{7.67}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XII@out{2.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XII@out{1.77}\else\def\zchieffCopulaCorrelationModel@XII@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XII@out}\newcommand\zchieffCopulaCorrelationModel@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XIII@out{\{"median": 3.59, "5th percentile": 3.04, "95th percentile": 5.02, "error plus": 1.42, "error minus": 0.55\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XIII@out{3.59}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XIII@out{3.04}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XIII@out{5.02}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XIII@out{1.42}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XIII@out{0.55}\else\def\zchieffCopulaCorrelationModel@XIII@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XIII@out}\newcommand\zchieffCopulaCorrelationModel@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XIV@out{\{"median": 300.0, "5th percentile": 300.0, "95th percentile": 300.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XIV@out{300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XIV@out{0.0}\else\def\zchieffCopulaCorrelationModel@XIV@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XIV@out}\newcommand\zchieffCopulaCorrelationModel@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XV@out{\{"median": 9.8, "5th percentile": 8.75, "95th percentile": 10.28, "error plus": 0.48, "error minus": 1.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XV@out{9.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XV@out{8.75}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XV@out{10.28}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XV@out{0.48}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XV@out{1.05}\else\def\zchieffCopulaCorrelationModel@XV@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XV@out}\newcommand\zchieffCopulaCorrelationModel@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XVI@out{\{"median": 32.74, "5th percentile": 26.91, "95th percentile": 36.24, "error plus": 3.5, "error minus": 5.83\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XVI@out{32.74}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XVI@out{26.91}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XVI@out{36.24}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XVI@out{3.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XVI@out{5.83}\else\def\zchieffCopulaCorrelationModel@XVI@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XVI@out}\newcommand\zchieffCopulaCorrelationModel@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XVII@out{\{"median": 0.18, "5th percentile": 0.09, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.09\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XVII@out{0.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XVII@out{0.09}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XVII@out{0.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XVII@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XVII@out{0.09}\else\def\zchieffCopulaCorrelationModel@XVII@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XVII@out}\newcommand\zchieffCopulaCorrelationModel@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XVIII@out{\{"median": 0.36, "5th percentile": 0.3, "95th percentile": 0.42, "error plus": 0.06, "error minus": 0.06\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XVIII@out{0.36}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XVIII@out{0.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XVIII@out{0.42}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XVIII@out{0.06}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XVIII@out{0.06}\else\def\zchieffCopulaCorrelationModel@XVIII@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XVIII@out}\newcommand\zchieffCopulaCorrelationModel@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XIX@out{\{"median": 0.14, "5th percentile": 0.11, "95th percentile": 0.18, "error plus": 0.04, "error minus": 0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XIX@out{0.14}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XIX@out{0.11}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XIX@out{0.18}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XIX@out{0.04}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XIX@out{0.03}\else\def\zchieffCopulaCorrelationModel@XIX@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XIX@out}\newcommand\zchieffCopulaCorrelationModel@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XX@out{\{"median": 0.18, "5th percentile": 0.13, "95th percentile": 0.25, "error plus": 0.07, "error minus": 0.05\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XX@out{0.18}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XX@out{0.25}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XX@out{0.07}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XX@out{0.05}\else\def\zchieffCopulaCorrelationModel@XX@out{??}\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XX@out}\newcommand\zchieffCopulaCorrelationModel@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffCopulaCorrelationModel@XXI@out{\{"median": 4.6, "5th percentile": 1.5, "95th percentile": 7.5, "error plus": 3.0, "error minus": 3.1, "correlated percentile": 98\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffCopulaCorrelationModel@XXI@out{4.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffCopulaCorrelationModel@XXI@out{1.5}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffCopulaCorrelationModel@XXI@out{7.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffCopulaCorrelationModel@XXI@out{3.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffCopulaCorrelationModel@XXI@out{3.1}\else\ifnum\pdfstrcmp{#1}{correlated percentile}=0\def\zchieffCopulaCorrelationModel@XXI@out{98}\else\def\zchieffCopulaCorrelationModel@XXI@out{??}\fi\fi\fi\fi\fi\fi\fi\zchieffCopulaCorrelationModel@XXI@out}\makeatother
\makeatletter\newcommand\zchieffLinearCorrelationModel[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@out{\{"param": \{"alpha\_1": \{"median": 1.57, "5th percentile": {-}0.74, "95th percentile": 2.85, "error plus": 1.28, "error minus": 2.32\}, "alpha\_2": \{"median": 4.53, "5th percentile": 3.23, "95th percentile": 6.15, "error plus": 1.62, "error minus": 1.3\}, "beta": \{"median": 1.14, "5th percentile": 0.07, "95th percentile": 2.68, "error plus": 1.54, "error minus": 1.07\}, "break\_mass": \{"median": 35.06, "5th percentile": 21.88, "95th percentile": 47.93, "error plus": 12.87, "error minus": 13.18\}, "delta\_m\_1": \{"median": 4.64, "5th percentile": 0.39, "95th percentile": 9.36, "error plus": 4.72, "error minus": 4.25\}, "delta\_m\_2": \{"median": 4.2, "5th percentile": 0.38, "95th percentile": 8.91, "error plus": 4.72, "error minus": 3.82\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.61, "error plus": 0.27, "error minus": 0.22\}, "lam\_1": \{"median": 0.6, "5th percentile": 0.34, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.26\}, "lamb": \{"median": 2.95, "5th percentile": 1.91, "95th percentile": 3.96, "error plus": 1.01, "error minus": 1.04\}, "mlow\_1": \{"median": 5.02, "5th percentile": 3.22, "95th percentile": 8.18, "error plus": 3.16, "error minus": 1.8\}, "mlow\_2": \{"median": 3.47, "5th percentile": 3.03, "95th percentile": 4.8, "error plus": 1.33, "error minus": 0.44\}, "mpp\_1": \{"median": 9.94, "5th percentile": 9.24, "95th percentile": 10.34, "error plus": 0.4, "error minus": 0.7\}, "mpp\_2": \{"median": 33.26, "5th percentile": 26.86, "95th percentile": 36.44, "error plus": 3.18, "error minus": 6.39\}, "mu\_chieff\_0": \{"median": 0.03, "5th percentile": {-}0.01, "95th percentile": 0.06, "error plus": 0.03, "error minus": 0.03\}, "ln\_sigma\_chieff\_0": \{"median": {-}2.23, "5th percentile": {-}2.45, "95th percentile": {-}2.03, "error plus": 0.2, "error minus": 0.22\}, "mu\_chieff\_1": \{"median": {-}0.02, "5th percentile": {-}0.13, "95th percentile": 0.09, "error plus": 0.11, "error minus": 0.12, "percentile exclude zero": 60\}, "ln\_sigma\_chieff\_1": \{"median": 0.96, "5th percentile": 0.56, "95th percentile": 1.27, "error plus": 0.31, "error minus": 0.4, "percentile exclude zero": 99\}\}, "ppd": \{\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\zchieffLinearCorrelationModel@out\zchieffLinearCorrelationModel@I\else\ifnum\pdfstrcmp{#1}{ppd}=0\let\zchieffLinearCorrelationModel@out\zchieffLinearCorrelationModel@II\else\def\zchieffLinearCorrelationModel@out{??}\fi\fi\fi\zchieffLinearCorrelationModel@out}\newcommand\zchieffLinearCorrelationModel@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@I@out{\{"alpha\_1": \{"median": 1.57, "5th percentile": {-}0.74, "95th percentile": 2.85, "error plus": 1.28, "error minus": 2.32\}, "alpha\_2": \{"median": 4.53, "5th percentile": 3.23, "95th percentile": 6.15, "error plus": 1.62, "error minus": 1.3\}, "beta": \{"median": 1.14, "5th percentile": 0.07, "95th percentile": 2.68, "error plus": 1.54, "error minus": 1.07\}, "break\_mass": \{"median": 35.06, "5th percentile": 21.88, "95th percentile": 47.93, "error plus": 12.87, "error minus": 13.18\}, "delta\_m\_1": \{"median": 4.64, "5th percentile": 0.39, "95th percentile": 9.36, "error plus": 4.72, "error minus": 4.25\}, "delta\_m\_2": \{"median": 4.2, "5th percentile": 0.38, "95th percentile": 8.91, "error plus": 4.72, "error minus": 3.82\}, "lam\_0": \{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.61, "error plus": 0.27, "error minus": 0.22\}, "lam\_1": \{"median": 0.6, "5th percentile": 0.34, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.26\}, "lamb": \{"median": 2.95, "5th percentile": 1.91, "95th percentile": 3.96, "error plus": 1.01, "error minus": 1.04\}, "mlow\_1": \{"median": 5.02, "5th percentile": 3.22, "95th percentile": 8.18, "error plus": 3.16, "error minus": 1.8\}, "mlow\_2": \{"median": 3.47, "5th percentile": 3.03, "95th percentile": 4.8, "error plus": 1.33, "error minus": 0.44\}, "mpp\_1": \{"median": 9.94, "5th percentile": 9.24, "95th percentile": 10.34, "error plus": 0.4, "error minus": 0.7\}, "mpp\_2": \{"median": 33.26, "5th percentile": 26.86, "95th percentile": 36.44, "error plus": 3.18, "error minus": 6.39\}, "mu\_chieff\_0": \{"median": 0.03, "5th percentile": {-}0.01, "95th percentile": 0.06, "error plus": 0.03, "error minus": 0.03\}, "ln\_sigma\_chieff\_0": \{"median": {-}2.23, "5th percentile": {-}2.45, "95th percentile": {-}2.03, "error plus": 0.2, "error minus": 0.22\}, "mu\_chieff\_1": \{"median": {-}0.02, "5th percentile": {-}0.13, "95th percentile": 0.09, "error plus": 0.11, "error minus": 0.12, "percentile exclude zero": 60\}, "ln\_sigma\_chieff\_1": \{"median": 0.96, "5th percentile": 0.56, "95th percentile": 1.27, "error plus": 0.31, "error minus": 0.4, "percentile exclude zero": 99\}\}}\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@III\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@IV\else\ifnum\pdfstrcmp{#1}{beta}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@V\else\ifnum\pdfstrcmp{#1}{break_mass}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@VI\else\ifnum\pdfstrcmp{#1}{delta_m_1}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@VII\else\ifnum\pdfstrcmp{#1}{delta_m_2}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@VIII\else\ifnum\pdfstrcmp{#1}{lam_0}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@IX\else\ifnum\pdfstrcmp{#1}{lam_1}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@X\else\ifnum\pdfstrcmp{#1}{lamb}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XI\else\ifnum\pdfstrcmp{#1}{mlow_1}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XII\else\ifnum\pdfstrcmp{#1}{mlow_2}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XIII\else\ifnum\pdfstrcmp{#1}{mpp_1}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XIV\else\ifnum\pdfstrcmp{#1}{mpp_2}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XV\else\ifnum\pdfstrcmp{#1}{mu_chieff_0}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XVI\else\ifnum\pdfstrcmp{#1}{ln_sigma_chieff_0}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XVII\else\ifnum\pdfstrcmp{#1}{mu_chieff_1}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XVIII\else\ifnum\pdfstrcmp{#1}{ln_sigma_chieff_1}=0\let\zchieffLinearCorrelationModel@I@out\zchieffLinearCorrelationModel@XIX\else\def\zchieffLinearCorrelationModel@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@I@out}\newcommand\zchieffLinearCorrelationModel@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@II@out{\{\}}\else\def\zchieffLinearCorrelationModel@II@out{??}\fi\zchieffLinearCorrelationModel@II@out}\newcommand\zchieffLinearCorrelationModel@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@III@out{\{"median": 1.57, "5th percentile": {-}0.74, "95th percentile": 2.85, "error plus": 1.28, "error minus": 2.32\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@III@out{1.57}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@III@out{{-}0.74}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@III@out{2.85}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@III@out{1.28}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@III@out{2.32}\else\def\zchieffLinearCorrelationModel@III@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@III@out}\newcommand\zchieffLinearCorrelationModel@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@IV@out{\{"median": 4.53, "5th percentile": 3.23, "95th percentile": 6.15, "error plus": 1.62, "error minus": 1.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@IV@out{4.53}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@IV@out{3.23}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@IV@out{6.15}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@IV@out{1.62}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@IV@out{1.3}\else\def\zchieffLinearCorrelationModel@IV@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@IV@out}\newcommand\zchieffLinearCorrelationModel@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@V@out{\{"median": 1.14, "5th percentile": 0.07, "95th percentile": 2.68, "error plus": 1.54, "error minus": 1.07\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@V@out{1.14}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@V@out{0.07}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@V@out{2.68}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@V@out{1.54}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@V@out{1.07}\else\def\zchieffLinearCorrelationModel@V@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@V@out}\newcommand\zchieffLinearCorrelationModel@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@VI@out{\{"median": 35.06, "5th percentile": 21.88, "95th percentile": 47.93, "error plus": 12.87, "error minus": 13.18\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@VI@out{35.06}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@VI@out{21.88}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@VI@out{47.93}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@VI@out{12.87}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@VI@out{13.18}\else\def\zchieffLinearCorrelationModel@VI@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@VI@out}\newcommand\zchieffLinearCorrelationModel@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@VII@out{\{"median": 4.64, "5th percentile": 0.39, "95th percentile": 9.36, "error plus": 4.72, "error minus": 4.25\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@VII@out{4.64}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@VII@out{0.39}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@VII@out{9.36}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@VII@out{4.72}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@VII@out{4.25}\else\def\zchieffLinearCorrelationModel@VII@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@VII@out}\newcommand\zchieffLinearCorrelationModel@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@VIII@out{\{"median": 4.2, "5th percentile": 0.38, "95th percentile": 8.91, "error plus": 4.72, "error minus": 3.82\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@VIII@out{4.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@VIII@out{0.38}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@VIII@out{8.91}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@VIII@out{4.72}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@VIII@out{3.82}\else\def\zchieffLinearCorrelationModel@VIII@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@VIII@out}\newcommand\zchieffLinearCorrelationModel@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@IX@out{\{"median": 0.34, "5th percentile": 0.13, "95th percentile": 0.61, "error plus": 0.27, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@IX@out{0.34}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@IX@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@IX@out{0.61}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@IX@out{0.27}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@IX@out{0.22}\else\def\zchieffLinearCorrelationModel@IX@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@IX@out}\newcommand\zchieffLinearCorrelationModel@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@X@out{\{"median": 0.6, "5th percentile": 0.34, "95th percentile": 0.82, "error plus": 0.21, "error minus": 0.26\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@X@out{0.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@X@out{0.34}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@X@out{0.82}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@X@out{0.21}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@X@out{0.26}\else\def\zchieffLinearCorrelationModel@X@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@X@out}\newcommand\zchieffLinearCorrelationModel@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XI@out{\{"median": 2.95, "5th percentile": 1.91, "95th percentile": 3.96, "error plus": 1.01, "error minus": 1.04\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XI@out{2.95}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XI@out{1.91}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XI@out{3.96}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XI@out{1.01}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XI@out{1.04}\else\def\zchieffLinearCorrelationModel@XI@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XI@out}\newcommand\zchieffLinearCorrelationModel@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XII@out{\{"median": 5.02, "5th percentile": 3.22, "95th percentile": 8.18, "error plus": 3.16, "error minus": 1.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XII@out{5.02}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XII@out{3.22}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XII@out{8.18}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XII@out{3.16}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XII@out{1.8}\else\def\zchieffLinearCorrelationModel@XII@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XII@out}\newcommand\zchieffLinearCorrelationModel@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XIII@out{\{"median": 3.47, "5th percentile": 3.03, "95th percentile": 4.8, "error plus": 1.33, "error minus": 0.44\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XIII@out{3.47}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XIII@out{3.03}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XIII@out{4.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XIII@out{1.33}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XIII@out{0.44}\else\def\zchieffLinearCorrelationModel@XIII@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XIII@out}\newcommand\zchieffLinearCorrelationModel@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XIV@out{\{"median": 9.94, "5th percentile": 9.24, "95th percentile": 10.34, "error plus": 0.4, "error minus": 0.7\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XIV@out{9.94}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XIV@out{9.24}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XIV@out{10.34}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XIV@out{0.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XIV@out{0.7}\else\def\zchieffLinearCorrelationModel@XIV@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XIV@out}\newcommand\zchieffLinearCorrelationModel@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XV@out{\{"median": 33.26, "5th percentile": 26.86, "95th percentile": 36.44, "error plus": 3.18, "error minus": 6.39\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XV@out{33.26}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XV@out{26.86}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XV@out{36.44}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XV@out{3.18}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XV@out{6.39}\else\def\zchieffLinearCorrelationModel@XV@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XV@out}\newcommand\zchieffLinearCorrelationModel@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XVI@out{\{"median": 0.03, "5th percentile": {-}0.01, "95th percentile": 0.06, "error plus": 0.03, "error minus": 0.03\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XVI@out{0.03}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XVI@out{{-}0.01}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XVI@out{0.06}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XVI@out{0.03}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XVI@out{0.03}\else\def\zchieffLinearCorrelationModel@XVI@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XVI@out}\newcommand\zchieffLinearCorrelationModel@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XVII@out{\{"median": {-}2.23, "5th percentile": {-}2.45, "95th percentile": {-}2.03, "error plus": 0.2, "error minus": 0.22\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XVII@out{{-}2.23}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XVII@out{{-}2.45}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XVII@out{{-}2.03}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XVII@out{0.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XVII@out{0.22}\else\def\zchieffLinearCorrelationModel@XVII@out{??}\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XVII@out}\newcommand\zchieffLinearCorrelationModel@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XVIII@out{\{"median": {-}0.02, "5th percentile": {-}0.13, "95th percentile": 0.09, "error plus": 0.11, "error minus": 0.12, "percentile exclude zero": 60\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XVIII@out{{-}0.02}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XVIII@out{{-}0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XVIII@out{0.09}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XVIII@out{0.11}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XVIII@out{0.12}\else\ifnum\pdfstrcmp{#1}{percentile exclude zero}=0\def\zchieffLinearCorrelationModel@XVIII@out{60}\else\def\zchieffLinearCorrelationModel@XVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XVIII@out}\newcommand\zchieffLinearCorrelationModel@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\zchieffLinearCorrelationModel@XIX@out{\{"median": 0.96, "5th percentile": 0.56, "95th percentile": 1.27, "error plus": 0.31, "error minus": 0.4, "percentile exclude zero": 99\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\zchieffLinearCorrelationModel@XIX@out{0.96}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\zchieffLinearCorrelationModel@XIX@out{0.56}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\zchieffLinearCorrelationModel@XIX@out{1.27}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\zchieffLinearCorrelationModel@XIX@out{0.31}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\zchieffLinearCorrelationModel@XIX@out{0.4}\else\ifnum\pdfstrcmp{#1}{percentile exclude zero}=0\def\zchieffLinearCorrelationModel@XIX@out{99}\else\def\zchieffLinearCorrelationModel@XIX@out{??}\fi\fi\fi\fi\fi\fi\fi\zchieffLinearCorrelationModel@XIX@out}\makeatother

